Compression for Quadratic Similarity Queries: Finite Blocklength and Practical Schemes

We study the problem of compression for the purpose of similarity identification, where similarity is measured by the mean square Euclidean distance between vectors. While the asymptotical fundamental limits of the problem - the minimal compression rate and the error exponent - were found in a previous work, in this paper we focus on the nonasymptotic domain and on practical, implementable schemes. We first present a finite blocklength achievability bound based on shape-gain quantization: The gain (amplitude) of the vector is compressed via scalar quantization and the shape (the projection on the unit sphere) is quantized using a spherical code. The results are numerically evaluated and they converge to the asymptotic values as predicted by the error exponent. We then give a nonasymptotic lower bound on the performance of any compression scheme, and compare to the upper (achievability) bound. For a practical implementation of such a scheme, we use wrapped spherical codes, studied by Hamkins and Zeger, and use the Leech lattice as an example for an underlying lattice. As a side result, we obtain a bound on the covering angle of any wrapped spherical code, as a function of the covering radius of the underlying lattice.

==> skeyval-core.tex <==
%++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++%
% This is file 'skeyval-core.tex', version 1.3, 2013/05/15.                %
%                                                                          %
% This package and accompanying files may be distributed and/or            %
% modified under the conditions of the LaTeX Project Public License,       %
% either version 1.3 of this license or any later version. The latest      %
% version of this license is in http://www.latex-project.org/lppl.txt      %
% and version 1.3 or later is part of all distributions of LaTeX           %
% version 2005/12/01 or later.                                             %
%                                                                          %
% The LPPL maintenance status of this software is 'author-maintained'.     %
%                                                                          %
% This software is provided 'as it is', without warranty of any kind,      %
% either expressed or implied, including, but not limited to, the          %
% implied warranties of merchantability and fitness for a particular       %
% purpose.                                                                 %
%                                                                          %
% The following files constitute the skeyval bundle and must be            %
% distributed as a whole:                                                  %
%                                                                          %
%  README, skeyval.sty, skeyval-core.tex, skeyval-for.tex,                 %
%  skeyval-view.sty, skeyval-ltxpatch.sty, skeyval-ltxcmds.tex,            %
%  skeyval-pstkey.sty, skeyval-pstkey.tex, skeyval-testclass.cls,          %
%  skeyval-testpkg.sty, skeyval-pokayoke1, skeyval-pokayoke2,              %
%  skeyval-view-pokayoke1.                                                 %
%                                                                          %
% Copyright (c) 2010-2013 Ahmed Musa (amusa22@gmail.com).                  %
%++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++%

\csname skeyval-core-loaded\endcsname
\expandafter\let\csname skeyval-core-loaded\endcsname\endinput

\begingroup
\catcode035 06 % #
\catcode064 11 % @
\catcode123 01 % {
\catcode125 02 % }
\catcode044 12 % ,
\def\skv@prova{\endgroup
  \def\do##1,{%
    \ifx\do##1\else
      \catcode##1\string=\the\catcode##1\relax
      \expandafter\do
    \fi
  }%
  \edef\skv@core@restorecodes{\do35,64,123,125,61,59,13,\do,}%
}
\skv@prova

\edef\skv@core@restorecodes{%
  \unexpanded\expandafter{\skv@core@restorecodes}%
  \endlinechar\the\endlinechar\relax
  \catcode`\^^M=\the\catcode`\^^M\relax
}
\endlinechar13 %
\catcode013 05 % ^^M
\catcode035 06 % #
\catcode064 11 % @
\catcode123 01 % {
\catcode125 02 % }
\catcode061 12 % =
\catcode044 12 % ,
\def\do#1=#2,{%
  \ifx\do#1\else
    \edef\skv@core@restorecodes{%
      \unexpanded\expandafter{\skv@core@restorecodes}%
      \catcode#1=\the\catcode#1\relax
    }%
    \catcode#1=#2\relax
    \expandafter\do
  \fi
}
\do 032=10,033=12,036=03,038=04,040=12,041=12,042=12,043=12,%
  059=12,045=12,047=12,058=12,063=12,091=12,093=12,126=13,13=5,\do=,%

\newdimen\skvz@\skvz@=0pt\relax
\newcount\skvm@ne\skvm@ne=-1\relax
\ifcase
  \ifx\eTeXversion\@undefined 0\else
    \ifnum\eTeXversion<\tw@ 0\else 1\fi
  \fi\relax
  \errhelp{This package requires eTeX version 2 or higher.}
  \errmessage{skeyval package: eTeX not loaded or old version.}
  \expandafter\endinput
\fi

\newif\ifskv@latex
\newif\ifskv@tempst
\ifx\ProvidesFile\@undefined
  \skv@latexfalse
  \message{File 'skeyval-core.tex' 2013/05/15 v1.3:
    Core of 'skeyval' key-value parser (AM)}
  \input skeyval-ltxcmds
\else
  \skv@latextrue
  \ProvidesFile{skeyval-core.tex}
    [2013/05/15 v1.3 Base file of skeyval package (AM)]
  \@addtofilelist{skeyval-core.tex}
  \long\def\@nodocument#1{%
    \@latex@error{'#1' appeared\on@line\space without
      \noexpand\begin{document}}\@ehd
  }
\fi

% skeyval-ltxcmds.tex defines \PackageError, etc:
\protected\def\skv@warn{\PackageWarningNoLine{skeyval}}
\protected\def\skv@err{\PackageError{skeyval}}
% No \protected for \skv@ehd:
\def\skv@ehd{%
  I have encountered a problem here. Try typing <return>
  \MessageBreak to proceed. If that doesn't work, type X then
  <return>\MessageBreak to quit.
}
\let\skvgenericexception\@latexerr
\protected\def\skvtracingall{%
  \tracinggroups\@ne\tracingifs\@ne\loggingall\tracingassigns\@ne
}
\let\skvloggingall\skvtracingall
\long\def\skviofii#1#2{#1}
\long\def\skviiofii#1#2{#2}
% A \relax'ed command should not be redefined, because we don't know
% if it is temporarily or permanently made \relax.
\long\def\skvifdefinable#1#2{%
  \ifdefined#1%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {\@latex@error{Command '\string#1' already defined}\skv@ehd}
  {#2}%
}
% \skvgenloop{<parser>}{<list>}{<1.parameter.callback>}
%
% 1. The parser may be empty. This is the case for nsv/tsv lists.
% 2. The normalization of the list, including dealing with active parsers,
%    is left to the caller.
% 3. \@iden will help remove spurious leading spaces.
%
\protected\def\skvgenloop#1#2#3{%
  \def\skv@gendo##1#1{%
    \ifx\skv@gendo##1\expandafter\@gobble\else\expandafter\@iden\fi
    {#3\expandafter\skv@gendo\@iden}%
  }%
  \expandafter\skv@gendo\@iden#2#1\skv@gendo#1%
}
% \skvrescan{<macro>}
\protected\def\skvrescan#1{%
  \begingroup
  \endlinechar\m@ne\newlinechar\m@ne
  \catcode`\@=11\relax
  \everyeof{\skv@rescan@guard}%
  \def\reserved@a##1\skv@rescan@guard{%
    \endgroup
    \edef#1{\unexpanded\expandafter{\@gobble##1}}%
  }%
  % \relax protects any blank space leading the content of #1:
  \expandafter\reserved@a\scantokens\expandafter{\expandafter\relax#1}%
}

% Process a comma list with a simple callback. This can't be used if #2
% isn't scannable or if scanning #2 will change the signature of
% its token list.
%
% \skv@commaact{<list>}{<1.parameter.callback>}
%
% Example:
%
%   \def\emptify{\skv@commaact{\def##1{}}}
%
\begingroup
\catcode`\,=\active
\protected\gdef\skv@commaact#1#2{%
  \begingroup
  \toks@{}%
  \def,##1{%
    \ifx\skv@commaact##1\else
      \ifx,##1%
        % Double comma seen:
        \expandafter\expandafter\expandafter,%
      \else
        \toks@\expandafter{\the\toks@#2}%
      \fi
    \fi
  }%
  \begingroup
  \edef\skv@tempa{\unexpanded{,#1}}%
  \catcode`\,=\active
  \skvrescan\skv@tempa
  % Add a trailing \skv@commaact, in case the list is ended by a comma (,):
  \expandafter\endgroup\skv@tempa,\skv@commaact
  \expandafter\endgroup\the\toks@
}
\endgroup

\protected\def\skvnewregister#1#2{%
  \def\skv@prova{#1}%
  \def\skv@provb{\bool}%
  % We don't want to expose \if while in the next conditional:
  \def\skv@provc{\if}%
  \ifx\skv@prova\skv@provb
    \let\skv@prova\skv@provc
  \fi
  \skv@commaact{#2}{%
    \skvifdefinable##1{%
      \csname new\expandafter\expandafter\expandafter\@gobble
      \expandafter\string\skv@prova\endcsname##1%
    }%
  }%
}
\let\skvnewregisters\skvnewregister
\skvnewregisters\toks{\skv@temptoks,\skv@toksa}

% Sometimes we change \bgroup temporarily to avoid \futurelet confusing
% it with explicit \bgroup character. The change does confuse \skvifnextchar
% if we used \bgroup in \skvifnextchar. Hence let us use \skv@orig@bgroup
% in \skvifnextchar:
\let\skv@orig@bgroup\bgroup
\let\skv@orig@egroup\egroup

\def\reserved@a#1{%
  \def\skvifnextisouter{%
    \expandafter\skv@ifnextisouter\meaning\skv@nextseen#1\relax
  }%
  \def\skv@ifnextisouter##1#1##2\relax{%
    \ifcat$##2$\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi
  }%
}
\expandafter\reserved@a\expandafter{\detokenize{outer macro}:}

% We modify LaTeX kernel's \@ifnextchar to eliminate the need for
% doubling the hash character in #2 or #3. \skv@nextseen may be needed
% outside the group; so we use \global.
\long\def\skvsimpleifnextchar#1#2#3{%
  \begingroup
  \let\reserved@d=#1%
  \edef\reserved@a{\endgroup\unexpanded{#2}}%
  \edef\reserved@b{\endgroup\unexpanded{#3}}%
  \global\futurelet\skv@nextseen\skv@simpleifnext
}
\def\skv@simpleifnext{%
  \ifx\skv@nextseen\@sptoken
    \let\skv@letnext\skv@simpleifn@xt
  \else
    \ifx\skv@nextseen\reserved@d
      \let\skv@letnext\reserved@a
    \else
      \let\skv@letnext\reserved@b
    \fi
  \fi
  \skv@letnext
}
\lowercase{\def\skv@simpleifn@xt} {%
  \global\futurelet\skv@nextseen\skv@simpleifnext
}

% Tests for \skvifnextchar:
%
% \outer\def\foo{}
% \iftrue\skvifnextchar*\relax\relax\foo\fi
% \iftrue\skvifnextchar*\relax\relax\fi
% \skvifnextchar*\relax\relax\iftrue\fi
%
\protected\long\def\skvifnextchar#1#2#3{%
  \skvsimpleifnextchar\skv@orig@bgroup{%
    \skvsimpleifnextchar{#1}{#2}{#3}%
  }{%
    % Test for \egroup, so that, eg, {\loggingall\LoadClass{article}}
    % doesn't fail because of the closing brace:
    \skvsimpleifnextchar\skv@orig@egroup{%
      \skvsimpleifnextchar{#1}{#2}{#3}%
    }{%
      \skvifnextisouter{%
        \skvsimpleifnextchar{#1}{#2}{#3}%
      }{%
        \skv@ifnextchar@a{#1}{#2}{#3}%
      }%
    }%
  }%
}
\long\def\skv@ifnextchar@a#1#2#3#4{%
  \edef\reserved@a{\skv@ifnextchar@b{#1}\skv@ifnextchar@b{#4}}%
  \expandafter\ifx\reserved@a
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {#2}{#3}#4%
}
\long\def\skv@ifnextchar@b#1{%
  \expandafter\skv@ifnextchar@c\string#1\relax\noboundary{#1}%
}
\long\def\skv@ifnextchar@c#1#2\noboundary#3{%
  \ifx\relax#2%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {#1}{\unexpanded{#3}}%
}
\let\skv@sav@ifnextchar\skvifnextchar
\protected\def\skvusesimpleifnextchar{%
  \let\skvifnextchar\skvsimpleifnextchar
}
\let\skvuselatexifnextchar\skvusesimpleifnextchar
\protected\def\skvuserobustifnextchar{%
  \let\skvifnextchar\skv@sav@ifnextchar
}

% Expandable \@testopt:
%
% Eg,
%     \def\macroa{\skvnewxtestopt\macrob{Mr.}}
%     \def\macrob[#1]#2{#1 #2}
%     \edef\testa{\expandafter\macroa\activespace{David Carlisle}}
%     \edef\testb{\macroa[Mr.]{Heiko Oberdiek}}
%
\long\def\skvnewxtestopt#1#2#3{%
  % #3 will be seen as a space only if that space is active. But
  % \skvifstrcmpTF will detokenize that space before comparison.
  \skvifstrcmpTF{ }{#3}{%
    \skvnewxtestopt#1{#2}%
  }{%
    \skvifstrcmpTF{#3}{[}%
      {#1[}{\skvifntypeTF{#3}{#1[#2]#3}{#1[#2]{#3}}}%
  }%
}

% Expandable \@ifnextchar:
%
% Eg,
%    \def\temp{\skvxifnextchar*{\def\x{T}}{\def\x{F}}}
%    \temp* (star seen) or \temp<some token> (star not seen)
%
% ** This can't be used to test the presence of explicit left brace.
%
\long\def\skvxifnextchar#1#2#3#4{%
  % #4 will be seen as a space only if that space is active. But
  % \skvifstrcmpTF will detokenize that space before comparison.
  \skvifstrcmpTF{ }{#4}{%
    \skvxifnextchar#1{#2}{#3}%
  }{%
    \skvifstrcmpTF{#4}{#1}{#2}{\skvifntypeTF{#4}{#3#4}{#3{#4}}}%
  }%
}

\long\def\skvgobbleleadingspaces{\skvsimpleifnextchar x{}{}}
\long\protected\def\skvstarorlong#1{%
  \skvifstar{\let\l@ngrel@x\relax#1}{\let\l@ngrel@x\long#1}%
}
\long\protected\def\skv@testopt#1#2{\skvifnextchar[{#1}{#1[{#2}]}}
\long\protected\def\skv@testpnopt#1#2{\skvifnextchar({#1}{#1({#2})}}
\long\protected\def\skvifstar#1{\skvifnextchar*{\@firstoftwo{#1}}}
\def\skv@def@#1#2#3{%
  \ifdefined#3%
    \ifx#3\relax\else
      \skv@err{Command \detokenize{#3} already exists}\skv@ehd
    \fi
  \fi
  \ifcat$\detokenize{#2}$\else
    \ifx#2p\expandafter\expandafter\expandafter\protected\fi
  \fi
  \l@ngrel@x\csname#1def\endcsname#3%
}
\def\skv@csdef@#1#2#3{%
  \def\skv@prova{\skv@def@{#1}{#2}}%
  \expandafter\skv@prova\csname#3\endcsname
}
\def\skv@redef@#1#2#3{%
  \ifcat$\detokenize{#2}$\else
    \ifx#2p\expandafter\expandafter\expandafter\protected\fi
  \fi
  \l@ngrel@x\csname#1def\endcsname#3%
}
\protected\def\skvrobustdef{\skvstarorlong{\skv@def@{}{p}}}
\skvrobustdef*\skvrobustredef{\skvstarorlong{\skv@redef@{}{p}}}
\skvrobustdef*\skvrobustgdef{\skvstarorlong{\skv@def@{g}{p}}}
\skvrobustdef*\skvnewdef{\skvstarorlong{\skv@def@{}{}}}
\skvrobustdef*\skvrenewdef{\skvstarorlong{\skv@redef@{}{}}}
\skvrobustdef*\skvnewedef{\skvstarorlong{\skv@def@{e}{}}}
\skvrobustdef*\skvnewgdef{\skvstarorlong{\skv@def@{g}{}}}
\skvrobustdef*\skvrobustcsdef{\skvstarorlong{\skv@csdef@{}{p}}}
\skvrobustdef*\skvnewcsdef{\skvstarorlong{\skv@csdef@{}{}}}
\skvrobustdef*\skvifplus#1{\skvifnextchar+{\@firstoftwo{#1}}}

\skvrobustdef*\skvshowcs#1{%
  \begingroup\expandafter\endgroup
  \expandafter\show\csname#1\endcsname
}
\skvrobustdef*\skvcomment{%
  \begingroup
  \def\do##1{\catcode`##1=12\relax}%
  \dospecials
  \skv@endcomment
}
\begingroup
\catcode`\!=0
\catcode`\\=12
!long!gdef!skv@endcomment#1\endcomment{!endgroup}
!endgroup
%\skvrobustdef\skv@c@mment#1\endcomment{\endgroup}

\skvnewedef*\skv@hashchar{\string#}
\let\nofilter\relax
% Don't use '=' at the end of the following definition; the user
% might have put '=':
\skvrobustdef*\skvnewlet#1{\skvifdefinable#1\relax\let#1 }
\skvnewlet\skv@nil\relax
\skvnewlet\skvrelax\relax
\skvnewdef*\skv@relaxtoks{\relax}
\skvnewdef*\skv@truetoks{true}
\skvnewdef*\skv@falsetoks{false}
\skvnewdef*\skv@nnil{\skv@nil}
\skvnewdef\skv@car#1#2\car@nil{#1}
\skvnewdef\skv@car@detok#1#2\car@nil{\detokenize{#1}}
\skvnewdef\skv@removetonnil#1\skv@nnil{}
\skvnewdef\skv@catchtonnil#1\skv@nnil{#1}
\long\def\@gobblethree#1#2#3{}
\skvnewdef\skv@gobbletoend#1\skv@gobble@nil{}
\skvnewlet\skv@gobble@nil\relax
\def\@space{ }
\let\then\iffalse
\skvnewdef\skvswap#1#2{#2#1}
\skvnewdef*\skv@quark{\@gobble\skv@quark}
\skvnewlet\skvrom\romannumeral
\skvnewdef*\skv@rej{^skv^}
\skvnewdef*\skv@dotna{.na}
\skvnewdef\skvafterfi#1\fi{\fi#1}
\skvnewdef\skvafterfifi@inneriscond#1\fi#2\fi{\fi#1\fi}
\skvnewdef\skvafterfifi#1\fi#2\fi{\fi\fi#1}
\skvnewdef\skvafterelsei#1\else#2\fi{\fi#1}
\skvnewlet\skvafterelse\skvafterelsei
\skvnewdef\skvafterelseii#1\else#2\fi{\fi#2}
\skvnewdef*\skv@simplearg{##1}
\skvnewlet\skvsanitizemacro\@onelevel@sanitize
% \skvaddtotoks{<token register>}{<token to add>}
\skvrobustdef*\skvaddtotoks#1#2{#1\expandafter{\the#1#2}}
\skvrobustdef*\skvoaddtotoks#1#2{#1\expandafter{\the\expandafter#1#2}}
\skvrobustdef*\skv@usetempst#1#2{%
  \edef#2{\skvifdefboolTF{skv@tempst}\skvexpandonce\unexpanded{#1}}%
}
\skvrobustdef*\skvtestifin#1#2{%
  \begingroup
  \long\def\in@@##1#1##2\in@@{%
    \edef\in@@{\unexpanded{##2}}%
    \expandafter\endgroup
    \ifx\in@@\@empty\in@false\else\in@true\fi
  }%
  \in@@#2{\in@@}#1\in@@
}
\skvrobustdef*\skvcsnewif#1{%
  \skvifstrcmpTF{#1}{x}{%
    \skv@err{Redefining primitve '\@backslashchar ifx'?}\skv@ehd
  }{%
    \csname newif\expandafter\endcsname\csname if#1\endcsname
  }%
}
\skvnewdef*\skv@zapornot#1{%
  \if#1%
    \expandafter\skvzapspaces
  \else
    \expandafter\@iden
  \fi
}
\skvnewdef\skvzapspaces#1{\skv@zapspaces.#1 \zap@nil}
\skvnewdef\skv@zapspaces#1 #2\zap@nil{%
  \skvifblankTF{#2}{%
    \@gobble#1%
  }{%
    \skv@zapspaces#1#2\zap@nil
  }%
}
\skvnewdef\skvxzapspaces#1#2{%
  \edef#2{.#1}%
  \edef#2{\expandafter\skv@zapspaces#2 \zap@nil}%
}
% \skvifleadspaceTF{<toks>}{<true>}{<false>}
\newcommand\skvifleadspaceTF[3]{%
  \romannumeral\csname
  @\skvifnullTF{#1}{second}{\iffalse{\fi\skv@ifleadspace.#1 x}}%
  oftwo\endcsname{0 #2}{0 #3}%
}
\skvnewdef\skv@ifleadspace#1 {%
  \expandafter\skvifnullTF\expandafter{\@gobble#1}{first}{second}%
  \expandafter\@gobble\expandafter{\iffalse}\fi
}

% \skvifldspaceTF is faster than \skvifleadspaceTF.
%
% \skvifldspaceTF{ }{}{} gives <true> as desired.
\begingroup
\lccode`\&=0 \catcode`\&=7 \lccode`\!=0 \catcode`\!=8
\lowercase{\endgroup
  \skvnewdef\skvifldspaceTF#1{\skv@ifldspace!#1! &}
  \skvnewdef\skv@ifldspace#1! #2&{\skvifblankFT{#2}}
  \skvnewdef\skvtrimspace#1{\skv@trimspace@a.#1& &}
  \skvnewdef\skv@trimspace@a#1 &{\skv@trimspace@b#1&}
  \skvnewdef\skv@trimspace@b#1&#2{%
    \unexpanded\expandafter{%
      \romannumeral0%
      \expandafter\skvifldspaceTF\expandafter{\@gobble#1}{%
        \@gobble#1%
      }{%
        \expandafter\@space\@gobble#1%
      }%
    }%
  }
}
\skvnewdef\skvotrimspace{\expandafter\skvtrimspace\expandafter}
\skvnewdef\skvxtrimspace#1{%
  \expandafter\skvtrimspace\expandafter{\romannumeral-`\q#1}%
}
\skvrobustdef*\skvdespace#1#2{\edef#2{\skvtrimspace{#1}}}
\skvrobustdef*\skvdespacecontent#1{%
  \edef#1{\expandafter\skvtrimspace\expandafter{#1}}%
}
\skvnewdef*\skvcsuse#1{%
  \skvifcsname#1\then
    \csname#1\expandafter\endcsname
  \fi
}
\skvrobustdef*\skvcsdef#1{\expandafter\def\csname#1\endcsname}
\skvrobustdef*\skvcsgdef#1{\expandafter\gdef\csname#1\endcsname}
\skvrobustdef*\skvcsedef#1{\expandafter\edef\csname#1\endcsname}
\skvrobustdef*\skvcsxdef#1{\expandafter\xdef\csname#1\endcsname}
\skvnewdef\skvaftercsname#1#2{%
  \expandafter\skvswap\expandafter{\csname#2\endcsname}{#1}%
}
\skvnewlet\skvaftercs\skvaftercsname
\skvnewdef*\skvifdef#1\then{\if0\skvifdefTF{#1}{0}{1}}
\skvnewdef*\skvifundef#1\then{\if0\skvifdefTF{#1}{1}{0}}
% \skvifcsname x\then\def\x{T}\else\def\x{F}\fi
\skvnewdef*\skvifcsname#1\then{\if0\skvifcsdefTF{#1}{0}{1}}
\skvnewdef*\skvifdefTF#1{%
  \skvifxTF{#1}\skv@undefined{%
    \@secondoftwo
  }{%
    \ifx\relax#1%
      \expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
}
\skvnewdef*\skvifdefFT#1{\skvifdefTF{#1}\@secondoftwo\@firstoftwo}
\skvnewdef*\skvifcsdefTF#1{%
  \skvifblankTF{#1}{%
    \expandafter\@secondoftwo\@gobble
  }{%
    \ifcsname#1\endcsname
      \expandafter\@firstofone
    \else
      \expandafter\expandafter\expandafter
      \@secondoftwo\expandafter\@gobble
    \fi
  }{%
    \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
}
\skvnewdef*\skvifcsdefFT#1{\skvifcsdefTF{#1}\@secondoftwo\@firstoftwo}
% Don't check for blank #1. For internal use:
\skvnewdef*\skvifnamedefTF#1{%
  \ifcsname#1\endcsname
    \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\expandafter\expandafter\@secondoftwo
    \else
      \expandafter\expandafter\expandafter\@firstoftwo
    \fi
  \else
    \expandafter\@secondoftwo
  \fi
}
\skvnewdef*\skvifnamedefFT#1{\skvifnamedefTF{#1}\@secondoftwo\@firstoftwo}
\skvnewdef*\skv@ifx@#1#2\skv@ifx@nil{\expandafter#1}
\skvnewdef*\skv@ifx@@#1#2\skv@ifx@nil{#1}
\skvnewdef*\skvifxTF#1#2{%
  \csname @\expandafter\expandafter\expandafter
  \ifx\skv@ifx@#1\batchmode\skv@ifx@nil\skv@ifx@@#2\noboundary\skv@ifx@nil
  first\else second\fi oftwo\endcsname
}
\skvnewdef*\skvifxFT#1#2{\skvifxTF{#1}{#2}\@secondoftwo\@firstoftwo}
\skvnewdef*\skv@ghost{\@gobble\skv@ghost}
\skvnewdef\skvifemptyTF#1{%
  \ifx#1\@empty\skv@ghost
  \expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
}
\skvnewdef\skvifcsemptyTF#1{\expandafter\skvifemptyTF\csname#1\endcsname}
\skvnewdef\skvifdefemptyTF#1{%
  \skvifblankTF{#1}\@secondoftwo{%
    \skvifntypeTF{#1}{%
      \skvifdefTF{#1}{\skvifxTF#1\@empty}{\@secondoftwo}%
    }{%
      \@secondoftwo
    }%
  }%
}
\begingroup
% Keep lccode, in case the test occurs in a table:
\lccode`\&=0 \catcode`\&=8
\lowercase{\endgroup
  \skvnewdef\skvifnullTF#1{%
    \csname @\ifcat&\detokenize{#1}&first\else second\fi oftwo\endcsname
  }
  \skvnewdef\skviflacus#1\then{\ifcat&\detokenize{#1}&}
}
\skvnewdef\skvifblankTF#1{%
  \expandafter\skvifnullTF\expandafter{\@gobble#1.}%
}
\skvnewdef\skvifblankFT#1{\skvifblankTF{#1}\@secondoftwo\@firstoftwo}

\skvnewdef*\skvifboolTF#1{%
  \skvifblankTF{#1}{%
    \@secondoftwo
  }{%
    \skvifcsdefTF{if#1}{%
      \csname @\csname if#1\endcsname
        first\else second\fi oftwo\endcsname
    }{%
      \skv@err{Undefined boolean '#1'}\skv@ehd
    }%
  }%
}
\skvnewdef*\skvifboolFT#1{\skvifboolTF{#1}\@secondoftwo\@firstoftwo}
% \skvifbool sw1\then <true> \else <false> \fi
\skvnewdef*\skvifbool#1\then{\if0\skvifboolTF{#1}01}
\skvnewdef*\skvifdefboolTF#1{%
  \csname @\csname if#1\endcsname first\else second\fi oftwo\endcsname
}
\skvnewdef*\skvifdefboolFT#1{\skvifdefboolTF{#1}\@secondoftwo\@firstoftwo}
\skvrobustdef*\skvaftergroupifboolTF#1\endgroup{%
  \skvifboolTF{#1}{\endgroup\@firstoftwo}{\endgroup\@secondoftwo}%
}
\skvrobustdef*\skvaftergroupifboolFT#1\endgroup{%
  \skvifboolTF{#1}{\endgroup\@secondoftwo}{\endgroup\@firstoftwo}%
}
% \skvifboolvalTF{<toks>}{<true>}{<false>}
\skvrobustdef*\skvifboolvalTF#1{%
  \skvxifinTF{,\expandafter\skvtrimspace\expandafter
    {\detokenize{#1}},}{,\detokenize{true,false},}%
}
\skvrobustdef*\skvxifboolvalTF#1{%
  \begingroup
  \edef\skv@prova{#1}%
  \skvdespacecontent\skv@prova
  \skvexpandtwoargs{\endgroup\skvifinTF}
    {,\skvoxdetok\skv@prova,}{,\detokenize{true,false},}%
}
% Generate error if <toks> is not a valid boolean value, otherwise
% execute #2:
% \skvifboolvalT{<toks>}{<true>}
\skvrobustdef*\skvifboolvalT#1#2{%
  \skvxifinTF{,\expandafter\skvtrimspace\expandafter
    {\detokenize{#1}},}{,\detokenize{true,false},}%
    {#2}{\skv@badboolerr{#1}}%
}
% Convert bool value (true or false) to switch value (00 or 01):
\skvrobustdef*\skvbooltoswitch#1#2{%
  \begingroup
  \def\reserved@a##1#1##2##3\skv@nil{%
    \def#2{##2}%
    \ifx#2\@nnil
      \skv@err{Bad boolean value '#1' can't be
        \MessageBreak converted to switch value}\@ehc
    \fi
  }%
  \reserved@a true{00}false{01}#1{\@nil}\skv@nil
  \skvaftergroupdef#2\endgroup
}
\skvrobustdef*\skv@badboolerr#1{%
  \skv@err{Invalid boolean value '#1'; expected 'true' or 'false'}\skv@ehd
}

% Switches have values of either 00 or 01.

% \skvifknobTF, unlike \skvifswitchTF, is for use with plain switches,
% ie, switches that have no separate namespace.
\skvnewdef*\skvifknobTF#1{%
  \if\@nameuse{#1}\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
}
\skvnewdef*\skvifknobFT#1{%
  \if\@nameuse{#1}\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi
}
% Switches and toggles have separate namespaces.
\skvrobustdef*\skvnewswitches#1{%
  \skvcommaloop{#1}\skv@prova{%
    \skvifcsdefTF{skv@switch@\skv@prova}{%
      \skv@err{Switch '\skvoxdetok\skv@prova' already exists}\skv@ehd
    }{%
      \skvcsdef{skv@switch@\skv@prova}{01}%
    }%
  }%
}
\skvnewlet\skvnewswitch\skvnewswitches
\skvnewdef*\skvifswitchTF#1{%
  \if
  \skvifcsdefTF{skv@switch@#1}{%
    \csname skv@switch@#1\endcsname
  }{%
    01%
  }%
  \expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
}
\skvnewdef*\skvifdefswitchTF#1{%
  \if\csname skv@switch@#1\endcsname
  \expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
}
\skvrobustdef*\skvswitchtrue#1{%
  \skvifcsdefTF{skv@switch@#1}{%
    \skvcsdef{skv@switch@#1}{00}%
  }{%
    \skv@err{No switch '\detokenize{#1}'}\skv@ehd
  }%
}
\skvrobustdef*\skvswitchfalse#1{%
  \skvifcsdefTF{skv@switch@#1}{%
    \skvcsdef{skv@switch@#1}{01}%
  }{%
    \skv@err{No switch '\detokenize{#1}'}\skv@ehd
  }%
}
\skvrobustdef*\skvnewtog#1{%
  \skvcommaloop{#1}\skv@prova{%
    \skvifcsdefTF{skv@toggle@\skv@prova}{%
      \skv@err{Switch '\skvoxdetok\skv@prova' already exists}\skv@ehd
    }{%
      \skvcslet{skv@toggle@\skv@prova}\@secondoftwo
    }%
  }%
}
\skvrobustdef*\skvdeftog#1{%
  \skvcommaloop{#1}\skv@prova{%
    \skvcslet{skv@toggle@\skv@prova}\@secondoftwo
  }%
}
\skvnewdef*\skviftogTF#1{%
  \skvifcsdefTF{skv@toggle@#1}{%
    \csname skv@toggle@#1\endcsname
  }{%
    \@secondoftwo
  }%
}
\skvnewdef*\skviftogFT#1{\skviftogTF{#1}\@secondoftwo\@firstoftwo}
\skvnewdef*\skvifdeftogTF#1{\csname skv@toggle@#1\endcsname}
\skvrobustdef*\skvsettogtrue#1{%
  \skvifcsdefTF{skv@toggle@#1}{%
    \skvcslet{skv@toggle@#1}\@firstoftwo
  }{%
    \skv@err{No toggle '\detokenize{#1}'}\skv@ehd
  }%
}
\skvrobustdef*\skvsettogfalse#1{%
  \skvifcsdefTF{skv@toggle@#1}{%
    \skvcslet{skv@toggle@#1}\@secondoftwo
  }{%
    \skv@err{No toggle '\detokenize{#1}'}\skv@ehd
  }%
}
% Allow 'f' to stop the search for number:
\skvnewdef\skvifcondTF#1\fi{%
  \csname @#1first\else second\fi oftwo\endcsname
}
\skvnewdef\skvifcondFT#1\fi{\skvifcondTF{#1}\fi\@secondoftwo\@firstoftwo}
% In case #1 isn't expandable. This is the difference between
% \skvifcondTF and \skvifconditionTF.
\skvnewdef\skvifconditionTF#1\fi{%
  #1\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\skvnewdef*\skvifnumTF#1#{\skvifcondTF\ifnum#1\fi}
\skvnewdef*\skvifdim#1#{\skvifcondTF\ifdim#1\fi}
\skvnewdef*\skvifnumFT#1#{\skvifnumTF#1{\@secondoftwo}{\@firstoftwo}}
\skvnewdef\skvalloftwo#1#2{#1#2}
% If '#1' is a single, non-space and non-braced token:
\skvnewdef\skvifntypeTF#1{%
  \csname @\if0\skv@strcmp
  {\skvexpandonce{\skvalloftwo#1{}{}}}{\unexpanded{#1{}}}%
  first\else second\fi oftwo\endcsname
}
\skvnewdef\skvxifntypeTF{\skvexpandarg\skvifntypeTF}
\skvrobustdef*\skvundef#1{\let#1\@undefined}
\skvrobustdef*\skvgundef#1{\global\let#1\@undefined}
\skvrobustdef*\skvcsundef#1{\skvcslet{#1}\@undefined}
\skvrobustdef*\skvcsgundef#1{\global\skvcslet{#1}\@undefined}
\skvrobustdef*\skvemptify#1{\skv@commaact{#1}{\def##1{}}}
\skvrobustdef*\skvinizero#1{\skv@commaact{#1}{\def##1{0}}}
\skvrobustdef*\skvundefcmdlist#1{%
  \skvcommaparse{#1}\skv@prova{\expandafter\skvundef\skv@prova}%
}
\skvrobustdef*\skvemptifycmds#1{%
  \skvcommaparse{#1}\skv@prova{\expandafter\def\skv@prova{}}%
}
% \skv@addtocollection{<toks>}
%
% Collect tokens in a group for later exiting the group with them:
%
\skvrobustdef*\skv@addtocollection#1{%
  \edef\skv@collection{%
    \ifdefined\skv@collection\skvexpandonce\skv@collection\fi
    \unexpanded{#1}%
  }%
}
% Don't use \do for \dl, in case \do appears as a garbage:
% \skvgarbageitems{\dl<cmd1>\gdl<cmd2>...}
\skvrobustdef*\skvgarbageitems{\skvappto\skv@garbagelist}
\skvrobustdef*\skvdumpgarbage{%
  \let\gdl\skvgundef\let\dl\skvundef
  \skv@garbagelist
  \def\skv@garbagelist{}%
}

\skvifdefTF\pdfstrcmp{%
  \let\skv@strcmp\pdfstrcmp
}{%
  \RequirePackage{pdftexcmds}%
  \skvifdefTF\pdf@strcmp{%
    \let\skv@strcmp\pdf@strcmp
  }{%
    \skv@err{Neither '\string\pdfstrcmp' nor '\string\pdf@strcmp' exists}\skv@ehd
  }%
}
\skvnewdef\skvifstrcmpTF#1#2{%
  \csname @\ifnum\skv@strcmp{\detokenize{#1}}%
    {\detokenize{#2}}=0first\else second\fi oftwo\endcsname
}
\skvnewdef*\skvifstrcmpFT#1#2{\skvifstrcmpTF{#1}{#2}\@secondoftwo\@firstoftwo}
\skvnewdef\skvifstreq#1#2\then{%
  \ifnum\skv@strcmp{\detokenize{#1}}{\detokenize{#2}}=\skvz@
}
\skvnewdef\skvoifstrcmpTF#1#2{%
  \csname @\ifnum\skv@strcmp{\skvexpandonce{#1}}%
    {\skvexpandonce{#2}}=0first\else second\fi oftwo\endcsname
}
\skvnewdef\skvxifstrcmpTF#1#2{%
  \csname @\ifnum\skv@strcmp{#1}{#2}=0first\else
    second\fi oftwo\endcsname
}
\skvrobustdef\skvcslet#1#2{\expandafter\let\csname#1\endcsname#2}
\skvrobustdef\skvnewcslet#1{%
  \skvifcsdefTF{#1}{%
    \skv@err{Command '\skvnoexpandcs{#1}' already defined}\skv@ehd
  }{%
    \skvcslet{#1}%
  }%
}
\skvrobustdef\skvletcs#1#2{%
  \begingroup\expandafter\endgroup\expandafter
  \let\expandafter#1\csname#2\endcsname
}
\skvrobustdef\skvnewletcs#1{%
  \skvifdefTF{#1}{%
    \skv@err{Command '\string#1' already defined}\skv@ehd
  }{%
    \skvletcs#1%
  }%
}
\skvrobustdef*\skvcsletcs#1#2{%
  \begingroup\expandafter\endgroup
  \expandafter\let\csname#1\expandafter
  \endcsname\csname#2\endcsname
}
\skvrobustdef\skvnewcsletcs#1{%
  \skvifcsdefTF{#1}{%
    \skv@err{Command '\skvnoexpandcs{#1}' already defined}\skv@ehd
  }{%
    \skvcsletcs{#1}%
  }%
}
\skvrobustdef*\skvglobalizecs#1{%
  \begingroup\expandafter\endgroup\expandafter
  \global\expandafter\let\csname#1\expandafter\endcsname
  \csname#1\endcsname
}
\skvrobustdef*\skvaftergroupdef#1\endgroup{%
  \skvexpanded{\endgroup\skvcmdexit#1}%
}
\skvrobustdef*\skvaftergroupcsdef#1\endgroup{%
  \skvexpanded{\endgroup\expandafter\skvcmdexit\csname#1\endcsname}%
}

% Taking commands and booleans out of a local group under \edef:
\skvnewdef*\skvcmdexit#1{%
  \skvifdefTF{#1}{%
    \edef\noexpand#1{\noexpand\unexpanded{\skvexpandonce{#1}}}%
  }{}%
}
\skvnewdef*\skvcsexit#1{%
  % If #1 is undefined, \skvexpandcsonce will make it relax. The
  % preliminary test in \skvcmdexit will deal with that situation.
  \skvaftercs\skvcmdexit{#1}%
}
% \edef\x{\endgroup\skvcmdexitloop{\x\y}}:
\skvnewdef*\skvcmdexitloop#1{\skv@cmdexitloop#1\end}
\skvnewdef*\skv@cmdexitloop#1{%
  \ifx\end#1\else\skvcmdexit{#1}\expandafter\skv@cmdexitloop\fi
}
\skvnewdef*\skvboolexit#1{%
  \expandafter\noexpand\csname\expandafter\@gobblethree
  \string#1#1true\else false\fi\endcsname
}
% \edef\x{\endgroup\skvboolexitloop{\ifboola\ifboolb}}:
\skvnewdef*\skvboolexitloop#1{\skv@boolexitloop#1\end}
\skvnewdef*\skv@boolexitloop#1{%
  \ifx\end#1\else\skvboolexit{#1}\expandafter\skv@boolexitloop\fi
}

\skvnewdef*\skvprotect#{%
  \ifx\protect\@typeset@protect\skv@protect\@firstofone\fi
  \ifx\protect\@unexpandable@protect\skv@protect\skvunexpandable\fi
  \ifx\protect\noexpand\skv@protect\unexpanded\fi
  \ifx\protect\string\skv@protect\detokenize\fi
  \relax\@firstofone
}
\skvnewdef*\skv@protect#1#2\relax\@firstofone{\fi#1}
\skvnewdef*\skvunexpandable#1{\unexpanded{\skvprotect{#1}}}
\skvrobustdef\skvifnotnil#1{%
  \begingroup
  \edef\skv@prova{\unexpanded{#1}}%
  \expandafter\endgroup\ifx\skv@prova\skv@nnil
  \expandafter\@gobble\else\expandafter\@firstofone\fi
}
% \skvadvanceno{<cmd>}{<number>}
\skvrobustdef*\skvsetnumber#1{%
  \begingroup
  \def\x{\edef\x{\endgroup\def\noexpand#1{\the\count@}}\x}%
  \afterassignment\x\count@
}
\skvnewlet\skvsetno\skvsetnumber
% \skvadvanceno{<cmd>}{<number>}
\skvrobustdef*\skvadvanceno{\skv@advanceno\relax}
\skvrobustdef*\skvgadvanceno{\skv@advanceno\global}
\skvrobustdef*\skv@advanceno#1#2#3{%
  % Raise error if #3 isn't an integer, \chardef'd or \countdef'd:
  \begingroup
  \count@#3\relax
  \endgroup
  \skvifdefTF#2{%
    #1\edef#2{\the\numexpr#2+#3\relax}%
  }{%
    \skv@err{Number '\string#2' is not defined}\skv@ehd
  }%
}
\skvrobustdef*\skvpushnumber#1{%
  \skvifdefTF#1{%
    \edef#1{\the\numexpr#1+1\relax}%
  }{%
    \def#1{0}%
  }%
}
\skvrobustdef*\skvpopnumber#1{%
  \skvifdefTF#1{%
    \edef#1{\the\numexpr#1+1\relax}%
  }{%
    \skv@err{Number '\string#1' is not defined}\skv@ehd
  }%
}

\skvrobustdef\skv@testst#1{%
  \skvifstar{\skv@tempsttrue#1}{\skv@tempstfalse#1}%
}
% For internal use:
\skvrobustdef\skv@i@ifstar#1{\@ifnextchar*{\@firstoftwo{#1}}}
\skvrobustdef\skv@i@testst#1{%
  \skv@i@ifstar{\skv@tempsttrue#1}{\skv@tempstfalse#1}%
}
\skvrobustdef\skv@testcl#1{%
  \skvifnextchar!{\skv@cltrue#1}{\skv@clfalse#1}%
}
\skvrobustdef\skv@teststopt#1#2{\skv@testst{\skv@testopt{#1}{#2}}}

% Remove spurious leading and trailing spaces before checking for outer brace.
% Such spaces do hide the outer brace.
% If we were to use \skvtrimspace for \skvifbracedTF, then the need
% for double \romannumeral will cause problems of premature expansion.
\begingroup
\lccode`\&=0 \catcode`\&=7
\skvnewgdef\skvifbracedTF#1{%
  \expandafter\skv@ifbraced@a\expandafter{%
    \romannumeral-`\q\skv@ifbraced@b.#1& &%
  }%
}
\skvnewgdef\skv@ifbraced@a#1{\skv@ifbraced@d#1\brace@nil{#1}}
\skvnewgdef\skv@ifbraced@b#1 &{\skv@ifbraced@c#1&}
\skvnewgdef\skv@ifbraced@c#1&#2{%
  \expandafter\skvifldspaceTF\expandafter{\@gobble#1}%
    {\@gobble#1}{\expandafter\@space\@gobble#1}%
}
\skvnewgdef\skv@ifbraced@d#1\brace@nil#2{%
  \skvifstrcmpTF{#1}{#2}\@secondoftwo\@firstoftwo
}
\endgroup

\skvnewdef\skvifbracedFT#1{\skvifbracedTF{#1}\@secondoftwo\@firstoftwo}

% \skvstripouterbraces{<nr>}<cmd>
% Example:
% \def\x{{{{X}}}}
% \skvstripouterbraces{2}\x
\skvrobustdef*\skvstripouterbraces#1#2{%
  \skvifemptyTF#2{}{%
    \begingroup
    \@tempcnta\skvz@
    \expandafter\skv@stripouterbraces#2\strip@nil{#2}{#1}%
  }%
}
\skvrobustdef*\skv@stripouterbraces#1\strip@nil#2#3{%
  \edef\skv@prova{\unexpanded{#1}}%
  \skvifxTF#2\skv@prova{%
    \skvaftergroupdef#2\endgroup
  }{%
    \advance\@tempcnta\@ne
    \skvifnumTF\@tempcnta=#3{%
      \let#2\skv@prova
      \skvaftergroupdef#2\endgroup
    }{%
      \let#2\skv@prova
      \expandafter\skv@stripouterbraces#2\strip@nil{#2}{#3}%
    }%
  }%
}
\skvrobustdef*\skvifescapedTF#1{%
  \begingroup\escapechar92\relax
  \edef\x{\expandafter\skv@car\string#1x\car@nil}%
  \expandafter\endgroup
  \csname @\ifx\x\@backslashchar first\else second\fi oftwo\endcsname
}
\skvnewdef\skvifescapedFT#1{\skvifescapedTF{#1}\@secondoftwo\@firstoftwo}
\skvnewdef*\skvremovescape#1{\expandafter\@gobble\string#1}
\skvnewdef*\skvgobblescape#1{%
  \skvifblankTF{#1}{}{%
    \skvifnumTF\escapechar>255{\string#1}{%
      \skvifnumTF\escapechar<0{\string#1}{%
        \skvifnumTF\escapechar=32{%
          \expandafter\@gobblespace\string#1%
        }{%
          \skvremovescape{#1}%
        }%
      }%
    }%
  }%
}
\skvnewdef*\skvoxdetok#1{\detokenize\expandafter{#1}}
\skvnewdef*\skvexpandonce#1{\unexpanded\expandafter{#1}}
\skvnewlet\skvxonce\skvexpandonce
\skvnewlet\skvxaft\expandafter
\skvnewdef*\skvexpandtwice#1{%
  \unexpanded\expandafter\expandafter\expandafter{#1}%
}
\skvnewdef*\skvexpandthrice#1{%
  \unexpanded\expandafter\expandafter\expandafter
  \expandafter\expandafter\expandafter\expandafter{#1}%
}
\skvnewdef*\skvnoexpandcs#1{\skvexpandonce{\csname#1\endcsname}}
\skvnewdef*\skvexpandcsonce#1{%
  \expandafter\skvexpandonce\expandafter{\csname#1\endcsname}%
}
\skvnewdef*\skvexpandcstwice#1{%
  \expandafter\skvexpandtwice\expandafter{\csname#1\endcsname}%
}
\skvnewdef*\skvexpandcsthrice#1{%
  \expandafter\skvexpandthrice\expandafter{\csname#1\endcsname}%
}
\skvrobustdef\skvexpanded#1{\begingroup\edef\x{\endgroup#1}\x}
\skvrobustdef\skvexpandarg#1#2{\skvexpanded{\unexpanded{#1}{#2}}}
\skvrobustdef\skvexpandargonce#1#2{%
  \skvexpanded{\unexpanded{#1}{\skvexpandonce{#2}}}%
}
\skvrobustdef*\skvexpandtwoargs#1#2#3{\skvexpanded{\unexpanded{#1}{#2}{#3}}}
\skvrobustdef*\skvexpandtwoargsonce#1#2#3{%
  \skvexpanded{\unexpanded{#1}{\skvexpandonce{#2}}{\skvexpandonce{#3}}}%
}
\skvrobustdef\skvexpandsecond#1#2{\skvexpanded{\unexpanded{#1}#2}}
\skvrobustdef\skvexpandsecondonce#1#2{%
  \skvexpanded{\unexpanded{#1}\skvexpandonce{#2}}%
}
\skvnewdef\skvexpandnext#1#2{\expandafter\skvswap\expandafter{#2}{#1}}
\skvnewdef\skvexpandbracenext#1#2{%
  \expandafter\skvswap\expandafter{\expandafter{#2}}{#1}%
}
\skvnewlet\skvexpbracenext\skvexpandbracenext
% Eg, \skvexpandintonext\x[\y], \skvexpandintonext\x{\y}.
% This isn't expandable, because #1 may not be just one token.
\skvnewdef\skvexpandintonext#1{%
  \begingroup
  \edef\reserved@a{\endgroup\unexpanded{#1}}%
  \expandafter\reserved@a\expandafter
}
\skvrobustdef*\skvifinTF#1#2{%
  \skvtestifin{#1}{#2}%
  \csname @\ifin@ first\else second\fi oftwo\endcsname
}
\skvrobustdef*\skvifinFT#1#2{\skvifinTF{#1}{#2}\@secondoftwo\@firstoftwo}
\skvrobustdef*\skvxifinTF#1#2{\skvexpandtwoargs\skvifinTF{#1}{#2}}
\skvrobustdef*\skvxifinFT#1#2{\skvxifinTF{#1}{#2}\@secondoftwo\@firstoftwo}
\skvrobustdef*\skvifindetokTF#1#2#3{%
  \skvexpandtwoargs\skvifinTF{#1\skvoxdetok{#2}#1}{#1\skvoxdetok{#3}#1}%
}
\skvnewdef\skviffound#1\in#2\then{\skvtestifin{#1}{#2}\ifin@}
\skvnewdef\skvxiffound#1\in#2\then{\skvexpandtwoargs\skvtestifin{#1}{#2}\ifin@}

% \skv@kvsplit{<kvpair>}{<parametered.callback>}
\skvrobustdef*\skv@kvsplit#1#2{%
  \begingroup
  \def\skv@tempa##1=##2=##3\skv@kvsplit{\endgroup#2}%
  \skv@tempa#1==\skv@kvsplit
}
\skvrobustdef*\skv@okvsplit#1{\skvexpbracenext\skv@kvsplit{#1}}
% \skv@slashsplit{<slashlist>}{<parametered.callback>}
% Patrons calling \skv@slashsplit should note that it may return
% ^skv^ for any missing components:
\skvrobustdef*\skv@slashsplit#1#2{%
  \begingroup
  \def\skv@tempa##1/##2/##3/##4/##5/##6/##7/##8/##9\skv@slashsplit{%
    \endgroup#2%
  }%
  \skv@tempa#1/^skv^/^skv^/^skv^/^skv^/^skv^/^skv^/^skv^/^skv^\skv@slashsplit
}
\skvrobustdef*\skv@oslashsplit#1{\skvexpbracenext\skv@slashsplit{#1}}

% \skv@splitpath@a{<path.macro>}{<pref.macro>}{<fam.macro>}
% Here, <path.macro> has the form {<pref>/<fam>}.
\skvrobustdef*\skv@splitpath@a#1#2#3{%
  \begingroup
  \ifx#1\@empty
    \skv@err{No key can have empty path}\skv@ehd
  \else
    \skv@oslashsplit{#1}{%
      \edef#2{\skvtrimspace{##1}}%
      \edef#3{\skvtrimspace{##2}}%
      \skvstripouterbraces{2}#2%
      \skvstripouterbraces{2}#3%
      \ifx#3\skv@rej
        \let#3#2%
        \let#2\skvdefaultprefix
      \fi
    }%
  \fi
  \skvexpanded{\endgroup\skvcmdexit#2\skvcmdexit#3}%
}
% \skv@splitpath@b{<path.macro>}{<pref.macro>}{<fam.macro>}
% Here, <path.macro> has the form {<pref>}{<fam>}.
% Here, we don't expect to find empty entries in #1, since
% \skv@splitpath@a wouldn't have made such an entry in #1. But don't
% mind, let us still test for empty.
\skvrobustdef*\skv@splitpath@b#1#2#3{%
  \begingroup
  \def\skv@prova##1##2\@nil{%
    \edef#2{\skvtrimspace{##1}}%
    \edef#3{\skvtrimspace{##2}}%
    \ifx#3\@empty
      \let#3#2%
      \let#2\skvdefaultprefix
    \fi
  }%
  \expandafter\skv@prova#1\@nil
  \skvexpanded{\endgroup\skvcmdexit#2\skvcmdexit#3}%
}
% \skv@formatpaths{<paths>}{<macro.to.reveive.formated.paths>}
%
% Format <paths> given in the form
%
%   {<pref1>/<fam1>},...,{<pref-n>/<fam-n>}
%
% into
%
%   \skv@pathdo{<pref1>}{<fam1>}...\skv@pathdo{<pref-n>}{<fam-n>}
%
\skvrobustdef*\skv@formatpaths#1#2{%
  \begingroup
  \skvifdefTF#2{}{\def#2{}}%
  \edef\skv@prova{#1}%
  \skvcsvnormalize[/]\skv@prova
  \skvcommaparse*\skv@prova\skv@prova{%
    \skv@splitpath@a\skv@prova\skv@tempa\skv@tempb
    \edef\skv@prova{{\skv@tempa}{\skv@tempb}}%
    \skvxifinTF{\skvoxdetok\skv@prova}{\skvoxdetok{#2}}{}{%
      \edef#2{\skvexpandonce#2\noexpand\skv@pathdo\skv@prova}%
    }%
  }%
  \skvaftergroupdef#2\endgroup
}
% \skv@makepaths{<prefix.macro>}{<families.macro>}{<pathlist.macro>}
%    {<wrapper.macro>}
%
% Attach prefix to families, to make pathlist. <prefix> must contain
% only one element.
%
\skvrobustdef*\skv@makepaths#1#2#3#4{%
  \begingroup
  \skv@ifnoprefix#1{\let#1\skvdefaultprefix}{}%
  \edef\skv@pref{#1}%
  \skvdespacecontent\skv@pref
  \skvstripouterbraces{2}\skv@pref
  \skv@ifoneprefix\skv@pref{%
    \skvifdefTF#3{}{\def#3{}}%
    \skvcommaparse*#2\skv@prova{%
      \skvstripouterbraces{2}\skv@prova
      \edef\skv@prova{{\skv@pref}{\skv@prova}}%
      \skvxifinTF{\skvoxdetok\skv@prova}{\skvoxdetok{#3}}{}{%
        \edef#3{\skvexpandonce{#3}\noexpand#4\skv@prova}%
      }%
    }%
  }{%
    \skv@err{Only one prefix allowed here}
      {The service you've called takes only one key prefix}%
  }%
  \skvaftergroupdef#3\endgroup
}
% \skv@ifoneprefix{<prefix>}
\skvrobustdef*\skv@ifoneprefix#1{%
  \skvxifinTF{,}{\skvoxdetok{#1}}{%
    \begingroup
    \def\skv@prova##1,##2\skv@nil{%
      \endgroup
      \skvifblankTF{##2}{%
        \def#1{##1}%
      }{%
        \@secondoftwo
      }%
    }%
    \expandafter\skv@prova#1\skv@nil
  }{%
    \@firstoftwo
  }%
}
% \skv@ifnoprefix{<prefix.macro>}
\skvrobustdef*\skv@ifnoprefix#1{%
  % Think twice before changing this conditional!
  \ifcase0%
    \ifx#1\skv@undefined\else\ifx#1\@empty\else 1\fi\fi\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\skvrobustdef*\skvifmacroTF#1{%
  \skvifntypeTF{#1}{%
    \begingroup
    \edef\skv@tempa##1{\def##1####1\detokenize{macro}:####2\skvrelax}%
    \skv@tempa\skv@tempa{%
      \expandafter\endgroup\ifx\@nnil##2\@nnil
        \expandafter\@secondoftwo
      \else
        \expandafter\@firstoftwo
      \fi
    }%
    \edef\skv@tempb##1{##1\detokenize{macro}:\skvrelax}%
    \skv@tempb{\expandafter\skv@tempa\meaning#1}%
  }{%
    \@secondoftwo
  }%
}
\skvrobustdef*\skvifmacroFT#1{\skvifmacroTF{#1}\@secondoftwo\@firstoftwo}
% Note: If there're more than 1 alpha/Alpha character, both \skvifloweralpha
% and \skvifupperalpha will return false. Hence double (or more) aphabetic
% characters can't be auto-completed by \skvautocompletelist.
\skvnewdef*\skvifloweralpha#1{%
  \skvifblankTF{#1}{%
    \@secondoftwo
  }{%
    \skvifntypeTF{#1}{%
      \skvifnumTF`#1>96{%
        \skvifnumTF`#1<123{\@firstoftwo}{\@secondoftwo}%
      }{%
        \@secondoftwo
      }%
    }{%
      \@secondoftwo
    }%
  }%
}
\skvnewdef*\skvifupperalpha#1{%
  \skvifblankTF{#1}{%
    \@secondoftwo
  }{%
    \skvifntypeTF{#1}{%
      \skvifnumTF`#1>64{%
        \skvifnumTF`#1<91{\@firstoftwo}{\@secondoftwo}%
      }{%
        \@secondoftwo
      }%
    }{%
      \@secondoftwo
    }%
  }%
}
% If there is a digit present in #1:
\skvnewdef*\skvifdigitpresentTF#1{%
  \skvifcondTF\if0\skvifblankTF{#1}{1}{\skv@ifdigitpresent#1\skv@nnil}\fi
}
\skvnewdef*\skv@ifdigitpresent#1{%
  \skvifxTF#1\skv@nnil{%
    1%
  }{%
    \skvifnumTF`#1>47{%
      \skvifnumTF`#1<58{%
        0\skv@removetonnil
      }{%
        \skv@ifdigitpresent
      }%
    }{%
      \skv@ifdigitpresent
    }%
  }%
}

\skvnewdef*\skvifalldigitTF#1{%
  \skvifcondTF\if0\skvifblankTF{#1}{1}{\skv@ifalldigit#1\skv@nnil}\fi
}
\skvnewdef*\skv@ifalldigit#1{%
  \skvifxTF#1\skv@nnil{0}{%
    \skvifnumTF`#1>47{%
      \skvifnumTF`#1<58{%
        \skv@ifalldigit
      }{%
        1\skv@removetonnil
      }%
    }{%
      1\skv@removetonnil
    }%
  }%
}

\skvnewdef*\skvifalphapresentTF#1{%
  \skvifcondTF\if0\skvifblankTF{#1}{1}{\skv@ifalphapresent#1\skv@nnil}\fi
}
\skvnewdef*\skv@ifalphapresent#1{%
  \skvifxTF#1\skv@nnil{%
    1%
  }{%
    \skvifnumTF`#1>96{%
      \skvifnumTF`#1<123{%
        0\skv@removetonnil
      }{%
        \skv@ifalphapresent
      }%
    }{%
      \skv@ifalphapresent
    }%
  }%
}
\skvnewdef*\skvifAlphapresentTF#1{%
  \skvifcondTF\if0\skvifblankTF{#1}{1}{\skv@ifAlphapresent#1\skv@nnil}\fi
}
\skvnewdef*\skv@ifAlphapresent#1{%
  \skvifxTF#1\skv@nnil{%
    1%
  }{%
    \skvifnumTF`#1>64{%
      \skvifnumTF`#1<91{%
        0\skv@removetonnil
      }{%
        \skv@ifAlphapresent
      }%
    }{%
      \skv@ifAlphapresent
    }%
  }%
}
\skvnewdef*\skvifprimitiveTF#1{%
  \expandafter\skv@ifprimitive\meaning#1\relax
}
\skvnewdef*\skv@ifprimitive#1#2\relax{%
  \skvifcondTF\if#1\@backslashchar\fi{%
    \skvifdigitpresentTF{#2}\@secondoftwo\@firstoftwo
  }{%
    \@secondoftwo
  }%
}

\begingroup
\catcode`\&=7
\skvnewgdef*\skvdefregistertester#1#2{%
  \begingroup
  \def\x##1{\skvnoexpandcs{skv@\skvremovescape#1test@##1}}%
  \edef\x{\endgroup
    \def\noexpand#2####1{%
      \unexpanded{\skvifxTF#1{##1}\@secondoftwo}{%
        \unexpanded{\skvifprimitiveTF{##1}\@secondoftwo}%
        {\noexpand\expandafter\x{a}\noexpand\meaning####1:&}%
      }%
    }%
    \def\x{a}####1:####2&{\x{b}####1\string#1&}%
    \def\x{b}####1\string#1####2&{\noexpand\skvifblankTF{####1}}%
  }\x
}
\endgroup
\skvdefregistertester\skip\skvifskipTF
\skvdefregistertester\count\skvifcountTF
\skvdefregistertester\dimen\skvifdimenTF
\skvdefregistertester\toks\skviftoksTF

% Converting units.
% Examples:
%  \edef\x{\skvconvertunit{10pt}{mm}}
%  \edef\x{\skvconvertunit{1in}{bp}}
\skvnewdef*\skvconvertunit#1#2{%
  \strip@pt\dimexpr#1*\p@/\dimexpr1#2\relax\relax#2%
}

% If all the tokens are digits or arithmetic:
\skvnewdef*\skvifallarithmeticTF#1{%
  \begingroup
  \skv@swatrue
  \skvifdimensionable{#1}{}{%
    \ifskv@isinteger\else
      \def\do##1##2{%
        \ifx\do##1\else
          \skvifinTF{##1}{0123456789.+-*/()}{}{%
            \skvifinTF{,##1##2,}
              {,em,ex,in,pt,pc,cm,mm,dd,cc,nd,nc,bp,sp,}{}{%
              \skv@swafalse
              \def\do####1\skvrelax{}%
            }%
          }%
          \expandafter\do
        \fi
        ##2%
      }%
      \do#1\do\skvrelax
    \fi
  }%
  \expandafter\endgroup\ifskv@swa
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}

\skvnewregister\bool{\ifskv@isinteger}

% In case the argument of \skvifintegerTF containes \numexpr:
\skvnewlet\skv@catch@nil\relax
% \skvensureinteger{<essence>}{<test token>}
\skvrobustdef*\skvensureinteger#1#2{%
  \begingroup
  \def\skv@prova##1\skv@catch@nil{%
    % If ##1 is empty or contains nothing before a \relax, it's fine:
    \ifx\relax##1\relax\else
      \skv@err{Token '#2' for '#1' isn't an integer}\skv@ehd
    \fi
  }%
  \afterassignment\skv@prova\skv@cnta#2\relax\skv@catch@nil
  \endgroup
}
\skvnewdef*\skv@validunit{em,ex,in,pt,pc,cm,mm,dd,cc,nd,nc,bp,sp}
\skvrobustdef*\skv@catchremainder#1\skv@catch@nil{%
  \endgroup\def\skv@elt{#1}%
}
\skvrobustdef*\skvifintegerTF#1{%
  \begingroup
  % Don't try '\numexpr0+#1' here:
  \afterassignment\skv@catchremainder
  \@tempcnta\numexpr0#1\relax\skv@catch@nil
  \skvifxTF\skv@elt\@empty{%
    \@firstoftwo
  }{%
    \skvifxTF\skv@elt\skv@relaxtoks\@firstoftwo\@secondoftwo
  }%
}
\skvrobustdef\skvoifinteger{\skvexpbracenext\skvifintegerTF}

% Test if a token #1 can be assigned to a \dimendef'd register. We assume
% that #1 isn't a complicated expression and isn't padded with trailing
% \relax's. A complicated expression will be something like
%
%       2pt+3ex-(3pt/4+1.45cc*3)
%
% which is much harder to parse and decide on.
%
% Examples:
%
% \skvifdimensionable{01}{\def\x{T}}{\def\x{F}}
% \skvifdimensionable{01pt}{\def\x{T}}{\def\x{F}}
% \skvifdimensionable{01abpt}{\def\x{T}}{\def\x{F}}
% \skvifdimensionable\paperwidth{\def\x{T}}{\def\x{F}}
% \skvifdimensionable{\skip0}{\def\x{T}}{\def\x{F}}
% \skvifdimensionable{1.2pt}{\def\x{T}}{\def\x{F}}
% \skvifdimensionable{1.2\relax pt}{\def\x{T}}{\def\x{F}}
% \skvifdimensionable{1pt\relax\skvrelax}{\def\x{T}}{\def\x{F}}
%
\skvrobustdef\skvifdimensionable#1{%
  \def\skv@dimunit{}%
  % Does 'pt' mean 0pt or 1pt? Make it an invalid input:
  \lowercase{\skvifindetokTF{,}{#1}}\skv@validunit{%
    \skv@err{Illegal step '#1': no number found with it}\skv@ehd
  }{}%
  \skv@isintegerfalse
  \skvifintegerTF{#1}{%
    \skv@isintegertrue\@secondoftwo
  }{%
    \expandafter\skv@ifdimensionable\skv@elt\skv@catch@nil
  }%
}
\skvrobustdef\skv@ifdimensionable#1#2\skv@catch@nil{%
  \skvifxTF\relax#1{%
    \skvifblankTF{#2}{%
      \skv@isintegertrue\@secondoftwo
    }{%
      \expandafter\skv@findunit\skv@elt\skv@catch@nil
    }%
  }{%
    \expandafter\skv@findunit\skv@elt\skv@catch@nil
  }%
}
\skvrobustdef\skv@findunit#1#2#3\skv@catch@nil{%
  \def\skv@provb{%
    \ifx\relax#2%
      \if\relax\detokenize{#3}\relax
        \expandafter\expandafter\expandafter\@firstoftwo
      \else
        \expandafter\expandafter\expandafter\@secondoftwo
      \fi
    \else
      \expandafter\@secondoftwo
    \fi
  }%
  \skvifstrcmpTF{.}{#1}{%
    % In this case, #1 must have come with a trailing \relax.
    % Remove it and re-start the test:
    \def\skv@prova##1##2\relax\skv@catch@nil{%
      \skvifdimensionable{##1##2}%
    }%
    \skv@prova#2#3\skv@catch@nil
  }{%
    % Check for a valid unit. May be a \dimendef'd token.
    \skvifinTF{,#1,}{,\hsize,\vsize,}{%
      \skv@provb
    }{%
      \skvifdimenTF{#1}{%
        \skv@provb
      }{%
        \lowercase{\skvifindetokTF{,}{#1#2}}\skv@validunit{%
          \def\skv@dimunit{#1#2}%
          % Check if #3 has only one (leading) \relax:
          \def\skv@prova##1##2##3\skv@catch@nil{%
            \def\elt{##1}\def\skv@elt{##2}%
          }%
          \skv@prova#3\skv@quark\skv@quark\skv@catch@nil
          \ifx\elt\skv@relaxtoks
            \def\skv@prova{\skv@quark}%
            \ifx\skv@elt\skv@prova
              \expandafter\expandafter\expandafter\@firstoftwo
            \else
              % \skv@elt might contain \relax, but never mind; let us end
              % the search here. The samething can be said of the tests in
              % \skv@provb.
              \expandafter\expandafter\expandafter\@secondoftwo
            \fi
          \else
            \expandafter\@secondoftwo
          \fi
        }{%
          \@secondoftwo
        }%
      }%
    }%
  }%
}

% Evaluating a dimensionable expression.
%
% 1. This can't parse expressions containing both * and / in one component,
%    eg, in 3pt*3/2. But (3pt*3)/2 or (3pt/2)*3 will pass.
%
% Examples:
%
% \skvifdimexpr{2bp*3/2}{<T>}{<F>} : fails
% \skvifdimexpr{1pt-2bp*3+(3cc-2ex)/2}{<T>}{<F>} : true
% \skvifdimexpr{(1pt-2bp+(3cc-2ex)/2)*5}{<T>}{<F>} : true
% \skvifdimexpr{1+(1pt-2bp+(3cc-2ex)/2)*5}{<T>}{<F>} : false
%
\skvrobustdef*\skvifdimexpr#1{%
  \begingroup
  \@tempcnta\skvz@
  \skv@dimexpr@beg
  \skv@dimexpr@bgroup#1(\skv@catch@nil
  \skv@dimexpr@end
  \skv@dimexpr@end@end
}
\skvrobustdef*\skv@dimexpr@beg{\begingroup\@tempcnta\skvz@}
\skvrobustdef*\skv@dimexpr@end{%
  \skv@dimexpr@end@end
  \skv@dimexpr@true\skv@dimexpr@false
}
\skvrobustdef*\skv@dimexpr@end@end{%
  \skvifnumTF\@tempcnta<\skvz@
    {\endgroup\@secondoftwo}{\endgroup\@firstoftwo}%
}
\skvrobustdef*\skv@dimexpr@true{\advance\@tempcnta\skvz@}
\skvrobustdef*\skv@dimexpr@false{\advance\@tempcnta\m@ne}
\skvrobustdef*\skv@dimexpr@bgroup#1(#2\skv@catch@nil{%
  \skv@dimexpr@egroup#1)\skv@catch@nil
  \skvifblankTF{#2}{}{%
    \skv@dimexpr@beg
    \skv@dimexpr@bgroup#2\skv@catch@nil
  }%
}
\skvrobustdef*\skv@dimexpr@egroup#1)#2\skv@catch@nil{%
  \skv@dimexpr@plus#1+\skv@catch@nil
  \skvifblankTF{#2}{}{%
    \skv@dimexpr@end
    \skv@dimexpr@egroup#2\skv@catch@nil
  }%
}
\skvrobustdef*\skv@dimexpr@plus#1+#2\skv@catch@nil{%
  \skv@dimexpr@minus#1-\skv@catch@nil
  \skvifblankTF{#2}{}{\skv@dimexpr@plus#2\skv@catch@nil}%
}
\skvrobustdef*\skv@dimexpr@minus#1-#2\skv@catch@nil{%
  \skvifblankTF{#1}{}{%
    \skvifinTF{*}{#1}{%
      \skvifinTF{/}{#1}{%
        \skv@err{I can't parse this: both star (*) and slash
          \MessageBreak (/) are in '#1'}\skv@ehd
      }{%
        \skvifblankTF{#1}{}{\skv@dimexpr@times#1*\skv@catch@nil}%
      }%
    }{%
      \skvifblankTF{#1}{}{\skv@dimexpr@divide#1/\skv@catch@nil}%
    }%
  }%
  \skvifblankTF{#2}{}{\skv@dimexpr@minus#2\skv@catch@nil}%
}
% Because of, eg, 2pt*3/2, the test for * is more subtle:
\skvrobustdef*\skv@dimexpr@times#1*#2\skv@catch@nil{%
  \skvifblankTF{#1}{}{%
    \skvifdimensionable{#1}\skv@dimexpr@true\skv@dimexpr@false
  }%
  \skvifblankTF{#2}{}{%
    \def\skv@prova##1*##2\skv@catch@nil{##1}%
    \skvexpbracenext\skv@dimexpr@integer{\skv@prova#2\skv@catch@nil}%
  }%
}
\skvrobustdef*\skv@dimexpr@divide#1/#2\skv@catch@nil{%
  \skvifblankTF{#1}{}{%
    \skvifdimensionable{#1}\skv@dimexpr@true\skv@dimexpr@false
  }%
  \skvifblankTF{#2}{}{%
    \def\skv@prova##1/##2\skv@catch@nil{##1}%
    \skvexpbracenext\skv@dimexpr@integer{\skv@prova#2\skv@catch@nil}%
  }%
}
\skvrobustdef*\skv@dimexpr@integer#1{%
  \skvifblankTF{#1}{}{%
    \skvifintegerTF{#1}\skv@dimexpr@true\skv@dimexpr@false
  }%
}

% \skvtrimlastparser{<parser>}<cmd>
\skvrobustdef\skvtrimlastparser#1#2{%
  \begingroup
  % The following \relax will not be cat-12, so it won't appear in #2:
  \def\skv@trim@a{%
    \skvxifinTF{\detokenize{#1}\relax}{\skvoxdetok{#2}\relax}{%
      \def\skv@trim@b####1#1\skv@normal@nil{%
        \edef#2{\unexpanded{####1}}%
        \skv@trim@a
      }%
      \expandafter\skv@trim@b#2\skv@normal@nil
    }{}%
  }%
  \skv@trim@a
  \skvaftergroupdef#2\endgroup
}

% Generate parameter characters from number #1 to #2:
\skvnewdef*\skvgenerateparameters#1#2{%
  \ifnum#1<\numexpr#2+1####\number#1%
    \expandafter\skvgenerateparameters
    \expandafter{\number\numexpr#1+1\expandafter}%
    \expandafter{\number#2\expandafter}%
  \fi
}

% Normalize non-parser-separated tokenlist. Preserve outer braces.
% \edef\x{\skvtsvnormalize{ x y {z}}}
\skvnewdef*\skvtsvnormalize#1{%
  \unexpanded\expandafter
    {\romannumeral-`\q\skv@tsvnormalize.#1 \skv@normal@nil}%
}
\skvnewdef*\skv@tsvnormalize#1 #2\skv@normal@nil{%
  \skvifblankTF{#2}
    {\expandafter\expandafter\expandafter\space
      \expandafter\noexpand\@gobble#1}
    {\skv@tsvnormalize#1#2\skv@normal@nil}%
}


% \skvnormalize{<csv/kv>}<parser>{<list>}<cmd>
\skvrobustdef*\skvnormalize#1#2#3#4{%
  \def\skv@prova##1#1##2##3\skv@nil{%
    \ifx\skv@nnil##2%
      \skv@err{Invalid list type '#1' for command \string\skvnormalize}\skv@ehd
    \fi
    \edef#4{\unexpanded{#3}}%
    ##2[#2]#4%
  }%
  \skv@prova csv\skvcsvnormalize kv\skvkvnormalize#1\skv@nnil\skv@nil
}
\skvnewdef*\skv@switch@inkv{01}
% \skvcsvnormalize[<parser>]<listcmd>
\skvrobustdef*\skvcsvnormalize{\skv@testopt\skv@csvnormalize,}
\skvrobustdef*\skv@csvnormalize[#1]#2{%
  \begingroup
  \skv@setupnormalizer{#1}%
  \skvswitchfalse{inkv}%
  \edef#2{\expandafter\skv@normalizelist\expandafter{#2}}%
  \skvaftergroupdef#2\endgroup
}
% \skvcsvnormalizeset{<cmda>{<token1>,<cmdb2>{<token2>},...}
\skvrobustdef*\skvcsvnormalizeset{\skv@testopt\skv@csvnormalizeset,}
\skvrobustdef*\skv@csvnormalizeset[#1]#2{%
  \begingroup
  \toks@{}%
  \skv@setupnormalizer{#1}%
  \skvswitchfalse{inkv}%
  \def\do##1##2,{%
    \skvifnotnil{##1}{%
      \edef##1{\skv@normalizelist{##2}}%
      \skvexpanded{\toks@{\the\toks@\skvcmdexit##1}}%
      \do
    }%
  }%
  \do#2,\skv@nil,%
  \expandafter\endgroup\the\toks@
}
% \skvkvnormalize{<kvlistcmd>}
\skvrobustdef*\skvkvnormalize#1{%
  \begingroup
  \skv@setupnormalizer{,}%
  \skvswitchtrue{inkv}%
  % We put '\skv@kvguard' at the end of #1 to preserve any trailing '='.
  % This can happen if a key has an empty value. But this can leave
  % a trailing space or <parser> in #1. We remove the trailing space
  % with \skvtrimspace.
  \edef#1{\expandafter\skv@normalizelist\expandafter{#1\skv@kvguard}}%
  \def\skv@kvnorm##1\skv@kvguard##2\skv@normal@nil{%
    \skv@parserequalerr##1##2,=\skv@normal@nil
    \edef#1{\skvtrimspace{##1##2}}%
    \skvtrimlastparser{,}#1%
  }%
  \expandafter\skv@kvnorm#1\skv@normal@nil
  \skvaftergroupdef#1\endgroup
}

\begingroup
\catcode`\~=13 \catcode`\!=13
\skvrobustgdef\skv@setupnormalizer#1{%
  \begingroup
  \lccode`\~=`#1 \lccode`\!=`\=
  \lowercase{\endgroup
    \def\skv@normalizelist##1{%
      \unexpanded\expandafter{\romannumeral-`\q
        \skv@activeparser#1##1#1~\skv@normal@nil}%
    }%
    \def\skv@activeparser##1~##2\skv@normal@nil{%
      \skvifblankTF{##2}{%
        \skvifdefswitchTF{inkv}{%
          \skv@activeequal##1!\skv@normal@nil
        }{%
          \skv@spaceparser##1 #1\skv@normal@nil
        }%
      }{%
        \skv@activeparser##1#1##2\skv@normal@nil
      }%
    }%
    \def\skv@activeequal##1!##2\skv@normal@nil{%
      \skvifblankTF{##2}{%
        \skv@spaceparser##1 #1\skv@normal@nil
      }{%
        \skv@activeequal##1=##2\skv@normal@nil
      }%
    }%
  }%
  \def\skv@spaceparser##1 #1##2\skv@normal@nil{%
    \skvifblankTF{##2}{%
      \skv@parserspace##1#1 \skv@normal@nil
    }{%
      \skv@spaceparser##1#1##2\skv@normal@nil
    }%
  }%
  \def\skv@parserspace##1#1 ##2\skv@normal@nil{%
    \skvifblankTF{##2}{%
      \skvifdefswitchTF{inkv}{%
        \skv@spaceequal##1 =\skv@normal@nil
      }{%
        \skv@doubleparser##1#1#1\skv@normal@nil
      }%
    }{%
      \skv@parserspace##1#1##2\skv@normal@nil
    }%
  }%
  \def\skv@spaceequal##1 =##2\skv@normal@nil{%
    \skvifblankTF{##2}{%
      \skv@equalspace##1= \skv@normal@nil
    }{%
      \skv@spaceequal##1=##2\skv@normal@nil
    }%
  }%
  \def\skv@equalspace##1= ##2\skv@normal@nil{%
    \skvifblankTF{##2}{%
      \skv@doubleparser##1#1#1\skv@normal@nil
    }{%
      \skv@equalspace##1=##2\skv@normal@nil
    }%
  }%
  \def\skv@doubleparser##1#1#1##2\skv@normal@nil{%
    \skvifblankTF{##2}{%
      \skvifdefswitchTF{inkv}{%
        \skv@doubleequal##1==\skv@normal@nil
      }{%
        \skvifblankTF{##1}{}{%
          \skv@remleadparser##1\skv@normal@nil
        }%
      }%
    }{%
      \skv@doubleparser##1#1##2\skv@normal@nil
    }%
  }%
  \def\skv@doubleequal##1==##2\skv@normal@nil{%
    \skvifblankTF{##2}{%
      \skvifblankTF{##1}{}{%
        \skv@remleadparser##1\skv@normal@nil
      }%
    }{%
      \skv@doubleequal##1=##2\skv@normal@nil
    }%
  }%
  \def\skv@remleadparser#1##1\skv@normal@nil{%
    \expandafter\space\noexpand##1%
  }%
  \def\skv@parserequalerr##1#1=##2\skv@normal@nil{%
    \skvifblankTF{##2}{}{%
      \skv@err{There is '#1=' in your key-value list}\skv@ehd
    }%
  }%
}
\endgroup

% Define a special parser normalizer that doesn't replace double parsers
% with single parser, because a double parser might mean an intentionally
% missing token/property of a key:
\begingroup
\catcode`\~=13
\skvrobustgdef*\skvdefinekeepdoubleparsernormalizer#1#2{%
  \begingroup
  \uccode`\~=`#1
  \uppercase{\endgroup
    \long\def#2##1{%
      \unexpanded\expandafter{\romannumeral-`\q
        \skv@keepdouble@activeparser##1~\skv@normal@nil}%
    }%
    \long\def\skv@keepdouble@activeparser##1~##2\skv@normal@nil{%
      \skvifblankTF{##2}
        {\skv@keepdouble@spaceparser##1 #1\skv@normal@nil}
        {\skv@keepdouble@activeparser##1#1##2\skv@normal@nil}%
    }%
  }%
  \long\def\skv@keepdouble@spaceparser##1 #1##2\skv@normal@nil{%
    \skvifblankTF{##2}
      {\skv@keepdouble@parserspace##1#1 \skv@normal@nil}
      {\skv@keepdouble@spaceparser##1#1##2\skv@normal@nil}%
  }%
  \long\def\skv@keepdouble@parserspace##1#1 ##2\skv@normal@nil{%
    \skvifblankTF{##2}
      {\skvifblankTF{##1}{}{\expandafter\space\noexpand##1}}
      {\skv@keepdouble@parserspace##1#1##2\skv@normal@nil}%
  }%
}
\endgroup

\skvdefinekeepdoubleparsernormalizer{/}\skvkeepdoubleslashnormalize

% \skvmacnormalize[<parser>]<listcmd>
\skvrobustdef*\skvmacnormalize{\skv@testopt\skv@macnormalize,}
\skvrobustdef*\skv@macnormalize[#1]#2{%
  \begingroup
  \skvsetupmacroparsernormalizer{#1}%
  \edef#2{\expandafter\skvmacroparsernormalize\expandafter{#2}}%
  \skvaftergroupdef#2\endgroup
}
% This is for normalizing lists like {x\\ y\\\\ z}, where \\ is
% a control sequence. Such parsers may be commands but we don't
% expect them to be active characters.
%
% Example:
%
%   \skvsetupmacroparsernormalizer{\\}
%   \edef\x{\skvmacroparsernormalize{x\\ y\\\\ z}}
%
\skvrobustdef*\skvsetupmacroparsernormalizer#1{%
  \long\def\skvmacroparsernormalize##1{%
    \unexpanded\expandafter{\romannumeral-`\q
      \skv@mac@spaceparser##1 #1\skv@normal@nil}%
  }%
  \long\def\skv@mac@spaceparser##1 #1##2\skv@normal@nil{%
    \skvifblankTF{##2}
      {\skv@mac@parserspace##1#1 \skv@normal@nil}
      {\skv@mac@spaceparser##1#1##2\skv@normal@nil}%
  }%
  \long\def\skv@mac@parserspace##1#1 ##2\skv@normal@nil{%
    \skvifblankTF{##2}
      {\skv@mac@doubleparser##1#1#1\skv@normal@nil}
      {\skv@mac@parserspace##1#1##2\skv@normal@nil}%
  }%
  \long\def\skv@mac@doubleparser##1#1#1##2\skv@normal@nil{%
    \skvifblankTF{##2}{ ##1}
      {\skv@mac@doubleparser##1#1##2\skv@normal@nil}%
  }%
}
% \skvletmanytocmd{<cmd list>}{<cmd>}
\skvrobustdef*\skvletmanytocmd#1#2{%
  \skvcommaparse{#1}\skv@prova{%
    \expandafter\let\skv@prova= #2%
  }%
}
% \skvnewletmanytocmd{<cmd list>}{<cmd>}
\skvrobustdef*\skvnewletmanytocmd#1#2{%
  \skvcommaparse{#1}\skv@prova{%
    \expandafter\skv@newcastcommand\skv@prova=#2=\cast@nil
  }%
}
% \skvcastcommands{<cmd list>}
%
%   <cmd list> -> {<cmd-a1>=<cmd-a2>,...,<cmd-b1>=<cmd-b2>}
%
% In <cmd list>, cast left-hand command to the right-hand command.
% Raise error if left-hand command already exists and isn't equal to
% the right-hand command.
%
% Example:
%
%   \skvcastcommands{\ifxx=\ifx,\fii=\fi}
%
\skvrobustdef*\skvcastcommands#1{%
  \def\skv@provb##1=##2=##3\cast@nil{\let##1= ##2}%
  \skvkvparse{#1}\skv@prova{%
    \expandafter\skv@provb\skv@prova==\cast@nil
  }%
}
% \skvnewcastcommands{<cmd list>}
%
%   <cmd list> -> {<cmd-a1>=<cmd-a2>,...,<cmd-b1>=<cmd-b2>}
%
\skvrobustdef*\skvnewcastcommands#1{%
  \skvkvparse{#1}\skv@prova{%
    \expandafter\skv@newcastcommand\skv@prova==\cast@nil
  }%
}
\skvrobustdef*\skv@newcastcommand#1=#2=#3\cast@nil{%
  \skvifdefTF{#1}{%
    \ifx#1#2\else
      \skv@err{Command \noexpand#1 already exists:
        \MessageBreak it can't be cast to \string#2}\skv@ehd
    \fi
  }{%
    \let#1= #2%
  }%
}
% \skvpushfunctions<base-fn>{<fn-list>}<counter-number>
%
% 1. <counter-number> is a number, not a counter.
% 2. See file skeyval-for.tex for \skvsavestate and \skvrestorestate.
%
\skvrobustdef*\skvpushfunctions#1#2#3{%
  \skvgadvanceno#3\@ne
  \begingroup
  \def\skv@prova##1{\skvremovescape{##1}@skv@\romannumeral#3}%
  \def\do##1{\let\noexpand##1\skvnoexpandcs{\skv@prova{##1}}}%
  \skvifcsdefTF{\skvremovescape{#1}@skv@stack}{}{%
    \skvcsdef{\skvremovescape{#1}@skv@stack}{}%
  }%
  \skvcsxdef{\skvremovescape{#1}@skv@stack}{%
    #2{\skvexpandcsonce{\skvremovescape{#1}@skv@stack}}%
  }%
  \def\do##1{\let\skvnoexpandcs{\skv@prova{##1}}\noexpand##1}%
  \skvexpanded{\endgroup#2}%
}
% \skvpopfunctions<base-fn><counter-number>
\skvrobustdef*\skvpopfunctions#1#2{%
  \begingroup
  \edef\skv@elt{\skvnoexpandcs{\skvremovescape{#1}@skv@stack}}%
  \expandafter\skvifdefTF\skv@elt{%
    \expandafter\ifx\skv@elt\@empty
      \skv@err{Stack of '\noexpand#1' is empty}\skv@ehd
    \fi
  }{%
    \skv@err{Stack of '\noexpand#1' is undefined}\skv@ehd
  }%
  \edef\skv@prova{\skvexpandtwice\skv@elt}%
  \edef\skv@provb##1##{\endgroup##1\gdef\skvexpandonce\skv@elt}%
  \expandafter\skv@provb\skv@prova
  \skvgadvanceno#2\m@ne
}

\chardef\skv@stackdepthlimit=6\relax
% #1=stack (a macro), #2=list, #3=max depth
\skvrobustdef*\skvbuildmacrostack#1#2#3{%
  \begingroup
  \escapechar92\relax
  \ifdefined#1%
    \skv@err{Stack \noexpand#1 already exists}\skv@ehd
  \else
    \def#1{}%
  \fi
  \@tempcnta\skvz@
  \def\do##1{%
    \noexpand\skv@elt\noexpand##1%
    \skvnoexpandcs{\skvremovescape{##1}@skv@\romannumeral\@tempcnta}%
  }%
  \def\skv@loop{%
    \advance\@tempcnta\@ne
    % Don't use \ifnum here, because #2 may contain booleans.
    \skvifnumTF\@tempcnta<\numexpr#3+1\relax{%
      \edef#1{\skvexpandonce#1.\romannumeral\@tempcnta.{#2}}%
      \skv@loop
    }{}%
  }%
  \skv@loop
  \skvaftergroupdef#1\endgroup
}
\skvrobustdef*\skvpushstate#1#2{\skv@pushorpopstate{#1}{#2}{+}}
\skvrobustdef*\skvpopstate#1#2{\skv@pushorpopstate{#1}{#2}{-}}
% #1: stack (a macro) as built by \skvbuildmacrostack
% #2: depth counter (macro-defined)
% #3: stack direction (+/-)
\skvrobustdef*\skv@pushorpopstate#1#2#3{%
  \if+#3\relax
    \skvgadvanceno#2\@ne
    \def\skv@elt##1##2{\let##2=##1}%
  \else
    \ifnum#2<\@ne
      \skv@err{Can't pop stack: depth currently less than 1}\skv@ehd
    \else
      \def\skv@elt##1##2{\let##1=##2}%
    \fi
  \fi
  \ifnum#2>\skv@stackdepthlimit
    \skv@err{Stack depth limit '\number\skv@stackdepthlimit' exceeded}\skv@ehd
  \fi
  \def\skv@prova##1{%
    \def\skv@prova####1.##1.####2####3\skv@nil{####2}%
    \expandafter\skv@prova#1\skv@nil
  }%
  \expandafter\skv@prova\expandafter{\romannumeral#2}%
  \let\skv@elt\relax
  \if-#3\skvgadvanceno#2\m@ne\fi
}

\skvrobustdef*\skvnewbools{\skv@testopt\skv@newbools{}}
\skvrobustdef*\skv@newbools[#1]#2{%
  \begingroup
  \toks@{}%
  \def\skv@prova{#2}%
  \skvcsvnormalize\skv@prova
  \def\do##1,{%
    \ifx\do##1\else
      \skvifcsdefTF{if#1##1}{%
        \skv@err{Boolean '\skvnoexpandcs{if#1##1}' already exists}\skv@ehd
      }{%
        \toks@\expandafter{\the\expandafter\toks@
          \csname newif\expandafter\endcsname\csname if#1##1\endcsname}%
      }%
      \expandafter\do
    \fi
  }%
  \expandafter\do\skv@prova,\do,%
  \expandafter\endgroup\the\toks@
}

% Some booleans:
%
% inset             = in \skvsetkeys
% viarootofsetkeys  = a key is being set via the root of the command
%                     \skvsetkeys. This is needed because sometimes we
%                     bypass the root of \skvsetkeys, eg, by calling
%                     \skv@setkeys@a.
% inclass           = in class file.
% kf                = key has been found while in \skvsetkeys.
% intry             = in 'try set keys'.
% insa              = in 'search also set keys'.
% success           = key has been found while in 'try set keys'.
% inopt             = in process/execute options.
% inpox             = in process options.
% inprepo           = presetting or post-setting keys.
% inoptionsec       = in skeyval package's options processing section.
%                     Some checks are done in that section.
%
\skvnewbools[skv@]{%
  inclass,inset,viarootofsetkeys,processvalueaslist,st,cl,pl,kf,inpox,inopt,%
  inprepo,tracingkeys,tempsw,swa,verbose,intry,insa,success,inoptionsec,%
  inreservedhandler,ignorepointers,addslots@appending%
}

\skvnewbools{indirectkeys}
\skvnewbools[skv]{indef,novalue,valuebraced}
\skvnewbools[dirkeys@]{saveunknownkeys}
% \skvnewcounts[<optional prefix>]{<name list>}
\skvrobustdef*\skvnewcounts{\skv@testopt\skv@newcounts{}}
\skvrobustdef*\skv@newcounts[#1]#2{%
  \begingroup
  \toks@{}%
  \def\skv@prova{#2}%
  \skvcsvnormalize\skv@prova
  \def\do##1,{%
    \ifx\do##1\else
      \skvifcsdefTF{#1##1}{%
        \skv@err{Counter '\skvnoexpandcs{#1##1}' already exists}\skv@ehd
      }{%
        \toks@\expandafter{\the\expandafter\toks@
          \csname newcount\expandafter\endcsname\csname#1##1\endcsname}%
      }%
      \expandafter\do
    \fi
  }%
  \expandafter\do\skv@prova,\do,%
  \expandafter\endgroup\the\toks@
}
\skvnewcounts[skv@]{tempcnt,cnta}
% \skvnewnumbers[<optional prefix>]{<name list>}
\skvrobustdef*\skvnewnumbers{\skv@testopt\skv@newnumbers{}}
\skvrobustdef*\skv@newnumbers[#1]#2{%
  \begingroup
  \toks@{}%
  \def\skv@prova{#2}%
  \skvcsvnormalize\skv@prova
  \def\do##1,{%
    \ifx\do##1\else
      \skvifcsdefTF{#1##1}{%
        \skv@err{Number '\skvnoexpandcs{#1##1}' already exists}\skv@ehd
      }{%
        \toks@\expandafter{\the\expandafter\toks@
          \expandafter\def\csname#1##1\endcsname{0}}%
      }%
      \expandafter\do
    \fi
  }%
  \expandafter\do\skv@prova,\do,%
  \expandafter\endgroup\the\toks@
}
\skvnewlet\skvnewnumber\skvnewnumbers
\skvnewnumbers[skv@]{keydepth,setkeysdepth,preposetdepth,makekeysdepth,
  usekeysdepth,trysetkeysdepth,trysetkeysidepth,gendepth}
\skvnewnumbers{dirkeys@depth}
\skvnewlet\skv@novalue\relax
\skvnewdef*\skv@novaluetoks{\skv@novalue}

% A fast key parsing scheme originally designed for \newforeach loop.
%
% \skvquickkeys.define{<family>}[<hp>]{<list>}
% \skvquickkeys.set{<family>}[<na>]{<kvlist>}
%
% 1. Quickly define and set command/store keys.
% 2. Pointers aren't used here, to speed up parsing. Use other key
%    machineries instead.
% 3. Package and class options can't be passed via quick keys.
% 4. When defining keys, the syntax of <list> is:
%
%    {<keya-1,...,keya-n>}/{<default>}/{<callback>}/{<choice list>}/{<arg>}
%    ;...;
%    {<keyb-1,...,keyb-n>}/{<default>}/{<callback>}/{<choice list>}/{<arg>}
%
%    Here, keys key1 and key2 will have the same default value, callback,
%    choice list and argument pattern.
%
% 5. The special keys '.exec' and '.exec code' will simply execute the
%    code <default>, without defining anything.
% 6. Use the token '.na' to indicate a missing item that isn't blank or empty.
% 7. The parser for defining the keys can be specified via \setquickkeysparser.
%    The default parser is semicolon (;).
%
% Example:
%  \skvquickkeys.define{fam}[mp@]{%
%    keya/true/\def\x##1{#1*##1}/true,false;
%    keyb;
%    keyc,keyd/aaa+bbb/\def\x##1{#1*##1*#2}/.na/#1+#2;
%  }
%
\skvnewdef*\skv@ifstrrejorempty#1{%
  \skvifstrcmpTF{#1}{^skv^}{%
    \@firstoftwo
  }{%
    \skvifblankTF{#1}%
  }%
}
\skvnewdef*\skv@ifstrrejordotna#1{%
  \skvifstrcmpTF{#1}{^skv^}{%
    \@firstoftwo
  }{%
    \skvifstrcmpTF{#1}{.na}%
  }%
}
\skvnewdef*\skv@ifstrnut#1{%
  \skvifstrcmpTF{#1}{^skv^}{%
    \@firstoftwo
  }{%
    \skvifstrcmpTF{#1}{.na}{%
      \@firstoftwo
    }{%
      \skvifblankTF{#1}%
    }%
  }%
}
\skvnewdef*\skv@ifcmdrejorempty#1{%
  \skvifxTF#1\skv@rej{%
    \@firstoftwo
  }{%
    \skvifemptyTF#1%
  }%
}
\skvnewdef*\skv@ifcmdrejordotna#1{%
  \skvifxTF#1\skv@rej{%
    \@firstoftwo
  }{%
    \skvifxTF#1\skv@dotna
  }%
}
\skvnewdef*\skv@ifcmdnut#1{%
  \skvifxTF#1\skv@rej{%
    \@firstoftwo
  }{%
    \skvifxTF#1\skv@dotna{%
      \@firstoftwo
    }{%
      \skvifemptyTF#1%
    }%
  }%
}
% \skv@qkeysgetkeynames{<kvlist.cmd>}{<return.cmd>}
\skvrobustdef*\skv@qkeysgetkeynames#1#2{%
  \begingroup
  \let#2\@empty
  \skvkvparse*#1\skv@prova{%
    \def\do##1=##2=##3\skv@nil{%
      \edef#2{\skvaddlist,#2##1}%
    }%
    \expandafter\do\skv@prova==\skv@nil
  }%
  \skvaftergroupdef#2\endgroup
}
\skvrobustdef*\skvsetquickkeysparser{\def\skv@qkeysparser}
\skvsetquickkeysparser{;}
\skvrobustdef*\skvquickkeys#1#{%
  \edef\skv@tempa{\skvtrimspace{#1}}%
  \skvxifstrcmpTF{\skvexpandonce\skv@tempa}{.define}{%
    \begingroup\endlinechar\m@ne
    \skv@defquickkeys
  }{%
    \skvxifstrcmpTF{\skvexpandonce\skv@tempa}{.set}{%
      \skv@setquickkeys
    }{%
      \skvxifstrcmpTF{\skvexpandonce\skv@tempa}{.preset}{%
        \skv@presetquickkeys
      }{%
        \skv@err{Unknown task for \string\skvquickkeys}\skv@ehd
      }%
    }%
  }%
}
\skvrobustdef*\skv@defquickkeys#1{\skv@testopt{\skv@defquickkeys@a{#1}}{}}
\skvrobustdef*\skv@defquickkeys@a#1[#2]#3{%
  \endgroup
  \edef\skv@qkeysfam{\skvtrimspace{#1}}%
  \edef\skv@tempa{\skvkeepdoubleslashnormalize{#3}}%
  \skvexpanded{\skvparselist*{\skv@qkeysparser}}\skv@tempa\skv@tempa{%
    \skv@oslashsplit\skv@tempa{%
      \skvifinTF{,##1,}{,.exec,.exec code,}{%
        ##2\relax
      }{%
        % Loop over key list, in case there are more than one key:
        \skvparselist{,}{##1}\skv@tempa{%
          % If ##2 is empty, the default will be empty:
          \skv@ifstrrejordotna{##2}{}{%
            \skvcsedef{\skv@qkeysfam/\skv@tempa/qkeys.def}{\unexpanded{##2}}%
          }%
          \skvcsedef{\skv@qkeysfam/\skv@tempa/qkeys.cbk}{%
            \skvifblankTF{#2}{}{%
              \skvcsletcs{#2\skv@tempa}{\skv@qkeysfam/\skv@tempa/qkeys.val}%
            }%
            \skv@ifstrrejordotna{##3}{}{\unexpanded{##3}}%
          }%
          \skv@ifstrnut{##4}{}{%
            \skvcsedef{\skv@qkeysfam/\skv@tempa/qkeys.chc}{\unexpanded{##4}}%
          }%
          \skv@ifstrnut{##5}{}{%
            \skvcsedef{\skv@qkeysfam/\skv@tempa/qkeys.arg}{\unexpanded{##5}}%
          }%
        }%
      }%
    }%
  }%
}

% \skvquickkeys.preset{<family>}{<kvlist>}
%
\skvrobustdef*\skv@presetquickkeys#1#2{%
  \edef\skv@prova{\unexpanded{#2}}%
  \skvkvnormalize\skv@prova
  \skvcslet{\skvtrimspace{#1}/qkeys.preset}\skv@prova
}

\skvnewnumbers[skv@]{setqkeysdepth}

% \skvquickkeys.set{<family>}[<na>]{<kvlist>}

\skvrobustdef*\skv@setquickkeys#1{\skv@testopt{\skv@setquickkeys@a{#1}}{}}
\skvrobustdef*\skv@setquickkeys@a#1[#2]#3{%
  \skvsavestate\skv@setquickkeys{%
    \do\skv@qkeysfam\do\skv@qkeysna\do\skv@qkeyskvlist
    \do\skv@qkeyscurrnames
  }\skv@setqkeysdepth
  \edef\skv@qkeysna{\unexpanded{#2}}%
  \skvcsvnormalize\skv@qkeysna
  \edef\skv@qkeyskvlist{\unexpanded{#3}}%
  \skvkvnormalize\skv@qkeyskvlist
  \edef\skv@qkeysfam{\skvtrimspace{#1}}%
  \def\skv@setqkeys@a##1##2{%
    \skvifcsdefTF{\skv@qkeysfam/##1/qkeys.cbk}{}{%
      \skv@err{Key '\skv@qkeysfam/##1'
        \MessageBreak is not defined}\skv@ehd
    }%
    \skvifstrcmpTF{##2}\skv@novalue{%
      \skvifcsdefTF{\skv@qkeysfam/##1/qkeys.def}{%
        \skvcsletcs{\skv@qkeysfam/##1/qkeys.val}{\skv@qkeysfam/##1/qkeys.def}%
      }{%
        \skv@err{No user value and no default
          \MessageBreak for key '\skv@qkeysfam/##1'}\skv@ehd
      }%
    }{%
      \skvcsedef{\skv@qkeysfam/##1/qkeys.val}{\unexpanded{##2}}%
    }%
    \skvletcs\skv@tempval{\skv@qkeysfam/##1/qkeys.val}%
    \skvletcs\reserved@a{\skv@qkeysfam/##1/qkeys.chc}%
    \skvifdefTF\reserved@a{%
      \skvxifinTF{,\skvoxdetok\skv@tempval,}{,\skvoxdetok\reserved@a,}{}{%
        \skv@err{Value '\skvoxdetok\skv@tempval' for key '##1'
          \MessageBreak is not in prescribed list
          \MessageBreak '\skvoxdetok\reserved@a'}\skv@ehd
      }%
    }{}%
    \skvifcsdefTF{\skv@qkeysfam/##1/qkeys.arg}{%
      \skvletcs\skv@argpattern{\skv@qkeysfam/##1/qkeys.arg}%
    }{%
      \let\skv@argpattern\skv@simplearg
    }%
    \skvletcs\skv@callback{\skv@qkeysfam/##1/qkeys.cbk}%
    \expandafter\expandafter\expandafter\def\expandafter\expandafter
      \expandafter\reserved@a\expandafter\skv@argpattern\expandafter
      \quickkeyseov\expandafter{\skv@callback}%
    \expandafter\reserved@a\skv@tempval\quickkeyseov
  }%
  \def\skv@setqkeys@b##1=##2=##3\skv@setqkeys@nil{%
    \skvxifinTF{,\detokenize{##1},}{,\skvoxdetok\skv@qkeysna,}{}{%
      \skv@setqkeys@a{##1}{##2}%
    }%
  }%
  \skvifcsdefFT{\skv@qkeysfam/qkeys.preset}{}{%
    \skv@qkeysgetkeynames\skv@qkeyskvlist\skv@qkeyscurrnames
    \def\skv@setqkeys@c##1=##2=##3\skv@setqkeys@nil{%
      \skvxifinTF{,\detokenize{##1},}{,\skvoxdetok\skv@qkeyscurrnames,}{}{%
        \let\skv@setquickkeys@a\skv@bad@setquickkeys@a
        \skv@setqkeys@b##1={##2}=##3\skv@setqkeys@nil
        \let\skv@setquickkeys@a\skv@sav@setquickkeys@a
      }%
    }%
    \skvletcs\skv@tempa{\skv@qkeysfam/qkeys.preset}%
    \skvkvparse*\skv@tempa\skv@tempa{%
      \expandafter\skv@setqkeys@c\skv@tempa=\skv@novalue=\skv@setqkeys@nil
    }%
  }%
  \skvkvparse*\skv@qkeyskvlist\skv@tempa{%
    \expandafter\skv@setqkeys@b\skv@tempa=\skv@novalue=\skv@setqkeys@nil
  }%
  \skvrestorestate\skv@setquickkeys\skv@setqkeysdepth
}
\skvnewlet\skv@sav@setquickkeys@a\skv@setquickkeys@a
\skvrobustdef*\skv@bad@setquickkeys@a{%
  \skv@err{'\string\skvquickkeys.set' can't be nested in a preset
    \MessageBreak key's callback: this will cause a cyclic call
    \MessageBreak to '\string\skvquickkeys.set'}\skv@ehd
}

% \skvinitializequickkeys{<fam>}[<na>]{<kvlist>}
\skvrobustdef*\skvinitializequickkeys#1{%
  \skv@testopt{\skv@initializequickkeys@a{#1}}{}%
}
\skvrobustdef*\skv@initializequickkeys@a#1[#2]#3{%
  \skvindeftrue
  \skv@setquickkeys{#1}[#2]{#3}%
  \skvindeffalse
}

\input skeyval-for

%  \skvifcase<comparator>{<teststr>}
%    {<cases>}
%  \elsedo
%    {<no match>}
%  \endif
%
% 1. \skvifcase is expandable but, to simplify the code, \elsedo is mandatory.
%    See \ltsifcases of ltxtools package; it is expandable and the 'else part'
%    can be omitted in it.
% 2. \skvifcasse and \skvifcases aren't expandable, but \elsedo isn't
%    mandatory.
%
% Example:
%
%  \skvifcase\skvifstrcmpTF{c}
%    {a}{do a}
%    {b}{do b}
%    {c}{do c}
%  \elsedo
%    no match%
%  \endif
%
% \skvifcase is expandable.
%
\skvnewdef\skvifcase#1#2#3\elsedo#4\endif{%
  % {#2}{#4} represent default action:
  \skv@ifcase{#1}{#2}#3{#2}{#4}\skv@casestop
}
\skvnewdef\skv@ifcase#1#2#3{%
  #1{#2}{#3}{%
    \skv@ifcase@domatch
  }{%
    \skv@ifcase@a{#1}{#2}%
  }%
}
\skvnewdef\skv@ifcase@a#1#2#3{\skv@ifcase{#1}{#2}}
\skvnewdef\skv@ifcase@domatch#1#2\skv@casestop{\skvtrimspace{#1}}

%  \skvifcasse{<teststr>}
%    {<cases>}
%  \elsedo
%    {<no match>}
%  \endif
%
% 1. \elsedo can be omitted by the user, ie, it is optional. See also
%    \skvifcases.
% 2. Because of the need to remove blank spaces before 'case',
%    \skvifcasse isn't expandable.
%
% Example:
%
%  \skvifcasse{x}
%     case{a}{\def\x{do a}}
%     case{b}{\def\x{do b}}
%     case{c}{\def\x{do c}}
%  \elsedo
%     \def\x{no match}
%  \endif
%
\skvrobustdef*\skvifcasse#1#2\endif{%
  \skvxifinTF{\detokenize{\elsedo}}{\detokenize{#2}}{%
    \begingroup
    \def\skv@prova##1\elsedo##2\skv@ifcasse@nil{%
      \endgroup
      \skv@ifcasse@a{#1}##1case{#1}{##2}\skv@casse@stop
    }%
    \skv@prova#2\skv@ifcasse@nil
  }{%
    \skv@ifcasse@a{#1}#2case{#1}{}\skv@casse@stop
  }%
}
\skvrobustdef*\skv@ifcasse@a#1{%
  \@ifnextchar\relax{\skv@ifcasse@b#1}{\skv@ifcasse@b#1}%
}
\skvrobustdef*\skv@ifcasse@b#1case#2{%
  \skvxifstrcmpTF{#1}{#2}{%
    \skv@ifcasse@domatch
  }{%
    \skv@ifcasse@c{#1}%
  }%
}
\skvrobustdef*\skv@ifcasse@c#1#2{\skv@ifcasse@a{#1}}
\skvrobustdef*\skv@ifcasse@domatch#1#2\skv@casse@stop{\skvtrimspace{#1}}

%  \skvifcases<teststr>\then
%    <cases>{<acts>}
%    <default>{<act>}
%  \fi
%
% 1. <default>{<act>} can be omitted by the user, ie, it is optional.
% 2. \skvifcases isn't expandable.
%
% Example:
%  \skvifcases x\then
%     case{a}{\def\x{do a}}
%     case{b}{\def\x{do b}}
%     case{c}{\def\x{do c}}
%     default{\def\x{no match}}
%  \fi
%
\skvrobustdef*\skvifcases#1\then#2\fi{%
  % Any space trailing #2 will be absorbed by ##3 of the following
  % \skv@prova.
  \begingroup
  \def\skv@prova##1default##2##3\skv@ifcases@nil{%
    \endgroup
    \skvifstrcmpTF{##2}{\@nil}{%
      \skv@ifcases@a{#1}##1case{#1}{}\skv@cases@stop
    }{%
      \skv@ifcases@a{#1}##1case{#1}{##2}\skv@cases@stop
    }%
  }%
  \skv@prova#2default{\@nil}\skv@ifcases@nil
}
\skvrobustdef*\skv@ifcases@a#1{%
  \@ifnextchar\relax{\skv@ifcases@b#1}{\skv@ifcases@b#1}%
}
\skvrobustdef*\skv@ifcases@b#1case#2{%
  \skvxifstrcmpTF{#1}{#2}{%
    \skv@ifcases@domatch
  }{%
    \skv@ifcases@c{#1}%
  }%
}
\skvrobustdef*\skv@ifcases@c#1#2{\skv@ifcases@a{#1}}
\skvrobustdef*\skv@ifcases@domatch#1#2\skv@cases@stop{#1}

% Evaluating a series of boolean expressions.
%
% Example:
%
% \skvifexprTF{%
%   not ( expr { \skvifdefTF\xa } and expr { \skvifemptyTF\xa } )
%   or ( expr { \skvifboolTF{@tempswa} } or expr { \skvifxTF\xa\xb } )
% }{%
%   \def\x{T}
% }{%
%   \def\x{F}
% }
\skvnewnumbers[skv@]{exprcnt}
\skvrobustdef*\skvifexprTF#1{%
  \begingroup
  \def\skv@expr@neg{01}%
  \skvsetno\skv@exprcnt\skvz@
  \skv@expr@beg
  \skv@expr@bgroup#1(\skv@expr@nil
  \skv@expr@end
  \skv@expr@end@end
}
\skvrobustdef*\skv@expr@beg{%
  \begingroup
  \def\skv@expr@neg{01}%
  \skv@exprcnt\skvz@
}
\skvrobustdef*\skv@expr@end{%
  \skv@expr@end@end\skv@expr@true\skv@expr@false
}
\skvrobustdef*\skv@expr@end@end{%
  \expandafter\endgroup\csname @\ifnum\skv@exprcnt<\skvz@
    second\else first\fi oftwo\endcsname
}
\skvrobustdef*\skv@expr@true{%
  \skvadvanceno\skv@exprcnt{\if\skv@expr@neg\m@ne\else\skvz@\fi}%
  \def\skv@expr@neg{01}%
}
\skvrobustdef*\skv@expr@false{%
  \skvadvanceno\skv@exprcnt{\if\skv@expr@neg\skvz@\else\m@ne\fi}%
  \def\skv@expr@neg{01}%
}
\skvrobustdef\skv@expr@bgroup#1(#2\skv@expr@nil{%
  \skv@expr@egroup#1)\skv@expr@nil
  \skvifblankTF{#2}{}{%
    \skv@expr@beg
    \skv@expr@bgroup#2\skv@expr@nil
  }%
}
\skvrobustdef\skv@expr@egroup#1)#2\skv@expr@nil{%
  \skv@expr@and#1and\skv@expr@nil
  \skvifblankTF{#2}{}{%
    \skv@expr@end
    \skv@expr@egroup#2\skv@expr@nil
  }%
}
\skvrobustdef\skv@expr@and#1and#2\skv@expr@nil{%
  \skv@expr@or#1or\skv@expr@nil
  \skvifblankTF{#2}{}{%
    \skv@exprcnt\ifnum\skv@exprcnt<\skvz@\m@ne\else\skvz@\fi
    \skv@expr@and#2\skv@expr@nil
  }%
}
\skvrobustdef\skv@expr@or#1or#2\skv@expr@nil{%
  \skv@expr@not#1not\skv@expr@nil
  \skvifblankTF{#2}{}{%
    \skv@exprcnt\ifnum\skv@exprcnt<\skvz@\skvz@\else\@ne\fi
    \skv@expr@or#2\skv@expr@nil
  }%
}
\skvrobustdef\skv@expr@not#1not#2\skv@expr@nil{%
  \skv@expr@do#1expr\skv@expr@nil
  \skvifblankTF{#2}{}{%
    \def\skv@expr@neg{00}%
    \skv@expr@not#2\skv@expr@nil
  }%
}
\skvrobustdef\skv@expr@do#1expr#2\skv@expr@nil{%
  \skvifblankTF{#1}{}{%
    \skv@err{Invalid \noexpand\skvifexprTF test expression}
      {The handicapped test part is: '\detokenize{#1}'}%
  }%
  \skvifblankTF{#2}{}{\skv@expr@do@a#2\skv@expr@nil}%
}
\skvrobustdef\skv@expr@do@a#1#2\skv@expr@nil{%
  \ignorespaces#1\skv@expr@true\skv@expr@false
  \skv@expr@do#2\skv@expr@nil
}

\skvnewdef\skvwhileexpr#1\do#2{%
  \skvifcondTF{#1}\fi{#2\skvwhileexpr{#1}\do{#2}}{}%
}

\skvbuildmacrostack\skv@keystate{%
  \do\skvcurrentprefix\do\skv@fams\do\skvcurrentfamily
  \do\skvcurrentkey\do\skv@header\do\skvcurrentpath\do\skv@na
  \do\skv@currentnames\do\ifskv@st\do\ifskv@pl\do\ifskv@kf\do\ifskvnovalue
  \do\skvcurrentvalue\do\CurrentOption\do\ifskv@intry\do\ifskv@success
  \do\ifskv@inpox\do\ifskv@inprepo\do\skv@pathdo\do\skv@rmkeys
  \do\ifskv@viarootofsetkeys\do\skv@currpref\do\skv@currfam
}\skv@stackdepthlimit

\skvbuildmacrostack\skv@dirkeys@state{%
  \do\dirkeys@pathlist\do\dirkeys@holderprefixtoks\do\dirkeys@parser
  \do\dirkeys@unknownkeysmacro\do\ifdirkeys@saveunknownkeys
  \do\ifindirectkeys\do\ifskvdfk@initialize\do\ifskvdfk@saveinitialvalues
}\skv@stackdepthlimit

\skvrobustdef\skvappto#1#2{\edef#1{\skvexpandonce{#1}\unexpanded{#2}}}
\skvrobustdef\skvxappto#1#2{\edef#1{\skvexpandonce{#1}#2}}
\skvrobustdef\skvgappto#1#2{\xdef#1{\skvexpandonce{#1}\unexpanded{#2}}}
\skvrobustdef\skvxgappto#1#2{\xdef#1{\skvexpandonce{#1}#2}}
\skvrobustdef\skvappendtomacro{\skv@testst{\skv@appendtomacro{app}{e}}}
\skvrobustdef\skvgappendtomacro{\skv@testst{\skv@appendtomacro{app}{x}}}
\skvrobustdef\skvprependtomacro{\skv@testst{\skv@appendtomacro{pre}{e}}}
\skvrobustdef\skvgprependtomacro{\skv@testst{\skv@appendtomacro{pre}{x}}}
\skvrobustdef\skv@appendtomacro#1#2#3#4{%
  \skvifescapedTF{#3}{%
    \@nameuse{#2def}#3{%
      \skvifstrcmpTF{#1}{app}{%
        \skvifdefTF#3{\skvexpandonce#3}{}%
        \skvifdefboolTF{skv@tempst}\skvexpandonce\unexpanded{#4}%
      }{%
        \skvifdefboolTF{skv@tempst}\skvexpandonce\unexpanded{#4}%
        \skvifdefTF#3{\skvexpandonce#3}{}%
      }%
    }%
  }{%
    \skv@err{Token '\detokenize{#3}' is not escaped}\skv@ehd
  }%
}

% \skvaddlist{<parser>}{<listcmd>}
% This is usually called under \edef. <listcmd> must have been
% initialized.
\skvnewdef*\skvaddlist#1#2{%
  \skvifemptyTF#2{}{\skvexpandonce#2\unexpanded{#1}}%
}
% \skvxaddtolist{<parser>}{<listcmd>}{<newitem>}
\skvrobustdef\skvxaddtolist#1#2#3{\edef#2{\skvaddlist#1#2#3}}
% \skvaddtolist[<parser>]{<listcmd>}{<newitem>}
\skvrobustdef*\skvaddtolist{\skv@teststopt{\skv@addtolist{}},}
\skvrobustdef*\skvgaddtolist{\skv@teststopt{\skv@addtolist{\global}},}
\skvrobustdef\skv@addtolist#1[#2]#3#4{%
  #1\edef#3{%
    \skvifdefTF#3{%
      \skvifemptyTF#3{}{\skvexpandonce#3#2}%
    }{}%
    \skvifdefboolTF{skv@tempst}\skvexpandonce\unexpanded{#4}%
  }%
}
% \skv@declarefilter{<filter.type>}
\skvrobustdef*\skv@declarefilter#1{%
  \edef\skv@filter##1##2{%
    \skvifblankTF{#1}{\let##2=##1}{%
      \skvifxTF#1\relax{\let##2=##1}{%
        \skvifstrcmpTF{#1}\nofilter{\let##2=##1}{%
          \unexpanded{#1}{##1}{##2}%
        }%
      }%
    }%
  }%
}

% \skvfiltermergelist![<parser>](<wrapper>)<cmd>{<sublist>}<filter>
%
% 1. The exclamation mark (!) implies that the outcome is globalized.
% 2. When there is no filter to be applied, \skvmergelist is faster
%    than \skvfiltermergelist.
% 3. <wrapper> will be applied to all the elements (new and old).
%    The default value of <wrapper> is \skvexpandonce.
% 4. Example:
%      \def\alist{a;b;c}
%      \def\wrap#1{{#1}}
%      \skvfiltermergelist[;](\wrap)\alist{a;d;e}\nofilter
%      \show\alist
%
\skvrobustdef*\skvfiltermergelist{%
  \skv@testcl{\skv@testopt\skv@filtermergelist,}%
}
\skvrobustdef*\skv@filtermergelist[#1]{%
  \skv@testpnopt{\skv@f@ltermergelist{#1}}\skvexpandonce
}
\skvrobustdef*\skv@f@ltermergelist#1(#2)#3#4#5{%
  \begingroup
  \skv@declarefilter{#5}%
  \skvifdefTF#3{\skvcsvnormalize[#1]#3}{\def#3{}}%
  \edef\skv@merga{\unexpanded{#4}}%
  \skvcsvnormalize[#1]\skv@merga
  \skvdolist*{#1}\skv@merga\skv@merga{%
    \@tempswatrue
    \skv@filter\skv@merga\skv@mergb
    \let\skv@mergc#3%
    \let#3\@empty
    \skvdolist*{#1}\skv@mergc\skv@mergc{%
      \skv@filter\skv@mergc\skv@mergd
      \ifx\skv@mergb\skv@mergd
        \@tempswafalse
        \edef#3{\skvaddlist#1#3#2{\skv@merga}}%
      \else
        \edef#3{\skvaddlist#1#3#2{\skv@mergc}}%
      \fi
    }%
    \if@tempswa
      \edef#3{\skvaddlist#1#3#2{\skv@merga}}%
    \fi
  }%
  \skvaftergroupdef#3\endgroup
  \ifskv@cl\global\let#3#3\fi
}
% \skvmergelist![<parser>](<wrapper>)<cmd>{<sublist>}
%
% 1. The exclamation mark (!) implies that the outcome is globalized.
% 2. <wrapper> will be applied to only the new elements. The default
%    value of <wrapper> is \skvexpandonce.
\skvrobustdef*\skvmergelist{\skv@testcl{\skv@testopt\skv@mergelist,}}
\skvrobustdef*\skv@mergelist[#1]{%
  \skv@testpnopt{\skv@m@rgelist{#1}}\skvexpandonce
}
\skvrobustdef*\skv@m@rgelist#1(#2)#3#4{%
  \begingroup
  \skvifdefTF#3{\skvcsvnormalize[#1]#3}{\def#3{}}%
  \edef\skv@tempa{\unexpanded{#4}}%
  \skvcsvnormalize[#1]\skv@tempa
  \skvdolist*{#1}\skv@tempa\skv@tempa{%
    \skvxifinTF{#1\skvoxdetok\skv@tempa#1}{#1\skvoxdetok#3#1}{}{%
      \edef#3{\skvaddlist#1#3#2{\skv@tempa}}%
    }%
  }%
  \skvaftergroupdef#3\endgroup
  \ifskv@cl\global\let#3#3\fi
}

% \skvfilterremoveelements!<cmd>{<sublist>}<filter>
% The exclamation mark (!) implies that the outcome is globalized.
% When there is no filter to be applied, \skvremoveelements is faster
% than \skvfilterremoveelements.
% \if@tempswa can be used to test if, at the end, anything was
% removed from #1.
\skvrobustdef*\skvfilterremoveelements{%
  \skv@testcl\skv@filterremoveelements
}
\skvrobustdef*\skv@filterremoveelements#1#2#3{%
  \begingroup
  \let\skv@origlist#1%
  \skv@declarefilter{#3}%
  \skvifdefTF#1{\skvkvnormalize#1}{\def#1{}}%
  \skvcommaparse{#2}\skv@rema\skv@rema{%
    \skv@filter\skv@rema\skv@remb
    \let\skv@remc#1\let#1\@empty
    \skvcommaloop*\skv@remc\skv@remc{%
      \skv@filter\skv@remc\skv@remd
      \ifx\skv@remb\skv@remd\else
        \edef#1{\skvaddlist,#1\skvexpandonce\skv@remc}%
      \fi
    }%
  }%
  \skvexpanded{\endgroup
    \skvcmdexit#1%
    \ifx#1\@empty
      \noexpand\@tempswatrue
    \else
      \ifx#1\skv@origlist\noexpand\@tempswafalse\else
        \noexpand\@tempswatrue\fi
    \fi
  }%
  \ifskv@cl\global\let#1#1\fi
}
% \skvremoveelements!<cmd>{<sublist>}
% The exclamation mark (!) implies that the outcome is globalized.
% \if@tempswa can be used to test if, at the end, anything was
% removed from #1.
\skvrobustdef*\skvremoveelements{\skv@testcl\skv@removeelements}
\skvrobustdef\skv@removeelements#1#2{%
  \begingroup
  \let\skv@origlist#1%
  \skvifdefTF#1{}{\def#1{}}%
  \edef\skv@rema{\unexpanded{#2}}%
  \skvcsvnormalize\skv@rema
  \let\skv@remb#1\let#1\@empty
  \skvcommaparse*\skv@remb\skv@tempa{%
    \skvxifinTF{,\skvoxdetok\skv@tempa,}{,\skvoxdetok\skv@rema,}{}{%
      \edef#1{\skvaddlist,#1\skvexpandonce\skv@tempa}%
    }%
  }%
  \skvexpanded{\endgroup
    \skvcmdexit#1%
    \ifx#1\@empty
      \noexpand\@tempswatrue
    \else
      \ifx#1\skv@origlist\noexpand\@tempswafalse\else
        \noexpand\@tempswatrue\fi
    \fi
  }%
  \ifskv@cl\global\let#1#1\fi
}

% \skvfilterreplaceelements!<listcmd>{<replacements>}<filter>
%
% <replacements> => {<old-1>}{<new-1>},...,{<old-n>}{<new-n>}
%
% An exclamation mark suffix (!) implies that the outcome is globalized.
% When there is no filter to be applied, \skvreplaceelements is only
% negligibly faster than \skvfilterreplaceelements. Hence \skvreplaceelements
% isn't defined in this package. When there is no <filter>, use \nofilter
% as the filter.
%
% Example:
%
% \def\cmd{a = 1 , b = 2 , c = 3}
% \skvfilterreplaceelements\cmd{{a = 1}{x = 1},{c = 3}{z=3}}\skv@getkeyname
%
\skvrobustdef*\skvfilterreplaceelements{%
  \skv@testcl\skv@filterreplaceelements
}
\skvrobustdef*\skv@filterreplaceelements#1#2#3{%
  \begingroup
  \skv@declarefilter{#3}%
  \skvifdefTF#1{\skvkvnormalize#1}{\def#1{}}%
  \def\do##1##2\skv@nil{%
    \ifx#3\skv@getkeyname
      \def\@do####1=####2=####3\skv@nil####4{%
        \edef####4{\skvtrimspace{####1}=\skvtrimspace{####2}}%
      }%
      \@do##1==\skv@nil\skv@old
      \@do##2==\skv@nil\skv@new
    \else
      \edef\skv@old{\unexpanded{##1}}%
      \edef\skv@new{\unexpanded{##2}}%
    \fi
  }%
  \skvcommaparse{#2}\skv@tempa{%
    \expandafter\do\skv@tempa\skv@nil
    \skv@filter\skv@old\skv@oldb
    \let\skv@tempb#1\let#1\@empty
    \skvcommaloop*\skv@tempb\skv@tempb{%
      \skv@filter\skv@tempb\skv@tempc
      \ifx\skv@tempc\skv@oldb
        \edef#1{\skvaddlist,#1\skvexpandonce\skv@new}%
      \else
        \edef#1{\skvaddlist,#1\skvexpandonce\skv@tempb}%
      \fi
    }%
  }%
  \skvaftergroupdef#1\endgroup
  \ifskv@cl\global\let#1#1\fi
}
\skvnewdef*\skvcurrentfullkey{\skv@header\skvcurrentkey}
\skvnewlet\skvcurrenttriple\skvcurrentfullkey
\skvrobustdef*\skvsetdefaultprefix#1{%
  \edef\skvdefaultprefix{\skvtrimspace{#1}}%
  \let\skv@defapf\skvdefaultprefix
}
\skvsetdefaultprefix{KV}
\skvrobustdef*\skv@makeprefix#1{%
  % It is required to first fully expand the prefix:
  \edef\skvcurrentprefix{#1}%
  \skvdespacecontent\skvcurrentprefix
}
% \skv@makeheader{<family>}
\skvrobustdef*\skv@makeheader#1{%
  % Fully expand the family, in case it is given as \skvcurrentfamily or
  % a local/temporary macro:
  \edef\skvcurrentfamily{#1}%
  \skvdespacecontent\skvcurrentfamily
  \ifx\skvcurrentprefix\@undefined
    \let\skvcurrentprefix\skvdefaultprefix
  \fi
  \edef\skv@header{%
    \ifx\skvcurrentprefix\@empty\else\skvcurrentprefix/\fi
    \ifx\skvcurrentfamily\@empty\else\skvcurrentfamily/\fi
  }%
  \ifx\skv@header\@empty
    \def\skv@header{/}%
    \let\skvcurrentpath\skv@header
  \else
    \def\reserved@a##1/\@nil{##1}%
    \edef\skvcurrentpath{\expandafter\reserved@a\skv@header\@nil}%
    \ifx\skvcurrentpath\@empty
      \def\skvcurrentpath{/}%
    \fi
  \fi
}
\skvrobustdef*\skv@testopta#1{%
  \skvifstar
    {\skv@sttrue\skv@t@stopta{#1}}
    {\skv@stfalse\skv@t@stopta{#1}}%
}
\skvrobustdef*\skv@t@stopta#1{\skvifplus{\skv@pltrue#1}{\skv@plfalse#1}}
\skvrobustdef*\skv@testoptb#1{%
  \skv@testopt{\skv@t@stoptb{#1}}\skvdefaultprefix
}
\skvrobustdef*\skv@t@stoptb#1[#2]#3{%
  \skv@makeprefix{#2}\skv@makeheader{#3}#1%
}
\skvrobustdef*\skv@testoptc#1{%
  \skv@testopt{\skv@t@stoptc{#1}}\skvdefaultprefix
}
\skvrobustdef*\skv@t@stoptc#1[#2]#3{%
  \skvxifinTF{,}{\detokenize{#2}}{%
    \skv@err{Only one prefix is allowed here,
      \MessageBreak but you gave '#2'}\skv@ehd
  }{%
    \skv@makeprefix{#2}%
    \edef\skv@fams{#3}%
    \skvxifinTF{,}{\detokenize{#3}}{%
      \skvcsvnormalize\skv@fams
    }{%
      \skvdespacecontent\skv@fams
    }%
    \skv@testopt#1{}%
  }%
}
% \skv@testoptd{<cmd>}{<pre-mp>}
\skvrobustdef*\skv@testoptd#1#2{%
  \skv@testoptb{%
    \edef\skv@provb{#2\skv@header}%
    \def\skv@prova{\skv@testopt{\skv@t@stoptd{#1}}}%
    \expandafter\skv@prova\expandafter{\skv@provb}%
  }%
}
% \skv@t@stoptd{<cmd>}[<mp>]{<key>}
\skvrobustdef*\skv@t@stoptd#1[#2]#3{%
  \skvifnextchar[{\skv@sttrue#1{#2}{#3}}{\skv@stfalse#1{#2}{#3}[]}%
}
\skvrobustdef*\skv@getkeyname#1#2{%
  \expandafter\skv@g@tkeyname#1=\skv@getname@nil#2%
}
\skvrobustdef*\skv@g@tkeyname#1=#2\skv@getname@nil#3{%
  \skv@strippointersfromkey{#1}%
  \let#3=\skvcurrentkey
}
\skvrobustdef*\skv@getkeyvalue#1#2{%
  \expandafter\skv@g@tkeyvalue#1==\skv@getvalue@nil#2%
}
\skvrobustdef*\skv@g@tkeyvalue#1={\skv@g@tk@yvalue#1=.}
\skvrobustdef*\skv@g@tk@yvalue#1=#2=#3\skv@getvalue@nil#4{%
  \edef#4{\unexpanded\expandafter{\@gobble#2}}%
  \skvexpbracenext\skvifbracedTF#4{%
    \skvvaluebracedtrue
  }{%
    \skvvaluebracedfalse
    \skvexpbracenext\skv@strippointersfromvalue#4%
  }%
  \let#4=\skvcurrentvalue
}
% \skv@getnamesofkeys{<kv list>}{<result macro>}
\skvrobustdef*\skv@getnamesofkeys#1#2{%
  \begingroup
  \edef\skv@prova{\unexpanded{#1}}%
  \skvkvnormalize\skv@prova
  \let#2\@empty
  \skvcommaloop*\skv@prova\skv@prova{%
    \expandafter\skv@g@tkeyname\skv@prova=\skv@getname@nil\skv@prova
    \edef#2{\skvaddlist,#2\skvexpandonce\skv@prova}%
  }%
  \skvaftergroupdef#2\endgroup
}
\skvnewdef*\skv@badkeynames{}
\skvnewdef*\skvaddbadkeynames{\skvappendtomacro\skv@badkeynames}
\skvrobustdef*\skv@definedefault#1#2{%
  \ifskv@inoptionsec\else
    \skvxifinTF{,\skvcurrentprefix,}{,skv,SKV,}{%
      \skvxifinTF{,\skvcurrentfamily,}{,skeyval,}{%
        \skv@err{Prefix/family '\skvcurrentpath' are reserved}\skv@ehd
      }{}%
    }{}%
  \fi
  \ifskv@tracingkeys
    \skvxifinTF{,#1,}{,\skv@badkeynames,}{%
      \skv@err{Key name '#1' not allowed}\skv@ehd
    }{}%
  \fi
  \skvcsedef{\skv@header#1.@defa}{%
    \skvnoexpandcs{\skv@header#1}{\unexpanded{#2}}%
  }%
  \skv@recordkey{#1}{#2}%
}

% 1. Record key and its initial/default value if the key appears in the
%    'needini' list of its family. The list 'needini' is made by the
%    command \skvsaveinitialvaluekeys.
% 2. To 'save initial values of keys', the key names must have been
%    entered by \skvsaveinitialvaluekeys in 'needini' list.
% 3. If a key has no default, then \skv@definedefault will not be called
%    and hence \skv@recordkey won't be invoked.
% 4. In \skvdefinekeys, if a key has no default, it won't be entered in
%    the 'needini' list. In \skvdefinekeys, an empty default value should
%    be indicated with a slash, eg, .cmd/keya/, .ord/keyb//,
%    or .ord/keyb/.na/.
% 5. In \skvdefinekeys, use the key/option '.save initial values' to
%    create 'needini' lists of families.
\skvrobustdef*\skv@recordkey#1#2{%
  \begingroup
  \skvifcsdefFT{\skvcurrentpath.@needini}{%
    \endgroup\skv@swafalse
  }{%
    \skv@swatrue
    \skvxifinTF{,#1,}{,\skvexpandcsonce{\skvcurrentpath.@needini},}{%
      \edef\skv@tempa{\skvtrimspace{#2}}%
      \edef\skv@tempa{%
        #1=\skvoifstrcmpTF{\skv@tempa}{true}{false}{\skvexpandonce\skv@tempa}%
      }%
      \skvletcs\skv@tempb{\skvcurrentpath.@inikv}%
      \skvifdefTF\skv@tempb{%
        \skvxifinTF{,\skvoxdetok\skv@tempa,}{,\skvoxdetok\skv@tempb,}{}{%
          \skvcsedef{\skvcurrentpath.@inikv}{%
            \skvaddlist,\skv@tempb\skvexpandonce\skv@tempa
          }%
        }%
      }{%
        \skvcsedef{\skvcurrentpath.@inikv}{\skvexpandonce\skv@tempa}%
      }%
    }{}%
  }%
  \ifskv@swa
    \expandafter\skvaftergroupdef\csname
      \skvcurrentpath.@inikv\expandafter\endcsname
      \expandafter\endgroup
  \fi
}

% Key will be given in the form <pointer>{<key>}. The command
% \skv@strippointersfromkey is called both when defining and setting keys.
%
% Notes:
%  1.  When setting keys, we also call \skv@replacepointers to replace
%      '.use value' pointer with the value of the key.
%  2.  There is no pointer '.save value', since the key's value is
%      always saved automatically.
%
% \skv@strippointersfromkey{<key name>}
% \skv@strippointersfromkey*{<key name cmd>}
%
% Return \skvcurrentkey.
%
\skvrobustdef*\skv@strippointersfromkey{%
  \skv@i@testst\skv@str@ppointersfromkey
}
\skvrobustdef*\skv@str@ppointersfromkey#1{%
  \begingroup
  \toks@{}%
  \skv@usetempst{#1}\skv@tempa
  % We can choose to ignore the search for pointers where we don't
  % use pointers. This is useful at least in one respect: during debugging
  % in non-pointer circumstances. In general, it is not advisable to ignore
  % pointers.
  \ifskv@ignorepointers\else
    \def\skv@tempb{\expandafter\skv@findpointer\expandafter{\skv@tempa}}%
    \def\skv@add##1{\edef\x{\toks@{\the\toks@##1}}\x}%
    \skv@tempb{.need value}\skv@tempa{%
      \skv@add{\skvcsdef{\skv@header\skv@tempa.@ndv}{}}%
    }{%
      \skv@tempb{.gneed value}\skv@tempa{%
        \skv@add{\skvcsgdef{\skv@header\skv@tempa.@ndv}{}}%
      }{%
        \skv@tempb{.forbid value}\skv@tempa{%
          \skv@add{\skvcsdef{\skv@header\skv@tempa.@fbv}{}}%
        }{%
          \skv@tempb{.gforbid value}\skv@tempa{%
            \skv@add{\skvcsgdef{\skv@header\skv@tempa.@fbv}{}}%
          }{}%
        }%
      }%
    }%
  \fi
  \skvexpanded{\endgroup
    \the\toks@
    % The following complication is because of, e.g., pntkeys:
    \edef\noexpand\skvcurrentkey{%
      \noexpand\unexpanded{\skvexpandonce\skv@tempa}%
    }%
  }%
}
% \skv@strippointersfromvalue{<key value>}
% \skv@strippointersfromvalue*{<key value cmd>}
%
% Strip pointers from a key's value. The pointers that may be used on
% values of keys are
%
%   .expand once process list   -> Expand value once and process the
%                                   expanded value as a list.
%   .expand twice process list  -> Expand value twice and process the
%                                   expanded value as a list.
%   .expand process list        -> Fully expand value and process the
%                                   expanded value as a list.
%   .eprocess list              -> Fully expand value and process the
%                                   expanded value as a list.
%   .process list               -> Process the given value as a list.
%   .list                       -> Process the given value as a list.
%   .expand once                -> Expand value once before parsing it.
%   .expand twice               -> Expand value twice before parsing it.
%   .expanded                   -> Fully expand value before parsing it.
%   .expand                     -> Fully expand value before parsing it.
%
% Return \skvcurrentvalue.
%
\skvrobustdef*\skv@strippointersfromvalue{%
  \skv@i@testst\skv@str@ppointersfromvalue
}
\skvrobustdef*\skv@str@ppointersfromvalue#1{%
  \begingroup
  \skv@usetempst{#1}\skv@tempa
  \ifskv@ignorepointers\else
    \def\skv@tempb{\expandafter\skv@findpointer\expandafter{\skv@tempa}}%
    % The following order is important, since '.expand' will match
    % '.expand once' and erroneously give the key's value as 'o'.
    \skv@tempb{.expand once process list}\skv@tempa{%
      \skv@processvalueaslisttrue
      \edef\skv@tempa{\skvexpandtwice\skv@tempa}%
    }{%
      \skv@tempb{.expand twice process list}\skv@tempa{%
        \skv@processvalueaslisttrue
        \edef\skv@tempa{\skvexpandthrice\skv@tempa}%
      }{%
        \skv@tempb{.expand process list}\skv@tempa{%
          \skv@processvalueaslisttrue
          \edef\skv@tempa{\skv@tempa}%
        }{%
          \skv@tempb{.eprocess list}\skv@tempa{%
            \skv@processvalueaslisttrue
            \edef\skv@tempa{\skv@tempa}%
          }{%
            \skv@tempb{.process list}\skv@tempa{%
              \skv@processvalueaslisttrue
            }{%
              \skv@tempb{.list}\skv@tempa{%
                \skv@processvalueaslisttrue
              }{%
                \skv@tempb{.expand once}\skv@tempa{%
                  \edef\skv@tempa{\skvexpandtwice\skv@tempa}%
                }{%
                  \skv@tempb{.expand twice}\skv@tempa{%
                    \edef\skv@tempa{\skvexpandthrice\skv@tempa}%
                  }{%
                    \skv@tempb{.expanded}\skv@tempa{%
                      \edef\skv@tempa{\skv@tempa}%
                    }{%
                      \skv@tempb{.expand}\skv@tempa{%
                        \edef\skv@tempa{\skv@tempa}%
                      }{}%
                    }%
                  }%
                }%
              }%
            }%
          }%
        }%
      }%
    }%
  \fi
  \let\skvcurrentvalue\skv@tempa
  \skvexpanded{\endgroup
    \skvcmdexit\skvcurrentvalue
    \skvboolexit\ifskv@processvalueaslist
  }%
}
\skvrobustdef*\skv@findpointer#1#2#3{%
  \def\skv@f@ndpointer##1#2##2##3\skv@pointer@nil{%
    \skvifstrcmpTF{##2}{\skv@nil}{%
      \@secondoftwo
    }{%
      % We don't want, eg, '<tokens>.expanded{value}', since in this case
      % applying \edef to the value macro may be unsafe on <tokens>:
      \skvifblankTF{##1}{}{%
        \skv@err{Nothing should come before the
          \MessageBreak pointer '#2' on key '##2'.
          \MessageBreak If you require the value of the key to be expanded,
          \MessageBreak you should have done the expansion yourself}\skv@ehd
      }%
      \edef#3{\skvtrimspace{##2}}%
      \@firstoftwo
    }%
  }%
  \skv@f@ndpointer#1#2{\skv@nil}\skv@pointer@nil
}
% \skv@extractpntkey@atdefkey{<toks>}{<cmd>}
%
% At define key, extract pseudo key name from a weird key name of the form
%
%     evaluate (?) as (?) using (?)
%
\skvrobustdef*\skv@extractpntkey@atdefkey#1#2{%
  \begingroup
  \@tempcnta\skvz@
  \def#2{}%
  \def\skv@prova##1(##2){%
    \def\skv@provb{##2}%
    \ifx\skv@provb\@nnil\else
      \advance\@tempcnta\@ne
      \edef#2{\skvexpandonce#2\skvtrimspace{##1}}%
      \expandafter\skv@prova
    \fi
  }%
  \skv@prova#1(\@nil)%
  \ifx#2\@empty
    \edef#2{\unexpanded{#1}}%
  \else
    % The number of arguments of the pseudo key is determined by the
    % number of closed parentheses:
    \skvcsedef{\skv@header#2.@x0arg}{\skvgenerateparameters{1}\@tempcnta}%
  \fi
  \skvexpanded{\endgroup
    \skvcmdexit#2%
    \skvcsexit{\skv@header#2.@x0arg}%
  }%
}
% \skv@extractpntkey@atsetkey{<toks>}
%
% At set key, extract pseudo key name from a weird key name of the form
%
%     evaluate (?) as (?) using (?)
%
\skvrobustdef*\skv@extractpntkey@atsetkey#1{%
  \begingroup
  \def\skvcurrentkey{}%
  \def\skvcurrentvalue{}%
  \def\skv@prova##1(##2){%
    \def\skv@provb{##2}%
    \ifx\skv@provb\@nnil\else
      \edef\skvcurrentkey{\skvxonce\skvcurrentkey\skvtrimspace{##1}}%
      \edef\skvcurrentvalue{\skvxonce\skvcurrentvalue{\skvtrimspace{##2}}}%
      \expandafter\skv@prova
    \fi
  }%
  \skv@prova#1(\@nil)%
  \ifx\skvcurrentkey\@empty
    \skv@err{No key name for a parenthesized key}\skv@ehd
    \expandafter\@nodocument
  \fi
  \skvexpanded{\endgroup
    \skvcmdexit\skvcurrentkey\skvcmdexit\skvcurrentvalue
  }%
}
\skvrobustdef*\skv@replacepointers#1{%
  \begingroup
  \let\skvcurrentvalue\@empty
  \let\skv@tempa\@empty
  \skvifbracedTF{#1}{%
    \skv@r@placepointers{#1}.use value\skv@nil
  }{%
    \skv@r@placepointers#1.use value\skv@nil
  }%
  \skvaftergroupdef\skvcurrentvalue\endgroup
}
% In the following scheme, if we have, eg,
%
%    key2=\dimexpr.use value{key1}*5\relax
%
% \dimexpr will be retained as part of the value of key2 in pointer
% replacement.
%
\skvrobustdef*\skv@r@placepointers#1.use value#2{%
  % In case #1 isn't empty:
  \edef\skvcurrentvalue{\skvexpandonce\skvcurrentvalue\unexpanded{#1}}%
  \edef\skv@prova{\unexpanded{#2}}%
  \skvifxTF\skv@prova\skv@nnil{}{%
    \skvifcsdefFT{\skv@header#2.@value}{%
      \skv@err{No value recorded for key '#2'; ignored}\skv@ehd
      \skv@r@placepointers
    }{%
      \skvxifinTF{,\detokenize{#2},}{,\skvoxdetok\skv@tempa,}{%
        \skv@err{Back linking of pointers;
          \MessageBreak pointer replacement canceled}\skv@ehd
      }{%
        \edef\skv@tempa{\skvaddlist,\skv@tempa\unexpanded{#2}}%
        \skvletcs\skv@prova{\skv@header#2.@value}%
        \skvexpbracenext\skvifbracedTF\skv@prova\skvexpbracenext\skvexpandnext
        \skv@r@placepointers\skv@prova
      }%
    }%
  }%
}

% Assign arguments to keys:
%
% \skvassignargs[<prefixes>]{<families>}{<keys>}{.<expansion type>{<arg>}}
%
% 1. Valid expansion types are .expand once, .expand twice, .expanded.
% 2. At set keys (not at define keys), the argument to the listed keys will
%    be expanded using the expansion type.
% 3. The argument will be assigned whether or not a key already has been
%    defined. This allows the user to define the key later, after its
%    argument has been fixed.
% 3. Under the macros \skvdefinekeys and \directkeys, there are equally
%    efficient handlers for assigning arguments to keys.
%
% Example:
%
%   \skvassignargs[KV1,KV2]{fam1,fam2}{keya,keyb}{.expanded{#1/#2}}
%
% The keys could then be set as
%
%   \skvsetkeys[KV1]{fam2}{keya=\vala/\valb}
%
% For each prefix and family, this will define parameterless functions
%
%   \<prefix>/<family>/<key>.@xxarg.
%
% which will be used at setkeys to define and execute the key's callback.
%
\skvrobustdef*\skvassignargs{\skv@testopt\skv@assignargs\skvdefaultprefix}
\skvrobustdef*\skv@assignargs[#1]#2#3#4{%
  \begingroup
  \let\skv@temparg\skv@simplearg
  \def\skv@expandertype{x0}%
  \edef\skv@tempa{\skvtrimspace{#4}}%
  \def\do##1##2{%
    \ifx\do##1\else
      \skvxifinTF{\detokenize{##1}}{\skvoxdetok\skv@tempa}{%
        \def\skv@prova####1##1####2####3\skv@arg@nil{%
          \edef\skv@temparg{\unexpanded{####2}}%
          \def\skv@expandertype{##2}%
        }%
        \expandafter\skv@prova\skv@tempa\skv@arg@nil
        \def\do####1\do\do{}%
      }{}%
      \expandafter\do
    \fi
  }%
  \do{.unexpanded}{x0}{.expand once}{x1}{.expand twice}{x2}%
    {.expanded}{xx}{.expand}{xx}\do\do
  \def\skv@tempc{}%
  % Loop over prefixes:
  \skvcommaparse{#1}\skv@tempa{%
    \skv@makeprefix\skv@tempa
    % Loop over families:
    \skvcommaparse{#2}\skv@tempa{%
      \skv@makeheader\skv@tempa
      % Loop over keys:
      \skvcommaparse{#3}\skv@tempa{%
        \edef\skv@tempc{%
          \skvexpandonce\skv@tempc
          \skvcsedef{\skv@header\skv@tempa.@\skv@expandertype arg}{%
            \noexpand\unexpanded{\skvexpandonce\skv@temparg}%
          }%
        }%
      }%
    }%
  }%
  \expandafter\endgroup\skv@tempc
}
% \skv@getexpander{<expander.type>}
%
% 1. <expander.type> is one of 'x0', 'x1', 'x2', 'xx', which had been
%    saved in a key-dependent macro.
%
% 2. \skv@getexpander returns macro \skvexpander, which will
%    contain one of \unexpanded, \skvexpandonce, \skvexpandtwice, \@iden.
%
\skvrobustdef*\skv@getexpander#1{%
  \begingroup
  \edef\skv@prova{\skvtrimspace{#1}}%
  \def\skv@provb##1{%
    \def\skv@provb####1##1####2####3\skv@nil{%
      \endgroup
      \def\skvexpander{####2}%
      \ifx\skvexpander\@nnil
        \skv@err{Unknown expansion type '\detokenize{##1}'}\skv@ehd
      \fi
    }%
    \skv@provb x0{\unexpanded},x1{\skvexpandonce},x2{\skvexpandtwice},%
      xx{\@iden},##1{\@nil}\skv@nil
  }%
  \expandafter\skv@provb\expandafter{\skv@prova}%
}
% \skv@getargpattern{<callback token list>}
%
% Get argument type from the key's callback. The valid tags are
%
%   .arg, .arg unexpanded, .arg expanded, .arg expand, .arg expand once,
%   .arg expand twice.
%
\skvrobustdef*\skv@getargpattern{%
  \let\skv@argpattern\@undefined
  \def\do##1##2{%
    \ifx\do##1\else
      \skvxifinTF{\detokenize{##1}}{\skvoxdetok\skv@callback}{%
        \def\skv@prova####1##1####2####3\skv@argpattern@nil{%
          \edef\skv@argpattern{\unexpanded{####2}}%
          \ifx\skv@argpattern\@empty
            \let\skv@argpattern\skv@simplearg
          \fi
          \edef\skv@callback{\skvtrimspace{####1}\skvtrimspace{####3}}%
        }%
        \expandafter\skv@prova\skv@callback\skv@argpattern@nil
        \def\skvexpandertype{##2}%
        \def\do####1\do\do{}%
      }{}%
      \expandafter\do
    \fi
  }%
  % The following order is important, to avoid incorrect match
  % of the search term:
  \do{.arg unexpanded}{x0}{.arg expand once}{x1}{.arg expand twice}{x2}%
    {.arg expanded}{xx}{.arg expand}{xx}{.arg}{x0}\do\do
  \ifdefined\skv@argpattern\else
    % Argument pattern might have been specified outside the key's
    % callback.
    \def\do##1{%
      \ifx\do##1\else
        \skvifnamedefTF{\skvcurrentfullkey.@##1arg}{%
          \skvletcs\skv@argpattern{\skvcurrentfullkey.@##1arg}%
          \def\skvexpandertype{##1}%
          \def\do####1\do{}%
        }{}%
        \expandafter\do
      \fi
    }%
    \do{xx}{x2}{x1}{x0}\do
  \fi
  \ifdefined\skv@argpattern
    % Possibly expand value:
    \skvstripouterbraces{2}\skv@argpattern
    \def\do##1##2{%
      \ifx\do##1\else
        \skvxifstrcmpTF{##2}\skvexpandertype{%
          \edef\skvcurrentvalue{%
            \expandafter##1\expandafter{\skvcurrentvalue}%
          }%
          \def\do####1\do\do{}%
        }{}%
        \expandafter\do
      \fi
    }%
    \do\@iden{xx}\skvexpandtwice{x2}\skvexpandonce{x1}\unexpanded{x0}\do\do
  \else
    \let\skv@argpattern\skv@simplearg
  \fi
}
% +++++++++++++ Ordinary keys:
%
% \skvordkey[<pref>]{<fam>}{<key>}[<defa>]{<callback>}
%
\skvrobustdef*\skvordkey{\skv@testoptb{\skv@ordkey{e}}}
\skvrobustdef*\skvordkeys{\skv@testoptb{\skv@ordkeys{e}}}
%
% \skvgordkey[<pref>]{<fam>}{<key>}[<defa>]{<callback>}
%
% Global ordinary keys. So far, these are needed only by \skvgdisablekey.
%
\skvrobustdef*\skvgordkey{\skv@testoptb{\skv@ordkey{x}}}
\skvrobustdef*\skvgordkeys{\skv@testoptb{\skv@ordkeys{x}}}
\skvrobustdef*\skv@ordkey#1#2{%
  \skv@strippointersfromkey{#2}%
  \skvexpanded{\skv@testopt{\skv@ordkey@a{#1}{\skvcurrentkey}}{^skv^}}%
}
\skvrobustdef*\skv@ordkey@a#1#2[#3]#4{%
  \skvifstrcmpTF{#3}{^skv^}{}{\skv@definedefault{#2}{#3}}%
  % The pointer '.hp' may be used to set a holder prefix for the key.
  \skvxifinTF{\detokenize{.hp}}{\detokenize{#4}}{%
    \def\skv@prova##1.hp##2##3\skv@ord@nil{%
      \let\skv@gobble@or@iden\@iden
      \edef\skv@hp{\unexpanded{##2}}%
      \edef\skv@callback{\unexpanded{##1##3}}%
    }%
    \skv@prova#4\skv@ord@nil
  }{%
    \let\skv@gobble@or@iden\@gobble
    \edef\skv@callback{\unexpanded{#4}}%
  }%
  \csname skvcs#1def\endcsname{\skv@header#2.@cbk}{%
    % This can be called in #3 access the value of ordinary key.
    % No prefix is used here, to reduce macro name:
    \skv@gobble@or@iden{\skvcslet{\skv@hp#2}\noexpand\skvcurrentvalue}%
    \skvexpandonce\skv@callback
  }%
}
\skvrobustdef*\skv@ordkeys#1#2{\skv@testopt{\skv@ordkeys@a{#1}{#2}}{^skv^}}
\skvrobustdef*\skv@ordkeys@a#1#2[#3]#4{%
  \skvcommaparse{#2}\skv@prova{%
    \skvexpbracenext\skv@strippointersfromkey\skv@prova
    \skvexpbracenext{\skv@ordkey@a{#1}}\skvcurrentkey[#3]{#4}%
  }%
}
% \skvvoidkey[<pref>]{<fam>}{<key>}[<defa>]{<callback>}
%
% A void key is an invalid key. A user who tries to set that key will
% automatically be told that the key is inadmissible. The author of an
% invalid key can also use <callback> to set a message.
%
\skvrobustdef*\skvvoidkey{\skv@testoptb\skv@voidkey}
\skvrobustdef*\skv@voidkey#1{%
  \skv@strippointersfromkey{#1}%
  \skvexpanded{\skv@testopt{\skv@voidkey@a{\skvcurrentkey}}{^skv^}}%
}
\skvrobustdef*\skv@voidkey@a#1[#2]#3{%
  \skvifstrcmpTF{#2}{^skv^}{}{\skv@definedefault{#1}{#2}}%
  \skvcsedef{\skv@header#1.@cbk}{%
    \unexpanded{#3}\relax
    \skv@err{Key '#1' of family '\skvcurrentpath'
      \MessageBreak has been set invalid by its author}\noexpand\skv@ehd
  }%
}
% \skvobsoletekey
%    [<pref>]{<fam>}{<obsolete key>}{<new key>}[<defa>]{<callback>}
%
% 1. An obsolete key is a key that is no longer in use and has
%    been replaced by a new key. A user who tries to set an obsolete
%    key will automatically be told that the key is obsolete and that
%    he/she should instead use the new key.
% 2. The author of an obsolete key can also use <callback> to set a
%    message for the user. <callback> can be empty.
% 3. Pointers can be used on both <obsolete key> and <new key>.
%
\skvrobustdef*\skvobsoletekey{\skv@testoptb\skv@obsoletekey}
\skvrobustdef*\skv@obsoletekey#1#2{%
  \skv@strippointersfromkey{#1}%
  \skvexpanded{%
    \skv@testopt{\skv@obsoletekey@a{\skvcurrentkey}{#2}}{^skv^}%
  }%
}
\skvrobustdef*\skv@obsoletekey@a#1#2[#3]#4{%
  \skvifstrcmpTF{#3}{^skv^}{}{\skv@definedefault{#1}{#3}}%
  \skvcsedef{\skv@header#1.@cbk}{%
    \unexpanded{#4}\relax
    \noexpand\skv@warn{Key '\skvcurrentpath/#1'
      \MessageBreak is now obsolete. Instead of using the obsolete
      \MessageBreak key '#1', I will now set the new key
      \MessageBreak '#2' with the value you have given for
      \MessageBreak key '#1'. You can avoid this warning by
      \MessageBreak using the new key '#2' instead of the
      \MessageBreak obsolete key '#1'}\noexpand\skv@ehd
  }%
}

%% Key names with parenthesized tokens.
%
% \skvpntkey[<pref>]{<fam>}{<key>}[<defa>]{<callback>}
%
% The tokens in parenthesis are removed when building the key name.
% Each parenthesis gives rise to one argument of the key's callback.
% When the key is set, the tokens in parenthesis are assigned to the
% arguments. It is the user's responsibility to catch those argument
% in the key's callback.
%
% Example - a key of three arguments:
%
%  \skvpntkey[KV]{fam}{evaluate (1) as (2) using (3)}{%
%    \def\oldcmd{#1}\def\newcmd{#2}\def\formula{#3}%
%    \def\x##1{#1*##1}%
%  }
%
%  \skvpntkey[KV]{fam}{evaluate (1) as (2) using (3)}[\x\y{\numexpr\x*2}]{%
%    \edef\x#2{#3}%
%  }
%
%  \skvshowcs{KV/fam/evaluateasusing/.@x0arg}
%
%  \skvsetkeys[KV]{fam}{evaluate (\x) as (\y) using (\numexpr\x*2)}
%
\skvrobustdef*\skvpntkey{\skv@testoptb\skv@pntkey}
\skvrobustdef*\skv@pntkey#1{%
  \skv@strippointersfromkey{#1}%
  \skvexpbracenext\skv@extractpntkey@atdefkey\skvcurrentkey\skvcurrentkey
  \skvexpanded{\skv@testopt{\skv@pntkey@a{\skvcurrentkey}}{^skv^}}%
}
\skvrobustdef*\skv@pntkey@a#1[#2]#3{%
  \skvifstrcmpTF{#2}{^skv^}{}{\skv@definedefault{#1}{#2}}%
  \skvcsedef{\skv@header#1.@cbk}{\unexpanded{#3}}%
}

%% Command keys:
%
% \skvcmdkey[<pref>]{<fam>}[<mp>]{<key>}[<defa>]{<callback>}
%
\skvrobustdef*\skvcmdkey{%
  \def\skv@zapsw{01}%
  \skv@testoptd\skv@cmdkey{cmd}%
}
% \skvzcmdkey will internally zap the spaces in the key's name, but the
% key user will not notice that: he can still use the key's name with
% spaces in it. The key's author could then use the zapped name internally
% in his code.
\skvrobustdef*\skvzcmdkey{%
  \def\skv@zapsw{00}%
  \skv@testoptd\skv@cmdkey{cmd}%
}
% When the key's value has doubled hash characters, xkeyval's definition
% of \skv@cmdkey fails:
\skvrobustdef*\skv@cmdkey#1#2[#3]#4{%
  \skv@strippointersfromkey{#2}%
  \skvifdefboolTF{skv@st}{\skv@definedefault\skvcurrentkey{#3}}{}%
  % This is to allow the key name to be expanded before possibly zapping
  % spaces in key name:
  \edef\skv@prova{#1\skvcurrentkey}%
  \edef\skv@prova{\expandafter\skv@zapornot\expandafter
    {\expandafter\skv@zapsw\expandafter}\expandafter{\skv@prova}}%
  \skvcsedef{\skv@header\skvcurrentkey.@cbk}{%
    \skvcslet{\skv@prova}\noexpand\skvcurrentvalue
    \unexpanded{#4}%
  }%
}
% \skvcmdkeys[<pref>]{<fam>}[<mp>]{<keys>}[<defa>]{<callback>}
\skvrobustdef*\skvcmdkeys{%
  \def\skv@zapsw{01}%
  \skv@testoptd\skv@cmdkeys{cmd}%
}
\skvrobustdef*\skvzcmdkeys{%
  \def\skv@zapsw{00}%
  \skv@testoptd\skv@cmdkeys{cmd}%
}
\skvrobustdef*\skv@cmdkeys#1#2[#3]#4{%
  \skvcommaparse{#2}\skv@tempa{%
    \skvexpanded{\skv@cmdkey{#1}{\skv@tempa}}[#3]{#4}%
  }%
}

%% List processor keys.
%
% \skvlistkey[<pref>]{<fam>}[<mp>]{<key>}[<defa>]{<callback>}
%
\skvrobustdef*\skv@getlistkeyparser#1{%
  \begingroup
  \let\skv@prova\undefined
  \skvxifinTF{\detokenize{\listsep}}{\detokenize{#1}}{%
    \skvxifinTF{\detokenize{\listparser}}{\detokenize{#1}}{%
      \skv@err{I find both \noexpand\listsep and \noexpand\listparser in the
        \MessageBreak callback of key '\skvcurrentfullkey'}\skv@ehd
    }{%
      \def\skv@prova{\listsep}%
    }%
  }{%
    \skvxifinTF{\detokenize{\listparser}}{\detokenize{#1}}{%
      \def\skv@prova{\listparser}%
    }{}%
  }%
  \skvifdefTF\skv@prova{%
    % Hide the parameter characters in #1 here:
    \edef\skv@provc{\unexpanded{#1}}%
    \def\skv@provb##1{%
      \def\skv@provb####1##1####2####3\skv@listparser@nil{%
        \skvifblankTF{####2}{%
          \def\skv@listparser{,}%
        }{%
          \edef\skv@listparser{\skvtrimspace{####2}}%
        }%
        \edef\skv@callback{\skvtrimspace{####1}\skvtrimspace{####3}}%
      }%
      \expandafter\skv@provb\skv@provc\skv@listparser@nil
    }%
    \expandafter\skv@provb\expandafter{\skv@prova}%
  }{%
    \def\skv@listparser{,}%
    \edef\skv@callback{\skvtrimspace{#1}}%
  }%
  \skvexpanded{\endgroup
    \skvcmdexit\skv@listparser\skvcmdexit\skv@callback
  }%
}
\skvnewlet\skvstopprocessinglistkey\skvbreakloop
\skvrobustdef*\skvlistkey{%
  \def\skv@zapsw{01}%
  \skv@testoptd\skv@listkey{list}%
}
\skvrobustdef*\skvzlistkey{%
  \def\skv@zapsw{00}%
  \skv@testoptd\skv@listkey{list}%
}
\skvrobustdef*\skv@listkey#1#2[#3]#4{%
  \skv@strippointersfromkey{#2}%
  \skvifdefboolTF{skv@st}{\skv@definedefault\skvcurrentkey{#3}}{}%
  % This is to allow the key name to be expanded before possibly zapping
  % spaces in key name:
  \edef\skv@provb{#1\skvcurrentkey}%
  \edef\skv@provb{\expandafter\skv@zapornot\expandafter
    {\expandafter\skv@zapsw\expandafter}\expandafter{\skv@provb}}%
  \skv@getlistkeyparser{#4}%
  % If there are more parameters in #4 than ####1, the next step
  % will raise an error:
  \skvxifinTF{\detokenize{##2}}{\skvoxdetok\skv@callback}{%
    \skv@err{A listkey can't have more than one
      \MessageBreak parameter character}\skv@ehd
  }{%
    \def\skv@prova{\skvcsdef{\skv@header\skvcurrentkey.@auxcbk}####1}%
    \expandafter\skv@prova\expandafter{\skv@callback}%
  }%
  \let\do\noexpand
  \skvcsedef{\skv@header\skvcurrentkey.@cbk}{%
    \skvcslet{\skv@provb}\do\skvcurrentvalue
    \edef\do\skv@prova{\do\unexpanded{####1}}%
    \do\skvstripouterbraces{2}\do\skv@prova
    % 1. \skvprocesslist processes an empty list.
    % 2. You can call \skvlistcount when processing listkeys, since
    %    \skvprocesslist initializes and increments it.
    \do\skvprocesslist*{\skv@listparser}\do\skv@prova\do\skv@prova{%
      \do\csname\skv@header\skvcurrentkey.@auxcbk%
      \do\expandafter\endcsname\do\expandafter{\do\skv@prova}%
    }%
  }%
  % A listkey must have a 1-parameter argument. We use the following
  % definition to enforce this requirement:
  \skvcsdef{\skv@header\skvcurrentkey.@listkey}{}%
}
% \skvlistkeys[<pref>]{<fam>}[<mp>]{<keys>}[<defa>]{<callback>}
\skvrobustdef*\skvlistkeys{%
  \def\skv@zapsw{01}%
  \skv@testoptd\skv@listkeys{list}%
}
\skvrobustdef*\skvzlistkeys{%
  \def\skv@zapsw{00}%
  \skv@testoptd\skv@listkeys{list}%
}
\skvrobustdef*\skv@listkeys#1#2[#3]#4{%
  \skvcommaparse{#2}\skv@tempa{%
    \skvexpanded{\skv@listkey{#1}{\skv@tempa}}[#3]{#4}%
  }%
}

%% Choice keys:
%
% The skeyval package allows holder-macro prefixes {<mp>} for choice keys.
%
%  \skvchoicekey[<pref>]{<fam>}[<mp>]{<keys>}[<bins>]{<choices>}
%     [<default>]{<callback>}
%  \skvchoicekey+[<pref>]{<fam>}[<mp>]{<keys>}[<bins>]{<choices>}
%     [<default>]{<callback>}{<fallback>}
%  \skvchoicekey*[<pref>]{<fam>}[<mp>]{<keys>}[<bins>]{<choices>}
%     [<default>]{<callback>}
%  \skvchoicekey*+[<pref>]{<fam>}[<mp>]{<keys>}[<bins>]{<choices>}
%     [<default>]{<callback>}{<fallback>}
%
%  \skvchoicekeys[KV]{fam}[mp@]{key1,key2}[\val\nr]{%
%    center.do=\def\vala{#1},
%    right.do=\def\valb{#1},
%    left.do=\def\valc{#1}
%  }[center]{\def\x##1{#1*##1}}
%
% \skv@preparenominations{00.or.01}{<altlist>}
\skvrobustdef*\skv@preparenominations#1#2{%
  \begingroup
  \def\skv@altlista{}%
  \def\skv@altlistb{}%
  \def\skv@provc##1.do=##2.do=##3\skv@choice@nil{%
    \if#1\lowercase{\fi
      \edef\skv@prova{\skvtrimspace{##1}}%
    \if#1}\fi
    \skvstripouterbraces{2}\skv@prova
    \edef\skv@altlista{%
      \skvaddlist,\skv@altlista\skvxonce\skv@prova
    }%
    \edef\reserved@a{%
      \skvnoexpandcs{\skvoxdetok\skv@prova @skvch}%
      {\skvtrimspace{##2}}%
    }%
    \edef\skv@altlistb{\skvxonce\skv@altlistb\skvxonce\reserved@a}%
  }%
  \skvcommaparse{#2}\skv@prova{%
    \expandafter\skv@provc\skv@prova.do=.do=\skv@choice@nil
  }%
  \ifx\skv@altlista\@empty
    \skv@err{No nominations (state pattern) for choice key}\skv@ehd
    \def\skv@altlistb{}%
  \fi
  \skvexpanded{\endgroup
    \skvcmdexit\skv@altlista\skvcmdexit\skv@altlistb
  }%
}
% \skv@executechoice{00 or 01}{<currentvalue>}{<altlist>}
\skvrobustdef*\skv@executechoice#1#2#3{%
  \begingroup
  \if#1\lowercase{\fi
    \edef\skv@prova{\skvtrimspace{#2}}%
  \if#1}\fi
  \skvstripouterbraces{2}\skv@prova
  \edef\do{%
    \expandafter\noexpand\csname\detokenize
    \expandafter{\skv@prova}@skvch\endcsname
  }%
  % Hide #3 in a macro to avoid confusing any parameter
  % characters in #3 with the parameters of \skv@prova:
  \edef\skv@provb{\unexpanded{#3}}%
  \edef\skv@prova{\def\noexpand\skv@prova####1\skvxonce\do####2####3}%
  \skv@prova\skv@choice@nil{%
    \toks@{##2}%
    \edef\skv@prova{\unexpanded{##2}}%
    \ifx\skv@prova\skv@nnil
      \skv@err{No state pattern match found for key
        \MessageBreak '\skvcurrentkey'}\skv@ehd
      \toks@{}%
    \fi
  }%
  \expandafter\expandafter\expandafter\skv@prova\expandafter
    \skv@provb\do{\skv@nil}\skv@choice@nil
  \expandafter\endgroup\the\toks@
}
\skvrobustdef*\skvchoicekey{%
  \skv@testopta{\skv@testoptb
    {\skv@testopt\skv@choicekey@a{choice\skv@header}}}%
}
\skvnewlet\skvchoicekeys\skvchoicekey
\skvrobustdef*\skv@choicekey@a[#1]#2{%
  \skvxifinTF{\skv@hashchar}{\detokenize{#2}}{%
    \skv@err{Hash character '\skv@hashchar' not allowed
      \MessageBreak in key name}\skv@ehd
  }{%
    \edef\skv@currlist{\unexpanded{#2}}%
    \edef\skv@hp{\skvtrimspace{#1}}%
    \skv@testopt\skv@choicekey@b{}%
  }%
}
\skvrobustdef*\skv@choicekey@b[#1]#2{%
  \edef\skv@bins{\unexpanded{#1}}%
  % Check the syntax of bins. This also helps catch wrong use syntax
  % of \skvchoicekeys: it's easy to get the syntax of \skvchoicekeys
  % wrong. The default value may have been put in place of bins.
  \ifx\skv@bins\@empty\else
    \skvtfor\skv@prova:=#1\do{%
      \skvexpbracenext\skvifescapedTF\skv@prova{}{%
        \skv@err{Token '\skvoxdetok\skv@prova' of bin of
          \MessageBreak choice key isn't escaped}\skv@ehd
      }%
    }%
  \fi
  \skvifblankTF{#2}{%
    \skv@err{No nominations (state pattern) for
      \MessageBreak choice keys '\skv@currlist'}\skv@ehd
  }{%
    \skvifboolTF{skv@st}{%
      \skv@preparenominations{00}{#2}%
    }{%
      \skv@preparenominations{01}{#2}%
    }%
  }%
  \skvifnextchar[\skv@choicekey@c{\skv@choicekey@c[^skv^]}%
}
\skvrobustdef*\skv@choicekey@c[#1]{%
  \edef\skv@default{\skvtrimspace{#1}}%
  % Choice can't have braced values, since that will make matching
  % to the state pattern difficult or impossible:
  \skvstripouterbraces{2}\skv@default
  \skvifdefboolTF{skv@pl}\skv@choicekey@e\skv@choicekey@d
}
\skvrobustdef*\skv@choicekey@d#1{%
  \skvexpanded{%
    \noexpand\skv@choicekey@f{{%
      \noexpand\skv@executechoice\ifskv@st{00}\else{01}\fi
        {####1}{\skvxonce\skv@altlistb}%
      \unexpanded{#1}%
    }}%
  }%
}
\skvrobustdef*\skv@choicekey@e#1#2{%
  \skvexpanded{%
    \noexpand\skv@choicekey@f{{%
      \noexpand\skv@executechoice\ifskv@st{00}\else{01}\fi
        {####1}{\skvxonce\skv@altlistb}%
      \unexpanded{#1}%
    }{\unexpanded{#2}}}%
  }%
}
\skvrobustdef*\skv@choicekey@f#1{%
  \edef\skv@prova##1##2{%
    \ifskv@st\noexpand\skv@sttrue\else\noexpand\skv@stfalse\fi
    \ifskv@pl\noexpand\skv@pltrue\else\noexpand\skv@plfalse\fi
    \noexpand\skv@checkchoice
    \ifx\skv@bins\@empty\else[\skvxonce\skv@bins]\fi
    {##1}{\skvxonce\skv@altlista}##2%
  }%
  \skv@temptoks\expandafter{\skv@prova{##1}{#1}}%
  % Why separate \skv@choicekey@g? It is needed by skeyval-view.sty:
  \skv@choicekey@g
}
\skvrobustdef*\skv@choicekey@g{%
  \skvcommaparse*\skv@currlist\skv@prova{%
    \skvexpbracenext\skv@strippointersfromkey\skv@prova
    \ifx\skv@default\skv@rej\else
      \skvexpanded{%
        \noexpand\skv@definedefault
          {\skvxonce\skvcurrentkey}{\skvxonce\skv@default}%
      }%
    \fi
    \skvcsedef{\skv@header\skvcurrentkey.@cbk}{%
      \skvcslet{\skv@hp\skvcurrentkey}\noexpand\skvcurrentvalue
      \the\skv@temptoks
    }%
  }%
}

\skvrobustdef*\skv@togkey@settog#1#2#3{%
  \edef\skv@prova{\skv@zapornot{#1}{#2}}%
  \csname skvsettog#3\expandafter\endcsname\expandafter{\skv@prova}%
}

%% Boolean keys:
%
% \skvboolkey[<pref>]{<fam>}[<mp>]{<key>}[<defa>]{<callback>}
% \skvboolkey+[<pref>]{<fam>}[<mp>]{<keys>}[<defa>]{<callback>}{<fallback>}
%
% Boolean keys create a store to receive the key's value and also create
% a boolean internally.
%
\skvrobustdef*\skvboolkey{%
  \def\skv@typetogkey{01}%
  \def\skv@zapsw{01}%
  \skv@t@stopta{\skv@testoptd\skv@boolkey{}}%
}
% \skvzboolkey will internally zap the spaces in the key's name and in
% the boolean that it creates internally, but the key user will not
% notice that: he will still be able to submit the original key's name
% with spaces in it. The key's author could then use the zapped key
% name and boolean in his code (internally).
\skvrobustdef*\skvzboolkey{%
  \def\skv@typetogkey{01}%
  \def\skv@zapsw{00}%
  \skv@t@stopta{\skv@testoptd\skv@boolkey{}}%
}
% \skv@boolkeys{<mp>}{<key>}[<default>]
\skvrobustdef*\skv@boolkey#1#2[#3]{%
  \skv@strippointersfromkey{#2}%
  \skvexpanded{%
    \ifskv@pl\skv@boolkey@b\else\skv@boolkey@a\fi
    {\skvcurrentkey}{#1\skvcurrentkey}%
  }{#3}%
}
% \skv@boolkey@a{<key>}{<mp.key>}{<default>}{<callback>}
\skvrobustdef*\skv@boolkey@a#1#2#3#4{%
  \def\skv@tempa{\skv@boolkey@c{#1}{#2}{#3}}%
  \skvifknobTF{skv@typetogkey}{%
    \expandafter\skv@tempa\expandafter{\expandafter{\expandafter
      \skv@togkey@settog\expandafter{\skv@zapsw}{#2}\skv@value#4}}%
  }{%
    \expandafter\skv@tempa\expandafter{\expandafter{\expandafter
      \csname\expandafter\skv@zapornot\expandafter{\skv@zapsw}{#2}%
      \skv@value\endcsname#4}}%
  }%
}
% \skv@boolkey@b{<key>}{<mp.key>}{<default>}{<callback>}{<fallback>}
\skvrobustdef*\skv@boolkey@b#1#2#3#4#5{%
  \def\skv@tempa{\skv@boolkey@c{#1}{#2}{#3}}%
  \skvifknobTF{skv@typetogkey}{%
    \expandafter\skv@tempa\expandafter{\expandafter{\expandafter
      \skv@togkey@settog\expandafter{\skv@zapsw}{#2}\skv@value#4}{#5}}%
  }{%
    \expandafter\skv@tempa\expandafter{\expandafter{\expandafter
      \csname\expandafter\skv@zapornot\expandafter{\skv@zapsw}{#2}%
      \skv@value\endcsname#4}{#5}}%
  }%
}
% \skv@boolkey@c{<key>}{<mp.key>}{<default>}{{<callback>}{<fallback>}}
\skvrobustdef*\skv@boolkey@c#1#2#3#4{%
  \if\skv@typetogkey
    \skvdeftog{\skv@zapornot{\skv@zapsw}{#2}}%
  \else
    \skvcsnewif{\skv@zapornot{\skv@zapsw}{#2}}%
  \fi
  \skvifdefboolTF{skv@st}{\skv@definedefault{#1}{#3}}{}%
  \edef\skv@tempa##1##2{%
    \noexpand\skv@sttrue
    \ifskv@pl\noexpand\skv@pltrue\else\noexpand\skv@plfalse\fi
    \skv@checkchoice[\noexpand\skv@value]{##1}{true,false}##2%
  }%
  \skv@temptoks\expandafter{\skv@tempa{##1}{#4}}%
  \skvcsedef{\skv@header#1.@cbk}{\the\skv@temptoks}%
}
%
% \skvboolkeys[<pref>]{<fam>}[<mp>]{<keys>}[<defa>]{<callback>}
% \skvboolkeys+[<pref>]{<fam>}[<mp>]{<keys>}[<defa>]{<callback>}{<fallback>}
%
\skvrobustdef*\skvboolkeys{%
  \def\skv@typetogkey{01}%
  \def\skv@zapsw{01}%
  \skv@t@stopta{\skv@testoptd\skv@boolkeys{}}%
}
\skvrobustdef*\skvzboolkeys{%
  \def\skv@typetogkey{01}%
  \def\skv@zapsw{00}%
  \skv@t@stopta{\skv@testoptd\skv@boolkeys{}}%
}
% \skv@boolkeys{<mp>}{<keys>}[<default>]
\skvrobustdef*\skv@boolkeys#1#2[#3]{%
  \skvifdefboolTF{skv@pl}\skv@boolkeys@b\skv@boolkeys@a{#2}{#1}{#3}%
}
% \skv@boolkeys@a{<keys>}{<mp>}{<default>}{<callback>}
\skvrobustdef*\skv@boolkeys@a#1#2#3#4{\skv@boolkeys@c{#1}{#2}{#3}{#4}{^skv^}}
% \skv@boolkeys@b{<keys>}{<mp>}{<default>}{<callback>}{<fallback>}
\skvrobustdef*\skv@boolkeys@b#1#2#3#4#5{\skv@boolkeys@c{#1}{#2}{#3}{#4}{#5}}
\skvrobustdef*\skv@boolkeys@c#1#2#3#4#5{%
  \skvcommaparse{#1}\skv@tempa{%
    \skvexpbracenext\skv@strippointersfromkey\skv@tempa
    \skvexpanded{%
      \skvifstrcmpTF{#5}{^skv^}{%
        \skv@boolkey@a{\skvcurrentkey}%
          {#2\skvcurrentkey}\unexpanded{{#3}{#4}}%
      }{%
        \skv@boolkey@b{\skvcurrentkey}%
          {#2\skvcurrentkey}\unexpanded{{#3}{#4}{#5}}%
      }%
    }%
  }%
}
%
% \skvbiboolkeys[<pref>]{<fam>}[<mp>]{<key1,key2>}[<defa>]
%    {<callback.for.key1>}{<callback.for.key2>}
% \skvbiboolkeys+[<pref>]{<fam>}[<mp>]{<key1,key2>}[<defa>]
%    {<callback.for.key1>}{<callback.for.key2>}{<fallback>}
%
% Example:
%
% \skvbiboolkeys+[KV]{fam}[mp@]{.need value{keya},keyb}[true]{%
%    \ifmp@keya\def\xa##1{##1}\fi
% }{%
%    \ifmp@keyb\def\xb##1{##1}\fi
% }{%
%    \skv@warn{Value '#1' is invalid}%
% }
%
\skvrobustdef*\skvbiboolkeys{%
  \def\skv@typetogkey{01}%
  \def\skv@zapsw{01}%
  \skv@t@stopta{\skv@testoptd\skv@biboolkeys{}}%
}
\skvrobustdef*\skvzbiboolkeys{%
  \def\skv@typetogkey{01}%
  \def\skv@zapsw{00}%
  \skv@t@stopta{\skv@testoptd\skv@biboolkeys{}}%
}
\skvrobustdef*\skv@biboolkeys#1#2[#3]{%
  \begingroup
  \edef\skv@currlist{\unexpanded{#2}}%
  \skvcsvnormalize\skv@currlist
  \@tempcnta\skvz@
  \skvcommaloop*\skv@currlist\skv@tempa{%
    \advance\@tempcnta\@ne
    \ifnum\@tempcnta>\tw@
      \skvbreakloop
    \fi
  }%
  \ifnum\@tempcnta=\tw@\else
    \skv@err{Number of bi-keys isn't 2:
      \MessageBreak ||\skv@currlist||}\skv@ehd
  \fi
  \skvexpanded{%
    \ifskv@pl\skv@biboolkeys@b\else\skv@biboolkeys@a\fi
    {\skv@currlist}%
  }{#1}{#3}%
}
% \skv@bilboolkeys@a{<key1,key2>}{<mp>}{<default>}{<callback1>}{<callback2>}
\skvrobustdef*\skv@biboolkeys@a#1#2#3#4#5{%
  \skv@biboolkeys@c{#1}{#2}{#3}{#4}{#5}{^skv^}%
}
% \skv@bilboolkeys@a{<key1,key2>}{<mp>}{<default>}
%    {<callback1>}{<callback2>}{<fallback>}
\skvrobustdef*\skv@biboolkeys@b#1#2#3#4#5#6{%
  \skv@biboolkeys@c{#1}{#2}{#3}{#4}{#5}{#6}%
}
\skvrobustdef*\skv@biboolkeys@c#1#2#3#4#5#6{%
  % Don't group the following: pointers will be lost outide the group.
  % 'bicallerid' is used to indicate that the master key is the one
  % that has instantiated the callback of the slave. This avoids
  % infinite re-entrance of \skvsetkeys.
  \edef\skv@default{\unexpanded{#3}}%
  \edef\skv@tempc{\unexpanded{#4}}%
  \edef\skv@tempd{\unexpanded{#5}}%
  \edef\skv@tempe{\unexpanded{#6}}%
  \toks@{}\def\skv@provd{}%
  \let\nx\noexpand
  \def\@do##1##2{%
    \skvifcsname\skv@header##1.@##2\then
      \edef\skv@provd{%
        \skv@provd
        \skvcsdef{\skv@header##1.@##2}{%
          \csname\skv@header##1.@##2\endcsname
        }%
      }%
    \fi
  }%
  \def\skv@provc##1##2##3##4{%
    \skvsettogtrue{\skv@header bicallerid/##3}%
    \skvxonce\@elt
    \nx\skvifxTF\nx\skvcurrentvalue\nx\skv@truetoks{%
      \nx\skviftogTF{\skv@header bicallerid/##4}{}{%
        \skvsetkeys[##1]{##2}{##4=false}%
      }%
    }{%
      \nx\skviftogTF{\skv@header bicallerid/##4}{}{%
        \skvsetkeys[##1]{##2}{##4=true}%
      }%
    }%
    \skvsettogfalse{\skv@header bicallerid/##3}%
  }%
  % \skv@provb{<KV>}{<fam>}{<primary.key>}{<secondary.key>}
  \def\skv@provb##1##2##3##4{%
    \@do{##3}{ndv}\@do{##3}{fbv}%
    \skvexpanded{%
      \toks@{\the\toks@
        \skvdeftog{\skv@header bicallerid/##3}%
        \skvifstrcmpTF{#6}{^skv^}{%
          \skv@boolkey@a
            {##3}{#2##3}{\skvxonce\skv@default}{%
              \skv@provc{##1}{##2}{##3}{##4}%
            }%
        }{%
          \skv@boolkey@b
            {##3}{#2##3}{\skvxonce\skv@default}{%
              \skv@provc{##1}{##2}{##3}{##4}%
            }{\skvxonce\skv@tempe}%
        }%
      }%
    }%
  }%
  \def\skv@prova##1,##2\skv@nil{%
    \skv@strippointersfromkey{##1}%
    \let\skv@tempa\skvcurrentkey
    \skv@strippointersfromkey{##2}%
    \let\skv@tempb\skvcurrentkey
    \skvexpanded{%
      \let\nx\@elt\nx\skv@tempc
      \nx\skv@provb{\skvcurrentprefix}{\skvcurrentfamily}%
        {\skv@tempa}{\skv@tempb}%
      \let\nx\@elt\nx\skv@tempd
      \nx\skv@provb{\skvcurrentprefix}{\skvcurrentfamily}%
        {\skv@tempb}{\skv@tempa}%
    }%
  }%
  \skv@prova#1\skv@nil
  \skvexpanded{\endgroup
    \skv@provd\the\toks@
  }%
}

%% Toggle keys:
%
% \skvtogkey[<pref>]{<fam>}[<mp>]{<key>}[<defa>]{<callback>}
% \skvtogkey+[<pref>]{<fam>}[<mp>]{<key>}[<defa>]{<callback>}{<fallback>}
%
\skvrobustdef*\skvtogkey{%
  \def\skv@typetogkey{00}%
  \def\skv@zapsw{01}%
  \skv@t@stopta{\skv@testoptd\skv@boolkey{}}%
}
\skvrobustdef*\skvztogkey{%
  \def\skv@typetogkey{00}%
  \def\skv@zapsw{00}%
  \skv@t@stopta{\skv@testoptd\skv@boolkey{}}%
}
\skvrobustdef*\skvtogkeys{%
  \def\skv@typetogkey{00}%
  \def\skv@zapsw{01}%
  \skv@t@stopta{\skv@testoptd\skv@boolkeys{}}%
}
\skvrobustdef*\skvztogkeys{%
  \def\skv@typetogkey{00}%
  \def\skv@zapsw{00}%
  \skv@t@stopta{\skv@testoptd\skv@boolkeys{}}%
}
% \skvbitogkeys[<pref>]{<fam>}[<mp>]{<key1,key2>}[<defa>]
%    {<callback.for.key1>}{<callback.for.key2>}
% \skvbitogkeys+[<pref>]{<fam>}[<mp>]{<key1,key2>}[<defa>]
%    {<callback.for.key1>}{<callback.for.key2>}{<fallback>}
\skvrobustdef*\skvbitogkeys{%
  \def\skv@typetogkey{00}%
  \def\skv@zapsw{01}%
  \skv@t@stopta{\skv@testoptd\skv@biboolkeys{}}%
}
\skvrobustdef*\skvzbitogkeys{%
  \def\skv@typetogkey{00}%
  \def\skv@zapsw{00}%
  \skv@t@stopta{\skv@testoptd\skv@biboolkeys{}}%
}
\skvrobustdef*\skvSignalkeyPresetException#1{%
  \edef\skv@signalpreseterr{\unexpanded{#1}}%
}
\skvSignalkeyPresetException{%
  \@latex@error{%
    Key '\skvcurrentfullkey'
    \MessageBreak is a signal key. It shouldn't have
    \MessageBreak been preset. Presetting signal keys
    \MessageBreak does lead to cyclic key setting
  }\skv@ehd
}

% Declare prefix and family and then define/set keys on them (without
% the need to give prefix and family). This can be handy if all the keys
% in a project have the same prefix and family.
%
% Example:
%
%   \skvsetprefix{KV}
%   \skvsetfamily{fam}
%   \skvdefineordkey{key1}[default]{\def\x##1{##1*#1}}
%   \skvprocesskeys{key1=value1}
%
\skvrobustdef*\skvsetprefix{\def\skv@currpref}
\skvrobustdef*\skvsetfamily{\def\skv@currfam}
\skvrobustdef*\skv@defineonmeta#1{%
  \ifdefined\skv@currpref\else
    \let\skv@currpref\skvdefaultprefix
  \fi
  \skvexpanded{\noexpand#1[\skv@currpref]{\skv@currfam}}%
}
\skvrobustdef*\skvdefineordkey{\skv@defineonmeta\skvordkey}
\skvrobustdef*\skvdefineordkeys{\skv@defineonmeta\skvordkeys}
\skvrobustdef*\skvdefinecmdkey{\skv@defineonmeta\skvcmdkey}
\skvrobustdef*\skvdefinecmdkeys{\skv@defineonmeta\skvcmdkeys}
\skvrobustdef*\skvdefineboolkey{\skv@defineonmeta\skvboolkey}
\skvrobustdef*\skvdefineboolkeys{\skv@defineonmeta\skvboolkeys}
\skvrobustdef*\skvdefinebiboolkeys{\skv@defineonmeta\skvbiboolkeys}
\skvrobustdef*\skvdefinetogkey{\skv@defineonmeta\skvtogkey}
\skvrobustdef*\skvdefinetogkeys{\skv@defineonmeta\skvtogkeys}
\skvrobustdef*\skvdefinechoicekey{\skv@defineonmeta\skvchoicekey}
\skvrobustdef*\skvdefinechoicekeys{\skv@defineonmeta\skvchoicekeys}
\skvrobustdef*\skvprocesskeys{\skv@defineonmeta\skvsetkeys}

% Signal-slot keys:
%
% \skvappendslots[<pref>]{<fam>}{<signal.keys>}{<slots>}
%     [<signal default>]{<signal callback>}
% \skvprependslots[<pref>]{<fam>}{<signal.keys>}{<slots>}
%     [<signal default>]{<signal callback>}
%
% Example:
%
%  \skvordkeys[KV]{fam}{keya,keyb}{\def\x##1{#1*##1}}
%  \skvappendslots[KV]{fam}{keyd,keye}{keya=.expanded{\vala},keyb=valb}
%     [def-d&e]{\def\y##1{#1*##1}}
%
% 1. <slots> must pre-exist. If slot key is undefined, then the signal-slot
%    system isn't useful here since the slot will serve no purpose.
%
% 2. If desired, use pointers/handlers .expanded, .expand once, .expand twice
%    on values of <slots>.
%
% 3. Here, it helps to consider <signal.keys> as parents (or signals/
%   subjects/observables) and <slots> as children (or slots/observers).
%
% 4. <signal.keys> can't be preset, to avoid cyclic setting of keys.
%    Consider the following, for a signal key in the preset list:
%
%       set any key on a path -> preset 'signal'
%       -> set 'slot' -> preset 'signal'.
%
%    In the attempt to set a slot key, the preset list (that includes
%    the signal key) will be instantiated.
%
\AtEndOfPackage{%
  \skvnewcastcommands{%
    \skvslotkeys=\skvappendslots,\skvstylekeys=\skvappendslots,
    \skvprependstyles=\skvprependslots,
    \skvappendstylesexpanded=\skvappendslotsexpanded,
    \skvprependstylesexpanded=\skvprependslotsexpanded,
    \skvaddstyles=\skvaddslots,
    \skvobserverkeys=\skvappendslots,
    \skvprependobservers=\skvprependslots,
    \skvappendobserversexpanded=\skvappendslotsexpanded,
    \skvprependobserversexpanded=\skvprependslotsexpanded,
    \skvaddobservers=\skvaddslots
  }%
}
\skvrobustdef*\skvappendslots{%
  \def\skv@type{app}%
  \let\skvexpanderpointer\@iden
  \skv@testoptb\skv@appendslots
}
\skvrobustdef*\skvprependslots{%
  \def\skv@type{prep}%
  \let\skvexpanderpointer\@iden
  \skv@testoptb\skv@appendslots
}
\skvrobustdef*\skvappendslotsexpanded{%
  \def\skv@type{app}%
  \def\skvexpanderpointer{.expanded}%
  \skv@testoptb\skv@appendslots
}
\skvrobustdef*\skvprependslotsexpanded{%
  \def\skv@type{prep}%
  \def\skvexpanderpointer{.expanded}%
  \skv@testoptb\skv@appendslots
}
\skvrobustdef*\skv@appendslots#1#2{%
  \skv@testopt{\skv@appendslots@a{#1}{#2}}{^skv^}%
}
% #1=signal keys, #2=slot keys, #3=signal default, #4=signal callback
\skvrobustdef*\skv@appendslots@a#1#2[#3]#4{%
  \skvcommaparse{#1}\skv@prova{%
    \skvexpbracenext\skv@strippointersfromkey\skv@prova
    \skvexpanded{%
      \skvifstrcmpTF{#3}{^skv^}{}{%
        % If the signal aready exists, the default value will be
        % overridden:
        \skv@definedefault{\skvcurrentkey}{\unexpanded{#3}}%
      }%
      \skv@appendslots@b{\skvcurrentkey}\unexpanded{{#2}{#4}}%
    }%
  }%
}
% \skv@appendslots@b{<signal>}{<slots>}{<signal.callback>}
\skvrobustdef*\skv@appendslots@b#1#2#3{%
  \def\skv@slotlist{}%
  \skvkvparse{#2}\skv@prova{%
    \skv@okvsplit\skv@prova{%
      \skvxifstrcmpTF{#1}{##1}{%
        \skv@err{Linking key '##1' to itself}\skv@ehd
      }{%
        % If slot key is undefined, then the signal-slot system isn't
        % useful, since the slot won't be able to do anything with the
        % emitted signal.
        \skvifcsdefTF{\skv@header##1.@cbk}{}{%
          \skv@err{Slot key '\skvcurrentpath/##1'
            \MessageBreak is undefined}\skv@ehd
        }%
      }%
      \edef\skv@slotlist{%
        \skvaddlist,\skv@slotlist\unexpanded{##1}=%
        \skvexpanderpointer{\unexpanded{##2}}%
      }%
    }%
  }%
  \edef\skv@elt{%
    % Signal keys shouldn't be preset, to avoid cyclic setting of keys.
    % See note above.
    \noexpand\skvifdefboolTF{skv@inprepo}{%
      \noexpand\skv@signalpreseterr
    }{%
      \noexpand\skvsetkeys[\skvcurrentprefix]%
        {\skvcurrentfamily}{\skvexpandonce\skv@slotlist}%
    }%
  }%
  % The signal key might already exists, especially when using
  % \skvaddslots:
  \edef\elt{%
    \skvifcsdefTF{\skv@header#1.@cbk}%
      {\skvexpandcsonce{\skv@header#1.@cbk}}{}%
  }%
  \skvcsedef{\skv@header#1.@cbk}{%
    \skvxifstrcmpTF{\skv@type}{prep}{%
      \skvexpandonce\skv@elt\skvtrimspace{#3}\skvexpandonce\elt
    }{%
      \skvexpandonce\elt\skvtrimspace{#3}\skvexpandonce\skv@elt
    }%
  }%
}
%
% \skvaddslots[<pref>]{<fam>}{<signals>}{<prepended.slots>}
%     {<appended.slots>}[<signal.default>]{<signal.callback>}
%
% Slot keys are observer keys that receive signals from signal
% (ie, subject) keys.
%
% Examples:
%
%   \skvordkeys[KV]{fam}{keya1,keyb1,keya2,keyb2}{\def\x##1{#1*##1}}
%   \skvaddslots[KV]{fam}{keyd,keye}{keya1=vala,keyb1=valb}
%      {keya2=vala,keyb2=.expanded{\valb}}[def-d&e]{\def\y##1{#1*##1}}
%
%   \skvordkeys{graph}{avertices,bvertices}[6]{\def\x##1{#1+##1}}
%   \skvaddslots{graph}{vertices}{avertices=4}{bvertices=8}[6]
%       {\def\y##1{#1*##1}}
%   \skvsetkeys{graph}{vertices=6}
%
\skvrobustdef*\skvaddslots{%
  \let\skvexpanderpointer\@iden
  \skv@testoptb\skv@addslots
}
\skvrobustdef*\skv@addslots#1#2#3{%
  \skv@testopt{\skv@addslots@a{#1}{#2}{#3}}{^skv^}%
}
% \skv@addslots@a{<signals>}{<prepended slots>}{<appended slots>}
%     [<signal default>]{<signal callback>}
\skvrobustdef*\skv@addslots@a#1#2#3[#4]#5{%
  \skvexpanded{%
    \skvprependslots[\skvcurrentprefix]{\skvcurrentfamily}%
      \unexpanded{{#1}{#2}[#4]{#5}}%
    % Without \ifskv@addslots@appending, when using \skvaddslots,
    % signal keys will otherwise be added in the database twice
    % (while treating prepended and appended slots).
    \noexpand\skv@addslots@appendingtrue
    \skvappendslots[\skvcurrentprefix]{\skvcurrentfamily}%
      \unexpanded{{#1}{#3}[#4]{#5}}%
    \noexpand\skv@addslots@appendingfalse
  }%
}

% Checking the admissible values of keys:
%
\skvrobustdef*\skvcheckchoice{\skv@testopta{\skv@testopt\skv@checkchoice{}}}
\skvrobustdef*\skv@checkchoice[#1]#2#3{%
  \begingroup
  \edef\skv@tempa{\skvtrimspace{#2}}%
  \def\skv@tempb{#3}%
  \skvcsvnormalize\skv@tempb
  \skvexpanded{%
    \ifskv@st\lowercase{\fi
      \ifcat$\detokenize{#1}$%
        \skv@checkchoice@b\skv@nil
        {\skvexpandonce\skv@tempa}{\skvexpandonce\skv@tempb}%
      \else
        \skv@checkchoice@a\unexpanded{#1}\skv@nil
        {\skvexpandonce\skv@tempa}{\skvexpandonce\skv@tempb}%
      \fi
    \ifskv@st}\fi
  }%
}
\skvrobustdef*\skv@checkchoice@a#1#2\skv@nil#3#4{%
  \def\skv@tempa{#2}%
  \skvifxTF\skv@tempa\@empty{%
    \skv@checkchoice@b#1{#3}{#4}%
  }{%
    \skv@checkchoice@c#1#2{#3}{#4}%
  }%
}
\skvrobustdef*\skv@checkchoice@b#1#2#3{%
  \def\skv@tempa{#1}%
  \ifx\skv@tempa\skv@nnil
    \def\skv@tempa{\endgroup}%
  \else
    \def\skv@tempa{\endgroup\def#1{#2}}%
  \fi
  \skvxifinTF{,\detokenize{#2},}{,\detokenize{#3},}{%
    \ifskv@pl
      \skvappendtomacro\skv@tempa{\@firstoftwo}%
    \else
      \skvappendtomacro\skv@tempa{\@firstofone}%
    \fi
  }{%
    \ifskv@pl
      \skvappendtomacro\skv@tempa{\@secondoftwo}%
    \else
      \skv@err{Value '\detokenize{#2}' is not allowed}\skv@ehd
      \skvappendtomacro\skv@tempa{\@gobble}%
    \fi
  }%
  \skv@tempa
}
\skvrobustdef*\skv@checkchoice@c#1#2#3#4{%
  \@tempcnta\skvz@
  \def\skv@tempa{#3}%
  \edef\skv@tempc{\unexpanded{#4}}%
  \skvcsvnormalize\skv@tempc
  \def\skv@prova{\endgroup\skvexpandonce\skv@tempc\noexpand}%
  \def\skv@tempb##1,{%
    \def\skv@provb{##1}%
    \ifx\skv@provb\skv@nnil
      \def\skv@tempc{\def#1{#3}\def#2{-1}}%
      \ifskv@pl
        \edef\skv@tempb{\skv@prova\@secondoftwo}%
      \else
        \skv@err{Value '\detokenize{#3}' is not allowed}\skv@ehd
        \edef\skv@tempb{\skv@prova\@gobble}%
      \fi
    \else
      \edef\skv@tempc{\def\unexpanded{#1{##1}\def#2}{\the\@tempcnta}}%
      \ifx\skv@provb\skv@tempa
        \ifskv@pl
          \edef\skv@tempb{\skv@prova\skv@checkchoice@d}%
        \else
          \edef\skv@tempb{\skv@prova\skv@checkchoice@e}%
        \fi
      \else
        \advance\@tempcnta\@ne
      \fi
    \fi
    \skv@tempb
  }%
  \expandafter\skv@tempb\skv@tempc,\skv@nil,%
}
\skvrobustdef*\skv@checkchoice@d#1\skv@nil,{\@firstoftwo}
\skvrobustdef*\skv@checkchoice@e#1\skv@nil,{\@firstofone}

% \skvifkeydefTF[<prefs>]{<fams>}{key}{<true>}{<false>}
%
% 1. The search will stop as soon as the key is found in one combination
%    of prefixes/families.
% 2. The prefix and header created here may be needed in #5 and #6. Hence
%    we put entry prefix and header on stack before commencing the search.
%
\skvrobustdef*\skvifkeydefTF{\skv@testopt{\skv@ifkeyundef0}\skvdefaultprefix}
\skvrobustdef*\skvifkeydefFT{\skv@testopt{\skv@ifkeyundef1}\skvdefaultprefix}
\skvrobustdef*\skv@ifkeyundef#1[#2]#3#4#5#6{%
  \skvpushstate\skv@keystate\skv@keydepth
  \edef\skv@prefs{#2}%
  \edef\skv@fams{#3}%
  \skvdespace{#4}\skvcurrentkey
  \skv@kffalse
  % Don't use \skvcurrentprefix in place of \skv@prova here.
  % We use \skv@prova here because \skv@tempa, \skvcurrentprefix and
  % \skvcurrentfamily might be in use already.
  \skvcommaparse*\skv@prefs\skv@prova{%
    \skv@makeprefix\skv@prova
    \skv@ifk@yundef
    % Break outer loop as needed:
    \ifskv@kf\skvbreakloop\fi
  }%
  \skvexpanded{%
    \skvifboolTF{skv@kf}{%
      \if0#1%
        \noexpand\@firstoftwo
      \else
        \noexpand\@secondoftwo
      \fi
    }{%
      \if0#1%
        \noexpand\@secondoftwo
      \else
        \noexpand\@firstoftwo
      \fi
    }%
  }{#5}{#6}%
  \skvpopstate\skv@keystate\skv@keydepth
}
\skvrobustdef*\skv@ifk@yundef{%
  \skvcommaparse*\skv@fams\skv@prova{%
    \skv@makeheader\skv@prova
    \skvifcsdefFT{\skv@header\skvcurrentkey.@cbk}{}{%
      \skv@kftrue\skvbreakloop
    }%
  }%
}
% \skvifkeyinfamiliesTF[<prefs>]{<fams>}{key}{<true>}{<false>}
%
% The search will be done on all combinations of prefixes/families. The
% callback <true> or <false> will be executed for ALL the combinations.
%
\skvrobustdef*\skvifkeyinfamiliesTF{%
  \skv@testopt{\skv@ifkeyinfamilies0}\skvdefaultprefix
}
% \skvdoonallpathsfound[<prefs>]{<fams>}{key}{<true>}
\skvrobustdef*\skvdoonallpathsfound{%
  \skv@testopt\skv@doonallpathsfound\skvdefaultprefix
}
\skvrobustdef*\skv@doonallpathsfound[#1]#2#3#4{%
  \skv@ifkeyinfamilies0[#1]{#2}{#3}{#4}{}%
}
% \skvdoonallpathsnotfound[<prefs>]{<fams>}{key}{<false>}
\skvrobustdef*\skvdoonallpathsnotfound{%
  \skv@testopt\skv@doonallpathsnotfound\skvdefaultprefix
}
\skvrobustdef*\skv@doonallpathsnotfound[#1]#2#3#4{%
  \skv@ifkeyinfamilies0[#1]{#2}{#3}{}{#4}%
}
\skvrobustdef*\skvifkeyinfamiliesFT{%
  \skv@testopt{\skv@ifkeyinfamilies1}\skvdefaultprefix
}
\skvrobustdef*\skv@ifkeyinfamilies#1[#2]#3#4#5#6{%
  \skvpushstate\skv@keystate\skv@keydepth
  \edef\skv@prefs{#2}%
  \edef\skv@fams{#3}%
  \skvdespace{#4}\skvcurrentkey
  \skvcommaparse*\skv@prefs\skv@prova{%
    \skv@makeprefix\skv@prova
    \skv@ifk@yinfamilies{#1}{#5}{#6}%
  }%
}
\skvrobustdef*\skv@ifk@yinfamilies#1#2#3{%
  \skvcommaparse*\skv@fams\skv@prova{%
    \skv@makeheader\skv@prova
    \skvexpanded{%
      \skvifcsdefTF{\skv@header\skvcurrentkey.@cbk}{%
        \if0#1%
          \noexpand\@firstoftwo
        \else
          \noexpand\@secondoftwo
        \fi
      }{%
        \if0#1%
          \noexpand\@secondoftwo
        \else
          \noexpand\@firstoftwo
        \fi
      }%
    }{#2}{#3}%
  }%
  \skvpopstate\skv@keystate\skv@keydepth
}
% \skvifkeyinfamilyTF{<prefix>/<family>}{<key>}
\skvnewdef*\skvifkeyinfamilyTF#1#2{%
  \skvifcsdefTF{\skvtrimspace{#1}/\skvtrimspace{#2}.@cbk}%
}
% \skvifkeyincurrentfamilyTF{<key>}
\skvnewdef*\skvifkeyincurrentfamilyTF#1{%
  \skvifcsdefTF{\skvcurrentpath/\skvtrimspace{#1}.@cbk}%
}
\skvnewlet\skvifkeyoncurrentpathTF\skvifkeyincurrentfamilyTF

% \skvifonekeyinfamilyTF{<prefix>/<family>}{<keys>}
%
% Given a list of keys, test if at least one of them is defined.
%
% Example:
%
%   \edef\x{\skvifonekeyinfamilyTF{KV/fam}{keya,keyb,keyc}{T}{F}}.
%
\skvnewdef*\skvifonekeyinfamilyTF#1#2{%
  \ifnum\numexpr0\skv@ifonekeydef{#1}#2,\@nnil,>\skvz@
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\skvnewdef*\skv@ifonekeydef#1#2,{%
  \ifx\@nnil#2%
    \expandafter\@gobble
  \else
    \skvifcsdefTF{\skvtrimspace{#1}/\skvtrimspace{#2}.@cbk}{+1}{+0}%
    \expandafter\skv@ifonekeydef
  \fi
  {#1}%
}

% \skvgetdefinedkeys[<pref>]{<fams>}{<keys>}
%
% 1. Get keys defined on the given paths.
% 2. Remove any redundant star (*) and plus (+) suffix on
%    \skvgetdefinedkeys.
%
\skvrobustdef*\skvgetdefinedkeys{%
  \skv@testopta{\skv@testopt\skv@getdefinedkeys\skvdefaultprefix}%
}
\skvrobustdef*\skv@getdefinedkeys[#1]#2#3{%
  \begingroup
  \skv@makeprefix{#1}%
  \def\skv@tempa{}%
  \skvcommaparse{#2}\skvcurrentfamily{%
    \skv@makeheader\skvcurrentfamily
    % Prepare to take defined keys outside the group:
    \skvxifinTF{\skvoxdetok\skv@header}{\skvoxdetok\skv@tempa}{}{%
      \edef\skv@tempa{%
        \skvexpandonce\skv@tempa
        \noexpand\skvcsexit{\skvcurrentpath.@definedkeys}%
      }%
    }%
    \skvcommaparse{#3}\skvcurrentkey{%
      \skvifcsdefFT{\skv@header\skvcurrentkey.@cbk}{}{%
        \skvletcs\skv@prova{\skvcurrentpath.@definedkeys}%
        \skvifdefTF\skv@prova{%
          \skvxifinTF{,\skvoxdetok\skvcurrentkey,}{,\skvoxdetok\skv@prova,}{}{%
            \skvcsedef{\skvcurrentpath.@definedkeys}{\skv@prova,\skvcurrentkey}%
          }%
        }{%
          \skvcsedef{\skvcurrentpath.@definedkeys}{\skvcurrentkey}%
        }%
      }%
    }%
  }%
  \skvexpanded{\endgroup\skv@tempa}%
}

% \skvvalueof{<pref>}{<family>}{<key>}
\skvnewdef*\skvvalueof#1#2#3{\skvcsuse{#1/#2/#3.@value}}
% \skvvalueofkey{<pref>/<family>/<key>}
\skvnewdef*\skvvalueofkey#1{\skvcsuse{#1.@value}}

% When <pref> isn't given, the following will use 'default KV' for <pref>.
% \skvprintvalue[<pref>]{<family>}{<key>}
\skvrobustdef*\skvprintvalue{\skv@testoptb\skv@printvalue}
\skvrobustdef*\skv@printvalue#1{\skvcsuse{\skv@header#1.@value}}

% \skvgetvalue{<pref>}{<family>}{<key>}<cmd>
\skvrobustdef*\skvgetvalue#1#2#3#4{\skvletcs#4{#1/#2/#3.@value}}

% \skvconveyvalue[<pref>]{<family>}{<key>}<cmd>
\skvrobustdef*\skvconveyvalue{\skv@testoptb\skv@conveyvalue}
\skvrobustdef*\skv@conveyvalue#1#2{\skvletcs#2{\skv@header#1.@value}}

% \skvgetinikv{<pref>}{<family>}<cmd>
\skvrobustdef*\skvgetinikv#1#2#3{\skvletcs#3{#1/#2.@inikv}}

% \skvconveyinikv[<pref>]{<family>}<cmd>
\skvrobustdef*\skvconveyinikv{\skv@testoptb\skv@conveyinikv}
\skvrobustdef*\skv@conveyinikv#1{\skvletcs#1{\skvcurrentpath.@inikv}}

% \skvkeyslet[<pref>]{<family>}{<list>}
%
%   <list> -> {<newkey1>,<newkey2>,...,<newkey-n>}={<oldkey>}
%
% Note: <oldkey> must be only one key, to avoid letting one newkey
% to two oldkeys.
%
\skvrobustdef*\skvkeyslet{\skv@testoptb\skv@keyslet}
\skvnewlet\skvkeyinherit\skvkeyslet
\skvrobustdef*\skv@keyslet#1{%
  \skvletcs\skv@inikv{\skvcurrentpath.@inikv}%
  \skvifdefFT\skv@inikv{}{%
    \skvexpbracenext\skv@getnamesofkeys\skv@inikv\skv@inikeys
  }%
  \def\skv@keyslet@do@a##1=##2=##3\skv@nil{%
    \skvifinTF{,}{##2}{%
      \skv@err{There more than one old key:\MessageBreak '##2'}\skv@ehd
    }{%
      \skvcommaparse{##1}\skv@prova{%
        \skvexpbracenext\skv@keyslet@do@b\skv@prova{##2}%
      }%
    }%
  }%
  \def\skv@keyslet@do@b##1##2{%
    \skvifnamedefFT{\skv@header##2.@cbk}{%
      \skv@err{Key '\skvcurrentpath/##2'\MessageBreak is undefined}\skv@ehd
    }{%
      \skvifnamedefTF{\skv@header##1.@cbk}{%
        \skv@err{Key '\skvcurrentpath/##1' is already defined}\skv@ehd
      }{}%
    }%
    \skvcommaloop{cbk,ndv,gnv,fbv,gfv}\skv@prova{%
      \skvcsletcs{\skv@header##1.@\skv@prova}{\skv@header##2.@\skv@prova}%
    }%
    \skvifnamedefTF{\skv@header##2.@defa}{%
      \edef\skvcurrentkey{##2}%
      \skv@getdefault\skvcurrentprefix\skvcurrentfamily\skvcurrentkey
        \skvcurrentvalue
      \skvcsedef{\skv@header##1.@defa}{%
        \skvnoexpandcs{\skv@header##1}{\skvexpandonce\skvcurrentvalue}%
      }%
      \skv@swatrue
    }{%
      \skv@swafalse
    }%
    \skvifdefFT\skv@inikv{}{%
      \skvxifinFT{,\detokenize{##2},}{,\skvoxdetok\skv@inikeys,}{}{%
        \skvcsedef{\skvcurrentpath.@inikv}{%
          \skvcsaddlist,{\skvcurrentpath.@inikv}%
          ##1\ifskv@swa=\skvexpandonce\skvcurrentvalue\fi
        }%
      }%
    }%
    \skvcommaloop{ignoredkeys,needini}\skv@prova{%
      \skvletcs\skv@tempa{\skvcurrentpath.@\skv@prova}%
      \skvifdefFT\skv@tempa{}{%
        \skvxifinFT{,\detokenize{##2},}{,\skvoxdetok\skv@tempa,}{}{%
          \skvcsedef{\skvcurrentpath.@\skv@prova}{%
            \skvaddlist,\skv@tempa##1%
          }%
        }%
      }%
    }%
  }%
  \skvkvparse{#1}\skv@prova{%
    \expandafter\skv@keyslet@do@a\skv@prova==\skv@nil
  }%
  \let\do\skvundef
  \do\skv@keyslet@do\do\skv@inikv\do\skv@inikeys
}

\skvrobustdef*\skv@disabledkeywarning#1{%
  \skv@warn{Key '\skvcurrentpath/#1' has been disabled
    \MessageBreak You can't set or reset key '#1' at this
    \MessageBreak late stage. Perhaps you should have set it
    \MessageBreak earlier \ifskv@latex in \noexpand\documentclass or
    \string\usepackage\fi}%
}
\skvrobustdef*\skv@disabledkeyerror#1{%
  \skv@err{Key '\skvcurrentpath/#1' has been disabled}%
    {You can't set or reset key '#1' at this
    \MessageBreak late stage. Perhaps you should have set it
    \MessageBreak earlier \ifskv@latex in \noexpand\documentclass or
    \string\usepackage\fi}%
}
% A key may be disabled long before \skvmessagetypefordisabledkey
% is called.
\skvrobustdef*\skvmessagetypefordisabledkey#1{%
  \edef\skv@prova{\skvtrimspace{#1}}%
  \def\skv@provb##1{%
    \def\skv@provb####1##1####2####3\@nil{%
      \ifcase####2\relax
        \let\skv@disabledkeymsg\skv@disabledkeywarning
      \or
        \let\skv@disabledkeymsg\skv@disabledkeywarning
      \or
        \let\skv@disabledkeymsg\skv@disabledkeyerror
      \or
        \let\skv@disabledkeymsg\@gobble
      \else
        \skv@err{Invalid message type '#1' for disabled keys}\skv@ehd
      \fi
    }%
    \skv@provb warn{0}warning{1}error{2}nothing{3}##1{10}\@nil
  }%
  \expandafter\skv@provb\expandafter{\skv@prova}%
}
\skvnewlet\skvdisabledkeysmessagetype\skvmessagetypefordisabledkey
\skvdisabledkeysmessagetype{warn}

\skvrobustdef*\skvdisablekeys{%
  \def\skv@disable@temp{\skv@ordkey@a{e}}%
  \skv@testoptb\skv@disablekeys
}
\skvrobustdef*\skvgdisablekeys{%
  \def\skv@disable@temp{\skv@ordkey@a{x}}%
  \skv@testoptb\skv@disablekeys
}
\skvrobustdef*\skv@disablekeys#1{%
  \skvcommaparse{#1}\skv@prova{%
    \skvifnamedefTF{\skv@header\skv@prova.@cbk}{%
      \skvifnamedefTF{\skv@header\skv@prova.@defa}{%
        \edef\skv@provb{\noexpand\skv@disable@temp{\skv@prova}[]}%
      }{%
        \edef\skv@provb{\noexpand\skv@disable@temp{\skv@prova}[^skv^]}%
      }%
      \expandafter\skv@provb\expandafter{\expandafter
        \skv@disabledkeymsg\expandafter{\skv@prova}}%
    }{%
      \skv@err{Key '\skv@prova' is undefined:
        \MessageBreak couldn't be disabled}\skv@ehd
    }%
  }%
  \skvundef\skv@disable@temp
}

% We split xkeyval's \presetkeys (which has both head and tail) into
% \skvpresetkeys (head only) and \skvpostsetkeys (tail only).
% We strengthen \presetkeys as \skvpreposetkeys.
%
% \skvpresetkeys[<pref>]{<fam>}{<keys>}
% \skvgpresetkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvpresetkeys{\skv@testopt\skv@presetkeys\skvdefaultprefix}
\skvrobustdef*\skv@presetkeys[#1]#2#3{\skvpreposetkeys[#1]{#2}{#3}{}}
\skvrobustdef*\skvgpresetkeys{\skv@testopt\skv@gpresetkeys\skvdefaultprefix}
\skvrobustdef*\skv@gpresetkeys[#1]#2#3{\skvgpreposetkeys[#1]{#2}{#3}{}}
\skvrobustdef*\skvpostsetkeys{\skv@testopt\skv@postsetkeys\skvdefaultprefix}
\skvrobustdef*\skv@postsetkeys[#1]#2#3{\skvpreposetkeys[#1]{#2}{}{#3}}
\skvrobustdef*\skvgpostsetkeys{\skv@testopt\skv@gpostsetkeys\skvdefaultprefix}
\skvrobustdef*\skv@gpostsetkeys[#1]#2#3{\skvgpreposetkeys[#1]{#2}{}{#3}}
\skvrobustdef*\skvpreposetkeys{\skv@clfalse\skv@testoptb\skv@preposetkeys}
\skvrobustdef*\skvgpreposetkeys{\skv@cltrue\skv@testoptb\skv@preposetkeys}
\skvrobustdef*\skv@preposetkeys#1#2{%
  \skvifblankTF{#1}{}{\skv@pr@posetkeys{#1}{preset}}%
  \skvifblankTF{#2}{}{\skv@pr@posetkeys{#2}{postset}}%
}
\skvrobustdef*\skv@pr@posetkeys#1#2{%
  \skvifcsdefFT{\skvcurrentpath.@#2}{%
    \skvnormalize{csv}{,}{#1}\skv@tempa
    \ifskv@cl\expandafter\global\fi
    \expandafter\def\csname\skvcurrentpath.@#2\expandafter
      \endcsname\expandafter{\skv@tempa}%
  }{%
    % Don't change \skv@filtermergelist to \skvfiltermergelist:
    \expandafter\skv@filtermergelist\csname\skv@header
      .@#2\endcsname{#1}\skv@getkeyname
  }%
}
% \skvremovepresetkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremovepresetkeys{%
  \skv@clfalse\skv@testoptb\skv@removepresetkeys
}
% \skvgremovepresetkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvgremovepresetkeys{%
  \skv@cltrue\skv@testoptb\skv@removepresetkeys
}
\skvrobustdef*\skv@removepresetkeys#1{%
  \skvifcsdefTF{\skvcurrentpath.@preset}{%
    \expandafter\skv@filterremoveelements\csname\skv@header
      .@preset\endcsname{#1}\skv@getkeyname
  }{%
    \skv@err{No preset keys defined for '\skvcurrentpath'}\skv@ehd
  }%
}
% \skvundefpresetkeys[<pref>]{<fam>}
\skvrobustdef*\skvundefpresetkeys{%
  \skv@clfalse\skv@testoptb\skv@undefpresetkeys
}
\skvrobustdef*\skvgundefpresetkeys{%
  \skv@cltrue\skv@testoptb\skv@undefpresetkeys
}
\skvrobustdef*\skv@undefpresetkeys{%
  \skvifcsdefFT{\skvcurrentpath.@preset}{%
    \skv@err{No preset keys defined for '\skvcurrentpath'}\skv@ehd
  }{%
    \ifskv@cl\expandafter\global\fi
    \skvcsundef{\skvcurrentpath.@preset}%
  }%
}

% \skvremovepostsetkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremovepostsetkeys{%
  \skv@clfalse\skv@testoptb\skv@removepostsetkeys
}
% \skvgremovepostsetkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvgremovepostsetkeys{%
  \skv@cltrue\skv@testoptb\skv@removepostsetkeys
}
\skvrobustdef*\skv@removepostsetkeys#1{%
  \skvifcsdefTF{\skvcurrentpath.@postset}{%
    \expandafter\skv@filterremoveelements\csname\skv@header
      .@postset\endcsname{#1}\skv@getkeyname
  }{%
    \skv@err{No postset keys defined for '\skvcurrentpath'}\skv@ehd
  }%
}
% \skvundefpostsetkeys[<pref>]{<fam>}
\skvrobustdef*\skvundefpostsetkeys{%
  \skv@clfalse\skv@testoptb\skv@undefpostsetkeys
}
\skvrobustdef*\skvgundefpostsetkeys{%
  \skv@cltrue\skv@testoptb\skv@undefpostsetkeys
}
\skvrobustdef*\skv@undefpostsetkeys{%
  \skvifcsdefFT{\skvcurrentpath.@postset}{%
    \skv@err{No postset keys defined for '\skvcurrentpath'}\skv@ehd
  }{%
    \ifskv@cl\expandafter\global\fi
    \skvcsundef{\skvcurrentpath.@postset}%
  }%
}

% \skvremovepreposetkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremovepreposetkeys{%
  \skv@clfalse\skv@testoptb\skv@removepreposetkeys
}
% \skvgremovepreposetkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvgremovepreposetkeys{%
  \skv@cltrue\skv@testoptb\skv@removepreposetkeys
}
\skvrobustdef*\skv@removepreposetkeys#1#2{%
  \skv@r@movepreposetkeys{#1}{preset}%
  \skv@r@movepreposetkeys{#2}{postset}%
}
\skvrobustdef*\skv@r@movepreposetkeys#1#2{%
  \skvifcsdefTF{\skvcurrentpath.@#2}{%
    \expandafter\skv@filterremoveelements\csname\skv@header
      .@#2\endcsname{#1}\skv@getkeyname
  }{%
    \skv@err{No preset keys defined for '\skvcurrentpath'}\skv@ehd
  }%
}
% \skvundefpreposetkeys[<pref>]{<fam>}
\skvrobustdef*\skvundefpreposetkeys{%
  \skv@clfalse\skv@testoptb\skv@undefpreposetkeys
}
\skvrobustdef*\skvgundefpreposetkeys{%
  \skv@cltrue\skv@testoptb\skv@undefpreposetkeys
}
\skvrobustdef*\skv@undefpreposetkeys{%
  \skvifcsdefFT{\skvcurrentpath.@preset}{%
    \skv@err{No preset keys defined for '\skvcurrentpath'}\skv@ehd
  }{%
    \ifskv@cl\expandafter\global\fi
    \skvcsundef{\skvcurrentpath.@preset}%
    \ifskv@cl\expandafter\global\fi
    \skvcsundef{\skvcurrentpath.@postset}%
  }%
}

%% Note about the absence of \skvsavevaluekeys (save-value-keys):
%
% All keys have their values saved in the macro '<header>.@value'.
% The value can be accessed via \skvgetvalue of \skvconveyvalue. When
% needed, the value can be taken outside a local group by using \global
% on the macro that has inherited the key's value via these commands.

% \skvneedvaluekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvneedvaluekeys{%
  \skv@clfalse\skv@testoptb\skv@needvaluekeys
}
\skvrobustdef*\skvgneedvaluekeys{%
  \skv@cltrue\skv@testoptb\skv@needvaluekeys
}
\skvrobustdef*\skv@needvaluekeys#1{%
  \skvcommaparse{#1}\skv@prova{%
    \ifskv@cl\expandafter\global\fi
    \skvcsdef{\skv@header\skv@prova.@ndv}{}%
  }%
}
% \skvremoveneedvaluekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremoveneedvaluekeys{%
  \skv@clfalse\skv@testoptb\skv@removeneedvaluekeys
}
\skvrobustdef*\skvgremoveneedvaluekeys{%
  \skv@cltrue\skv@testoptb\skv@removeneedvaluekeys
}
\skvrobustdef*\skv@removeneedvaluekeys#1{%
  \skvcommaparse{#1}\skv@prova{%
    \ifskv@cl\expandafter\global\fi
    \skvcsundef{\skv@header\skv@prova.@ndv}%
  }%
}

% \skvforbidvaluekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvforbidvaluekeys{%
  \skv@clfalse\skv@testoptb\skv@forbidvaluekeys
}
\skvrobustdef*\skvgforbidvaluekeys{%
  \skv@cltrue\skv@testoptb\skv@forbidvaluekeys
}
\skvrobustdef*\skv@forbidvaluekeys#1{%
  \skvcommaparse{#1}\skv@prova{%
    \ifskv@cl\expandafter\global\fi
    \skvcsdef{\skv@header\skv@prova.@fbv}{}%
  }%
}
% \skvremoveforbidvaluekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremoveforbidvaluekeys{%
  \skv@clfalse\skv@testoptb\skv@removeforbidvaluekeys
}
\skvrobustdef*\skvgremoveforbidvaluekeys{%
  \skv@cltrue\skv@testoptb\skv@removeforbidvaluekeys
}
\skvrobustdef*\skv@removeforbidvaluekeys#1{%
  \skvcommaparse{#1}\skv@prova{%
    \ifskv@cl\expandafter\global\fi
    \skvcsundef{\skv@header\skv@prova.@fbv}%
  }%
}
% \skvoptionkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvoptionkeys{%
  \skv@clfalse\skv@testoptb{\skv@optionkeys{}}%
}
\skvrobustdef*\skvgoptionkeys{%
  \skv@cltrue\skv@testoptb{\skv@optionkeys{}}%
}
% \skvnonoptionkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvnonoptionkeys{%
  \skv@clfalse\skv@testoptb{\skv@optionkeys{non}}%
}
\skvrobustdef*\skvgnonoptionkeys{%
  \skv@cltrue\skv@testoptb{\skv@optionkeys{non}}%
}
\skvrobustdef*\skv@optionkeys#1#2{%
  \skvcommaparse{#2}\skv@prova{%
    \ifskv@cl\expandafter\global\fi
    \skvcsdef{\skv@header\skv@prova.@#1opt}{}%
  }%
}
% \skvremoveoptionkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremoveoptionkeys{%
  \skv@clfalse\skv@testoptb{\skv@removeoptionkeys{}}%
}
\skvrobustdef*\skvgremoveoptionkeys{%
  \skv@cltrue\skv@testoptb{\skv@removeoptionkeys{}}%
}
% \skvremovenonoptionkeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremovenonoptionkeys{%
  \skv@clfalse\skv@testoptb{\skv@removenonoptionkeys{non}}%
}
\skvrobustdef*\skvgremovenonoptionkeys{%
  \skv@cltrue\skv@testoptb{\skv@removenonoptionkeys{non}}%
}
\skvrobustdef*\skv@removeoptionkeys#1#2{%
  \skvcommaparse{#2}\skv@prova{%
    \ifskv@cl\expandafter\global\fi
    \skvcsundef{\skv@header\skv@prova.@#1opt}%
  }%
}
% Save the default/initial values of keys:
% \skvsaveinitialvaluekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvsaveinitialvaluekeys{%
  \skv@clfalse\skv@testoptb\skv@saveinitialvaluekeys
}
% \skvgsaveinitialvaluekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvgsaveinitialvaluekeys{%
  \skv@cltrue\skv@testoptb\skv@saveinitialvaluekeys
}
\skvrobustdef*\skv@saveinitialvaluekeys#1{%
  \skvifcsdefFT{\skvcurrentpath.@needini}{%
    \edef\skv@tempa{\unexpanded{#1}}%
    \skvcsvnormalize\skv@tempa
    \ifskv@cl\expandafter\global\fi
    \skvcsedef{\skvcurrentpath.@needini}{\skvexpandonce\skv@tempa}%
  }{%
    \expandafter\skv@filtermergelist\csname
    \skvcurrentpath.@needini\endcsname{#1}\skv@getkeyname
  }%
}
% \skvremovesaveinitialvaluekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremovesaveinitialvaluekeys{%
  \skv@clfalse\skv@testoptb\skv@removesaveinitialvaluekeys
}
% \skvgremovesaveinitialvaluekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvgremovesaveinitialvaluekeys{%
  \skv@cltrue\skv@testoptb\skv@removesaveinitialvaluekeys
}
\skvrobustdef*\skv@removesaveinitialvaluekeys#1{%
  \skvifcsdefFT{\skvcurrentpath.@needini}{%
    \skv@err{No save-initial keys defined for '\skvcurrentpath'}\skv@ehd
  }{%
    \expandafter\skv@filterremoveelements\csname
      \skvcurrentpath.@needini\endcsname{#1}\skv@getkeyname
  }%
}
% \skvundefsaveinitialvaluekeys[<pref>]{<fam>}
\skvrobustdef*\skvundefsaveinitialvaluekeys{%
  \skv@clfalse\skv@testoptb\skv@undefsaveinitialvaluekeys
}
% \skvgundefsaveinitialvaluekeys[<pref>]{<fam>}
\skvrobustdef*\skvgundefsaveinitialvaluekeys{%
  \skv@cltrue\skv@testoptb\skv@undefsaveinitialvaluekeys
}
\skvrobustdef*\skv@undefsaveinitialvaluekeys{%
  \skvifcsdefFT{\skvcurrentpath.@needini}{%
    \skv@err{No save-initial keys defined for '\skvcurrentpath'}\skv@ehd
  }{%
    \csname skv\ifskv@cl g\fi csundef\endcsname{\skvcurrentpath.@needini}%
  }%
}

% While setting keys, ignore the listed keys.
% \skvignorekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvignorekeys{\skv@clfalse\skv@testoptb\skv@ignorekeys}
\skvrobustdef*\skvgignorekeys{\skv@cltrue\skv@testoptb\skv@ignorekeys}
\skvrobustdef*\skv@ignorekeys#1{%
  \skvifcsdefTF{\skvcurrentpath.@ignoredkeys}{%
    \expandafter\skv@filtermergelist\csname
      \skvcurrentpath.@ignoredkeys\endcsname{#1}\skv@getkeyname
  }{%
    \edef\skv@tempa{\unexpanded{#1}}%
    \skvcsvnormalize[,]\skv@tempa
    \ifskv@cl\expandafter\global\fi
    \skvcsedef{\skvcurrentpath.@ignoredkeys}{\skvexpandonce\skv@tempa}%
  }%
}
% \skvremoveignorekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvremoveignorekeys{%
  \skv@clfalse\skv@testoptb\skv@removeignorekeys
}
% \skvgremoveignorekeys[<pref>]{<fam>}{<keys>}
\skvrobustdef*\skvgremoveignorekeys{%
  \skv@cltrue\skv@testoptb\skv@removeignorekeys
}
\skvrobustdef*\skv@removeignorekeys#1{%
  \skvifcsdefFT{\skvcurrentpath.@ignoredkeys}{%
    \skv@err{No ignore keys defined for '\skvcurrentpath'}\skv@ehd
  }{%
    \expandafter\skv@filterremoveelements\csname
      \skvcurrentpath.@ignoredkeys\endcsname{#1}\skv@getkeyname
  }%
}
% \skvundefignorekeys[<pref>]{<fam>}
\skvrobustdef*\skvundefignorekeys{%
  \skv@clfalse\skv@testoptb\skv@undefignorekeys
}
% \skvgundefignorekeys[<pref>]{<fam>}
\skvrobustdef*\skvgundefignorekeys{%
  \skv@cltrue\skv@testoptb\skv@undefignorekeys
}
\skvrobustdef*\skv@undefignorekeys{%
  \skvifcsdefFT{\skvcurrentpath.@ignoredkeys}{%
    \skv@err{No ignore keys defined for '\skvcurrentpath'}\skv@ehd
  }{%
    \csname skv\ifskv@cl g\fi csundef\endcsname
    {\skvcurrentpath.@ignoredkeys}%
  }%
}
%
% Adding to the callback of existing keys.
%
% \skvaddkeycode[<pref>]{<fam>}{<key>}{<precode>}{<postcode>}
\skvrobustdef*\skvaddkeycode{\skv@testoptb\skv@addkeycode}
\skvrobustdef*\skv@addkeycode#1#2#3{%
  \skv@prependkeycode{prep}{#1}{#2}%
  \skv@prependkeycode{app}{#1}{#3}%
}
\skvnewlet\skvaddtocallback\skvaddkeycode
% \skvprependkeycode[<pref>]{<fam>}{<key>}{<code>}
\skvrobustdef*\skvprependkeycode{\skv@testoptb{\skv@prependkeycode{prep}}}
\skvrobustdef*\skvappendkeycode{\skv@testoptb{\skv@prependkeycode{app}}}
\skvnewlet\skvprependtocallback\skvprependkeycode
\skvnewlet\skvapendtocallback\skvappendkeycode
\skvrobustdef*\skv@prependkeycode#1#2#3{%
  \edef\skvcurrentkey{\skvtrimspace{#2}}%
  \skvifcsdefTF{\skv@header\skvcurrentkey.@cbk}{%
    \skvcsedef{\skv@header\skvcurrentkey.@cbk}{%
      \skvifstrcmpTF{#1}{prep}{%
        \skvtrimspace{#3}%
        \skvexpandcsonce{\skv@header\skvcurrentkey.@cbk}%
      }{%
        \skvexpandcsonce{\skv@header\skvcurrentkey.@cbk}%
        \skvtrimspace{#3}%
      }%
    }%
  }{%
    \skvcsedef{\skv@header\skvcurrentkey.@cbk}{\skvtrimspace{#3}}%
  }%
}
\skvrobustdef*\skvsetkeys{%
  \skv@viarootofsetkeystrue
  \skv@testopta{\skv@testoptc\skv@setkeys@a}%
}
\skvrobustdef*\skvsetrmkeys{%
  \skv@viarootofsetkeystrue
  \skv@testopta{\skv@testoptc\skv@setrmkeys}%
}
\skvrobustdef*\skv@setrmkeys[#1]{%
  % Only one prefix is allowed here. \skv@testoptc has created
  % \skvcurrentprefix and \skv@fams.
  \skvifdefTF\skv@rmkeys{%
    \skvexpbracenext{\skv@setkeys@a[#1]}\skv@rmkeys
  }{}%
}
% \skv@setkeys@a[<ignored.list>]{<kvlist>}
\skvrobustdef*\skv@setkeys@a[#1]#2{%
  % \skvexecuteoptions calls \skv@setkeys@a. So this is the place for
  % \skv@insettrue:
  \skv@insettrue
  % \skv@testoptc has created \skvcurrentprefix and \skv@fams.
  \skvifdefboolTF{skv@intry}{}{%
    \skv@getnamesofkeys{#2}\skv@currentnames
  }%
  % Both #1 and #2 will be normalized in \skv@setkeys@b.
  \skv@setprepokeys{#1}{preset}%
  \skv@setkeys@b{#2}{#1}%
  \skv@setprepokeys{#1}{postset}%
  \ifnum\skv@setkeysdepth=\skvz@
    \skv@insetfalse
    \skv@viarootofsetkeysfalse
  \fi
  % Don't do \let\CurrentOption\@empty here.
}
\skvnewlet\skv@sav@setkeys@a\skv@setkeys@a
\skvrobustdef*\skv@badsetkeysinpreset[#1]#2{%
  \skv@err{%
    \noexpand\skvsetkeys or \noexpand\skvsetrmkeys can't be nested in a preset
    \MessageBreak key's callback: this will cause a cyclic call
    \MessageBreak to \noexpand\skvsetkeys or \noexpand\skvsetrmkeys
  }\skv@ehd
}
\skvrobustdef*\skv@setprepokeys#1#2{%
  \skv@inprepotrue
  \let\skv@setkeys@a\skv@badsetkeysinpreset
  % Preposet keys doesn't use \skv@fams in \skv@setkeys@d; it
  % branches off to \skv@setkeys@e. Hence the following loop is in
  % order.
  \skvecommaloop*\skv@fams\skvcurrentfamily{%
    \skv@makeheader\skvcurrentfamily
    \skvletcs\reserved@a{\skvcurrentpath.@#2}%
    \skvifdefFT\reserved@a{}{%
      \skvexpandtwoargs\skv@setkeys@b{\skvexpandonce\reserved@a}%
        {\skvaddlist,\skv@currentnames\unexpanded{#1}}%
    }%
  }%
  \let\skv@setkeys@a\skv@sav@setkeys@a
  \skv@inprepofalse
}
% \skv@setkeys@b{<kvlist>}{<ignored.list>}
%
% \skv@keydepth is called in places other than by \skvsetkeys. Hence we
% need an independent \skv@setkeysdepth here.
%
\skvrobustdef*\skv@setkeys@b#1#2{%
  % \skv@setprepokeys calls \skv@setkeys@b. So this is the place to
  % advance \skv@setkeysdepth.
  \skvgadvanceno\skv@setkeysdepth\@ne
  \ifnum\skv@setkeysdepth>\skv@stackdepthlimit\relax
    \skv@err{\noexpand\skvsetkeys is nested too deeply.
      \MessageBreak Maybe there has been infinite reentry}\skv@ehd
  \fi
  % \skv@na can't be anywhere else, not in \skv@setkeys@a.
  \edef\skv@na{\unexpanded{#2}}%
  \skvifemptyTF\skv@na{}{\skvcsvnormalize\skv@na}%
  \skvkvparse{#1}\CurrentOption{%
    \skv@processvalueaslistfalse
    % Expand the key name twice, in case the key and its value
    % are hidden in a macro. A maverick might do just that.
    \expandafter\expandafter\expandafter
      \skv@setkeys@c\CurrentOption=\skv@novalue=\skv@setkeys@nil
  }%
  \skvgadvanceno\skv@setkeysdepth\m@ne
}
\skvrobustdef*\skv@setkeys@c#1={%
  \skvxifinTF{(}{\detokenize{#1}}{%
    \skvxifinTF{)}{\detokenize{#1}}{%
      % A pntkey can't carry pointers:
      \edef\skvcurrentkey{\unexpanded{#1}}%
      \let\skv@tkey\skvcurrentkey
      \skv@strippointersfromkey*\skvcurrentkey
      \skv@strippointersfromvalue*\skvcurrentkey
      \ifx\skvcurrentvalue\skv@tkey
        \skv@extractpntkey@atsetkey{#1}%
        \def\skv@ispntkey{00}%
        \ifx\skvcurrentvalue\@empty
          \skvnovaluetrue
        \else
          \skvnovaluefalse
        \fi
      \else
        \skv@err{A parenthesized key can't have pointers}\skv@ehd
      \fi
    }{%
      \skv@err{Key value has '(' but no ')'}
        {The value of a parenthesized key must have both opening
          \MessageBreak parenthesis '(' and closing ')'.}%
    }%
  }{%
    \def\skv@ispntkey{01}%
    \skv@g@tkeyname#1=\skv@getname@nil\skvcurrentkey
  }%
  % ##1=value:
  \def\skv@prova##1=##2\skv@setkeys@nil{%
    \skvifknobTF{skv@ispntkey}{%
      % \skv@extractpntkey@atsetkey would have extracted key name and
      % value for the pntkey.
    }{%
      \edef\skvcurrentvalue{\skvexpandonce{\@gobble##1}}%
      \ifx\skvcurrentvalue\skv@novaluetoks
        \skvnovaluetrue
        \def\skvcurrentvalue{}%
      \else
        \skvnovaluefalse
      \fi
      \skvexpbracenext\skvifbracedTF\skvcurrentvalue{%
        \skvvaluebracedtrue
      }{%
        \skvvaluebracedfalse
        \skv@strippointersfromvalue*\skvcurrentvalue
      }%
    }%
    \ifx\skvcurrentkey\@empty
      \ifx\skvcurrentvalue\@empty\else
        \skv@err{Current key is nil, but you have a value for it:
          \MessageBreak\skvoxdetok\skvcurrentvalue}\skv@ehd
      \fi
    \fi
    \skvifdefboolTF{skv@processvalueaslist}{%
      % You can use the pointer '.process list', etc, on the current value to
      % signify that the value be processed as a list, in the
      % manner of a list key. This scheme is costlier than defining the
      % key as a listkey, using \skvlistkey, but it is more versatile.
      % This allows any key to accept and process a value that is a list,
      % irrespective of its argument pattern.
      \skv@processvalueaslist
    }{%
      \edef\CurrentOption{%
        \skvcurrentkey
        \ifx\skvcurrentvalue\@empty\else=\skvxonce\skvcurrentvalue\fi
      }%
      \skv@setkeys@d
    }%
  }%
  \skv@prova.%
}
\skvrobustdef*\skv@processvalueaslist{%
  \skvpushstate\skv@keystate\skv@keydepth
  \skvifemptyTF\skvcurrentvalue{%
    \let\CurrentOption\skvcurrentkey
    \skv@setkeys@d
  }{%
    \skvcommaparse*\skvcurrentvalue\skvcurrentvalue{%
      \edef\CurrentOption{%
        \skvcurrentkey
        \ifx\skvcurrentvalue\@empty\else=\skvxonce\skvcurrentvalue\fi
      }%
      \skv@setkeys@d
    }%
  }%
  \skvpopstate\skv@keystate\skv@keydepth
}
\skvrobustdef*\skv@setkeys@d{%
  \begingroup
  \skv@swatrue
  \skvxifinTF{,\skvcurrentkey,}{,\skv@na,}{\skv@swafalse}{}%
  \skvletcs\skv@tempa{\skvcurrentpath.@ignoredkeys}%
  \skvifdefTF\skv@tempa{%
    \skvxifinTF{,\skvcurrentkey,}{,\skv@tempa,}{\skv@swafalse}{}%
  }{}%
  \skvaftergroupifboolFT skv@swa\endgroup{}{%
    \skv@kffalse
    \skvifdefboolTF{skv@inprepo}{%
      \skv@setkeys@e
    }{%
      \skvifdefboolTF{skv@pl}{%
        % Set the key in all families in which it exists.
        \skvecommaloop*\skv@fams\skvcurrentfamily{%
          \skv@makeheader\skvcurrentfamily
          \skv@setkeys@e
        }%
      }{%
        % Stop searching as soon as the key is found in one family.
        \skvcommaloop*\skv@fams\skvcurrentfamily{%
          \skv@makeheader\skvcurrentfamily
          \skv@setkeys@e
          \ifskv@kf\skvbreakloop\fi
        }%
      }%
    }%
    \skvifdefboolTF{skv@kf}{%
      \skvifdefboolTF{skv@inpox}{%
        \ifskv@inclass\skvafterfi
          \expandafter\skv@removeoption\expandafter{\CurrentOption}%
        \fi
      }{}%
    }{%
      \skvifdefboolTF{skv@inpox}{%
        \skvifcsdefTF{\skvcurrentpath.@famhandler}{%
          \begingroup
          \let\elt\skvexpandonce
          \skvexpanded{\endgroup
            \skvnoexpandcs{\skvcurrentpath.@famhandler}%
              {\elt\skvcurrentprefix}{\elt\skvcurrentfamily}%
              {\elt\skvcurrentkey}{\elt\skvcurrentvalue}%
          }%
        }{%
          \skvifcsdefTF{skv@dox@\@currname.\@currext}{%
            \skvcsuse{skv@dox@\@currname.\@currext}%
          }{%
            \ifx\@currext\@clsextension\else
              \skv@err{%
                Unknown option '\skvcurrentfullkey'
                \MessageBreak for \@cls@pkg\space'\@currname'
              }{%
                The option '\skvcurrentfullkey'
                \MessageBreak was not declared in \@cls@pkg\space'\@currname'.
                \MessageBreak Perhaps you misspelled its name.
                \MessageBreak Try typing <return> to proceed.
              }%
            \fi
          }%
        }%
      }{%
        \skvifdefboolTF{skv@st}{%
          \skv@setkeys@f
        }{%
          \skvifcsdefTF{\skvcurrentpath.@famhandler}{%
            \begingroup
            \let\elt\skvexpandonce
            \skvexpanded{\endgroup
              \skvnoexpandcs{\skvcurrentpath.@famhandler}%
              {\elt\skvcurrentprefix}{\elt\skvcurrentfamily}%
              {\elt\skvcurrentkey}{\elt\skvcurrentvalue}%
            }%
          }{%
            % \ifskv@viarootofsetkeys is true, then \skvsetkeys is nested
            % in the callback of a .try key. In that case, throw the exception:
            \ifskv@intry
              \ifskv@viarootofsetkeys
                \skv@err{Key '\skvcurrentfullkey'
                  \MessageBreak is undefined}\skv@ehd
              \fi
            \else
              \skv@err{Key '\skvcurrentfullkey'
                \MessageBreak is undefined}\skv@ehd
            \fi
          }%
        }%
      }%
    }%
  }%
}
\skvrobustdef*\skv@setkeys@e{%
  \skvifcsdefFT{\skv@header\skvcurrentkey.@cbk}{%
    \ifskv@intry\skv@successfalse\fi
  }{%
    \skv@kftrue
    \ifskv@intry\skv@successtrue\fi
    \ifskv@inpox
      \skvifcsname\skv@header\skvcurrentkey.@nonopt\then
        \skv@err{Key '\skvcurrenttriple'
          \MessageBreak is a non-option key but it has appeared
          \MessageBreak as a class or package option}\skv@ehd
      \fi
    \else
      \skvifcsname\skv@header\skvcurrentkey.@opt\then
        \skv@err{Key '\skvcurrenttriple'
          \MessageBreak is an option key but it has appeared
          \MessageBreak outside class or package option list}\skv@ehd
      \fi
    \fi
    \ifskvnovalue
      \skvifcsdefTF{\skv@header\skvcurrentkey.@ndv}{%
        \skv@err{Key '\skvcurrenttriple'
          \MessageBreak requires a user value.
          \MessageBreak Maybe it's a signal key}\skv@ehd
      }{%
        \skvifcsdefTF{\skv@header\skvcurrentkey.@defa}{%
          \skv@getdefault\skvcurrentprefix\skvcurrentfamily
            \skvcurrentkey\skvcurrentvalue
          % Check if the default value is braced:
          \skvexpbracenext\skvifbracedFT\skvcurrentvalue{}{%
            \skvvaluebracedtrue
          }%
        }{%
          \skv@err{No value specified for key
            \MessageBreak'\skvcurrenttriple'
            \MessageBreak and no default value}\skv@ehd
        }%
      }%
    \else
      \skvifcsdefTF{\skv@header\skvcurrentkey.@fbv}{%
        \skv@err{Key '\skvcurrenttriple' doesn't
          \MessageBreak accept a user value: key value forbidden.}\skv@ehd
      }{}%
    \fi
    \skvifemptyTF\skvcurrentvalue{}{%
      \expandafter\skv@replacepointers\expandafter{\skvcurrentvalue}%
    }%
    \skvletcs\skv@callback{\skv@header\skvcurrentkey.@cbk}%
    \skv@getargpattern
    \edef\skv@callback{%
      \let\noexpand\this\noexpand\skvcurrentkey
      \skvexpandonce\skv@callback
    }%
    % 1. Strip outer braces of \skvcurrentvalue, so that the argument can be
    %    grabbed by the, possibly multi-parametered, callback function.
    % 2. The argument has been obtained from possible explicit definition
    %    of the argument. But if the obtained argument is simple, then the
    %    argument in the key's call may be more complex:
    \ifx\skv@argpattern\skv@simplearg\else
      \ifcsname\skv@header\skvcurrentkey.@listkey\endcsname
        \skv@err{A listkey must have only a one-parameter argument}\skv@ehd
      \else
        \skvstripouterbraces{2}\skvcurrentvalue
        \skvvaluebracedfalse
      \fi
    \fi
    \skvcslet{\skv@header\skvcurrentkey.@value}\skvcurrentvalue
    \skvpushstate\skv@keystate\skv@keydepth
    \expandafter\expandafter\expandafter\def\expandafter\expandafter
      \expandafter\skv@prova\expandafter\skv@argpattern\expandafter
      \skeyvaleov\expandafter{\skv@callback}%
    \skvifxTF\skv@argpattern\skv@simplearg{%
      \expandafter\skv@prova\expandafter{\skvcurrentvalue}\skeyvaleov
    }{%
      \expandafter\skv@prova\skvcurrentvalue\skeyvaleov
    }%
    \skvpopstate\skv@keystate\skv@keydepth
  }%
}
% Save rm keys:
\skvrobustdef*\skv@setkeys@f{%
  \skvexpanded{%
    \skvmergelist\noexpand\skv@rmkeys{\skvexpandonce\CurrentOption}%
    % The boolean \ifdirkeys@saveunknownkeys is, by default, false.
    % The default value of \dirkeys@unknownkeysmacro is \skvfaillist.
    \ifindirectkeys
      \ifdirkeys@saveunknownkeys
        \skvmergelist\skvexpandonce\dirkeys@unknownkeysmacro
          {{\skvcurrentprefix}/{\skvcurrentfamily}/%
          {\skvexpandonce\CurrentOption}}%
      \fi
    \fi
  }%
}
% \skv@getdefault{<pref>}{<fam>}{<key>}{<return.macro>}
\skvrobustdef*\skv@getdefault#1#2#3#4{%
  \begingroup
  \let\elt\relax
  \edef\skv@prova{\elt{#1}/\elt{#2}/\elt{#3}}%
  \let\elt\skvtrimspace
  \edef\skv@prova{\skv@prova}%
  \def\skv@g@tdefault##1##2\skv@nil{%
    \edef\skv@provb{\skvremovescape{##1}}%
    \@onelevel@sanitize\skv@prova
    \ifx\skv@prova\skv@provb
      \skvcsdef{\skv@prova}####1{\edef#4{\unexpanded{####1}}}%
      \csname\skv@prova.@defa\endcsname
    \else
      \skv@err{The default value syntax of key
        \MessageBreak '\skv@prova' doesn't conform to
        \MessageBreak skeyval format. Maybe another package
        \MessageBreak has abused the format}
        {I can't extract the default value of key '\skv@prova'.}%
    \fi
  }%
  % <default.macro><key.macro>
  \expandafter\expandafter\expandafter\skv@g@tdefault
    \csname\skv@prova.@defa\endcsname\skv@nil
  \skvaftergroupdef#4\endgroup
}
% Set keys using their default values:
% \skvinitializekeys[<pref>]{<fams>}[<ignored.keys>]
\skvrobustdef*\skvinitializekeys{\skv@testoptc\skv@initializekeys}
% #1: ignored keys
\skvrobustdef*\skv@initializekeys[#1]{%
  \begingroup
  \def\skv@tempe{}%
  % \skv@testoptc has created \skvcurrentprefix and \skv@fams.
  \skvcommaloop*\skv@fams\skv@tempa{%
    \skv@makeheader\skv@tempa
    \skvletcs\skv@tempa{\skvcurrentpath.@inikv}%
    \skvifdefFT\skv@tempa{%
      \skv@err{No 'save initial value' keys defined in family
        \MessageBreak'\skvcurrentpath'}\skv@ehd
    }{%
      % '\skvcurrentpath.@poxkeys' is the list of keys that have been
      % instantiated as current pacakge options.
      \skvletcs\skv@tempc{\skvcurrentpath.@poxkeys}%
      \skvifdefFT\skv@tempc{%
        \edef\skv@tempe{%
          \skvexpandonce\skv@tempe
          \skvsetkeys[\skvcurrentprefix]{\skvcurrentfamily}%
          [#1]{\skvexpandonce\skv@tempa}%
        }%
      }{%
        % Filter pox (instantiated package/article options) list members.
        % Pox keys can't be initialized.
        \def\skv@tempd{}%
        \skvcommaloop*\skv@tempa\skv@tempa{%
          \expandafter\skv@g@tkeyname\skv@tempa=\skv@getname@nil\skv@tempb
          \skvxifinTF{,\skvoxdetok\skv@tempb,}{,\skvoxdetok\skv@tempc,}{}{%
            \edef\skv@tempd{%
              \skvaddlist,\skv@tempd\skvexpandonce\skv@tempa
            }%
          }%
        }%
        \edef\skv@tempe{%
          \skvexpandonce\skv@tempe
          \skvsetkeys[\skvcurrentprefix]{\skv@fams}[#1]%
          {\skvexpandonce\skv@tempd}%
        }%
      }%
    }%
  }%
  \expandafter\endgroup\skv@tempe
}

%+++++++++++++++++++++ Compactly define keys +++++++++++++++++++++++++%
%
% \skvdefinekeys*+[<pref>]{<fams>}[<hp>]{<list>}
% * -> define only new keys.
% + -> define in all the given families.
%
% The only difference between \skvedefinekeys and \skvdefinekeys is the
% value of \endlinechar.
%
% Examples:
%
% \skvdefinekeys*+[KVA]{fam1,fam2}[thp@]{%
%    .initialize keys after define=true,
%    .save initial values,
%    .prepend to every key name=X@,
%    .ord/{keya,keyb}/{default-a},
%    .cmd/{keyc,keyd}/,
%    .zcmd/key e/\def\cmde##1{##1}/
%      \edef\y{\detokenize\expandafter{\thp@keye}}\def\x##1{#1*key e*##1},
%    .choice/keyf/center/{center.do=\def\x##1{#1*##1},left,right}/
%      \def\f##1{#1*##1}/\@@warning{Invalid value for keyf},
%    .zbool/show center/true/\edef\cmd{\ifthp@showcenter Yes\else No\fi}/
%      \@@warning{Invalid value for show center},
%    .arg/{key1,key2}/{#1/#2},
%    .arg/key3/{#1+#2},
%    .exec/\def\x##1{##1},
%    .exec code=\def\y##1{##1},
% }
% \skvshowcs{KVA/fam1/keyb.@defa}
% \def\keybval{xx}
% \skvsetkeys[KVA]{fam1}{keyb=.expand once{\keybval}}
%
\skvnewbools[skvdfk@]{saveinitialvalues,initialize}
% '.initialize' means set the keys with their default values after
% they've been defined. Leave this as ordinary keys, not zbool keys,
% since the key names contain dot (.). Zapping the spaces in the
% key name will not lead to a boolean of the \ifhp@key:

\skvordkey[SKV]{definekeys}{.initialize}[true]{%
  \skvifboolvalT{#1}{%
    \csname skvdfk@initialize#1\endcsname
  }%
}

% Save default values as a kv list in macro <header>.@needini:
\skvordkey[SKV]{definekeys}{.save initial values}[true]{%
  \skvifboolvalT{#1}{%
    \csname skvdfk@saveinitialvalues#1\endcsname
  }%
}
\skvordkey[SKV]{definekeys}{.parser}[,]{%
  \skvifntypeTF{#1}{%
    \def\skvdfk@parser{#1}%
    \skvstripouterbraces{2}\skvdfk@parser
  }{%
    \skv@err{Parser '#1' is invalid; must be a single character}\@ehd
  }%
}
\skvrobustdef*\skvsetdefinekeysparser{\def\skvdfk@parser}
\skvsetdefinekeysparser{,}
\skvrobustdef*\skvsetupdefinekeys#1{\skvsetkeys[SKV]{definekeys}{#1}}

\skvsetupdefinekeys{.initialize=false,.save initial values=false}

% Set aliases for handlers used in \skvdefinekeys:
\skvrobustdef*\skvtypecastfordefinekeys#1{%
  \begingroup
  \def\skv@tempa{}%
  \skvkvparse{#1}\skv@prova{%
    \skv@okvsplit\skv@prova{%
      \def\skv@keytypecast####1{%
        \skvifcsdefTF{skvdfk@typealias@####1}{%
          \skv@err{Key type alias '####1' already defined}\skv@ehd
        }{%
          \skvifstrcmpTF{##2}{^skv^}{%
            \skv@err{Key type alias '####1' has no master}\skv@ehd
          }{%
            \edef\skv@tempa{%
              \skvexpandonce\skv@tempa
              \skvcsdef{skvdfk@typealias@####1}{##2}%
            }%
          }%
        }%
      }%
      \skvcommaparse{##1}\skv@prova{%
        \expandafter\skv@keytypecast\expandafter{\skv@prova}%
      }%
    }%
  }%
  \expandafter\endgroup\skv@tempa
}
\skvtypecastfordefinekeys{%
  {.singleton,.state pattern}=.choice,
  .exec code=.exec,
  {.arg,.args}=.argx0,
  .arg expand once=.argx1,
  .arg expand twice=.argx2,
  .arg expanded=.argxx,
  {.initialize keys after define,.initialize after define,
    .initialize keys}=.initialize,
  {.save initial values,.save initial values of keys}=.saveini,
  {.prepend to key name,.prepend to every key name}=.preptokey,
  {.append to key name,.append to every key name}=.apptokey,
  {.prepend to callback,.prepend to every callback}=.preptocode,
  {.append to callback,.append to every callback}=.apptocode,
  {.exec after define,.after define}=.afterdef,
}
\skvnewdef*\skvdfk@afterdefine@hook{}
\skvrobustdef*\skvafterdefinekeys{%
  \skvgappendtomacro\skvdfk@afterdefine@hook
}
\skvrobustdef*\skvdfk@testopta#1{%
  \skvifstar{%
    \skv@sttrue
    \skvifplus
      {\skv@pltrue\skvdfk@testoptb#1}
      {\skv@plfalse\skvdfk@testoptb#1}%
  }{%
    \skv@stfalse
    \skvifplus
      {\skv@pltrue\skvdfk@testoptb#1}
      {\skv@plfalse\skvdfk@testoptb#1}%
  }%
}
\skvrobustdef*\skvdfk@testoptb#1{%
  \skv@testopt{\skvdfk@t@stoptb{#1}}\skvdefaultprefix
}
\skvrobustdef*\skvdfk@t@stoptb#1[#2]#3{%
  \skvxifinTF{,}{\detokenize{#2}}{%
    \skv@err{Only one prefix is allowed when calling
      \MessageBreak \noexpand\skvdefinekeys or similar commands,
      \MessageBreak but you gave '#2'}\skv@ehd
  }{%
    % The prefix and families here deserve separate names, to avoid
    % confusing them with those required for setting the keys of the
    % macro \skvdefinekeys.
    \edef\skv@checkkeyexist{\ifskv@st00\else01\fi}%
    \edef\skvdfk@pref{#2}%
    \skvxifinTF{,}{\detokenize{#3}}{%
      \edef\skvdfk@fams{#3}%
      \skvcsvnormalize\skvdfk@fams
    }{%
      \edef\skvdfk@fams{#3}%
      \skvdespacecontent\skvdfk@fams
    }%
    \skv@testopt#1{userhp@}%
  }%
}
\skvrobustdef*\skvedefinekeysifdefinable{\skvedefinekeys*}
% \skvedefinekeys has no stack, since everything is done in a local group.
% It is \skvmakekeys that has a stack.
\skvrobustdef*\skvedefinekeys{%
  \begingroup
  \endlinechar\m@ne
  \skvdfk@testopta\skv@definekeys@a
}
\skvrobustdef*\skvdefinekeys{%
  \begingroup
  \skvdfk@testopta\skv@definekeys@a
}
\skvrobustdef*\skv@definekeys@a[#1]#2{%
  \skvindeftrue
  \def\skv@validtypes{%
    .ord,.cmd,.zcmd,.bool,.zbool,.tog,.ztog,.choice,.choice*,%
    .exec,.afterdef,.initialize,.saveini,.argx0,.argx1,.argx2,.argxx,%
    .preptokey,.apptokey,.preptocode,.apptocode%
  }%
  \def\iftypeis##1\then{%
    \ifnum\skv@strcmp{\skvoxdetok\skv@type}{\detokenize{##1}}=\skvz@
  }%
  \def\do##1{\def##1{}}%
  \do\skv@prependtoeverykeyname\do\skv@appendtoeverykeyname
  \do\skv@prependtoeverycallback\do\skv@appendtoeverycallback
  % Take \skvindeftrue outside the current scope:
  \def\skv@accumulateonfams{\skvindeftrue}%
  \edef\skv@hp{#1}%
  \skvdespacecontent\skv@hp
  \skv@makeprefix\skvdfk@pref
  \edef\skvdfk@currlist{\skvkeepdoubleslashnormalize{#2}}%
  \def\skv@definekeys@b##1{%
    \skv@makeheader{##1}%
    \def\skv@accumulateonkeys{}%
    \def\skvdfk@keys{}%
    \def\skvdfk@keyvals{}%
    \skvexpbracenext\skv@definekeys@c\skvdfk@currlist
  }%
  % If the plus variant is not specified, just take and use the first
  % family.
  \skvifdefboolTF{skv@pl}{%
    \skvcommaloop*\skvdfk@fams\skv@tempa{%
      \skvexpbracenext\skv@definekeys@b\skv@tempa
    }%
  }{%
    \def\skv@prova##1,##2\skv@nil{%
      \skv@definekeys@b{##1}%
    }%
    \expandafter\skv@prova\skvdfk@fams,\skv@nil
  }%
  \edef\skv@accumulateonfams{%
    \skvxonce\skv@accumulateonfams
    \skvxonce\skvdfk@afterdefine@hook\relax
  }%
  \expandafter\endgroup\skv@accumulateonfams
  \skvindeffalse
  % 1. No need to reinitialize \skvdfk@afterdefine@hook here. Any changes
  %    done within the exited group haven't survived outside the group.
  % 2. Don't call \skvdfk@initializefalse and \skvdfk@saveinitialvaluesfalse
  %    here while in \directkeys: \skvdefinekeys is reentered for each path.
  %    \ifskvdfk@initialize and \ifskvdfk@saveinitialvalues are in the
  %    stack of \directkeys
  \ifindirectkeys\else
    \skvdfk@initializefalse\skvdfk@saveinitialvaluesfalse
  \fi
}
\skvrobustdef*\skv@definekeys@c#1{%
  \edef\skv@igkeys{%
    \skvifcsname\skvcurrentpath.@ignoredkeys\then
      \skvexpandcsonce{\skvcurrentpath.@ignoredkeys}%
    \fi
  }%
  \def\skv@splita##1/##2/{\skv@splitb##1/##2/.}%
  \def\skv@splitb##1/##2/##3/##4/##5/##6/##7/##8/##9\skv@split@nil{%
    \skvxifinTF{\skv@hashchar}{\detokenize{##2}}{%
      \skv@err{Key name(s) '\detokenize{##2}' contain hash character}\skv@ehd
    }{%
      % In case we have, eg, .exec=\def\x{?} instead of .exec/\def\x{?}:
      \skvxifinTF{=}{\detokenize{##1}}{%
        \skv@kvsplit{##1}{%
          \edef\skv@type{\skvtrimspace{####1}}%
          \edef\skv@itemtwo{\skvtrimspace{####2}}%
        }%
      }{%
        \edef\skv@type{\unexpanded{##1}}%
        \edef\skv@itemtwo{\unexpanded{##2}}%
      }%
    }%
    \skvifcsname skvdfk@typealias@\skv@type\then
      \edef\skv@type{\@nameuse{skvdfk@typealias@\skv@type}}%
    \fi
    \edef\skv@default{\skvexpandonce{\@gobble##3}}%
    % To avoid mixing parameter characters in \skv@prova:
    \edef\skv@rest{\unexpanded{{##4}/{##5}/{##6}/{##7}/{##8}/{##9}}}%
    \skvexpbracenext\skv@definekeys@d\skv@type
  }%
  \def\skv@splitc##1/##2/##3/##4/##5/##6/##7/##8/##9\skv@split@nil{%
    \edef\skv@itemfour{\unexpanded{##4}}%
    \edef\skv@itemfive{\unexpanded{##5}}%
    \edef\skv@itemsix{\unexpanded{##6}}%
    \skvifknobTF{skv@isarg}{%
      \skvdfk@definearg{##1}{##2}{##3}%
    }{%
      \if\skv@checkkeyexist
        \skvifcsname\skv@header##2.@cbk\then
          \skv@err{Key '\skvcurrenttriple' already exists}\skv@ehd
        \fi
      \fi
      \if\skv@ischoice
        \skv@ifcmdnut\skv@itemfour{%
          \skv@err{Empty nominations (state pattern) for
            \MessageBreak choice key '##2'}\skv@ehd
        }{}%
      \fi
      \edef\skvdfk@keys{\skvaddlist,\skvdfk@keys##2}%
      \skvxifboolvalTF{\skvexpandonce\skv@default}\in@true\in@false
      \edef\skvdfk@keyvals{%
        \skvaddlist,\skvdfk@keyvals
        \skv@ifcmdrejordotna\skv@default{}{%
          ##2=\skvifdefboolTF{in@}{false}{\skvexpandonce\skv@default}%
        }%
      }%
      \if\skv@isboolorchoice
        \if\skv@ischoice
          \let\skv@altact\skv@itemsix
        \else
          % bool or tog:
          \let\skv@altact\skv@itemfive
        \fi
        \skv@ifcmdnut\skv@altact{\let\skv@altact\skvkeyvalueerror}{}%
      \fi
      \iftypeis.choice*\then
        \def\skv@prova####1*{\def\skv@typeb{####1}}%
        \expandafter\skv@prova\skv@type
      \else
        \let\skv@typeb\skv@type
      \fi
      % Remove leading dot (.):
      \edef\skv@typeb{\expandafter\@gobble\skv@typeb}%
      \edef\skv@accumulateonkeys{%
        \skvexpandonce\skv@accumulateonkeys
        \skvnoexpandcs{skv\skv@typeb key}%
        \iftypeis.choice*\then*\fi
        \if\skv@isboolorchoice+\fi
        [\skvcurrentprefix]{\skvcurrentfamily}%
        \if\skv@needhp[\skv@hp]\fi
        {##2}%
        \if\skv@ischoice
          [\unexpanded{\skvuserinput\skvorder}]{\skvxonce\skv@itemfour}%
        \fi
        % default:
        \skv@ifcmdrejordotna\skv@default{}{[{\skvxonce\skv@default}]}%
        {% Key callback:
          \skvxonce\skv@prependtoeverycallback
          % If choice key, then the callback is item 5, otherwise
          % it's item 4:
          \if\skv@ischoice
            \skv@ifcmdnut\skv@itemfive{}{\skvxonce\skv@itemfive}%
          \else
            \skv@ifcmdnut\skv@itemfour{}{\skvxonce\skv@itemfour}%
          \fi
          \skvxonce\skv@appendtoeverycallback
        }%
        % Second branch of callback for '+' variants, now used for all
        % boolean and choice keys:
        \if\skv@isboolorchoice{\skvexpandonce\skv@altact}\fi
      }%
    }%
  }%
  \skvexpanded{\skvparselist{\skvdfk@parser}}{#1}\skv@prova{%
    \expandafter\skv@splita\skv@prova
      /^skv^/^skv^/^skv^/^skv^/^skv^/^skv^/^skv^/^skv^\skv@split@nil
  }%
  % 1. \skv@accumulateonfams is a two-layer stack: there're loops on
  %    families and keys.
  % 2. To save initial values of keys, the key names should be
  %    entered by \skvsaveinitialvaluekeys in 'needini' list. This is
  %    the case even when the boolean '.initialize' is true. See below.
  % 3. The boolean '.save initial values' is the one that will invoke
  %    \skvsaveinitialvaluekeys below.
  \def\@elt{%
    [\skvcurrentprefix]{\skvcurrentfamily}{\skvxonce\skvdfk@keyvals}%
  }%
  \edef\skv@accumulateonfams{%
    \skvexpandonce\skv@accumulateonfams
    \ifskvdfk@saveinitialvalues
      \noexpand\skvsaveinitialvaluekeys\@elt
    \fi
    \skvexpandonce\skv@accumulateonkeys
    \ifskvdfk@initialize
      \noexpand\skvsetkeys\@elt
    \fi
  }%
}
\skvrobustdef*\skv@definekeys@d#1{%
  \skvxifinFT{,#1,}{,\skv@validtypes,}{%
    \skv@err{Invalid key type '#1' in \string\skvdefinekeys}\skv@ehd
  }{%
    \@tempswatrue
    \iftypeis.exec\then
      \@tempswafalse
      \edef\skv@accumulateonkeys{%
        \skvexpandonce\skv@accumulateonkeys\skvexpandonce\skv@itemtwo
      }%
    \else
      \iftypeis.initialize\then
        \@tempswafalse
        \skv@ifcmdnut\skv@itemtwo{%
          \edef\skv@itemtwo{true}%
        }{%
          \skvexpbracenext\skvifboolvalT\skv@itemtwo\relax
        }%
        \csname skvdfk@initialize\skv@itemtwo\endcsname
        \edef\skv@accumulateonfams{%
          \skvexpandonce\skv@accumulateonfams
          \noexpand\csname skvdfk@initialize\skv@itemtwo\endcsname
        }%
      \else
        \iftypeis.saveini\then
          \@tempswafalse
          \skv@ifcmdnut\skv@itemtwo{%
            \edef\skv@itemtwo{true}%
          }{%
            \skvexpbracenext\skvifboolvalT\skv@itemtwo\relax
          }%
          \csname skvdfk@saveinitialvalues\skv@itemtwo\endcsname
          \edef\skv@accumulateonfams{%
            \skvexpandonce\skv@accumulateonfams
            \noexpand\csname skvdfk@saveinitialvalues\skv@itemtwo
              \endcsname
          }%
        \else
          \iftypeis.preptokey\then
            \@tempswafalse
            \let\skv@prependtoeverykeyname\skv@itemtwo
          \else
            \iftypeis.apptokey\then
              \@tempswafalse
              \let\skv@appendtoeverykeyname\skv@itemtwo
            \else
              \iftypeis.preptocode\then
                \@tempswafalse
                \let\skv@prependtoeverycallback\skv@itemtwo
              \else
                \iftypeis.apptocode\then
                  \@tempswafalse
                  \let\skv@appendtoeverycallback\skv@itemtwo
                \fi
              \fi
            \fi
          \fi
        \fi
      \fi
    \fi
    \skvifdefboolTF{@tempswa}{%
      % Leave these tests here, so that they aren't repeated for each
      % key in the next loop:
      \def\do##1{\def##1{01}}%
      \do\skv@isboolorchoice\do\skv@ischoice\do\skv@needhp\do\skv@isarg
      \skvifinTF{,#1,}{,.choice,.choice*,}{%
        \skvstripouterbraces{2}\skv@default
        \def\do##1{\def##1{00}}%
        \do\skv@ischoice\do\skv@isboolorchoice\do\skv@needhp
      }{%
        \skvifinTF{,#1,}{,.bool,.zbool,.tog,.ztog,}{%
          \def\skv@isboolorchoice{00}%
          \def\skv@needhp{00}%
        }{%
          \skvifinTF{,#1,}{,.cmd,.zcmd,}{%
            \def\skv@needhp{00}%
          }{%
            \skvifinTF{,#1,}{,.argx0,.argx1,.argx2,.argxx,}{%
              \def\skv@isarg{00}%
            }{}%
          }%
        }%
      }%
      \skvcommaloop*\skv@itemtwo\skv@tempa{%
        \skv@strippointersfromkey*\skv@tempa
        \edef\skvcurrentkey{%
          \skv@prependtoeverykeyname\skvcurrentkey
          \skv@appendtoeverykeyname
        }%
        \let\do\skvoxdetok
        \skvxifinTF{,\do\skvcurrentkey,}{,\do\skv@igkeys,}{}{%
          \edef\do{%
            \noexpand\skv@splitc#1/\skvcurrentkey/%
              {\skvexpandonce\skv@default}/\skvexpandonce\skv@rest
          }%
          \do\skv@split@nil
        }%
      }%
    }{%
      \skvifinFT{,#1,}{,.preptokey,.apptokey,.preptocode,.apptocode,}{}{%
        \let\skv@tempa\skv@itemtwo
        \skv@strippointersfromkey*\skv@itemtwo
        \let\skv@itemtwo\skvcurrentkey
        \ifx\skv@tempa\skv@itemtwo\else
          \skv@err{The token ||\skvoxdetok\skv@itemtwo||
            \MessageBreak shouldn't contain pointers for the
            given key type or requested action}\skv@ehd
        \fi
      }%
    }%
  }%
}
%
% Assigning arguments within \skvdefinekeys:
%
% Eg, using the type .arg:
%
%   .arg/{key1,key2}/{#1/#2}
%
\skvrobustdef*\skvdfk@definearg#1#2#3{%
  \begingroup
  \def\skv@prova.arg##1\skv@nil{%
    \edef\skv@prova{\skvtrimspace{##1}}%
  }%
  \skv@prova#1\skv@nil
  \edef\skv@accumulateonkeys{%
    \skvexpandonce\skv@accumulateonkeys
    \skvcsedef{\skv@header#2.@\skv@prova arg}{%
      \noexpand\unexpanded{\unexpanded{#3}}%
    }%
  }%
  \skvaftergroupdef\skv@accumulateonkeys\endgroup
}

%+++++++++++++++++++++++ Keys for \skvmakekeys +++++++++++++++++++++++%
% Example:
% \skvmakekeys[
%    .prefix=KVA, .families={fam1,fam2}, .hp=thp@, .all new,
%    .define in all families, .initialize=true, .endlinechar=-1
% ]{%
%    .ord/{keya,keyb}/{default-a},
%    .cmd/{keyc,keyd}/,
%    .zcmd/key e/\def\cmde##1{##1}/
%      \edef\y{\detokenize\expandafter{\thp@keye}}\def\x##1{#1*key e*##1},
%    .choice/keyf/center/{center.do=\def\x##1{#1*##1},left,right},
%    .zbool/show center/true/\edef\cmd{\ifthp@showcenter Yes\else No\fi}
% }
% \skvshowcs{KVA/fam1/keyb.@defa}
% \def\keybval{xx}
% \skvsetkeys[KVA]{fam1}{keyb=.expand once{\keybval}}

\skvedefinekeys*[SKV]{makekeys}[skvmk@]{%
  .ord/{.new,.all new,.all are new}/true/
    \edef\skvmk@allnew{0\skvifstrcmpTF{#1}{true}{0}{1}}
  ,
  .ord/{.initialize,.initialize after define,.initialize keys after define}
    /true/
    \skvifboolvalT{#1}{%
      \csname skvdfk@initialize#1\endcsname
    }%
  ,
  .ord/.save initial values,.save initial values of keys/true/
    \skvifboolvalT{#1}{%
      \csname skvdfk@saveinitialvalues#1\endcsname
    }%
  ,
  .ord/{.endlinechar,.endline character}/13/
    \def\skvmk@endlinechar{#1},
  .ord/{.define in all families,.in all families}/true/
    \edef\skvmk@inallfams{0\skvifstrcmpTF{#1}{true}{0}{1}}
  ,
  .ord/.prefix/\skvdefaultprefix/
    \skviflacus#1\then
      \let\skvmk@pref\skvdefaultprefix
    \else
      \edef\skvmk@pref{#1}%
      \skvstripouterbraces{2}\skvmk@pref
    \fi
  ,
  .ord/{.family,.families}/\skv@nil/
    \skviflacus#1\then
      \skv@err{Key family is empty\on@line}\skv@ehd
    \else
      \edef\skvmk@fams{#1}%
      \skvstripouterbraces{2}\skvmk@fams
    \fi
  ,
   .ord/{.holder prefix,.hp}/userhp@/\edef\skvmk@hp{#1}
}

% Default settings for keys of \skvmakekeys. Presetting keys will be
% inefficient here, since many of the keys have complements. It will be
% necessary to include all the complements in the preset list, but doing
% this will be inefficient.
\skvsetkeys[SKV]{makekeys}{%
  .prefix,.family,.hp,.new=false,.define in all families=false,
  .endlinechar=13,.initialize=false,.save initial values=false
}
\skvrobustdef*\skvmakekeys{\skv@testopt\skv@makekeys{}}
\skvrobustdef*\skv@makekeys[#1]#2{%
  \skvpushfunctions\skvmakekeys{%
    \do\skvmk@pref\do\skvmk@fams\do\skvmk@allnew\do\skvmk@hp
    \do\skvmk@endlinechar\do\skvmk@inallfams\do\ifskvdfk@initialize
    \do\ifskvdfk@saveinitialvalues
  }\skv@makekeysdepth
  \skvsetkeys[SKV]{makekeys}{#1}%
  \ifx\skvmk@fams\skv@nnil
    \skv@err{No family specified for \string\skvmakekeys}\skv@ehd
  \fi
  % The following \begingroup is ended in \skv@definekeys:
  \begingroup
  \skvexpanded{%
    \endlinechar=\skvmk@endlinechar\relax
    \skvdfk@testopta\skv@definekeys@a
    \if\skvmk@allnew*\fi\if\skvmk@inallfams+\fi
    [\skvmk@pref]{\skvmk@fams}%
    [\ifx\skvmk@hp\@empty userhp@\else\skvmk@hp\fi]%
  }%
  {#2}%
  \skvpopfunctions\skvmakekeys\skv@makekeysdepth
}

\skvrobustdef*\skvkeyvalueerror{%
  \skv@getinnoval\CurrentOption
  \skv@err{Erroneous value '\skv@ival' for key or option
    \MessageBreak'\skvcurrentkey'}{Invalid key value encountered.}%
}

\skvrobustdef*\skv@getinnoval#1{%
  \begingroup
  \skv@okvsplit{#1}{%
    \edef\skv@provb{\detokenize{##2}}%
    \skvifxTF\skv@provb\@empty{%
      \def\skv@ival{???}%
    }{%
      \skv@getshortformofcontent{30}\skv@provb\skv@ival
    }%
  }%
  \skvaftergroupdef\skv@ival\endgroup
}
% \skv@getshortformofcontent{<nr>}{<toks.cmd>}{<result.cmd>}
\skvrobustdef*\skv@getshortformofcontent#1#2#3{%
  \begingroup
  \edef\skv@prova{\detokenize\expandafter{#2}}%
  \def#3{}\@tempcnta\skvz@
  \def\do##1{%
    \def\skv@prova{##1}%
    \skvifxTF\skv@prova\skv@nnil{}{%
      \advance\@tempcnta\@ne
      \ifnum\@tempcnta<#1\relax
        \edef#3{#3\ifx\next\@sptoken\@space\fi##1}%
      \else
        \def\@do####1\skv@nil{}%
      \fi
      \@do
    }%
  }%
  \def\@do{\futurelet\next\do}%
  \expandafter\@do\skv@prova\skv@nil
  \skvaftergroupdef#3\endgroup
}

% +++++++++++ User-defined handlers for unknown keys. +++++++++++++%
%
% \skvunknownkeyhandler[<prefixes>]{<families>}{<handler>}
%
% Note: See skeyval.sty for \skvunknownoptionhandler.
%
% Eg, for keya undefined in KV/fam:
%
% \skvunknownkeyhandler[KV]{fam}{%
%   \skvordkey[#1]{#2}{#3}[#4]{\def\x##1{##1xx#4}}%
% }
% \skvsetkeys[KV]{fam}{unknownkey=val}
%
\skvrobustdef*\skvunknownkeyhandler{%
  \skv@testopt\skv@unknownkeyhandler\skvdefaultprefix
}
% For each prefix and family, this will define the functions
% \<prefix>/<family>/.@famhandler of 4 parameters (prefix, family,
% key name, current value).
\skvrobustdef*\skv@unknownkeyhandler[#1]#2#3{%
  \skvcommaloop{#1}\skv@tempa{%
    \skv@makeprefix\skv@tempa
    \skvcommaloop{#2}\skv@tempb{%
      \skv@makeheader\skv@tempb
      \skvcsdef{\skvcurrentpath.@famhandler}##1##2##3##4{#3}%
    }%
  }%
}

%%++++++++++++++++++++++ Keys for \skvusekeys: +++++++++++++++++++++++%%
% Example:
% \skvusekeys[
%    .prefix=KVA,.families={fam1,fam2},.set in all families,
%    .save rm keys
% ]{%
%    key1=value1, key2=value2
% }
\skvmakekeys[
  .prefix=SKV,.family=usekeys,.hp=skvuk@,.endlinechar=-1
]{%
  .ord/{.save rm,.save rm keys,.save unknown keys}/true/
    \edef\skvuk@saverm{\skvifstrcmpTF{#1}{true}{00}{01}}
  ,
  .ord/{.set in all families,.in all families}/true/
    \edef\skvuk@inallfams{\skvifstrcmpTF{#1}{true}{00}{01}}
  ,
  .ord/.prefix/\skvdefaultprefix/
    \skviflacus#1\then
      \let\skvuk@pref\skvdefaultprefix
    \else
      \edef\skvuk@pref{#1}%
      \skvstripouterbraces{2}\skvuk@pref
    \fi
  ,
  .ord/{.family,.families}/\skv@nil/
    \skviflacus#1\then
      \skv@err{Key family is empty\on@line}\skv@ehd
    \else
      \edef\skvuk@fams{#1}%
      \skvstripouterbraces{2}\skvuk@fams
    \fi
  ,
  .ord/{.path,paths}/\skv@nil/
    \skvifblankTF{#1}{%
      \skv@err{Key family is empty\on@line}\skv@ehd
    }{%
      \edef\skv@tempa{#1}%
      \ifx\skv@tempa\skv@nnil
        \skv@err{No path specified for \string\skvusekeys}\skv@ehd
      \else
        \skvstripouterbraces{2}\skv@tempa
        \skv@splitpath@a\skv@tempa\skvuk@pref\skvuk@fams
      \fi
    }%
  ,
}

% Default settings for keys of \skvusekeys:
\skvsetkeys[SKV]{usekeys}{%
  .prefix,.family,.set in all families=false,.save rm=false%
}

\skvrobustdef*\skvusekeys{\skv@testopt\skv@usekeys{}}
\skvrobustdef*\skv@usekeys[#1]#2{%
  \skvpushfunctions\skvusekeys{%
    \do\skvuk@fams\do\skvuk@pref\do\skvuk@inallfams\do\skvuk@saverm
  }\skv@usekeysdepth
  \skvsetkeys[SKV]{usekeys}{#1}%
  \ifx\skvuk@fams\skv@nnil
    \skv@err{No family specified for \string\skvusekeys}\skv@ehd
  \fi
  \skvexpanded{%
    \noexpand\skvsetkeys\if\skvuk@saverm*\fi\if\skvuk@inallfams+\fi
    [\skvuk@pref]{\skvuk@fams}{\unexpanded{#2}}%
  }%
  \skvpopfunctions\skvusekeys\skv@usekeysdepth
}

%++++++++++ Utilities for handlers of the macro \directkeys +++++++++++%

\skvnewlet\skvhandlereov\relax
% Undefine \dirkeys@handler@, in case a handler function is called
% without the handler name. Handler functions usually require
% 'dirkeys@handler@<handler.name>'.
\skvundef\dirkeys@handler@

\skvrobustdef*\skvsetdirectkeysparser{\def\dirkeys@parser}
\skvsetdirectkeysparser{,}
\skvrobustdef*\directkeys{\skv@testst\skv@dirkeys@parse@a}
\skvrobustdef*\skv@dirkeys@parse@a{%
  \begingroup
  \ifskv@tempst\endlinechar\m@ne\fi
  \skv@dirkeys@parse@b
}
\skvrobustdef*\skv@dirkeys@parse@b#1{%
  \endgroup
  \skvpushstate\skv@dirkeys@state\dirkeys@depth
  \indirectkeystrue
  \def\dirkeys@pathlist{}%
  \def\dirkeys@holderprefixtoks{}%
  \dirkeys@saveunknownkeysfalse
  \skvdfk@initializefalse
  \skvdfk@saveinitialvaluesfalse
  \edef\skv@tempa{\unexpanded{#1}}%
  \skvstripouterbraces{2}\skv@tempa
  % Normalize with respect to equality (=) and comma (,), since
  % \skvkvnormalize can't normalize with respect to \dirkeys@parser
  % that isn't comma (,). \skvparselist will normalize with respect
  % to \dirkeys@parser:
  \skvkvnormalize\skv@tempa
  \def\skv@dirkeys@split##1=##2=##3\dirkeys@nil{%
    \edef\skv@tempa{\unexpanded{##2}}%
    \skvstripouterbraces{2}\skv@tempa
    \skvdespacecontent\skv@tempa
    % Get the first token, to test if it's \directkeys. If it is, then
    % we have a nested \dirkeys:
    \expandafter\skvifxTF\skv@car##1x\car@nil\directkeys{%
      \skvifemptyTF\skv@tempa{%
        ##1\relax
      }{%
        \skv@err{Something wrong with use of \string\dirkeys:
          \MessageBreak equals ('=') found after \string\dirkeys}\skv@ehd
      }%
    }{%
      \skv@ensurehandlerdot{##1}%
      \skvifcsdefTF{dirkeys@handler@##1}{%
        \csname dirkeys@handler@##1\expandafter\endcsname
          \skv@tempa\skvhandlereov
      }{%
        \skv@err{Unknown handler '\detokenize{##1}'
          \MessageBreak in command \string\directkeys, or no '=' sign
          \MessageBreak after handler name}\skv@ehd
      }%
    }%
  }%
  % Normalize with respect to \dirkeys@parser:
  \skvexpanded{\skvparselist*{\dirkeys@parser}}\skv@tempa\skv@tempa{%
    \expandafter\skv@dirkeys@split\skv@tempa==\dirkeys@nil
  }%
  \indirectkeysfalse
  \skvpopstate\skv@dirkeys@state\dirkeys@depth
}
\skvrobustdef*\dirkeys@setdefaultpath{%
  \ifx\dirkeys@pathlist\@empty
    \ifskv@inopt
      \edef\dirkeys@pathlist{%
        \noexpand\skv@pathdo{KV}{\@currname.\@currext}%
      }%
    \else
      \skv@err{No key can have empty or nil path/family}\skv@ehd
    \fi
  \fi
  \ifx\dirkeys@holderprefixtoks\@empty
    \def\dirkeys@holderprefixtoks{user@}%
  \fi
}
\skvnewnumbers[skv@]{pathdepth}
\skvrobustdef*\skv@pushpathdo{%
  \edef\skv@pathdepth{\the\numexpr\skv@pathdepth+1}%
  \skvcslet{skv@pathdo@\romannumeral\skv@pathdepth}\skv@pathdo
}
\skvrobustdef*\skv@poppathdo{%
  \skvletcs\skv@pathdo{skv@pathdo@\romannumeral\skv@pathdepth}%
  \edef\skv@pathdepth{\the\numexpr\skv@pathdepth-1}%
}
\skvrobustdef*\dirkeys@dodefinekeys#1#2{%
  \begingroup
  % #2 may contain parameter characters that may be confused with
  % ##1 and ##2 below. Hence we put it in the macro \skv@tempb.
  % Note: Ignored keys are omitted by \skvdefinekeys.
  \edef\skv@tempb{\unexpanded{#2}}%
  \def\skv@tempa{}%
  \def\skv@pathdo##1##2{%
    \edef\skv@tempa{%
      \skvexpandonce\skv@tempa
      \skvdefinekeys#1[##1]{##2}%
      [\dirkeys@holderprefixtoks]{\skvexpandonce\skv@tempb}%
    }%
  }%
  \dirkeys@pathlist
  \expandafter\endgroup\skv@tempa
}
% \dirkeys@definetypekeys{<type>}{<star.or.empty>}{<keylist>}
\skvrobustdef*\dirkeys@definetypekeys#1#2#3{%
  \begingroup
  \def\skv@tempa{}%
  \skvexpanded{\skvparselist{\skvdfk@parser}}{#3}\skv@prova{%
    \edef\skv@tempa{%
      \skvexpandonce\skv@tempa
      \ifx\skv@tempa\@empty\else\skvdfk@parser\fi
      .#1/\skvexpandonce\skv@prova
    }%
  }%
  \skvexpanded{\endgroup
    \dirkeys@dodefinekeys{#2}{\skvexpandonce\skv@tempa}%
  }%
}
\skvrobustdef*\dirkeys@setkeys#1#2#3#4{%
  \begingroup
  % #1 may contain parameter characters that may be confused with
  % ##1 and ##2 below. Hence we put it in the macro \skv@tempb:
  \edef\skv@tempb{\unexpanded{#4}}%
  \def\skv@tempa{}%
  \def\skv@pathdo##1##2{%
    \edef\skv@tempa{%
      \skvexpandonce\skv@tempa
      #3\ifdirkeys@saveunknownkeys*\else#1\fi
      [##1]{##2}[\skvcsuse{##1/##2/.@ignoredkeys}]%
      \skvifstrcmpTF{#2}{rm}{}{{\skvexpandonce\skv@tempb}}%
    }%
  }%
  \dirkeys@pathlist
  \expandafter\endgroup\skv@tempa
}

% This is used by prepostsetkeys, etc.
% \dirkeys@dolistedkeys@a{<key.list>}{<callback>}
\skvrobustdef*\dirkeys@dolistedkeys@a#1#2{%
  \begingroup
  \def\skv@tempd{}%
  % ##1=prefix, ##2=family
  \def\skv@pathdo##1##2{%
    \def\skv@tempb{}%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvcommaparse{#1}\skv@tempa{%
      \skvxifinTF{,\skvoxdetok\skv@tempa,}{,\skvoxdetok\skv@igkeys,}{}{%
        \edef\skv@tempb{\skvaddlist,\skv@tempb\skvexpandonce\skv@tempa}%
      }%
    }%
    \edef\skv@tempd{%
      \skvexpandonce\skv@tempd
      \skvifemptyTF\skv@tempb{}{%
        \noexpand#2[##1]{##2}{\skvexpandonce\skv@tempb}%
      }%
    }%
  }%
  \dirkeys@pathlist
  \expandafter\endgroup\skv@tempd
}

% \dirkeys@dolistedkeys@b{<callback>}
\skvrobustdef*\dirkeys@dolistedkeys@b#1{%
  \begingroup
  \def\skv@tempa{}%
  % ##1=prefix, ##2=family
  \def\skv@pathdo##1##2{%
    \edef\skv@tempa{%
      \skvexpandonce\skv@tempa
      \unexpanded{\skv@makeprefix{##1}\skv@makeheader{##2}#1}%
    }%
  }%
  \dirkeys@pathlist
  \expandafter\endgroup\skv@tempa
}
\skvrobustdef*\skv@getmaintoks#1#2{%
  \def\skv@prova##1#2##2#2##3\skv@nil{%
    \edef\skvcurrentmaintoks{\skvtrimspace{##1}}%
    \skvstripouterbraces{2}\skvcurrentmaintoks
    \ifx\skvcurrentmaintoks\@empty
      \skv@err{No main key in '\detokenize{#1}'}\skv@ehd
    \fi
    \edef\skvcurrentsub{\unexpanded{##2}}%
    \ifx\skvcurrentsub\skv@novaluetoks
      \def\skvcurrentsub{}%
    \else\skvafterfi
      \skvdespacecontent\skvcurrentsub
      \skvstripouterbraces{2}\skvcurrentsub
    \fi
  }%
  \skv@prova#1#2\skv@novalue#2\skv@nil
}

% Pushing and popping path or holder prefix.
%
\skvnewnumbers[dirkeys@meta]{pathdepth,hpdepth}
\skvrobustdef*\dirkeys@pushmeta#1{%
  \skvifcasse{#1}
    case{path}{\def\@elt{pathlist}}
    case{hp}{\def\@elt{holderprefixtoks}}
  \elsedo
    \skv@err{Unknown meta type '#1'}\skv@ehd
  \endif
  \skvaftercs\skvgadvanceno{dirkeys@meta#1depth}\@ne
  \edef\skv@elt{\skvrom\csname dirkeys@meta#1depth\endcsname}%
  \skvcsletcs{dirkeys@\@elt @meta@\skv@elt}{dirkeys@\@elt}%
}
\skvrobustdef*\dirkeys@popmeta#1{%
  \skvifcase\skvifstrcmpTF{#1}%
    {path}{\def\@elt{pathlist}}%
    {hp}{\def\@elt{holderprefixtoks}}%
  \elsedo
    \skv@err{Unknown meta type '#1'}\skv@ehd
  \endif
  \edef\skv@elt{\skvrom\csname dirkeys@meta#1depth\endcsname}%
  \skvcsletcs{dirkeys@\@elt}{dirkeys@\@elt @meta@\skv@elt}%
  \skvaftercs\skvgadvanceno{dirkeys@meta#1depth}\m@ne
}

% Assigning admissible values to keys. The handlers here are:
%
% .state pattern, .state pattern expanded, .state pattern expand once,
% .state pattern expand twice.
%
% \dirkeys@savechoice{<list>}{<expander.type>}
%
% 1. <list> has the form
%
%      {<key1,...,keyn>}/{<ch1>.do={<act1>},...,<ch-n>.do={<act-n>}}
%              ,...,
%      <keyx-n>/{<ch1>.do={<act1>},...,<ch-n>.do={<act-n>}}
%
% 2. If it didn't exist, the main key (eg, the above <key1>) will be
%    defined with an empty default value and an empty callback.
%
\skvrobustdef*\dirkeys@savechoice#1#2{%
  \begingroup
  \def\skv@tempd{}%
  \edef\skv@tempa{\unexpanded{#1}}%
  \skvcsvnormalize[/]\skv@tempa
  \skvcommaparse*\skv@tempa\skv@tempa{%
    \skvexpbracenext\dirkeys@s@vechoice\skv@tempa{#2}%
  }%
  \expandafter\endgroup\skv@tempd
}
\skvrobustdef*\dirkeys@s@vechoice#1#2{%
  \skv@getmaintoks{#1}{/}%
  \skvkvnormalize\skvcurrentsub
  \def\skv@pathdo##1##2{%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvcommaparse*\skvcurrentmaintoks\skv@tempb{%
      \skvxifinTF{,\skv@tempb,}{,\skv@igkeys,}{}{%
        \skvifcsdefTF{##1/##2/\skv@tempb.@cbk}{}{%
          \edef\skv@tempd{%
            \skvexpandonce\skv@tempd
            \skvordkey[##1]{##2}{\skv@tempb}[]{}%
          }%
        }%
        \def\skv@choicelist{}%
        \skvcommaloop*\skvcurrentsub\skv@tempa{%
          \def\skv@prova####1.do=####2.do=####3\skv@nil{%
            \edef\skv@choicelist{%
              \skvexpandonce\skv@choicelist
              {\skvtrimspace{####1}}{\skvtrimspace{####2}}%
            }%
          }%
          \expandafter\skv@prova\skv@tempa.do=.do=\skv@nil
        }%
      }%
      \edef\skv@tempd{%
        \skvexpandonce\skv@tempd
        \skvappendkeycode[##1]{##2}{\skv@tempb}%
          {\dirkeys@executechoice{#2}{########1}%
          {\skvexpandonce\skv@choicelist}}%
      }%
    }%
  }%
  \dirkeys@pathlist
}
% \dirkeys@executechoice{<expansion.type>}{<curr.value>}{<choices.and.cbks>}
\skvrobustdef*\dirkeys@executechoice#1#2#3{%
  \skv@getexpander{#1}%
  \edef\skv@prova{\skvexpander{#2}}%
  \skvdespacecontent\skv@prova
  \def\do##1##2##3\skv@nil{%
    \edef\skv@provb{\unexpanded{##1}}%
    \skvifxTF\skv@provb\skv@prova{%
      ##2%
    }{%
      \skvifblankTF{##3}{%
        \skv@err{No choice match found for key '\skvcurrentkey'}\skv@ehd
      }{%
        \do##3\skv@nil
      }%
    }%
  }%
  \do#3\skv@nil
}

% Slot/style keys represent a limited signal-slot (or subject-observer)
% concept from Java.
%
% The handlers here are:
%
% .slot, .slot value expanded, .slot expand once, .slot expand twice,
% .prepend slot, .prepend slot value expanded, .prepend slot expand once,
% .prepend slot expand twice, .append slot, .append slot value expanded,
% .append slot expand once, .append slot expand twice
%
% Note that the handlers are preceded by 'append' or 'prepend'.
%
% \dirkeys@saveslots{<list>}{<append.or.prepend>}{<expander.type>}
%
% 1. <list> has the form
%
%    {<signal key1>,...,<signal key-n>}/{<slot1=val1>,...,<slot-n=val-n>}
%                            ,...,
%    {<signal key1>,...,<signal key-n>/{<slot1=val1>,...,<slot-n=val-n>}
%
% 2. Here the slots are linked with each signal key. When the signal key is
%    set, the associated slots will be set with the given values.
%
% 3. Examples:
%
%    a) The following example means that keyc and keyd are signals
%       (representations for the actions on their right, ie, for setting
%       the slots 'keya=\someright, keyb=\keybval' when keyc or keyd is set).
%       The values of keya and keyb will be expanded twice before the
%       keys are set:
%
%       .append slot expand twice={keyc,keyd}/{keya=\someright,keyb=\keybval}.
%
%    b) In the following example, #1 will be the value of keye and/or keyf
%       when they're set. The values of keye and keyf will be fully expanded
%       before they're assigned to keyc and keyd:
%
%       .prepend slot value expanded={keye,keyf}/{keyc=#1,keyd=#1}
%
\skvrobustdef*\dirkeys@saveslots#1#2#3{%
  \begingroup
  \skv@getexpander{#3}%
  \def\skv@tempd{}%
  \edef\skv@tempa{\unexpanded{#1}}%
  \skvcsvnormalize[/]\skv@tempa
  \skvcommaparse*\skv@tempa\skv@tempa{%
    \skvexpbracenext\dirkeys@s@veslots\skv@tempa{#2}%
  }%
  \expandafter\endgroup\skv@tempd
}
\skvrobustdef*\dirkeys@s@veslots#1#2{%
  \skv@getmaintoks{#1}{/}%
  \skvcsvnormalize\skvcurrentmaintoks
  \skvkvnormalize\skvcurrentsub
  \def\skv@pathdo##1##2{%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvcommaloop*\skvcurrentmaintoks\skv@signalkey{%
      \skvxifinTF{,\skv@signalkey,}{,\skv@igkeys,}{}{%
        \skvifcsdefTF{##1/##2/\skv@signalkey.@cbk}{}{%
          % Signal keys should always be set with a value. If they were
          % undefined before being designated as a signal key, then
          % clearly they should have no default. The empty callback will
          % later be replaced by signal emitters to the slots.
          \edef\skv@tempd{%
            \skvexpandonce\skv@tempd
            \skvordkey[##1]{##2}{.need value{\skv@signalkey}}{}%
          }%
        }%
        % Insert expanders in the sub list:
        \def\skv@slotlist{}%
        \skvcommaloop*\skvcurrentsub\skv@tempa{%
          \skv@okvsplit\skv@tempa{%
            \skvxifstrcmpTF{\skv@signalkey}{####1}{%
              \skv@err{Linking key '####1' to itself}\skv@ehd
            }{%
              % Slot keys must always be predefined, otherwise the signal
              % will be useless:
              \skvifcsdefTF{##1/##2/####1.@cbk}{}{%
                \skv@err{Slot key '####1' is undefined}\skv@ehd
              }%
            }%
            \skvxifinTF{,####1,}{,\skv@igkeys,}{}{%
              \edef\skv@slotlist{%
                \skvaddlist,\skv@slotlist\unexpanded{####1}=%
                \skvexpandonce\skvexpander{\unexpanded{####2}}%
              }%
            }%
          }%
        }%
      }%
      \edef\skv@tempd{%
        \skvexpandonce\skv@tempd
        % The slots contain value expanders \@firstofone, \unexpanded, etc.
        % They will be expanded by the next \skvexpanded when the main key
        % is set.
        \skvifstrcmpTF{#2}{app}{\skvappendkeycode}{\skvprependkeycode}%
          [##1]{##2}{\skv@signalkey}{%
          % Signal keys shouldn't be preset, to avoid cyclic setting
          % of keys. See note above.
          \noexpand\skvifdefboolTF{skv@inprepo}{%
            \noexpand\skv@signalpreseterr
          }{%
            % The following \skvexpanded works on expanders of slot values:
            \skvexpanded{\skvsetkeys[##1]{##2}{\skvexpandonce\skv@slotlist}}%
          }%
        }%
      }%
    }%
  }%
  \dirkeys@pathlist
}

%% +++++++++++++++ Linking keys:
%
% The handlers here are:
%
% .link, .link expanded, .link expand once, .link expand twice,
% .prepend link, .prepend link expanded, .prepend link expand once,
% .prepend link expand twice,
% .append link, .append link expanded, .append link expand once,
% .append link expand twice
%
% \dirkeys@savelinks{<list>}{<append.or.prepend>}{<expander.type>}
%
% 1.  <list> has the form
%
%      {<linkkey-1>,..,<linkkey-n>}/{<parentkey-1>,...,<parentkey-n>}
%
% 2.  The parent key will be set (with the value of link key) whenever the
%     link key is set.
% 3.  If the link key didn't exist, it will be defined as an ordinary key
%     with the default value of the parent key. In this way, setting a
%     link key without value won't give rise to a 'no value and no default
%     error'.
% 4.  Example: Link keyb and keyc to existing keya:
%
%        .link={keyb,keyc}/keya
%
%     This is equivalent to:
%
%        .slot={{keyb,keyc}/keya=#1} OR .style={{keyb,keyc}/keya=#1}
%
%     This will link keyb and keyc to keya, such that when keyb and
%     keyc are set, keya too will be set with their values.
%
\skvrobustdef*\dirkeys@savelinks#1#2#3{%
  \begingroup
  \def\skv@tempe{}%
  \edef\skv@tempa{\unexpanded{#1}}%
  \skvcsvnormalize[/]\skv@tempa
  \skvcommaparse*\skv@tempa\skv@tempa{%
    \skvexpbracenext\skv@getmaintoks\skv@tempa{/}%
    \skvcsvnormalize\skvcurrentmaintoks
    \def\skv@tempd{}%
    \skvcommaparse*\skvcurrentsub\skv@tempb{%
      \edef\skv@tempd{%
        \skvaddlist,\skv@tempd\skvexpandonce\skv@tempb=####1%
      }%
    }%
    \edef\skv@tempe{%
      \skvaddlist,\skv@tempe
      {\skvexpandonce\skvcurrentmaintoks}/{\skvexpandonce\skv@tempd}%
    }%
  }%
  \expandafter\endgroup\expandafter\dirkeys@saveslots
    \expandafter{\skv@tempe}{#2}{#3}%
}
% ++++++++++++ Storing values of keys:
%
% The handlers here are:
%
% .store value in, .store expanded value in, .store expanded once value in,
% .store expanded twice value in.
%
% \dirkeys@savestores{<list>}{<expander.type>}
%
% 1. <list> has the form
%
%    <key-1>/<cmd-1>,...,<key-n>/<cmd-n>
%
% 2. Examples:
%
%    .store expanded twice value in={keyc/\valc,keyd/\vald}
%
\skvrobustdef*\dirkeys@savestores#1#2{%
  \begingroup
  \skv@getexpander{#2}%
  \def\skv@tempd{}%
  \edef\skv@tempa{\unexpanded{#1}}%
  \skvcsvnormalize[/]\skv@tempa
  \skvcommaparse*\skv@tempa\skv@tempa{%
    \skv@oslashsplit\skv@tempa{%
      \skvifstrcmpTF{##2}{^skv^}{%
        \skv@err{No holder commands for key(s) '\detokenize{##1}'}\skv@ehd
      }{%
        \skvcommaparse{##1}\skv@tempa{%
          \skvexpbracenext\dirkeys@s@vestore\skv@tempa{##2}%
        }%
      }%
    }%
  }%
  \expandafter\endgroup\skv@tempd
}
\skvrobustdef*\dirkeys@s@vestore#1#2{%
  \def\skv@pathdo##1##2{%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvxifinTF{,#1,}{,\skv@igkeys,}{}{%
      \skvifcsdefFT{##1/##2/#1.@cbk}{%
        \skv@err{Key '#1' isn't defined
          \MessageBreak on path '##1/##2'}\skv@ehd
      }{%
        \edef\skv@tempd{%
          \skvexpandonce\skv@tempd
          \skvprependkeycode[##1]{##2}{#1}{%
            \skvletcs\noexpand\reserved@a{##1/##2/#1.@value}%
            \edef\noexpand#2{%
              % Don't use \skvcurrentvalue here, since this
              % changes when .setkeys is nested:
              \skvexpandonce\skvexpander{\noexpand\reserved@a}%
            }%
          }%
        }%
      }%
    }%
  }%
  \dirkeys@pathlist
}

\skvrobustdef*\dirkeys@keyslet#1{%
  \def\skv@pathdo##1##2{%
    \skv@makeprefix{##1}%
    \skv@makeheader{##2}%
    \skv@keyslet{#1}%
  }%
  \dirkeys@pathlist
}

% #1: <key-1>=<arg-1>,...,<key-n>=<arg-n>
% #2: <arg.expander.type>
%
\skvrobustdef*\dirkeys@assignarg#1#2{%
  \begingroup
  % Don't take #1 inside \skv@pathdo because it contains parameter
  % characters:
  \edef\skv@tempd{\unexpanded{#1}}%
  \def\skv@tempe{}%
  \skvkvnormalize\skv@tempd
  \def\skv@pathdo##1##2{%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvcommaloop*\skv@tempd\skv@tempa{%
      \skv@okvsplit\skv@tempa{%
        \skvxifinTF{,####1,}{,\skv@igkeys,}{}{%
          \skvifcsdefTF{##1/##2/####1.@cbk}{%
            \skvifblankTF{####2}{}{%
              \edef\skv@tempe{%
                \skvexpandonce\skv@tempe\unexpanded{%
                  \skvcsedef{##1/##2/####1.@#2arg}{\unexpanded{####2}}%
                }%
              }%
            }%
          }{%
            \skv@err{Key '####1' is undefined
              \MessageBreak in family '##1/##2'}\skv@ehd
          }%
        }%
      }%
    }%
  }%
  \dirkeys@pathlist
  \expandafter\endgroup\skv@tempe
}

% Use the default values of <keys> to set the keys.
% \dirkeys@setwithdefaults[<pref>]{<fam>}{<keys>}
\skvrobustdef*\dirkeys@setwithdefaults[#1]#2#3{%
  \begingroup
  \def\skv@defaultlist{}%
  \skvcommaparse{#3}\skvcurrentkey{%
    \skvletcs\skv@prova{#1/#2/\skvcurrentkey.@defa}%
    \skvifdefTF\skv@prova{%
      \skv@getdefault{#1}{#2}\skvcurrentkey\skvcurrentvalue
      \edef\skv@defaultlist{%
        \skvaddlist,\skv@defaultlist
        \skvcurrentkey=\skvexpandonce\skvcurrentvalue
      }%
    }{%
      \skv@err{No default value for key '\skvcurrentkey'
        \MessageBreak in family '#1/#2'}\skv@ehd
    }%
  }%
  \skvexpanded{\endgroup
    \skvsetkeys*+[#1]{#2}{\skvexpandonce\skv@defaultlist}%
  }%
}
\skvrobustdef*\dirkeys@setunknownkeyhandler#1{%
  \begingroup
  \edef\skv@tempa{\unexpanded{#1}}%
  \def\skv@tempb{}%
  \toks@{##1##2##3##4}%
  \def\skv@pathdo##1##2{%
    \skv@makeprefix{##1}%
    \skv@makeheader{##2}%
    \edef\skv@tempb{%
      \skvexpandonce\skv@tempb\protected
      \skvcsdef{\skvcurrentpath.@famhandler}\the\toks@{%
        \skvexpandonce\skv@tempa
      }%
    }%
  }%
  \dirkeys@pathlist
  \expandafter\endgroup\skv@tempb
}

%%++++++++++++++++++++++++++  Try setting keys +++++++++++++++++++++++%%
%
% \skvtrysetkeys[<paths>]{<keyvals>}
%
% \directkeys{
%   .try set keys={<options>}, where
%    <options> includes <paths> and key-value list (see below).
% }
%
% Try to set a given key-value list on the paths given by the independent
% <paths> of \skvtrysetkeys. If called within \directkeys (via the handler
% '.try set keys'), \skvtrysetkeys will ignore the paths that are currently
% prevailing within \directkeys. That is, within \directkeys, the handler
% '.try set keys' acts independent of local circumstances of \directkeys
% and uses its own paths from <options>.
%
% Save the known/found keys in the macro suggested by the option
% <success list macro>. The user can inspect this macro to see the found
% keys. When many families are given by the user, the success list is likely
% to be smaller than failed list.
%
% Raise an error if the number of successful families is less than
% the minimum threshold <min success>. The default value of <min success>
% is 1. The options <min success> and <lower goal> are synonymous.
%
% \skvtrysetkeys is similar to \skvsetkeys*+ (ie, \skvsetkeys with the
% options *+), but in this case we have <try> (ie, the maximum total number
% of attempts - families to search for a given key) before backing off,
% and <upper goal> (the maximum number of successful families in which a key
% should be set).
%
% \skvtrysetkeys too will set existing preset and postset keys in the
% given families.
%
% The options of \skvtrysetkeys are:
%
% .try:
%      The maximum number of the sum of successful and unsuccessful
%      attempts that should be made to set a key in the given SFs. The
%      default value of <try> is 100.
% .upper goal/.max success:
%      The max. number of search families (SF) in which a given key should
%      be set/executed, if the key existed in those families. The number of
%      SFs may be more than <upper goal>, but the key may not need to be
%      executed in all of them. The default value of <upper goal> is 1.
% .lower goal/.min success:
%      The min. number of search families (SF) in which a given key should
%      be set/executed. For any key, if <hits> is less than <lower goal>
%      an error will be flagged. The default of this is 0, meaning that
%      by default no error message will be returned if a key isn't found
%      on any of the paths.
% .path/.paths:
%      Paths to search <pref1>/<fam1>,...,<pref-n>/<fam-n>.
% .prefix
%      The prefix to search (default: KV). The number of prefixes can't
%      be more than 1. If you have multiple prefixes, then use the
%      .paths key. The given prefix will be prepended to all the given
%      families.
% .families/.family
%      The families to search <fam1>,...,<fam-n>.
% .ignore keys:
%      Ignored keys. These keys will not be set even if they are found.
% .save known keys:
%      The boolean that directs that known/found keys should be saved
%      in a macro.
% .save known keys in/success list macro/success list:
%      The macro into which to save known keys. Each known key is
%      saved in the format <pref>/<fam>/<key>. The user can
%      inspect this macro to see the found keys. The default macro is
%      \skvsuccesslist.
% .save unknown keys:
%      The boolean that directs that unknown keys should be saved
%      in a macro.
% .save unknown keys in/fail list macro/fail list:
%      The macro into which to save unknown keys. Each unknown key is
%      saved in the format <pref>/<fam>/<key>. The user can
%      inspect this macro to see the unknown keys. The default macro is
%      \skvfaillist.
% .path exception
%      The user-supplied action (code) to take when a key hasn't been found
%      on the curent path of the given paths. The default path exception
%      is nil.
% .hits exception
%      The user-supplied action (code) to take when the number of hits is
%      less than preferred minimum success. This may specify retrying on
%      some other paths. The default exception is an error message.
%
% NOTES:
%
% 1. When the paths are many, the user has to be right in choosing the
%    options '.try', '.upper goal' and '.lower goal', otherwise not
%    enough paths will be searched. For example, if you want some 'keya'
%    to be set on paths KV1/fam1, KV1/fam2, KV2/fam1, KV2/fam2, and you
%    set '.try=2' or '.upper goal=2', then only 2 paths will be traversed;
%    not the desired 4.

\skvedefinekeys[SKV]{skvtryset}[skvtry@]{%
  .initialize keys after define,
  .ord/{.try,.max attempt,.max attempts,.total}/100/
    \skvensureinteger{.max attempt}{#1}%
    \def\skvtry@maxattempts{#1}%
    \skvstripouterbraces{2}\skvtry@maxattempts
    \edef\skvtry@maxattempts{\number\skvtry@maxattempts}%
    \ifnum\skvtry@maxattempts<\@ne
      \skv@err{The max. number of attempts ('try')
        \MessageBreak can't be less than 1}\skv@ehd
    \fi
  ,
  .ord/{.upper goal,.max success,.max hits}/1/
    \skvensureinteger{upper goal}{#1}%
    \def\skvtry@maxsuccess{#1}%
    \skvstripouterbraces{2}\skvtry@maxsuccess
    \edef\skvtry@maxsuccess{\number\skvtry@maxsuccess}%
    \ifnum\skvtry@maxsuccess<\@ne
      \skv@err{The max. number of successful attempts
        \MessageBreak ('upper goal') can't be less than 1}\skv@ehd
    \fi
  ,
  .ord/{.min success,.lower goal,.goal}/0/
    \skvensureinteger{lower goal}{#1}%
    \def\skvtry@minsuccess{#1}%
    \skvstripouterbraces{2}\skvtry@minsuccess
    \edef\skvtry@minsuccess{\number\skvtry@minsuccess}%
    \ifnum\skvtry@minsuccess<\skvz@
      \skv@err{The min. number of successful attempts
        \MessageBreak ('lower goal') can't be less than 0}\skv@ehd
    \fi
  ,
  % #1=<pref1>/<fam1>,...,<pref-n>/<fam-n>
  .ord/{.path,.paths,.add path,.add paths}/\skv@nil/{
    \edef\skv@tempa{#1}%
    \skvstripouterbraces{2}\skv@tempa
    \ifx\skv@tempa\skv@nnil\def\skv@tempa{}\fi
    \ifx\skv@tempa\@empty\else
      \skvcommaparse*\skv@tempa\skv@prova{%
        \skv@splitpath@a\skv@prova\skv@tempa\skv@tempb
        \edef\skv@prova{{\skv@tempa}{\skv@tempb}}%
        \skvxifinTF{\skvoxdetok\skv@prova}{\skvoxdetok\skvtry@pathlist}{}{%
          \edef\skvtry@pathlist{%
            \skvexpandonce\skvtry@pathlist\noexpand\skvtry@pathdo\skv@prova
          }%
        }%
      }%
      \ifskv@insa
        \begingroup
        \def\skv@pathdo##1##2{%
          \edef\skv@prova{\detokenize{{##1}{##2}}}%
          \skvxifinTF{\skv@prova}{\skvoxdetok\skvtry@pathlist}{}{%
            \edef\skvtry@pathlist{%
              \skvexpandonce\skvtry@pathlist
              \noexpand\skvtry@pathdo{##1}{##2}%
            }%
          }%
        }%
        \dirkeys@pathlist
        \skvaftergroupdef\skvtry@pathlist\endgroup
      \fi
    \fi
  },
  % Prefix is used in making \skvtry@pathlist in .family:
  .ord/{.prefix}/\skvdefaultprefix/
      \skv@ifoneprefix{#1}{%
        \def\skvtry@pref{#1}
        \skvstripouterbraces{2}\skvtry@pref
      }{%
        \skv@err{Only one prefix is allowed in '.try set keys'}\skv@ehd
      }
  ,
  .ord/.prefixes//
    \ifskvindef\else
      \skv@err{Key '.prefixes' not defined; try '.paths'}\skv@ehd
    \fi
  ,
  .ord/{.family,.families}/\skv@nil/
    \edef\skvtry@fams{#1}
    \ifskvindef\else
      \ifx\skvtry@fams\skv@nnil
        \skv@err{No family specified for command
          \MessageBreak\string\skvtrysetkeys or handler '.try set keys'}\skv@ehd
      \fi
    \fi
    \skvstripouterbraces{2}\skvtry@fams
    \skv@makepaths\skvtry@pref\skvtry@fams\skvtry@pathlist\skvtry@pathdo
  ,
  .ord/{.ignore keys}//
    \def\skvtry@igkeys{#1}
    \ifx\skvtry@igkeys\@empty\else
      \skvstripouterbraces{2}\skvtry@igkeys
    \fi
  ,
  .ord/{.save known keys in,.success list,.success list macro}/
    \skvsuccesslist/
    \skviflacus#1\then
      \def\skvtry@knownkeyslistmacro{\skvsuccesslist}%
    \else
      \def\skvtry@knownkeyslistmacro{#1}
    \fi
    \skvstripouterbraces{2}\skvtry@knownkeyslistmacro
  ,
  .ord/{.save unknown keys in,.fail list,.fail list macro}/
    \skvfaillist/
    \skviflacus#1\then
      \def\skvtry@unknownkeyslistmacro{\skvfaillist}%
    \else
      \def\skvtry@unknownkeyslistmacro{#1}
    \fi
    \skvstripouterbraces{2}\skvtry@unknownkeyslistmacro
  ,
  % Exception on each path, if key isn't found:
  .ord/{.if any path fails,.if a path fails,.if path fails}//
    \edef\skvtry@pathexception{\unexpanded{#1}}
    \skvstripouterbraces{1}\skvtry@pathexception
  ,
  % Exception to be triggered after all paths have been searched and the key
  % isn't found:
  .ord/{.if hits less than target,.if hits less than goal,
    .if hits are less than goal}//
    \edef\skvtry@hitsexception{\unexpanded{#1}}
    \skvstripouterbraces{1}\skvtry@hitsexception
  ,
}

% \skvtrysetkeys[<options>]{<kvlist>}
\skvrobustdef*\skvtrysetkeys{\skv@testopt\skv@trysetkeys{}}
\skvrobustdef*\skv@trysetkeys[#1]#2{%
  \skvpushfunctions\skvtrysetkeys{%
    \do\skvtry@maxattempts\do\skvtry@hitsexception\do\skvtry@pathexception
    \do\skvtry@minsuccess\do\skvtry@maxsuccess\do\skvtry@igkeys
    \do\skvtry@knownkeyslistmacro\do\skv@tempknownkeys
    \do\skvtry@unknownkeyslistmacro\do\skv@tempunknownkeys
    \do\skv@triedlist\do\CurrentOption\do\skvtry@pref\do\skvtry@fams
    \do\skvtry@pathlist\do\skv@pathdo\do\skvcurrentkey\do\skvcurrentpath
    \do\skvcurrentprefix\do\skvcurrentfamily
  }\skv@trysetkeysdepth
  % Initialize \skvtry@pathlist; see the definition of the keys of
  % \skvtrysetkeys above.
  \def\skvtry@pathlist{}%
  \skvsetkeys[SKV]{skvtryset}{#1}%
  \ifx\skvtry@pathlist\@empty
    \skv@err{No families in which to 'try' to set keys}\skv@ehd
  \fi
  % To avoid repeated computation of \skv@currentnames in \skv@setkeys@a
  % for each key in the next loop:
  \skv@getnamesofkeys{#2}\skv@currentnames
  \expandafter\def\skvtry@knownkeyslistmacro{}%
  \expandafter\def\skvtry@unknownkeyslistmacro{}%
  \skvemptify{\skv@tempknownkeys,\skv@tempunknownkeys,\skv@triedlist}%
  \skv@intrytrue
  \skvcommaparse{#2}\CurrentOption{%
    \expandafter\skv@g@tkeyname\CurrentOption=\skv@getname@nil\skvcurrentkey
    \skvifemptyTF\skvtry@igkeys{%
      \@firstofone
    }{%
      \skvxifinTF{,\skvcurrentkey,}{,\skvtry@igkeys,}{}%
    }{%
      % \skv@triedlist saves non-ignored list:
      \edef\skv@triedlist{\skvaddlist,\skv@triedlist\skvcurrentkey}%
      \skvpushfunctions\skv@trysetkeys@istate{%
        \do\CurrentOption\do\skvcurrentkey\do\skv@attempts
        \do\skv@hits\do\skv@failedattempts\do\ifskv@success\do\skvtry@pathdo
      }\skv@trysetkeysidepth
      \skv@successfalse
      \skvinizero{\skv@attempts,\skv@hits,\skv@failedattempts}%
      \def\skvtry@pathdo##1##2{%
        \edef\skv@fams{##2}%
        \skv@makeprefix{##1}%
        % \ifskv@st is 'false' because we always save unknown keys while
        % in .try; and the branch for \ifskv@st is never taken when
        % in .try (see \skv@setkeys@d).
        \skv@stfalse\skv@plfalse\skv@viarootofsetkeysfalse
        \skvexpbracenext{\skv@setkeys@a[]}\CurrentOption
        \edef\skv@attempts{\the\numexpr\skv@attempts+1}%
        \ifskv@success
          \edef\skv@hits{\the\numexpr\skv@hits+1}%
          \edef\skv@tempknownkeys{%
            \skvaddlist,\skv@tempknownkeys\skvcurrenttriple
          }%
        \else
          % \skv@failedattempts is currently unused.
          \edef\skv@failedattempts{\the\numexpr\skv@failedattempts+1}%
          \edef\skv@tempunknownkeys{%
            \skvaddlist,\skv@tempunknownkeys\skvcurrenttriple
          }%
          \expandafter\expandafter\expandafter\skvtry@pathexception
        \fi
        \ifnum\skv@hits<\skvtry@maxsuccess\relax
          \ifnum\skv@attempts<\skvtry@maxattempts\relax\else
            \let\skvtry@pathdo\@gobbletwo
          \fi
        \else
          \let\skvtry@pathdo\@gobbletwo
        \fi
      }%
      \skvtry@pathlist
      \ifnum\skv@hits<\skvtry@minsuccess\relax
        \ifx\skv@triedlist\@empty
          \skv@err{Empty try list; all keys were probably ignored}\skv@ehd
        \else
          \ifx\skvtry@hitsexception\@empty
            \skv@err{Success target '\skvtry@minsuccess' wasn't reached
              \MessageBreak for key '\skvcurrentkey' by
              \ifskv@insa'.search also set'\else
              '.try set keys' or \noexpand\skvtrysetkeys\fi.
              \MessageBreak Actual hits were '\skv@hits'}\skv@ehd
          \else
            \expandafter\expandafter\expandafter\expandafter\expandafter
            \expandafter\expandafter\skvtry@hitsexception
          \fi
        \fi
      \fi
      \skvpopfunctions\skv@trysetkeys@istate\skv@trysetkeysidepth
    }%
  }%
  \ifx\skv@triedlist\@empty
    \skv@warn{Empty try list in '.try set keys';
      \MessageBreak all keys were probably ignored}\skv@ehd
  \fi
  \expandafter\let\skvtry@knownkeyslistmacro\skv@tempknownkeys
  \expandafter\let\skvtry@unknownkeyslistmacro\skv@tempunknownkeys
  \ifnum\skv@trysetkeysdepth=\@ne
    \skv@intryfalse\skv@insafalse
    \let\do\skvundef
    \do\skv@triedlist\do\skv@attempts\do\skv@hits\do\skv@failedattempts
    \do\skv@tempknownkeys\do\skv@tempunknownkeys
  \fi
  \skvpopfunctions\skvtrysetkeys\skv@trysetkeysdepth
}
% In \directkeys, \dirkeys@trysetkeys will be called instead of \skvtrysetkeys:
\skvrobustdef*\dirkeys@trysetkeys#1{%
  \begingroup
  \@tempcnta\skvz@
  \def\skv@tempc{}\def\skv@tempd{}%
  % Prepare to preserve outer brace in key value:
  \def\skv@tempa##1={%
    \begingroup
    \let\bgroup\relax
    \@ifnextchar\skv@orig@bgroup{%
      \endgroup\@tempswatrue\skv@tempb##1=%
    }{%
      \endgroup\@tempswafalse\skv@tempb##1=%
    }%
  }%
  % Because of the need to preserve outer braces in key values, don't
  % use \skv@kvsplit here.
  \def\skv@tempb##1=##2=##3\skv@nil{%
    \skvxifinTF{,##1,}{,.key values,.kv,.kv list,}{%
      \advance\@tempcnta\@ne
      \skvifnumTF\@tempcnta>\@ne{%
        \skv@err{Multiple entries for key
          \MessageBreak '.key values' or '.kv' or '.kv list'}\skv@ehd
      }{%
        \edef\skv@tempd{\skvifstrcmpTF{##2}{^skv^}{}{\unexpanded{##2}}}%
      }%
    }{%
      \edef\skv@tempc{%
        \skvaddlist,\skv@tempc##1%
        \skvifstrcmpTF{##2}{^skv^}{}{%
          =\if@tempswa{\fi\unexpanded{##2}\if@tempswa}\fi
        }%
      }%
    }%
  }%
  \skvkvparse{#1}\skv@prova{%
    \expandafter\skv@tempa\skv@prova=^skv^=\skv@nil
  }%
  \ifx\skv@tempd\@empty
    \skv@err{No key-value pairs for handler '.try set keys'}\skv@ehd
  \fi
  \skvexpanded{\endgroup
    \noexpand\skv@trysetkeys[\skvexpandonce\skv@tempc]%
      {\skvexpandonce\skv@tempd}%
  }%
}

%%+++++++++++++++++++++++++ 'search also' set keys +++++++++++++++++++%%
%
% \skvsasetkeys[<options>]{<keyvals>}
% .sa set keys={<options>}
%
% When using '.sa set keys', the key '.key values' must be part of
% <options>.
%
% 1. The only difference between \skvsasetkeys and \skvtrysetkeys is that,
%    when in \directkeys, the values of the option 'paths' of \skvsasetkeys
%    are added to the current active paths from the lists
%    \dirkeys@pathlist. Outside of \directkeys, the commands
%    \skvsasetkeys and \skvtrysetkeys are the same.
%
% 2. All the options of \skvtrysetkeys apply to \skvsasetkeys.

\skvnewlet\skvsasetkeys\skvtrysetkeys
\skvrobustdef*\dirkeys@sasetkeys#1{%
  \skv@insatrue
  \dirkeys@trysetkeys{#1}%
}
% \dirkeys@addpaths{<paths>}
% Elements of <path> will have the form '{<pref>}/{<fam>}'
\skvrobustdef*\dirkeys@addpaths#1{%
  \skv@formatpaths{#1}\dirkeys@pathlist
}
% \dirkeys@removepaths{<list>}
\skvrobustdef*\dirkeys@removepaths#1{%
  \begingroup
  \edef\skv@tempa{\unexpanded{#1}}%
  \skvcsvnormalize[,]\skv@tempa
  \skvcsvnormalize[/]\skv@tempa
  \def\skv@tempb{}%
  \def\skv@pathdo##1##2{%
    \skvxifinTF{,\detokenize{##1/##2},}{,\skvoxdetok\skv@tempa,}{}{%
      \edef\skv@tempb{%
        \skvexpandonce\skv@tempb
        \noexpand\skv@pathdo{##1}{##2}%
      }%
    }%
  }%
  \dirkeys@pathlist
  \let\dirkeys@pathlist\skv@tempb
  \skvaftergroupdef\dirkeys@pathlist\endgroup
}
% \dirkeys@removefams{<list>}
\skvrobustdef*\dirkeys@removefams#1{%
  \begingroup
  \edef\skv@tempa{\unexpanded{#1}}%
  \skvcsvnormalize\skv@tempa
  \def\skv@tempb{}%
  \def\skv@pathdo##1##2{%
    \skvxifinTF{,\detokenize{##2},}{,\skvoxdetok\skv@tempa,}{}{%
      \edef\skv@tempb{%
        \skvexpandonce\skv@tempb
        \noexpand\skv@pathdo{##1}{##2}%
      }%
    }%
  }%
  \dirkeys@pathlist
  \let\dirkeys@pathlist\skv@tempb
  \skvaftergroupdef\dirkeys@pathlist\endgroup
}
% \dirkeys@collectpaths{<pref.macro>}{<fam.macro>}{<ig.macro>}
% Collect current prefixes in <pref.macro>, families in <fam.macro> and
% ignored keys in <ig.macro>.
\skvrobustdef*\dirkeys@collectpaths#1#2#3{%
  \begingroup
  \skvemptify{#1,#2,#3}%
  \def\skv@pathdo##1##2{%
    \skvxifinTF{,##1,}{,#1,}{}{\edef#1{\skvaddlist,#1##1}}%
    \skvxifinTF{,##2,}{,#2,}{}{\edef#2{\skvaddlist,#2##2}}%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \edef#3{\skvaddlist,#3\skv@igkeys}%
  }%
  \dirkeys@pathlist
  \let\do\skvcmdexit
  \skvexpanded{\endgroup\do#1\do#2\do#3}%
}
% Remove leading and trailing slashes in #1.
\skvrobustdef*\skv@trimslashes#1{%
  \begingroup
  \def\skv@tempa{%
    \skvxifinFT{\skvrelax/}{\skvrelax#1}{}{%
      \def\do/##1\skv@nil{\def#1{##1}}%
      \expandafter\do#1\skv@nil
      \skv@tempa
    }%
  }%
  \skv@tempa
  \def\skv@tempa{%
    \skvxifinFT{/\skvrelax}{#1\skvrelax}{}{%
      \def\do##1/\skv@nil{\def#1{##1}}%
      \expandafter\do#1\skv@nil
      \skv@tempa
    }%
  }%
  \skv@tempa
  \skvaftergroupdef#1\endgroup
}

% \dirkeys@addtocodeorvalue{app.or.pre}{cbk.or.value}{<list>}
% <list> has the form <key1>={<value1>},...,<key-n>={<value-n>}
\skvrobustdef*\dirkeys@addtocodeorvalue#1#2#3{%
  \begingroup
  % Hid the list from the parameters of \skv@pathdo:
  \edef\skv@tempa{\unexpanded{#3}}%
  \def\skv@tempb{}%
  % ##1=prefix, ##2=family
  \def\skv@pathdo##1##2{%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvkvparse*\skv@tempa\skv@tempa{%
      \skv@okvsplit\skv@tempa{%
        \skvxifinTF{,\detokenize{####1},}{,\skvoxdetok\skv@igkeys,}{}{%
          \skvletcs\skv@prova{##1/##2/####1.@#2}%
          \skvifdefFT\skv@prova{%
            \skv@err{Key '####1' isn't in family
              \MessageBreak '##1/##2'}\skv@ehd
          }{%
            \skvcsedef{##1/##2/####1.@#2}{%
              \skvifstrcmpTF{#1}{pre}{%
                \skvtrimspace{####2}\skvexpandonce\skv@prova
              }{%
                \skvexpandonce\skv@prova\skvtrimspace{####2}%
              }%
            }%
            % To take the new macros outside the group:
            \edef\skv@tempb{%
              \skvexpandonce\skv@tempb
              \noexpand\skvcsexit{##1/##2/####1.@#2}%
            }%
          }%
        }%
      }%
    }%
  }%
  \dirkeys@pathlist
  \skvexpanded{\endgroup\skv@tempb}%
}

% \dirkeys@assigndefault{<kvlist>}
\skvrobustdef*\dirkeys@assigndefault#1{%
  \begingroup
  % Hid the list from the parameters of \do:
  \edef\skv@tempa{\unexpanded{#1}}%
  \def\skv@tempb{}%
  % ##1=prefix, ##2=family
  \def\skv@pathdo##1##2{%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvkvparse*\skv@tempa\skv@tempa{%
      \expandafter\skv@kvsplit\expandafter{\skv@tempa}{%
        \skvxifinTF{,\detokenize{####1},}{,\skvoxdetok\skv@igkeys,}{}{%
          \skvifcsdefTF{##1/##2/####1.@cbk}{%
            \skvcsedef{##1/##2/####1.@defa}{%
              \skvnoexpandcs{##1/##2/####1}{\skvtrimspace{####2}}%
            }%
            % To take the new defaults outside the group:
            \edef\skv@tempb{%
              \skvexpandonce\skv@tempb
              \noexpand\skvcsexit{##1/##2/####1.@defa}%
            }%
          }{%
            \skv@err{Key '####1' is not in family '##1/##2'}\skv@ehd
          }%
        }%
      }%
    }%
  }%
  \dirkeys@pathlist
  \skvexpanded{\endgroup\skv@tempb}%
}

% \dirkeys@assignvalue{<kvlist>}
\skvrobustdef*\dirkeys@assignvalue#1{%
  \begingroup
  % Hid the list from the parameters of \do:
  \edef\skv@tempa{\unexpanded{#1}}%
  \def\skv@tempb{}%
  % ##1=prefix, ##2=family
  \def\skv@pathdo##1##2{%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvkvparse*\skv@tempa\skv@tempa{%
      \expandafter\skv@kvsplit\expandafter{\skv@tempa}{%
        \skvxifinTF{,\detokenize{####1},}{,\skvoxdetok\skv@igkeys,}{}{%
          \skvifcsdefTF{##1/##2/####1.@cbk}{%
            \skvcsedef{##1/##2/####1.@value}{\skvtrimspace{####2}}%
            \edef\skv@tempb{%
              \skvexpandonce\skv@tempb
              \noexpand\skvcsexit{##1/##2/####1.@value}%
            }%
          }{%
            \skv@err{Key '####1' isn't in family '##1/##2'}\skv@ehd
          }%
        }%
      }%
    }%
  }%
  \dirkeys@pathlist
  \skvexpanded{\endgroup\skv@tempb}%
}

% \dirkeys@inheritproperty{value.or.cbk.or.defa}{<list>}
\skvrobustdef*\dirkeys@inheritproperty#1#2{%
  \begingroup
  \def\skv@tempb{}%
  % Hid the list from the parameters of \do:
  \edef\skv@tempa{\unexpanded{#2}}%
  % ##1=prefix, ##2=family
  \def\skv@pathdo##1##2{%
    \skvletcs\skv@igkeys{##1/##2/.@ignoredkeys}%
    \skvifdefTF\skv@igkeys{}{\def\skv@igkeys{}}%
    \skvkvparse*\skv@tempa\skv@tempa{%
      \skv@oslashsplit\skv@tempa{%
        % \skv@oslashsplit may return ^skv^ for ####1 or ####2, but
        % this doesn't matter here, since they will show that the keys
        % aren't defined.
        \skvxifinTF{,\detokenize{####1},}{,\skvoxdetok\skv@igkeys,}{}{%
          \ifcase\skvifcsdefTF{##1/##2/####1.@cbk}{0}{1}%
            \skvifcsdefTF{##1/##2/####2.@cbk}{0}{1}\relax
            \edef\skv@tempb{%
              \skvexpandonce\skv@tempb
              \skvcsletcs{##1/##2/####1.@#1}{##1/##2/####2.@#1}%
            }%
          \else
            \skv@err{Key '####1' or '####2' isn't in family '##1/##2'}\skv@ehd
          \fi
        }%
      }%
    }%
  }%
  \dirkeys@pathlist
  \expandafter\endgroup\skv@tempb
}

% \dirkeys@setbooleanhandler{<handler>}{<boolean>}{<bool.value>}
\skvrobustdef*\dirkeys@setbooleanhandler#1#2#3{%
  \skvifcsdefTF{if#2}{%
    \skvifblankTF{#3}{%
      \csname#2true\endcsname
    }{%
      \skvifboolvalTF{#3}{%
        \csname#2#3\endcsname
      }{%
        \skv@err{Invalid value '\detokenize{#3}' for handler '#1':
          \MessageBreak its expects either 'true' or 'false'}\skv@ehd
      }%
    }%
  }{%
    \skv@err{No boolean '\detokenize{#2}'}\skv@ehd
  }%
}

\skvrobustdef*\skv@ensurehandlerdot#1{%
  \if.\skv@car@detok#1x\car@nil\else
    \skv@err{A dot (.) must lead handler name '#1'}\skv@ehd
  \fi
}
\skvrobustdef*\dirkeys@handlerloop#1{%
  \edef\skv@tempa{\unexpanded{#1}}%
  \skvstripouterbraces{2}\skv@tempa
  \skvkvparse*\skv@tempa
}
\skvnewdef*\dirkeys@reservedhandlers{}
\skvrobustdef*\skv@reservedhandlererr{%
  \skv@err{Handler '##1' is reserved.
    \MessageBreak Reserved handlers can't be redefined whatsoever}\skv@ehd
}
\skvrobustdef*\dirkeys@defhandlers@aux#1{%
  \skvxifinTF{,#1,}{,\dirkeys@reservedhandlers,}{%
    \skv@reservedhandlererr
  }{%
    \ifskv@inreservedhandler
      \edef\dirkeys@reservedhandlers{%
        \dirkeys@reservedhandlers
        \ifx\dirkeys@reservedhandlers\@empty\else,\fi#1%
      }%
    \fi
    \edef\skv@collection{%
      \skvexpandonce\skv@collection
      \protected\skvcsdef{dirkeys@handler@#1}\skvxonce\skv@param{%
        % We can call \skvcurrenthandler in \skv@body, but when the
        % handler is cast into another handler, the inheriting handler
        % will not be the one in \skvcurrenthandler.
        \def\noexpand\skvcurrenthandler{#1}%
        \skvexpandonce\skv@body
      }%
    }%
  }%
}
% \dirkeys@defhandlers{<flag>}{<kvlist>}
%
% <flag> indicates if we're in <new> (01) or <define> (00) handler.
%
% <kvlist> -> {<handlers-1>}={<defn>},...,{<handlers-n>}={<defn>}
%
\skvrobustdef*\dirkeys@defhandlers#1#2{%
  \begingroup
  \def\skv@collection{}%
  \def\skv@param{####1\skvhandlereov}%
  \def\skv@defhandlers@do##1{%
    \skv@ensurehandlerdot{##1}%
    \skvifknobTF{#1}{%
      \dirkeys@defhandlers@aux{##1}%
    }{%
      \skvifcsdefTF{dirkeys@handler@##1}{%
        \skv@err{Handler '##1' arealdy exists}\skv@ehd
      }{%
        \dirkeys@defhandlers@aux{##1}%
      }%
    }%
  }%
  \dirkeys@handlerloop{#2}\skv@prova{%
    \skv@okvsplit\skv@prova{%
      % Hide the parameter characters in body:
      \edef\skv@prova{\unexpanded{##1}}%
      \skvstripouterbraces{2}\skv@prova
      \edef\skv@body{\unexpanded{##2}}%
      \skvcommaparse*\skv@prova\skv@prova{%
        \expandafter\skv@defhandlers@do\expandafter{\skv@prova}%
      }%
    }%
  }%
  \skvexpanded{\endgroup
    \skvexpandonce\skv@collection
    \skvcmdexit\dirkeys@reservedhandlers
  }%
}
\skvnewlet\dirkeysdefhandlers\dirkeys@defhandlers
% \dirkeys@defnarghandlers{<flag>}{<list>}
%
% Define handlers of more than one argument. This is slightly more
% expensive than '.new handlers':
%
% <flag> indicates whether we're in <new> (01) or <define> (00) handler.
%
\skvrobustdef*\dirkeys@defnarghandlers#1#2{%
  \begingroup
  \def\skv@collection{}%
  \def\skv@defhandlers@do##1{%
    \skv@ensurehandlerdot{##1}%
    \def\skv@prova####1####2\handler@nil{%
      \edef\skv@param{\skvgenerateparameters{1}{####1}\skvhandlereov}%
      \edef\skv@body{\unexpanded{####2}}%
      \skvifknobTF{#1}{%
        \dirkeys@defhandlers@aux{##1}%
      }{%
        \skvifcsdefTF{dirkeys@handler@##1}{%
          \skv@err{Handler '##1' arealdy exists}\skv@ehd
        }{%
          \dirkeys@defhandlers@aux{##1}%
        }%
      }%
    }%
    \expandafter\skv@prova\skv@provb\handler@nil
  }%
  \dirkeys@handlerloop{#2}\skv@prova{%
    \skv@okvsplit\skv@prova{%
      \edef\skv@prova{\unexpanded{##1}}%
      \skvstripouterbraces{2}\skv@prova
      % Here \skv@body is in \skv@defhandlers@do.
      \edef\skv@provb{\unexpanded{##2}}%
      \skvcommaparse*\skv@prova\skv@prova{%
        \expandafter\skv@defhandlers@do\expandafter{\skv@prova}%
      }%
    }%
  }%
  \skvexpanded{\endgroup
    \skvexpandonce\skv@collection
    \skvcmdexit\dirkeys@reservedhandlers
  }%
}
\skvnewlet\dirkeysdefnarghandlers\dirkeys@defnarghandlers

% \dirkeys@handlerlet{<flag>}{<kvlist>}
%
% 1. <flag> is either 00 (for define) or 01 (for new handler).
% 2. <kvlist> has the form
%
%       {<child handler list>}={<parent handler>}
%
\skvrobustdef*\dirkeys@handlerlet#1#2{%
  \begingroup
  \def\skv@collection{}%
  \def\skv@handlerlet@do##1##2{%
    \skvifblankTF{##1}{}{%
      \skvxifinTF{,##1,}{,\dirkeys@reservedhandlers,}{%
        \skv@reservedhandlererr
      }{%
        \ifskv@inreservedhandler
          \edef\dirkeys@reservedhandlers{%
            \dirkeys@reservedhandlers
            \ifx\dirkeys@reservedhandlers\@empty\else,\fi##1%
          }%
        \fi
        \skvifknobTF{#1}{}{%
          \skvifnamedefFT{dirkeys@handler@##1}{}{%
            \skv@err{Handler '##1' arealdy exists}\skv@ehd
          }%
        }%
        \edef\skv@collection{%
          \skvexpandonce\skv@collection
          \skvcsletcs{dirkeys@handler@##1}{dirkeys@handler@##2}%
        }%
      }%
    }%
  }%
  \dirkeys@handlerloop{#2}\skv@tempa{%
    \skv@okvsplit\skv@tempa{%
      \skvifnamedefTF{dirkeys@handler@##2}{%
        \skvcommaparse{##1}\skv@prova{%
          \skvexpbracenext\skv@handlerlet@do\skv@prova{##2}%
        }%
      }{%
        \skv@err{Handler '##2' doesn't exist}\skv@ehd
      }%
    }%
  }%
  \expandafter\endgroup\skv@collection
}
\skvrobustdef*\skvusehandler#1#2{%
  \skv@ensurehandlerdot{#1}%
  \skvifnamedefTF{dirkeys@handler@#1}{%
    \csname dirkeys@handler@#1\endcsname#2\skvhandlereov
  }{%
    \skv@err{Handler '#1' is undefined}\skv@ehd
  }%
}

% The macro that contains the default command in which unknown keys
% will be saved by some handlers of \directkeys:
\skvnewdef*\dirkeys@unknownkeysmacro{\skvfaillist}

% Notes:
% 1.  '.new reserved handlers' must be defined outsied \directkeys,
%     since we have used it here to defines every other handler.
% 2.  It defines definable handlers of one or more arguments. See also
%     '.define handlers' later on (within the next call of \directkeys).
%
\skvrobustcsdef*{dirkeys@handler@.new reserved handlers}#1\skvhandlereov{%
  \skv@inreservedhandlertrue
  \dirkeys@defhandlers{01}{#1}%
  \skv@inreservedhandlerfalse
}
\directkeys*{%
  % Defining new handlers that can't be overloaded:
  .new reserved handlers={
    % '.new reserved handlers' and '.define reserved handlers' are the
    % same thing since reserved handlers can't be overridden or overloaded.
    {.new reserved handler,.define reserved handlers,
      .define reserved handler}={
      \skvusehandler{.new reserved handlers}{#1}
    },
    {.exec,.exec code}={#1},
    {.define handler,.define handlers}={
      \dirkeys@defhandlers{00}{#1}
    },
    {.new handler,.new handlers}={
      \dirkeys@defhandlers{01}{#1}
    },
    {.define narg handler,.define narg handlers}={
      \dirkeys@defnarghandlers{00}{#1}
    },
    {.new narg handler,.new narg handlers}={
      \dirkeys@defnarghandlers{01}{#1}
    },
    % See comment above about '.new reserved handlers':
    {.new reserved narg handler,.new reserved narg handlers,
      .define reserved narg handler,.define reserved narg handlers}={
      \skv@inreservedhandlertrue
      \dirkeys@defnarghandlers{01}{#1}
      \skv@inreservedhandlerfalse
    },
    {.reserve handlers,.reserve handler}={
      \edef\skv@prova{\unexpanded{#1}}%
      \skvstripouterbraces{2}\skv@prova
      \skvcsvnormalize\skv@prova
      \edef\dirkeys@reservedhandlers{
        \dirkeys@reservedhandlers
        \ifx\dirkeys@reservedhandlers\@empty\else,\fi\skv@prova
      }
    },
    {.kill handler,.kill handlers}={
      \dirkeys@handlerloop{#1}\skv@tempa{
        \skvifcsdefTF{dirkeys@handler@\skv@tempa}{
          \skvcsundef{dirkeys@handler@\skv@tempa}
        }{
          \skv@err{Handler '\skv@tempa' is undefined}\skv@ehd
        }
      }
    },
    .use handler=\skvusehandler{#1},
    % Allow override:
    {.handler let*,.handlers let*,.let handler*,.let handlers*,
      .force handler let}={
      \dirkeys@handlerlet{00}{#1}
    },
    % Disallow override:
    {.handler let,.handlers let,.let handler,.let handlers}={
      \dirkeys@handlerlet{01}{#1}
    },
    % Let and reserved handlers:
    {.handler let reserved,.handlers let reserved}={
      \skv@inreservedhandlertrue
      \dirkeys@handlerlet{01}{#1}
      \skv@inreservedhandlerfalse
    },
    {.paths,.path,.change path,.change paths,.cd}={
      \def\dirkeys@pathlist{}\dirkeys@addpaths{#1}
    },
    {.add path,.add paths}={
      \dirkeys@addpaths{#1}
    },
    {.ignore path,.ignore paths}={
      \dirkeys@removepaths{#1}
    },
    {.restore path,.restore paths}={
      \dirkeys@addpaths{#1}
    },
    % Prefix is used in building \dirkeys@pathlist in '.family' handler.
    % There must be only one current prefix. Use .path to submit multiple
    % prefixes and families.
    {.prefix,.change prefix}={
      \skv@ifoneprefix{#1}{
        \edef\dirkeys@pref{#1}
        \skvstripouterbraces{2}\dirkeys@pref
      }{
        \skv@err{List of prefixes isn't allowed for handler
          \MessageBreak '.prefix' in \string\directkeys. You can use
          \MessageBreak '.paths' to submit multiple prefixes and
          \MessageBreak families}\skv@ehd
      }
    },
    % Since there can be only one prefix, you couldn't ignore it.
    {.prefixes,.change prefixes,.ignore prefix,.ignore prefixes}={
      \skv@err{No handler '\skvcurrenthandler'}\skv@ehd
    },
    % See .change path for .cd:
    {.families,.family,.change family,.change families,.cf}={
      \edef\dirkeys@fams{#1}
      \skvstripouterbraces{2}\dirkeys@fams
      \def\dirkeys@pathlist{}%
      \skv@makepaths\dirkeys@pref\dirkeys@fams\dirkeys@pathlist\skv@pathdo
    },
    {.add family,.add families}={
      \edef\dirkeys@fams{#1}
      \skvstripouterbraces{2}\dirkeys@fams
      \skv@makepaths\dirkeys@pref\dirkeys@fams\dirkeys@pathlist\skv@pathdo
    },
    {.ignore family,.ignore families}={
      \dirkeys@removefams{#1}
    },
    {.restore family,.restore families}={
      \skvusehandler{.add family}{#1}
    },
    {.ignore key,.ignore keys}={
      \skv@pushpathdo
      \def\skv@pathdo##1##2{
        \expandafter\skvmergelist\csname##1/##2/.@ignoredkeys\endcsname{#1}
      }
      \dirkeys@pathlist
      \skv@poppathdo
    },
    {.restore key,.restore keys}={
      \skv@pushpathdo
      \def\skv@pathdo##1##2{
        \expandafter\skvremoveelements
          \csname##1/##2/.@ignoredkeys\endcsname{#1}
      }
      \dirkeys@pathlist
      \skv@poppathdo
    },
    {.holder prefix,.hp}={
      \def\dirkeys@holderprefixtoks{#1}
    },
    % There is no need pushing prefix or family, since they're made
    % into paths by their key callbacks.
    {.push path,.push paths}={
      \dirkeys@pushmeta{path}
    },
    {.pop path,.pop paths}={
      \dirkeys@popmeta{path}
    },
    {.push holder prefix,.push hp}={
      \dirkeys@pushmeta{hp}
    },
    {.pop holder prefix,.pop hp}={
      \dirkeys@popmeta{hp}
    },
    .save unknown keys={
      \dirkeys@setbooleanhandler
        {.save unknown keys}{dirkeys@saveunknownkeys}{#1}
    },
    .save unknown keys in={
      \skvifblankTF{#1}{%
        \skv@err{Empty value for handler '.save unknown keys in'}\skv@ehd
      }{
        \skvifescapedTF{#1}{
          \dirkeys@saveunknownkeystrue
          \def\dirkeys@unknownkeysmacro{#1}
        }{
          \skv@err{Token '\detokenize{#1}' is not escaped}\skv@ehd
        }
      }
    },
    {.define key,.define keys}={
      \dirkeys@dodefinekeys{}{#1}
    },
    {.new key,.new keys}={
      \dirkeys@dodefinekeys{*}{#1}
    },
    {.define ordinary key,.define ordinary keys,.define ord keys}={
      \dirkeys@definetypekeys{ord}{}{#1}
    },
    {.new ordinary key,.new ordinary keys,.new ord keys}={
      \dirkeys@definetypekeys{ord}{*}{#1}
    },
    {.define command key,.define command keys,.define cmd keys}={
      \dirkeys@definetypekeys{cmd}{}{#1}
    },
    {.new command key,.new command keys,.new cmd keys}={
      \dirkeys@definetypekeys{cmd}{*}{#1}
    },
    {.define boolean key,.define boolean keys,.define bool keys}={
      \dirkeys@definetypekeys{bool}{}{#1}
    },
    {.new boolean key,.new boolean keys,.new bool keys}={
      \dirkeys@definetypekeys{bool}{*}{#1}
    },
    {.define toggle key,.define toggle keys,.define tog keys}={
      \dirkeys@definetypekeys{bool}{}{#1}
    },
    {.new toggle key,.new toggle keys,.new tog keys}={
      \dirkeys@definetypekeys{bool}{*}{#1}
    },
    {.define choice key,.define choice keys}={
      \dirkeys@definetypekeys{choice}{}{#1}
    },
    {.new choice key,.new choice keys}={
      \dirkeys@definetypekeys{choice}{*}{#1}
    },
    {.initialize keys after define,.initialize after define}={
      \dirkeys@setbooleanhandler
        {.initialize keys after define}{skvdfk@initialize}{#1}
    },
    {.save initial values of keys,.save initial values}={
      \dirkeys@setbooleanhandler
        {.save initial values of keys}{skvdfk@saveinitialvalues}{#1}
    },
    {.set keys,.setkeys,.set}={
      \dirkeys@setkeys{}{}\skvsetkeys{#1}
    },
    {.set keys*,.setkeys*,.set*,.setkeys save unknown,
     .set keys save unknown}={
      \dirkeys@setkeys{*}{}\skvsetkeys{#1}
    },
    {.set rmkeys,.setrmkeys,.set remaining keys}={
      \skvifblankTF{#1}{
        \dirkeys@setkeys{}{rm}\skvsetrmkeys{}
      }{
        \skv@err{Key 'set rmkeys' can't have value:
          \MessageBreak Instead use the key 'ignore keys'
          \MessageBreak to suggest keys to be ignored
          \MessageBreak when setting 'rmkeys'}\skv@ehd
      }
    },
    {.set rmkeys*,.setrmkeys*,.set remaining keys*}={
      \skvifblankTF{#1}{
        \dirkeys@setkeys{*}{rm}\skvsetrmkeys{}
      }{
        \skv@err{Key 'set rmkeys*' can't have value:
        \MessageBreak Instead use the handler '.ignore keys' to suggest keys
        \MessageBreak to be ignored when setting rmkeys}\skv@ehd
      }
    },
    % '.try set keys' doesn't use the active prefixes and families within
    % \directkeys. The prefix, families and other options are to be supplied
    % in the argument #1. The key .key values (or .kv) is used to
    % supply the key-value pairs.
    % .try set keys={<options>}
    {.try set keys,.try set,.try}={
      \dirkeys@trysetkeys{#1}
    },
    % 'search also' set keys.
    % .sa set keys={<options>}
    {.search also set keys,.sa set keys}={
      \dirkeys@sasetkeys{#1}
    },
    {.presetkeys,.preset keys}={
      \dirkeys@dolistedkeys@a{#1}\skv@presetkeys
    },
    .gpreset keys={
      \dirkeys@dolistedkeys@a{#1}\skv@gpresetkeys
    },
    .remove preset keys={
      \dirkeys@dolistedkeys@a{#1}\skvremovepresetkeys
    },
    .gremove preset keys={
      \dirkeys@dolistedkeys@a{#1}\skvgremovepresetkeys
    },
    .undefine preset keys={
      \skv@clfalse\dirkeys@dolistedkeys@b\skv@undefpresetkeys
    },
    .gundefine preset keys={
      \skv@cltrue\dirkeys@dolistedkeys@b\skv@undefpresetkeys
    },
    {.postsetkeys,.postset keys}={
      \dirkeys@dolistedkeys@a{#1}\skv@postsetkeys
    },
    .gpostset keys={
      \dirkeys@dolistedkeys@a{#1}\skv@gpostsetkeys
    },
    .remove postset keys={
      \dirkeys@dolistedkeys@a{#1}\skvremovepostsetkeys
    },
    .gremove postset keys={
      \dirkeys@dolistedkeys@a{#1}\skvgremovepostsetkeys
    },
    .undefine postset keys={
      \skv@clfalse\dirkeys@dolistedkeys@b\skv@undefpostsetkeys
    },
    .gundefine postset keys={
      \skv@cltrue\dirkeys@dolistedkeys@b\skv@undefpresetkeys
    },
    .option keys={
      \dirkeys@dolistedkeys@a{#1}\skvoptionkeys
    },
    .goption keys={
      \dirkeys@dolistedkeys@a{#1}\skvgoptionkeys
    },
    .remove option keys={
      \dirkeys@dolistedkeys@a{#1}\skvremoveoptionkeys
    },
    .gremove option keys={
      \dirkeys@dolistedkeys@a{#1}\skvgremoveoptionkeys
    },
    .nonoption keys={
      \dirkeys@dolistedkeys@a{#1}\skvnonoptionkeys
    },
    .gnonoption keys={
      \dirkeys@dolistedkeys@a{#1}\skvgnonoptionkeys
    },
    .remove nonoption keys={
      \dirkeys@dolistedkeys@a{#1}\skvremovenonoptionkeys
    },
    .gremove nonoption keys={
      \dirkeys@dolistedkeys@a{#1}\skvgremovenonoptionkeys
    },
    .need value keys={
      \dirkeys@dolistedkeys@a{#1}\skvneedvaluekeys
    },
    .gneed value keys={
      \dirkeys@dolistedkeys@a{#1}\skvgneedvaluekeys
    },
    .remove need value keys={
      \dirkeys@dolistedkeys@a{#1}\skvremoveneedvaluekeys
    },
    .gremove need value keys={
      \dirkeys@dolistedkeys@a{#1}\skvgremoveneedvaluekeys
    },
    .forbid value keys={
      \dirkeys@dolistedkeys@a{#1}\skvforbidvaluekeys
    },
    .gforbid value keys={
      \dirkeys@dolistedkeys@a{#1}\skvgforbidvaluekeys
    },
    .remove forbid value keys={
      \dirkeys@dolistedkeys@a{#1}\skvremoveforbidvaluekeys
    },
    .gremove forbid value keys={
      \dirkeys@dolistedkeys@a{#1}\skvgremoveforbidvaluekeys
    },
    .save initial value keys={
      \dirkeys@dolistedkeys@a{#1}\skvsaveinitialvaluekeys
    },
    .gsave initial value keys={
      \dirkeys@dolistedkeys@a{#1}\skvgsaveinitialvaluekeys
    },
    .remove save initial value keys={
      \dirkeys@dolistedkeys@a{#1}\skvremovesaveinitialvaluekeys
    },
    .gremove save initial value keys={
      \dirkeys@dolistedkeys@a{#1}\skvgremovesaveinitialvaluekeys
    },
    .undefine save initial value keys={
      \dirkeys@dolistedkeys@a{#1}\skvundefsaveinitialvaluekeys
    },
    .gundefine save initial value keys={
      \dirkeys@dolistedkeys@a{#1}\skvgundefsaveinitialvaluekeys
    },
    {.disable keys,.disable key}={
      \dirkeys@dolistedkeys@a{#1}\skvdisablekeys
    },
    {.disabled key message type,.disabled key exception type}={
      \skvdisabledkeysmessagetype{#1}
    },
    % Choices are always appended; never prepended, since the parent
    % key must first be set before choices are executed.
    % <key1>/{<ch1>.do={<act1>},...,<ch-n>.do={<act-n>}},...,
    %    <key-n>/{<ch1>.do={<act1>},...,<ch-n>.do={<act-n>}}
    {.state pattern,.choice,.nominations}={
      \dirkeys@savechoice{#1}{x0}
    },
    .state pattern expand once={
      \dirkeys@savechoice{#1}{x1}
    },
    .state pattern expand twice={
      \dirkeys@savechoice{#1}{x2}
    },
    {.state pattern expanded,.estate pattern,.enominations,.echoice}={
      \dirkeys@savechoice{#1}{xx}
    },
    % {<key-i>,...,<key-j>}/{<slotlist-ij>},...,
    %    {<key-n>,...,<key-m>}/{<slotlist-nm>}:
    {.append slot,.append slots,.slot,.slots,.style,.styles,.observers}={
      \dirkeys@saveslots{#1}{app}{x0}
    },
    {.prepend slot,.prepend slots}={
      \dirkeys@saveslots{#1}{prep}{x0}
    },
    {.append slot value expanded,.append slot expanded,
      .append slots value expanded,.append slots expanded,
      .eslot,.eslots,.estyle,.estyles}={
      \dirkeys@saveslots{#1}{app}{xx}
    },
    {.prepend slot value expanded,.prepend slot expanded,
      .prepend slots value expanded,.prepend slots expanded}={
      \dirkeys@saveslots{#1}{prep}{xx}
    },
    {.append slot expand value once,.append slot expand once,
      .append slots expand value once,.append slots expand once,
      .slot expand once,.slots expand once,.style expand once,
      .styles expand once}={
      \dirkeys@saveslots{#1}{app}{x1}
    },
    {.prepend slot expand value once,.prepend slot expand once,
      .prepend slots expand value once,.prepend slots expand once}={
      \dirkeys@saveslots{#1}{prep}{x1}
    },
    {.append slot expand value twice,.append slot expand twice,
      .append slots expand value twice,.append slots expand twice,
      .slot expand twice,.slots expand twice,.style expand twice,
      .styles expand twice}={
      \dirkeys@saveslots{#1}{app}{x2}
    },
    {.prepend slot expand value twice,.prepend slot expand twice,
      .prepend slots expand value twice,.prepend slots expand twice}={
      \dirkeys@saveslots{#1}{prep}{x2}
    },
    % {<linklist-1>}/<mainkeylist-1>,...,{<linklist-n>}/<mainkeylist-n>:
    {.append link,.append links,.link,.links}={
      \dirkeys@savelinks{#1}{app}{x0}
    },
    {.prepend link,.prepend links}={
      \dirkeys@savelinks{#1}{prep}{x0}
    },
    {.append link expanded value,.append link expanded,
      .append links expanded value,.append links expanded,.elink,.elinks}={
      \dirkeys@savelinks{#1}{app}{xx}
    },
    {.prepend link expanded value,.prepend link expanded,
      .prepend links expanded value,.prepend links expanded}={
      \dirkeys@savelinks{#1}{prep}{xx}
    },
    {.append link expand value once,.append link expand once,
      .append links expand value once,.append links expand once,
      .link expand once,.links expand once}={
      \dirkeys@savelinks{#1}{app}{x1}
    },
    {.prepend link expand value once,.prepend link expand once,
      .prepend links expand value once,.prepend links expand once}={
      \dirkeys@savelinks{#1}{prep}{x1}
    },
    {.append link expand value twice,.append link expand twice,
      .append links expand value twice,.append links expand twice,
      .link expand twice,.links expand twice}={
      \dirkeys@savelinks{#1}{app}{x2}
    },
    {.prepend link expand value twice,.prepend link expand twice,
      .prepend links expand value twice,.prepend links expand twice}={
      \dirkeys@savelinks{#1}{prep}{x2}
    },
    % .store value in={key1,key2}/<cmd>:
    .store value in={
      \dirkeys@savestores{#1}{x0}
    },
    {.store expanded value in,.store evalue in}={
      \dirkeys@savestores{#1}{xx}
    },
    .store expanded once value in={
      \dirkeys@savestores{#1}{x1}
    },
    .store expanded twice value in={
      \dirkeys@savestores{#1}{x2}
    },
    {.list break,.listbreak,.break list}={
      \skvbreaklooptrue
    },
    {.arg,.args}={
      \dirkeys@assignarg{#1}{x0}
    },
    % Expand arguments of keys at key setting time, not at key definition:
    {.arg expanded,.args expanded}={
      \dirkeys@assignarg{#1}{xx}
    },
    {.arg expand once,.args expand once}={
      \dirkeys@assignarg{#1}{x1}
    },
    {.arg expand twice,.args expand twice}={
      \dirkeys@assignarg{#1}{x2}
    },
    {.use defaults,.set with defaults}={
      \dirkeys@dolistedkeys@a{#1}\dirkeys@setwithdefaults
    },
    {.unknown key handler,.unknown option handler}={
      \dirkeys@setunknownkeyhandler{#1}
    },
    % Redefine the default value macros of keys.
    % .default values={keya=vala,...,keyn=valn}
    {.default value,.default values,.default,.defaults}={
      \dirkeys@assigndefault{#1}
    },
    % Change the current values of keys.
    % .assign values={keya=vala,...,keyn=valn}
    {.assign value,.assign values}={
      \dirkeys@assignvalue{#1}
    },
    {.inherit,.keys let,.key let}={
      \dirkeys@keyslet{#1}
    },
    % A key inherits value from a key.
    % .inherit values={keya1/keya2,...,keyn1/keyn2}
    {.inherit value,.inherit values}={
      \dirkeys@inheritproperty{value}{#1}
    },
    {.inherit callback,.inherit callbacks,.inherit code}={
      \dirkeys@inheritproperty{cbk}{#1}
    },
    {.inherit default,.inherit defaults}={
      \dirkeys@inheritproperty{defa}{#1}
    },
    % .prepend values={key1=val1,...,keyn=valn}
    {.prepend value,.prepend values}={
      \dirkeys@addtocodeorvalue{pre}{value}{#1}
    },
    {.append value,.append values}={
      \dirkeys@addtocodeorvalue{app}{value}{#1}
    },
    % .prepend code={key1=code1,...,keyn=coden}
    {.prepend code,.prepend codes}={
      \dirkeys@addtocodeorvalue{pre}{cbk}{#1}
    },
    {.append code,.append codes}={
      \dirkeys@addtocodeorvalue{app}{cbk}{#1}
    },
  },
  .new narg handlers={
    % All the parameters would have been despaced when '.no such key'
    % is called. #1=prefix, #2=family, #3=key, #4=value.
    .no such key={4}{
      \skvifcsdefTF{#1@#2@handler}{
        \csname#1@#2@handler\endcsname{#1}{#2}{#3}{#4}
      }{
        \skv@err{Key '#3' is not in family '#1/#2'}\skv@ehd
      }
    },
    .add slot={2}{
      \skvusehandler{.prepend slot}{#1}
      \skvusehandler{.append slot}{#2}
    },
    .add code={2}{
      \skvusehandler{.prepend code}{#1}
      \skvusehandler{.append code}{#2}
    },
    .add value={2}{
      \skvusehandler{.prepend value}{#1}
      \skvusehandler{.append value}{#2}
    },
    % .get value={<pref>}{<fam>}{<key>}<cmd>
    .get value={4}{
      \skvifnamedefTF{#1/#2/#3.@value}{
        \skvifescapedTF{#4}{
          \skvletcs#4{#1/#2/#3.@value}
        }{
          \skv@err{Token '\detokenize{#4}' isn't escaped}\skv@ehd
        }
      }{
        \skv@err{Key '#3' isn't defined or has
          \MessageBreak no value in '#1/#2'}\skv@ehd
      }
    },
    % .set boolean handler={<handler>}{<boolean>}{<boolean.value>}
    %   See example use above.
    .set boolean handler={3}{
      \dirkeys@setbooleanhandler{#1}{#2}{#3}
    },
  },
  .handlers let reserved={
    {.disabled option message type,
      .message type when disabled key is invoked,
      .message type when disabled option is invoked
    }=.disabled key message type,
  },
}

% \skvpatchcmd[<prefix>]{<cmd>}{<search>}{<replace>}{<success>}{<fail>}
%
\skvrobustdef*\skvpatchcmd{%
  \begingroup
  \@makeother{\#}\endlinechar\m@ne
  \skv@testopt\skv@patchcmd{####1}%
}
\skvrobustdef*\skv@patchcmd[#1]#2#3#4{%
  \ifskv@tracingkeys
    \typeout{^^J** Debugging patches: command '\string#2'}%
  \fi
  \skv@p@tchcmd{#1}{#2}{#3}{#4}%
}
\skvrobustdef*\skv@p@tchcmd#1#2#3#4{%
  \skvifpatchableTF{#2}{#3}{#4}{%
    \skv@patchdebug{++}{Command is patchable}%
    \skv@patchdebug{==}{Patching has begun}%
    \begingroup
    \edef\skv@tempa##1##2{%
      \def##1####1\detokenize{macro:}####2->####3\skvrelax{%
        #1\def\string#2####2{##2####3\skvrelax}%
      }%
      \def##2####1\detokenize{#3}####2\skvrelax{####1\detokenize{#4}####2}%
      \edef##1{##1\meaning#2\skvrelax}%
    }%
    \skv@tempa\skv@tempa\skv@tempb
    \skv@scantoksd\endgroup\skv@tempa
    \skv@patchdebug{==}{Patching completed successfully}%
    \@firstoftwo
  }{%
    \skv@patchdebug{--}{Patching couldn't be completed}%
    \@secondoftwo
  }%
}
\skvrobustdef*\skv@patchdebug#1#2{%
  \ifskv@tracingkeys\typeout{[debug] #1 #2.}\fi
}
\skvrobustdef*\skvifpatchableTF#1#2#3{%
  \endgroup
  \skvifdefFT{#1}{%
    \skv@patchdebug{--}{Command not defined}%
    \@secondoftwo
  }{%
    \skv@patchdebug{++}{Command is defined}%
    \skvifmacroTF{#1}{%
      \skv@patchdebug{++}{Command is a macro}%
      \skvifscannableTF{#1}{%
        \skv@patchdebug{++}{Macro can be retokenized safely after patching}%
        \skvifpatternTF{#2}{#1}{%
          \skv@patchdebug{++}{Requested search pattern found}%
          \@firstoftwo
        }{%
          \skv@patchdebug{--}{Requested search pattern not found}%
          \@secondoftwo
        }%
      }{%
        \skv@patchdebug{--}{Nested commands or parameters}%
        \@secondoftwo
      }%
    }{%
      \skv@patchdebug{--}{Macro can't be retokenized safely after patching}%
      \@secondoftwo
    }%
  }%
}
\skvrobustdef*\skveveryscan{%
  \everyeof{\noexpand}%
  \endlinechar\m@ne
  \makeatletter
  \catcode`\ =10
  \catcode`\\=0
  \catcode`\{\@ne
  \catcode`\}\tw@
}
\skvrobustdef*\skv@scantoksd#1#2{%
  \skvexpandsecond{#1\skveveryscan\scantokens}{%
    {#2}\everyeof{\the\everyeof}%
    \noexpand\endlinechar\the\endlinechar\relax
    \catcode`\noexpand\@=\the\catcode`\@\relax
    \catcode`\noexpand\ =\the\catcode`\ \relax
    \catcode`\noexpand\\=\the\catcode`\\\relax
    \catcode`\noexpand\{=\the\catcode`\{\relax
    \catcode`\noexpand\}=\the\catcode`\}\relax
  }%
}
\skvrobustdef*\skvifscannableTF#1{%
  % Fails if the content of #1 is already detokenized.
  \begingroup
  \edef\skv@tempa##1{%
    \def##1####1\detokenize{macro}:####2->####3\skvrelax{%
      ####1\def\string\skv@tempa####2{####3}%
    }%
    \edef##1{##1\meaning#1\skvrelax}%
  }%
  \skv@tempa\skv@tempa
  \makeatletter\everyeof{\noexpand}\endlinechar\m@ne
  \scantokens\expandafter{\skv@tempa}\relax
  \expandafter\endgroup
  \ifx#1\skv@tempa
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\skvrobustdef\skvifpatternTF#1#2{%
  \begingroup
  \edef\skv@tempa##1{\def##1####1\detokenize{#1}####2\skvrelax}%
  \skv@tempa\skv@tempa{%
    \expandafter\endgroup\ifx\\##2\\%
      \expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
  \edef\skv@tempb##1{##1\detokenize{#1}\skvrelax}%
  \skv@tempb{\expandafter\skv@tempa\meaning#2}%
}
\edef\skv@begindoctoks{\string\begin\string{\string\document\string}}
\skvrobustdef*\skvAtBeginEnvironment#1{%
  \skvaftercs\skvappendtomacro{lps@atbegin@#1@hook}%
}
\skvrobustdef*\skvAtEndEnvironment#1{%
  \skvaftercs\skvappendtomacro{lps@atend@#1@hook}%
}

\skvpatchcmd\begin
  {\csname#1\endcsname}
  {\skvcsuse{lps@atbegin@#1@hook}\csname#1\endcsname}
  {}
  {\skv@err{Patching '\string\begin' failed!\MessageBreak
     '\string\skvAtBeginEnvironment' will not work\@gobble}\@ehd
  }

\skvpatchcmd\end
  {\csname end#1\endcsname}
  {\skvcsuse{lps@atend@#1@hook}\csname end#1\endcsname}
  {}
  {\skv@err{Patching '\string\end' failed!\MessageBreak
     '\string\skvAtEndEnvironment' will not work\@gobble}\@ehd
  }

\skv@core@restorecodes

\endinput

%% End of file 'skeyval-core.tex'.


==> skeyval-for.tex <==
%++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++%
% This is file 'skeyval-for.tex', version 1.3, 2013/05/15.                 %
%                                                                          %
% This package and accompanying files may be distributed and/or            %
% modified under the conditions of the LaTeX Project Public License,       %
% either version 1.3 of this license or any later version. The latest      %
% version of this license is in http://www.latex-project.org/lppl.txt      %
% and version 1.3 or later is part of all distributions of LaTeX           %
% version 2005/12/01 or later.                                             %
%                                                                          %
% The LPPL maintenance status of this software is 'author-maintained'.     %
%                                                                          %
% This software is provided 'as it is', without warranty of any kind,      %
% either expressed or implied, including, but not limited to, the          %
% implied warranties of merchantability and fitness for a particular       %
% purpose.                                                                 %
%                                                                          %
% The following files constitute the skeyval bundle and must be            %
% distributed as a whole:                                                  %
%                                                                          %
%  README, skeyval.sty, skeyval-core.tex, skeyval-for.tex,                 %
%  skeyval-view.sty, skeyval-ltxpatch.sty, skeyval-ltxcmds.tex,            %
%  skeyval-pstkey.sty, skeyval-pstkey.tex, skeyval-testclass.cls,          %
%  skeyval-testpkg.sty, skeyval-pokayoke1, skeyval-pokayoke2,              %
%  skeyval-view-pokayoke1.                                                 %
%                                                                          %
% Copyright (c) 2010-2013 Ahmed Musa (amusa22@gmail.com).                  %
%++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++%

\begingroup%
\let\e\endlinechar\edef\p{\the\e}\e13\edef\n{\the\catcode\e}%
\xdef\skv@for@restorecatcodes{%
  \let\noexpand\skv@for@restorecatcodes\relax%
  \endlinechar=\p\relax\catcode\number\e=\n\relax%
  \catcode\string`\noexpand`\string=\the\catcode\string``\relax%
  \catcode\string`\noexpand=\string=\the\catcode\string`=\relax%
}%
\endgroup%
\endlinechar\string=13\relax%
\catcode13\string=5\relax%
\catcode\string``\string=12\relax
\catcode\string`=\string=12\relax
\def\skvgobble#1{}
\def\do#1{\catcode`\expandafter\skvgobble\string#1=\the\catcode`#1\relax}
\edef\skv@for@restorecatcodes{%
  \unexpanded\expandafter{\skv@for@restorecatcodes}%
  \do\ \do\%\do\@\do\(\do\)\do\[\do\]\do\|\do\:\do\;\do\,\do\.%
  \do\>\do\<\do\!\do\*\do\+\do\-\do\^\do\_\do\&\do\$\do\~\do\'%
  \do\"\do\
}
\catcode`\ =10\relax
\catcode`\@=11 \catcode`\(=12 \catcode`\)=12 \catcode`\[=12
\catcode`\]=12 \catcode`\|=12 \catcode`\:=12 \catcode`\;=12
\catcode`\,=12 \catcode`\*=12 \catcode`\+=12 \catcode`\-=12
\catcode`\<=12 \catcode`\>=12 \catcode`\!=12 \catcode`\.=12
\catcode`\^=07 \catcode`\_=08 \catcode`\&=04 \catcode`\$=03
\catcode`\~=13 \catcode`\%=14 \catcode`\'=12 \catcode`\"=12

\csname skeyval-for-loaded\endcsname
\expandafter\let\csname skeyval-for-loaded\endcsname\endinput

\ifx\ProvidesFile\@undefined
  \message{File 'skeyval-for.tex' 2013/05/15 v1.3
    Loops for skeyval package (AM)}
\else
  \ProvidesFile{skeyval-for.tex}
    [2013/05/15 v1.3 Loops for skeyval package (AM)]
  \@addtofilelist{skeyval-for.tex}
\fi

\skvrobustdef*\skv@nostackerr{%
  \skv@err{You've called an empty stack}\skv@ehd
}
% \skvsavestate<base-fn>{<fn-list>}<counter-number>
%
% See file skeyval-core.tex for \skvpushfunctions and \skvpopfunctions.
%
\skvrobustdef*\skvsavestate#1#2#3{%
  \skvgadvanceno#3\@ne
  \begingroup
  \let\s\string\escapechar\m@ne
  \def\skv@prova##1{\s##1@skv@\romannumeral#3}%
  \def\do##1{\let\noexpand##1\skvnoexpandcs{\skv@prova{##1}}}%
  \skvifcsdefTF{\s#1@skv@stack}{}{\skvcsdef{\s#1@skv@stack}{\nostack}}%
  \skvcsxdef{\s#1@skv@stack}{#2{\skvexpandcsonce{\s#1@skv@stack}}}%
  \def\do##1{\let\skvnoexpandcs{\skv@prova{##1}}\noexpand##1}%
  \edef\reserved@a{\endgroup#2}\reserved@a
}
% \skvrestorestate<base-fn><counter-number>
\skvrobustdef*\skvrestorestate#1#2{%
  \begingroup
  \let\nostack\skv@nostackerr
  \edef\skv@elt{\skvnoexpandcs{\skvremovescape#1@skv@stack}}%
  \expandafter\ifx\skv@elt\relax
    \skv@err{Stack of '\noexpand#1' is undefined}\skv@ehd
  \fi
  \edef\skv@prova{\skvexpandtwice\skv@elt}%
  \edef\skv@provb##1##{\endgroup##1\gdef\skvexpandonce\skv@elt}%
  \expandafter\skv@provb\skv@prova
  \skvgadvanceno#2\m@ne
}
\skvnewregisters\bool{%
  \ifbreakallforeachloops,\ifskvbreakloop,\ifforeachlastitem,
  \ifskvprocessempty,\ifskv@foreach@swa,\ifskv@foreach@swb,
  \ifskv@foreach@parenthesis,\ifskv@useemptylist,\ifskv@inforeach,
}
\skvnewlet\skvbreakloop\skvbreaklooptrue
\skvnewlet\breaknewforeach\skvbreaklooptrue
% \breakallforeachloops will break all current loops (inner and outer):
\skvnewdef*\breakallforeachloops{%
  \skvbreaklooptrue\breakallforeachloopstrue
}

\skvnewnumbers[skv@]{csvdepth,dolistdepth}
%
% \skvdolist{<parser>}{<list>}<holdercmd>{<callback>}
% \skvdolist*{<parser>}{<listcmd>}<holdercmd>{<callback>}
% \skvparselist{<parser>}{<list>}<holdercmd>{<callback>}
% \skvparselist*{<parser>}{<listcmd>}<holdercmd>{<callback>}
% \skvprocesslist{<parser>}{<list>}<holdercmd>{<callback>}
% \skvprocesslist*{<parser>}{<listcmd>}<holdercmd>{<callback>}
%
% 1. These macros can process both csv and tsv/nsv lists. Use empty
%    <parser> for tsv lists.
% 2. These macros can be nested to any depth, with different parsers
%    on each level.
% 3. \skvdolist and \skvparselist will not process an empty list, but
%    \skvprocesslist will do so.
% 4. For comma lists, \skvcommaloop and \skvcommaparse are faster.
%    See later.
% 5. For processing kv lists, use \skvparsekvlist.
% 6. The preservation of outer braces isn't a priority in this loop.
%
\skvrobustdef*\skvdolist{\skv@useemptylistfalse\skv@testst\skv@dolist}
\skvrobustdef*\skv@dolist#1#2#3#4{%
  \skv@usetempst{#2}#3%
  % \skvlistcount is used by listkeys.
  \skvsavestate\skvdolist{%
    \do\skv@dolist@callback
    \do\skv@dolist@a\do\skvlistcount\do\ifskv@useemptylist
  }\skv@dolistdepth
  \edef\skv@dolist@callback{\unexpanded{#4}}%
  \def\skvlistcount{0}%
  \def\skv@dolist@a##1##2#1{%
    \skvifstrcmpTF{##2}{\skv@dolist@nil}{%
      % To allow nesting of loop:
      \skvbreakloopfalse
    }{%
      \edef##1{\unexpanded{##2}}%
      \edef\skvlistcount{\the\numexpr\skvlistcount+1}%
      \skv@dolist@callback\relax
      \ifskvbreakloop
        \skvbreakloopfalse
        \begingroup
        \def\skv@dolist@a####1####2\skv@dolist@nil#1{%
          \endgroup
          \edef\skvremainder{\unexpanded{####2}}%
        }%
      \fi
      \skv@dolist@a{##1}%
    }%
  }%
  \ifskv@useemptylist
    \def\reserved@a##1##2##3{##3}%
  \else
    \let\reserved@a\skvifemptyTF
  \fi
  \reserved@a#3{}{%
    \expandafter\skv@dolist@a\expandafter#3#3#1\skv@dolist@nil#1%
  }%
  \skvrestorestate\skvdolist\skv@dolistdepth
}
% First normalize the list before parsing.
\skvrobustdef*\skvparselist{\skv@useemptylistfalse\skv@testst\skv@parselist}
\skvrobustdef*\skvprocesslist{\skv@useemptylisttrue\skv@testst\skv@parselist}
\skvrobustdef*\skv@parselist#1#2#3{%
  \skv@usetempst{#2}#3%
  \skvcsvnormalize[#1]#3%
  \skv@tempsttrue
  \skv@dolist{#1}#3#3%
}

\skvnewlet\foreachlistbreaker\relax
\skvnewlet\foreachlistpauser\relax
\skvnewdef*\skv@listbreakertoks{\foreachlistbreaker}
\skvnewdef*\skv@listpausertoks{\foreachlistpauser}
\skvnewlet\skvprocessempty\skvprocessemptytrue

% Reversing tokens:
\skvnewdef*\skvreverse#1{\skv@reverse#1\skv@reverse@stop}
\skvnewdef*\skv@reverse#1#2\skv@reverse@stop{%
  \if\relax\detokenize{#2}\relax\skv@reverse@stop\fi
  \skv@reverse#2\skv@reverse@stop\skvreversedo{#1}%
}
\skvnewdef*\skv@reverse@stop#1\skv@reverse@stop{\fi}
\let\skvreversedo\@iden

\skvrobustdef*\skv@removetrailingparser#1#2{%
  \skvxifinTF{\detokenize{#1}\relax}{\skvoxdetok#2\relax}{%
    \def\skv@prova##1#1\skv@trim@nil{\unexpanded{##1}}%
    \edef#2{\expandafter\skv@prova#2\skv@trim@nil}%
  }{}%
}

% \skvrecurse<body>\while<\if...>\fi
%
% On entry, the condition is checked before the body is executed.
%
% \@tempcnta\z@
% \skvrecurse{
%   \advance\@tempcnta\@ne
%   \@tempcntb\z@
%   \skvrecurse
%     \advance\@tempcntb\@ne
%     \typeout{Doing \the\@tempcnta,\the\@tempcntb}
%   \while
%     \ifnum\@tempcntb<3
%   \fi
%  }
% \while
%   \ifnum\@tempcnta<4
% \fi
%
\skvnewcounts{skv@recurse@cnt}
\skvrobustdef\skvrecurse#1\while#2\fi{%
  \skv@recurse@cnt\skvz@
  \@expandtwoargs\skv@dobody{\skvtrimspace{#2}}{\skvtrimspace{#1}}%
}
\skvrobustdef\skv@dobody#1#2{%
  \advance\skv@recurse@cnt\@ne
  \ifnum\skv@recurse@cnt>10000\relax
    \@latex@error{Possibly an infinite loop in \string\skvrecurse}
      {Maybe you didn't increment some counter or
        \MessageBreak the termination condition was never satisfied.}%
  \fi
  #1\relax\expandafter\@iden\else\expandafter\@gobble\fi
  {#2\relax\skv@dobody{#1}{#2}}%
}

% A version of LaTeX's \@tfor that can parse undoubled parameter
% characters and terminate the loop by using \skvbreakloop.
%
% \skvtfor<holder.cmd>:={<list>}\do{<callback>}
% \skvtfor*<holder.cmd>:={<listcmd>}\do{<callback>}
%
% Example:
%
%  \skvnewregister\count{\nr}
%  \skvtfor\x:=a \ifx {\def\x#1{#1}} \fi\do{%
%    \nr\z@
%    \skvtfor\y:=12345\do{%
%      \typeout{Doing: \detokenize\expandafter{\x}--\y}%
%      \advance\nr\@ne
%      \ifnum\nr>\tw@\skvbreakloop\fi
%    }
%  }
%
\skvnewdef*\skv@tfor@nil{\skv@tfor@nil}
\skvrobustdef*\skvtfor{\skv@testst\skv@tfor}
\skvrobustdef*\skv@tfor#1:={\skv@tf@r#1 }
\skvrobustdef\skv@tf@r#1#2\do#3{%
  \edef#1{\skvtrimspace{#2}}%
  \edef#1{\skvifdefboolTF{skv@tempst}\skvexpandtwice\skvexpandonce{#1}}%
  \skvifemptyTF#1{}{%
    \skvbreakloopfalse
    \expandafter\skv@tforloop#1\skv@tfor@nil\skv@tfor#1{#3}%
  }%
}
\skvrobustdef\skv@tforloop#1#2\skv@tfor#3#4{%
  \edef#3{\unexpanded{#1}}%
  \skvifxTF#3\skv@tfor@nil{%
    \skvbreakloopfalse
  }{%
    #4\relax
    \ifskvbreakloop
      \skvbreakloopfalse
      \begingroup
      \def\skv@tforloop##1\skv@tfor@nil\skv@tfor##2##3{%
        \endgroup
        \edef\skvremainder{\unexpanded{##1}}%
      }%
    \fi
    \skv@tforloop#2\skv@tfor#3{#4}%
  }%
}

%+++++++++++++++      Non-expandable comma loops       ++++++++++++++%%
%
% 1. These follow from \skvdolist and \skvparselist, but they are
%    specialized for comma lists and they are faster, since they don't
%    stack any state.
% 2. There is no fear of parameter characters in <callback> being mixed
%    with those of \skv@commaloop@picknext.
% 3. These loops can be nested to any depth.
% 4. The preservation of outer braces isn't a priority in these loops.
%
% \skvcommaloop{<list>}<holder-cmd>{<callback>}
% \skvcommaloop*{<listcmd>}<holder-cmd>{<callback>}
%
% Example:
%
%   \skvcommaloop{x#1,y#1}\tempa{\edef\xx#1{#1\tempa}}
%
\skvrobustdef*\skvcommaloop{\skv@testst\skv@commaloop}
\skvrobustdef\skv@commaloop#1#2#3{%
  \skv@usetempst{#1}#2%
  % Don't put \skvcsvnormalize#2 here. Use \skvcommaparse instead.
  % Some callers of \skvcommaloop already have their lists normalized.
  \skvifxTF#2\@empty{}{%
    \skvbreakloopfalse
    \skvexpandnext{\skv@commaloop@picknext#2{#3}}#2,\skv@commaloop@nil,%
  }%
}
\skvrobustdef\skv@commaloop@picknext#1#2#3,{%
  \skvifstrcmpTF{#3}{\skv@commaloop@nil}{%
    \skvbreakloopfalse
  }{%
    \edef#1{\unexpanded{#3}}%
    #2\relax
    \ifskvbreakloop
      \skvbreakloopfalse
      \begingroup
      \long\def\skv@commaloop@picknext##1##2##3\skv@commaloop@nil,{%
        \endgroup
        \edef\skvremainder{\unexpanded{##3}}%
      }%
    \fi
    \skv@commaloop@picknext#1{#2}%
  }%
}
%
% \skvecommaloop{<list>}<cmd>{<callback>}
% \skvecommaloop*{<listcmd>}<cmd>{<callback>}
%
% \skvecommaloop is as \skvcommaloop but will execute <callback>
% once when <list> is empty. This is needed for processing empty
% families.
%
\skvrobustdef\skvecommaloop{\skv@testst\skv@ecommaloop}
\skvrobustdef\skv@ecommaloop#1#2#3{%
  \edef#2{\unexpanded{\skv@commaloop@picknext#2{#3}}}%
  \ifskv@tempst\expandafter\expandafter\fi#2#1,\skv@commaloop@nil,%
}
%
% \skvcommaparse{<list>}<cmd>{<callback>}
% \skvcommaparse*{<listcmd>}<cmd>{<callback>}
%
% \skvcommaparse is as \skvcommaloop but will first normalize <list>
% using \skvcsvnormalize.
%
\skvrobustdef*\skvcommaparse{\skv@testst\skv@commaparse}
\skvrobustdef\skv@commaparse#1#2#3{%
  \skv@usetempst{#1}#2%
  \skvcsvnormalize#2%
  \skvcommaloop*#2#2{#3}%
}
% \skvkvparse{<list>}<cmd>{<callback>}
% \skvkvparse*{<listcmd>}<cmd>{<callback>}
%
% 1. \skvkvparse is as \skvcommaloop but will first normalize <list> using
%    \skvkvnormalize.
% 2. It is meant for processing key-value lists.
%
\skvrobustdef*\skvkvparse{\skv@testst\skv@kvparse}
\skvnewlet\skvparsekvlist\skvkvparse
\skvrobustdef\skv@kvparse#1#2#3{%
  \skv@usetempst{#1}#2%
  \skvkvnormalize#2%
  \skvcommaloop*#2#2{#3}%
}
% \skvcountelements[<parser>]{<list>}{<return.cmd>}
% \skvcountelements*[<parser>]{<listcmd>}{<return.cmd>}
\skvrobustdef*\skvcountelements{\skv@teststopt\skv@countelements,}
\skvrobustdef*\skv@countelements[#1]#2#3{%
  \begingroup
  \skv@usetempst{#2}\skv@tempa
  \@tempcnta\skvz@
  \skvdolist*{#1}\skv@tempa\skv@prova{%
    \advance\@tempcnta\@ne
  }%
  \edef#3{\the\@tempcnta}%
  \skvaftergroupdef#3\endgroup
}
% If the number of elements in a list is equal or greater than <nr>.
% \skvifelementcount[<parser>]{<list>}{<nr>}{<true>}{<false>}
% \skvifelementcount*[<parser>]{<listcmd>}{<nr>}{<true>}{<false>}
\skvrobustdef*\skvifelementcount{\skv@teststopt\skv@ifelementcount,}
\skvrobustdef*\skv@ifelementcount[#1]#2#3{%
  \begingroup
  \skv@usetempst{#2}\skv@tempa
  \@tempcnta\skvz@
  \skv@swafalse
  \skvdolist*{#1}\skv@tempa\skv@prova{%
    \advance\@tempcnta\@ne
    \ifnum\@tempcnta=#3\relax
      \skv@swatrue\skvbreakloop
    \fi
  }%
  \expandafter\endgroup\ifskv@swa
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}

% \skv@foreach@normalize[<parser>]<listcmd>
\skvrobustdef*\skv@foreach@normalize{\skv@testopt\skv@foreach@norm@lize,}
\skvrobustdef*\skv@foreach@norm@lize[#1]#2{%
  \skvxifntypeTF{\detokenize{#1}}\skvcsvnormalize\skvmacnormalize[#1]#2%
}

% \newforeach[<options>] <holders> {<list>} {<callback>}
% \newforeach*[<options>] <holders> {<listcmd>} {<callback>}
% \newforeach[<options>] <holders> in {<list>} do {<callback>}
% \newforeach*[<options>] <holders> in {<listcmd>} do {<callback>}
% \newforeach[<options>] <holders> in {<list>} <callback> ;
% \newforeach*[<options>] <holders> in {<listcmd>} <callback> ;
%
% 1. <callback> is the code that will be executed for each element
%    of the list. It will refer to the holder macros <holders>.
%
% 3. Elements of the form (a,b) and [a,b] are grabbed together.
%
% 4. Use \breaknewforeach to break out of the loop prematurely.
%
% 5. \newforeach can be nested.
%
% 6. The star (*) variant of \newforeach is equivalent to using the
%    key 'list is a macro' (or *) in <options>.
%
% \skv@foreach@holderdepth must be different from \foreachnestdepth,
% to avoid confusing two different stacks.
\skvnewnumbers{foreachnestdepth,skv@foreach@holderdepth,%
  skv@foreach@nra,skv@warnsubparser}
% \newforeach will not accept \skvifstreq or \skvifstrcmpTF because
% they don't start with '\if'. So we introduce \ifforeachstrcmp:
\skvnewlet\ifforeachstrcmp\skvifstreq
\skvnewdef*\skv@foreach@onlyinitially{}
\skvrobustdef*\skvforeachonlyinitially#1{%
  \edef\skv@foreach@onlyinitially{%
    \skvexpandonce\skv@foreach@onlyinitially
    \unexpanded{#1}%
  }%
}
% \skv@foreach@addtocallback{<pre.or.post>}{<code.to.add>}
\skvrobustdef*\skv@foreach@addtocallback#1#2{%
  \skvcsedef{skv@foreach@#1callback}{%
    \skvifcsdefFT{skv@foreach@#1callback}{}{%
      \skvexpandcsonce{skv@foreach@#1callback}%
    }%
    % No \unexpanded for #2 here, since #2 is to be expanded:
    #2%
  }%
}

\skvnewlet\skv@foreach@codemark\relax
\skvrobustdef*\skv@foreach@addtohook#1#2#3{%
  \begingroup
  \skvifdefTF#2{}{\def#2{}}%
  \edef\x{\detokenize{\skv@foreach@codemark#3\skv@foreach@codemark}}%
  \skvxifinTF\x{\skvoxdetok#2}{}{%
    \edef#2{%
      \skvifstrcmpTF{#1}{pre}{%
        \skv@foreach@codemark\unexpanded{#3}\skv@foreach@codemark
        \skvexpandonce{#2}%
      }{%
        \skvexpandonce{#2}%
        \skv@foreach@codemark\unexpanded{#3}\skv@foreach@codemark
      }%
    }%
  }%
  \skvaftergroupdef#2\endgroup
}

% \prependtobeginforeach[<depths>]{<code>}
\skvrobustdef*\prependtobeginforeach{%
  \skv@testopt{\skv@atbeginforeach{pre}}{}%
}
% \appendtobeginforeach[<depths>]{<code>}
\skvrobustdef*\appendtobeginforeach{%
  \skv@testopt{\skv@atbeginforeach{app}}{}%
}
\skvnewlet\atbeginforeach\appendtobeginforeach
\skvrobustdef*\skv@atbeginforeach#1[#2]#3{%
  \skvifblankTF{#2}{%
    \skvaftercsname{\skv@foreach@addtohook{#1}}%
      {skv@foreach@atbeginhook@\skvrom\@ne}{#3}%
  }{%
    \skvcommaloop{#2}\skv@tempa{%
      \skvaftercsname{\skv@foreach@addtohook{#1}}%
        {skv@foreach@atbeginhook@\skvrom\number\skv@tempa}{#3}%
    }%
  }%
}
% \prependtoendforeach[<depths>]{<code>}
\skvrobustdef*\prependtoendforeach{%
  \skv@testopt{\skv@atendforeach{pre}}{}%
}
% \appendtoendforeach[<depths>]{<code>}
\skvrobustdef*\appendtoendforeach{%
  \skv@testopt{\skv@atendforeach{app}}{}%
}
\skvnewlet\atendforeach\appendtoendforeach
\skvrobustdef*\skv@atendforeach#1[#2]#3{%
  \skvifblankTF{#2}{%
    \skvaftercsname{\skv@foreach@addtohook{#1}}%
      {skv@foreach@atendhook@\skvrom\@ne}{#3}%
  }{%
    \skvcommaloop{#2}\skv@tempa{%
      \skvaftercsname{\skv@foreach@addtohook{#1}}%
        {skv@foreach@atendhook@\skvrom\number\skv@tempa}{#3}%
    }%
  }%
}
% \atbeginforeachondepth{<depths>}{<code>}
\skvrobustdef*\atbeginforeachondepth#1#2{%
  \appendtobeginforeach[#1]{#2}%
}
% \atendforeachondepth{<depths>}{<code>}
\skvrobustdef*\atendforeachondepth#1#2{%
  \appendtoendforeach[#1]{#2}%
}

% \skv@foreach@fi@toks must use \detokenize. Don't change to \string!
\skvnewedef*\skv@foreach@fi@toks{\detokenize{\fi}}
\skvnewedef*\skv@foreach@if@toks{\string\if}

% \skv@foreach@ifacceptkv and \skv@foreach@maketester must come
% before the initialization of keys:
\skvrobustdef*\skv@foreach@ifacceptkv#1#2{%
  \def\next{}%
  \ifskvindef\else
    \edef\skv@prova{\unexpanded{#1}}%
    \ifnum0>\numexpr0\ifx\skv@prova\@empty-1\else
      \ifx\skv@prova\@nnil-1\else+0\fi\fi\relax\relax
      \skv@err{Invalid syntax '\detokenize{#1}'}\skv@ehd
    \else
      \edef\next{\unexpanded{#2}}%
    \fi
  \fi
  \next
}
\skvrobustdef*\skv@foreach@ifholderisonecmd#1#2#3{%
  \skvifntypeTF{#2}{%
    \skvifescapedTF{#2}{%
      #3%
    }{%
      \skv@err{Value of key '#1' must
      \MessageBreak be escaped: the holder macro
      \MessageBreak to be evaluated}\skv@ehd
    }%
  }{%
    \skv@err{Value of key '#1' must
      \MessageBreak be only one token: the holder
      \MessageBreak macro to be evaluated}\skv@ehd
  }%
}
% \skv@foreach@maketester{<cond>}<cond.tester.cmd>{<flag>}
%
% 1. Only balanced conditionals beginning with \if... and ending with \fi
%    are allowed. Restricting the type of allowed conditionals is
%    necessary for auto syntax checking.
% 2. <flag> is either 0 or 1, signifying whether or not the condition
%    should be entered in postcallback. This is because
%    \skv@foreach@maketester is called (by key 'loop stopper') for
%    formating the premature exit condition and (in
%    \skv@foreach@parsecountin and \skv@foreachfox@parsecountin) for the
%    condition for counting an item of the list. In the latter case,
%    there is no need to enter the formated
%    condition in the postcallback, since it it is entered in the
%    'afterprecallback' or (in the case of \foreachfox) in 'precallback'.
%
%    Examples: \ifnum\x>10\fi, \ifx\x\cmd\fi.
%
\skvrobustdef*\skv@foreach@maketester#1#2#3{%
  % Make '#1' innocent in a macro, in case it contains parameter
  % characters. \skv@prova will appear only in the error message.
  \begingroup
  \edef\skv@prova{\detokenize{#1}}%
  \skvifblankTF{#1}{%
    \skv@err{A blank conditional has been given in
      \MessageBreak\string\newforeach or a similar command}\skv@ehd
  }{%
    \skvxifinTF{\skv@foreach@fi@toks\relax}{\detokenize{#1}\relax}{%
      \skvxifinTF{\relax\skv@foreach@if@toks}{\relax\detokenize{#1}}{%
        \edef#2{\noexpand\skvifconditionTF\unexpanded{#1}}%
        \ifnum#3=\@ne
          \skv@foreach@addtocallback{post}{%
            \unexpanded{\skvifconditionTF#1}{\noexpand\skvbreakloop}{}%
          }%
        \fi
      }{%
        \skv@err{Invalid conditional '\skv@prova'}
          {Invalid, possibly unbalanced, conditional '\skv@prova'}%
      }%
    }{%
      \skv@err{Invalid conditional '\skv@prova'}\skv@ehd
    }%
  }%
  \skvexpanded{\endgroup
    \skvcmdexit#2%
    \ifnum#3=\@ne
      \skvcmdexit\skv@foreach@postcallback
    \fi
  }%
}
\skvquickkeys.define{skeyval/foreach}{%
  .exec/
    \def\skv@foreach@parser{,}
    \def\skv@foreach@subparser{/}
  ;
  parser/{,}/
    \edef\skv@foreach@parser{\unexpanded{#1}}
    \skvstripouterbraces{2}\skv@foreach@parser
    \skvxifntypeTF{\detokenize{#1}}{%
      \begingroup
      % It is assumed that every n-type parser and subparser
      % must have catcode 12:
      \skvexpandnext{\catcode`}\skv@foreach@parser=12\relax
      \skvrescan\skv@foreach@parser
      \skvaftergroupdef\skv@foreach@parser\endgroup
    }{}
  ;
  subparser/{/}/
    \edef\skv@foreach@subparser{\unexpanded{#1}}
    \skvstripouterbraces{2}\skv@foreach@subparser
    \skvxifntypeTF{\detokenize{#1}}{
      \begingroup
      \skvexpandnext{\catcode`}\skv@foreach@subparser=12\relax
      \skvrescan\skv@foreach@subparser
      \skvaftergroupdef\skv@foreach@subparser\endgroup
    }{}
  ;
  terminator,callback terminator/{;}/
    \edef\skv@foreach@terminator{\unexpanded{#1}}%
    \skvstripouterbraces{2}\skv@foreach@terminator
  ;
  % process up to = <nr>
  % Maximum number of items to process:
  process up to,process up to number//
    \skviflacus#1\then\else
      \skvensureinteger{process up to}{#1}%
      \def\skv@foreach@processupto{#1}%
      \skvstripouterbraces{2}\skv@foreach@processupto
    \fi
  ;
  process empty list/true/
    \edef\skv@foreach@processempty{0\skvifstrcmpTF{true}{#1}01}%
    /true,false
  ;
  % 'break=<condition>'
  % Break list processing when <condition> is satisfied. <condition> must
  % be a balanced plain TeX conditional. Eg, 'exit when={\ifnum\x=20\fi}'.
  % Notice the use of outer braces in '{\ifnum\x=20\fi}'. This avoids
  % conflicting the two equality signs: for the key-value and for number
  % testing.
  .exec/\let\skv@foreach@exittester\@secondoftwo;
  break,loop stopper,exit when/\if01\fi/
    \edef\skv@tempa{\unexpanded{#1}}%
    \skvstripouterbraces{2}\skv@tempa
    \skvexpbracenext\skv@foreach@maketester\skv@tempa
      \skv@foreach@exittester\@ne
  ;
  % Java-type of continue: If the user wants to ignore the callback for
  % some items, he can instantiate the key 'condition=<condition>'.
  % <condition> must be a balanced plain TeX conditional. Eg,
  % continue={\ifnum\x=20\fi}.
  .exec/\let\skv@foreach@continuetester\@secondoftwo;
  continue,ignore callback/\if01\fi/
    \edef\skv@tempa{\unexpanded{#1}}%
    \skvstripouterbraces{2}\skv@tempa
    \skvexpbracenext\skv@foreach@maketester\skv@tempa
      \skv@foreach@continuetester\skvz@
  ;
  % Eg, 'evaluate = \x as \z using \numexpr\x*2'. 'as' and 'using', and the
  % tokens after them, can be missing, but the formula must be complete.
  evaluate/\@nil/
    \skv@foreach@ifacceptkv{#1}{%
      \skv@foreach@parseevaluate{#1}%
    }%
  ;
  % The evaluator \numexpr will invariably be used internally for this key.
  % 'as' and 'using' are illegal here. This is only a shortcut for 'evaluate'.
  evaluate num,evaluate number/\@nil/
    \skv@foreach@ifacceptkv{#1}{%
      \skv@foreach@ifholderisonecmd{evaluate number}{#1}{%
        \skv@foreach@parseevaluate{#1as#1using\numexpr#1}%
      }%
    }%
  ;
  % The evaluator \dimexpr will invariably be used internally for this key.
  % 'as' and 'using' are illegal here. This is only a shortcut for 'evaluate'.
  evaluate dim,evaluate dimension/\@nil/
    \skv@foreach@ifacceptkv{#1}{%
      \skv@foreach@ifholderisonecmd{evaluate dimension}{#1}{%
        \skv@foreach@parseevaluate{#1as#1using\dimexpr#1}%
      }%
    }%
  ;
  % Eg, 'expand=\x'.
  % Fully expand holder macro. This is equivalent to, eg, edef\x{\x}.
  % 'as' and 'using' are illegal here. This is only a shortcut for 'evaluate'.
  expand,expanded/\@nil/
    \skv@foreach@ifacceptkv{#1}{%
      \skv@foreach@ifholderisonecmd{expand}{#1}{%
        \skv@foreach@parseevaluate{#1as#1using#1}%
      }%
    }%
  ;
  % Eg, 'pgf parse = \x as \xe using \x*3'. 'as' and 'using', and the
  % tokens after them, can be present or missing.
  % \pgfmathparse is always used for this key.
  pgf evaluate,pgf parse,pgfmath parse/\@nil/
    \skv@foreach@ifacceptkv{#1}{%
      \skv@foreach@parsepgfmathparse{#1}%
    }%
  ;
  % count in = \y all \x satisfying <condition> initially <value>
  % Eg,
  %    count in = \p all \x satisfying \ifnum\x>4\fi, or
  %    count in = \p all \x satisfying \skvifnumTF\x>4
  % The counting is not additive, meaning that the counter is initialized
  % to zero on each depth.
  count in,count/\@nil/
    \skv@foreach@ifacceptkv{#1}{%
      \skv@foreach@parsecountin{#1}%
    }%
  ;
  % Eg, 'remember=\x as \y initially A':
  remember/\@nil/
    \skv@foreach@ifacceptkv{#1}{%
      \skv@foreach@parseremember{#1}%
    }%
  ;
  % Eg, 'recall=\x initially A'.
  % 'recall' is as 'remember', but will save the value of the holder macro
  % in \<foreachlast><holder>. 'as' is invalid/illegal here, since a
  % retainer macro is built internally:
  retain,recall,call up/\@nil/
    \skv@foreach@ifacceptkv{#1}{%
      \skv@foreach@parserecall{#1}%
    }%
  ;
  item counter,counter/\foreachdefaultitemcounter/
    \skvifescapedTF{#1}{%
      \def\skv@foreach@itemcounter{#1}%
    }{%
      \skv@err{Non-escaped value '\detokenize{#1}'
        \MessageBreak for key 'item counter'}\skv@ehd
    }%
  ;
  list breaker/\foreachlistbreaker/
    \edef\skv@prova{\unexpanded{#1}}%
    \ifx\skv@prova\@empty
      \skv@err{Invalid empty value for key 'list breaker'}\skv@ehd
    \else
      \let\skv@listbreakertoks\skv@prova
    \fi
  ;
  list pauser/\foreachlistpauser/
    \edef\skv@prova{\unexpanded{#1}}%
    \ifx\skv@prova\@empty
      \skv@err{Invalid empty value for key 'list pauser'}\skv@ehd
    \else
      \let\skv@listpausertoks\skv@prova
    \fi
  ;
  % Remember outside the loop the holder values. Of course, this
  % means remembering only the latest values.
  recover holder values,recover holder values after loop/true/
    \edef\skv@foreach@recoverholders{0\skvifstrcmpTF{true}{#1}01}%
    /true,false
  ;
  % This default value of 'link' is required by \skvautocompletelist:
  .exec code/\def\skv@foreach@link{\@nil};
  link/\@nil/
    \edef\skv@prova{\unexpanded{#1}}%
    \ifcase0%
      \ifx\skv@prova\@empty 1\fi
      \ifx\skv@prova\@nnil 1\fi\relax
      \edef\skv@foreach@link{\unexpanded{#1}}%
      \skvstripouterbraces{2}\skv@foreach@link
    \fi
  ;
  grow/\@nil/
    \edef\skv@prova{\unexpanded{#1}}%
    \ifx\skv@prova\@nnil\else
      \skvcsedef{skv@foreach@grow#1}{00}
      \edef\skv@prova{\skvifstrcmpTF{#1}{left}{right}{left}}%
      \skvcsedef{skv@foreach@grow\skv@prova}{01}%
    \fi
    /left,right
  ;
  .exec/
    \def\skv@foreach@growleft{01}
    \def\skv@foreach@growright{01}
  ;
  grow left/true/
    \edef\skv@foreach@growleft{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  grow right/true/
    \edef\skv@foreach@growright{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  % Keep the decimals in rounded numbers or dimensions when list is
  % auto-completed. The value value of this key is 'true'.
  keep decimals/true/
    \edef\skv@foreach@keepdecimals{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  keep high decimals,keep only high decimals/true/
    \edef\skv@foreach@keephighdecimals{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  % This key means that, eg, for \x/\y, do \let\y=\x if \y has no
  % user value, ie, if the user gives as an item 'a' instead of
  % 'a/b' or 'a/a'.
  inherit,transfer macro values/true/
    \edef\skv@foreach@inherit{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  expand before fill,expand list before fill/true/
    \edef\skv@foreach@expandbeforefill{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  expand list once,x1,list is a macro,macro list/true/
    \edef\skv@foreach@expandlistonce{0\skvifstrcmpTF{true}{#1}01}%
    /true,false
  ;
  expand list twice,x2/true/
    \edef\skv@foreach@expandlisttwice{0\skvifstrcmpTF{true}{#1}01}%
    /true,false
  ;
  % Don't use 'expand' for this key, to avoid confusing it with
  % the 'expand' for holder macros:
  expand list,fully expand list,expand list fully,xx/true/
    \edef\skv@foreach@expandlistfully{0\skvifstrcmpTF{true}{#1}01}%
    /true,false
  ;
  reverse list,reverse,reflect/true/
    \edef\skv@foreach@reverselist{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  % 'hide parameters' can be used to avoid doubling the parameter
  % characters in the callback.
  hide parameters/true/
    \edef\skv@foreach@hideparameters{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
}

% The following keys don't need presetting. The user must supply
% values when they are called. In internal loops, their values will
% have to be revised from those of the outer loop.
%
%    link,evaluate,,evaluate num,evaluate dim,expand,count in,
%    process up to,grow
%
\skvquickkeys.preset{skeyval/foreach}{%
  parser,subparser,loop stopper,callback terminator,process up to,
  process empty list=false,item counter,list breaker,list pauser,
  recover holder values=false,grow left=false,grow right=false,
  keep decimals=true,keep high decimals=false,inherit=false,
  expand before fill=false,reverse list=false,expand list once=false,
  expand list twice=false,expand list fully=false,hide parameters=false
}

\skvnewdef*\skv@foreach@kvlist{}
% \setupforeach{<kvlist>}
\skvrobustdef*\setupforeach#1{%
  \skvifblankTF{#1}{}{%
    \skvaddtolist\skv@foreach@kvlist{#1}%
  }%
}
\skvrobustdef*\skv@foreach@setkeys#1{%
  \def\reserved@a{\skvquickkeys.set{skeyval/foreach}}%
  \expandafter\reserved@a\expandafter{\skv@foreach@kvlist,#1}%
}

% evaluate=<holder.macro> as <child.macro> using <formula>
%
% 1. Evaluation is done with \edef unless \pgfmathparse is present
%    in <formula> or key 'pgf evaluate' is called.
%
% 2. <formula> must be a valid formula, eg,
%
%      \pgfmathparse\x*2
%      \pgfmathparse{exp(50)*\x*2+sin(.5*pi)*60}
%      \numexpr\x*2
%      \skvexpandonce\x
%
%    or simply
%
%    'evaluate \x as \x using <empty>'
%
%    The latter is equivalent to asking for full expansion. See also
%    the keys 'evaluate num', 'evaluate dim', and 'expand'.
%
% 3. This allows <formula> to be generic.
%
\skvrobustdef*\skv@foreach@parseevaluate#1{%
  \begingroup
  \def\skv@tempxifin##1##2{%
    \skvxifinTF{\detokenize{##1}}{\detokenize{##2}}%
  }%
  \skv@foreach@swafalse
  \def\skv@tempd{}%
  \def\skv@tempa##1as##2using##3\skv@nil{%
    \edef\skv@prova{\skvtrimspace{##1}}%
    \edef\skv@provb{\skvtrimspace{##2}}%
    \edef\skv@provc{\skvtrimspace{##3}}%
    \ifx\skv@prova\@empty
      \skv@err{Value of key 'evaluate' has no holder macro}\skv@ehd
    \else
      \expandafter\skvifescapedTF\expandafter{\skv@prova}{%
        \expandafter\skvifntypeTF\expandafter{\skv@prova}{}{%
          \skv@err{Value of key 'evaluate': more than 1
            \MessageBreak token \skvoxdetok\skv@prova.
            \MessageBreak I can't find holder macro}\skv@ehd
        }%
      }{%
        \skv@err{Value of key 'evaluate':
          \MessageBreak holder macro \skvoxdetok\skv@prova not escaped}\skv@ehd
      }%
    \fi
    \ifx\skv@provb\@empty
      \skv@err{Value of key 'evaluate' has no child macro}\skv@ehd
    \else
      \expandafter\skvifescapedTF\expandafter{\skv@provb}{%
        \expandafter\skvifntypeTF\expandafter{\skv@provb}{}{%
          \skv@err{Value of key 'evaluate': more than 1
            \MessageBreak token \skvoxdetok\skv@provb.
            \MessageBreak I can't find child macro}\skv@ehd
        }%
      }{%
        \skv@err{Value of key 'evaluate':
          \MessageBreak child \skvoxdetok\skv@provb not escaped}\skv@ehd
      }%
    \fi
    \ifx\skv@provc\@empty
      \skv@err{Value of key 'evaluate' has no formula or
        \MessageBreak holder macro to be expanded}\skv@ehd
    \fi
    \skv@tempxifin{\pgfmathparse}{##3}{%
      \def\skv@tempc####1\pgfmathparse####2\skv@nil{%
        \ifx\@nnil####1\@nnil
          \skv@foreach@swatrue
        \else
          \skv@err{Invalid token \detokenize{####1}
            \MessageBreak before \string\pgfmathparse}\skv@ehd
        \fi
      }%
      \skv@tempc##3\skv@nil
    }{%
      \skv@tempxifin{\numexpr}{##3}{%
        \def\skv@tempd{\relax}%
      }{%
        \skv@tempxifin{\dimexpr}{##3}{%
          \def\skv@tempd{\relax}%
        }{%
          \def\skv@tempd{}%
        }%
      }%
    }%
  }%
  \skv@tempxifin{using}{#1}{%
    \skv@tempxifin{as}{#1}{%
      % 'as' and 'using' are present: maybe there is a formula.
      \skv@foreach@swbtrue
      \skv@tempa#1\skv@nil
    }{%
      \skv@err{Value of key 'evaluate':
        \MessageBreak there is 'using', but no 'as'}\skv@ehd
    }%
  }{%
    % No formula given. Maybe the key is 'expand' or still 'evaluate'
    % but without formula.
    \skv@foreach@swbfalse
    \skv@tempxifin{as}{#1}{%
      \def\skv@tempb##1as##2##3\skv@nil{%
        \ifx\@nnil##1\@nnil
          \skv@err{Value of key 'evaluate' has no holder macro}\skv@ehd
        \else
          \ifx\@nnil##2%
            \skv@err{Value of key 'evaluate' has no child macro}\skv@ehd
          \else
            \skv@tempa##1as##2using##1\skv@nil
          \fi
        \fi
      }%
      \skv@tempb#1{\@nnil}\skv@nil
    }{%
      % No 'as' or 'using': #1 should be only the holder macro:
      \ifx\@nnil#1\@nnil
        \skv@err{Value of key 'evaluate' has no holder macro}\skv@ehd
      \else
        \skvifntypeTF{#1}{%
          % Expand the holder macro:
          \skv@tempa#1as#1using#1\skv@nil
        }{%
          \skv@err{Value of key 'evaluate': more than 1
            \MessageBreak token '\detokenize{#1}'.
            \MessageBreak I can't find holder macro}\skv@ehd
        }%
      \fi
    }%
  }%
  \skv@foreach@addtocallback{afterpre}{%
    \ifskv@foreach@swa
      % <formula> has the syntax \pgfmathparse{\x}.
      \skvexpandonce\skv@provc
      \let\skvexpandonce\skv@provb\noexpand\pgfmathresult
    \else
      % <formula> has the syntax \numexpr\x*2 or \dimexpr\x*2.
      % \ifskv@foreach@swb is true when a formula has been given.
      \edef\skvexpandonce\skv@provb{%
        \ifskv@foreach@swb\noexpand\the\fi
        \skvexpandonce\skv@provc\skv@tempd
      }%
    \fi
  }%
  \skvaftergroupdef\skv@foreach@afterprecallback\endgroup
}

% pgfmath parse=<holder.macro> as <child.macro> using <formula>
%
% 1. Evaluation is always done with \pgfmathparse.
%
% 2. <formula> must be \pgfmathparse-able.
%
\skvrobustdef*\skv@foreach@parsepgfmathparse#1{%
  \begingroup
  \ifdefined\pgfmathparse\else
    \skv@err{No \string\pgfmathparse; 'pgfmath' module not loaded}\skv@ehd
  \fi
  \def\skv@tempxifin##1##2{%
    \skvxifinTF{\detokenize{##1}}{\detokenize{##2}}%
  }%
  \skv@foreach@swafalse
  \def\skv@tempa##1as##2using##3\skv@nil{%
    \edef\skv@prova{\skvtrimspace{##1}}%
    \edef\skv@provb{\skvtrimspace{##2}}%
    \edef\skv@provc{\skvtrimspace{##3}}%
    \ifx\skv@prova\@empty
      \skv@err{Value of key 'pgfmath parse' has no holder macro}\skv@ehd
    \else
      \expandafter\skvifescapedTF\expandafter{\skv@prova}{%
        \expandafter\skvifntypeTF\expandafter{\skv@prova}{}{%
          \skv@err{Value of key 'pgfmath parse': more than 1
            \MessageBreak token \skvoxdetok\skv@prova.
            \MessageBreak I can't find holder macro}\skv@ehd
        }%
      }{%
        \skv@err{Value of key 'pgfmath parse':
          \MessageBreak holder macro \skvoxdetok\skv@prova not escaped}\skv@ehd
      }%
    \fi
    \ifx\skv@provb\@empty
      \skv@err{Value of key 'pgfmath parse' has no child macro}\skv@ehd
    \else
      \expandafter\skvifescapedTF\expandafter{\skv@provb}{%
        \expandafter\skvifntypeTF\expandafter{\skv@provb}{}{%
          \skv@err{Value of key 'pgfmath parse': more than 1
            \MessageBreak token \skvoxdetok\skv@provb.
            \MessageBreak I can't find child macro}\skv@ehd
        }%
      }{%
        \skv@err{Value of key 'pgfmath parse':
          \MessageBreak child \skvoxdetok\skv@provb not escaped}\skv@ehd
      }%
    \fi
    \ifx\skv@provc\@empty
      \skv@err{Value of key 'pgfmath parse' has no formula or
        \MessageBreak holder macro to be expanded}\skv@ehd
    \fi
    \skv@tempxifin{\pgfmathparse}{##3}{%
      \def\skv@tempc####1\pgfmathparse####2\skv@nil{%
        \ifx\@nnil####1\@nnil
          \skv@foreach@swatrue
        \else
          \skv@err{Invalid token \detokenize{####1}
            \MessageBreak before \string\pgfmathparse}\skv@ehd
        \fi
      }%
      \expandafter\skv@tempc\skv@provc\skv@nil
    }{%
      \skv@tempxifin{\numexpr}{##3}{%
        \skv@err{Value of key 'pgfmath parse':
          \MessageBreak\noexpand\numexpr not allowed}\skv@ehd
      }{%
        \skv@tempxifin{\dimexpr}{##3}{%
          \skv@err{Value of key 'pgfmath parse':
            \MessageBreak\noexpand\dimexpr not allowed}\skv@ehd
        }{%
          \skv@foreach@swatrue
          \edef\skv@provc{\noexpand\pgfmathparse{\skvexpandonce\skv@provc}}%
        }%
      }%
    }%
  }%
  \skv@tempxifin{using}{#1}{%
    \skv@tempxifin{as}{#1}{%
      % 'as' and 'using' are present: maybe there is a formula.
      \skv@tempa#1\skv@nil
    }{%
      \skv@err{Value of key 'pgfmath parse':
        \MessageBreak there is 'using', but no 'as'}\skv@ehd
    }%
  }{%
    \skv@tempxifin{as}{#1}{%
      \def\skv@tempb##1as##2##3\skv@nil{%
        \ifx\@nnil##1\@nnil
          \skv@err{Value of key 'pgfmath parse' has no holder macro}\skv@ehd
        \else
          \ifx\@nnil##2%
            \skv@err{Value of key 'pgfmath parse' has no child macro}\skv@ehd
          \else
            \skv@tempa##1as##2using##1\skv@nil
          \fi
        \fi
      }%
      \skv@tempb#1{\@nnil}\skv@nil
    }{%
      % No 'as' or 'using': #1 should be only the holder macro:
      \ifx\@nnil#1\@nnil
        \skv@err{Value of key 'pgfmath parse' has no holder macro}\skv@ehd
      \else
        \skvifntypeTF{#1}{%
          % Evaluate the holder macro:
          \skv@tempa#1as#1using#1\skv@nil
        }{%
          \skv@err{Value of key 'pgfmath parse': more than 1
            \MessageBreak token '\detokenize{#1}'.
            \MessageBreak I can't find holder macro}\skv@ehd
        }%
      \fi
    }%
  }%
  \skv@foreach@addtocallback{afterpre}{%
    \ifskv@foreach@swa
      \skvexpandonce\skv@provc
      \let\skvexpandonce\skv@provb\noexpand\pgfmathresult
    \fi
  }%
  \skvaftergroupdef\skv@foreach@afterprecallback\endgroup
}

% count in = \y all \x satisfying <condition> initially <value>
%
% 1. <condition> must be a balanced and valid TeX conditional, like
%
%    \ifnum\x>2\fi, \ifx\x\@empty\fi
%
% 2. The aim is to allow general conditions (not only those involving
%    numerals) to be submitted.
%
% 3. PGF's \foreach doesn't have this feature; it has only a general
%    counter, eg,
%
%    '\foreach \x [count=\xi] in {a,...,e}'.
%
%    Generic counting is available in \newforeach by default, without
%    user request. The macros \foreachcurrentitem, \foreachitemcount,
%    \foreachnextitem are always available on each nesting level. The
%    boolean \ifforeachlastitem is also always available, to indicate when
%    the last item of the list has been reached:
%
%    \ifforeachlastitem \typeout{Processing last entry of the list} \fi
%
% 4. Counting is done from 1 (zero) unless <value> is given after
%    'initially'.
%
\skvrobustdef*\skv@foreach@parsecountin#1{%
  \begingroup
  \def\skv@tempxifin##1##2{%
    \skvxifinTF{\detokenize{##1}}{\detokenize{##2}}%
  }%
  \def\skv@tempa##1\skv@nil{%
    \skv@tempxifin{initially}{##1}{%
      \skv@tempb##1\skv@nil
    }{%
      \skv@tempb##1initially\skv@nil
    }%
  }%
  \def\skv@tempb##1all##2satisfying##3initially##4\skv@nil{%
    \edef\skv@prova{\skvtrimspace{##1}}%
    \edef\skv@provb{\skvtrimspace{##2}}%
    \edef\skv@provc{\skvtrimspace{##3}}%
    \edef\skv@provd{\skvtrimspace{##4}}%
    \ifx\skv@prova\@empty
      \skv@err{Value of key 'count' has no counter macro}\skv@ehd
    \else
      \expandafter\skvifescapedTF\expandafter{\skv@prova}{%
        \expandafter\skvifntypeTF\expandafter{\skv@prova}{}{%
          \skv@err{Value of key 'count in': more than 1
            \MessageBreak token \skvoxdetok\skv@prova.
            \MessageBreak I can't find counter macro}\skv@ehd
        }%
      }{%
        \skv@err{Value of key 'count':\MessageBreak
          counter macro \skvoxdetok\skv@prova not escaped}\skv@ehd
      }%
    \fi
    \ifx\skv@provd\@empty
      \expandafter\def\skv@prova{0}%
    \else
      \skvifintegerTF\skv@provd{%
        \expandafter\let\skv@prova\skv@provd
      }{%
        \skv@err{Value of key 'count':\MessageBreak
          initial \skvoxdetok\skv@provd not an integer}\skv@ehd
      }%
    \fi
    \skv@foreach@swafalse
    \ifx\skv@provc\@empty
      % No tester but there may be a holder macro to test. The holder
      % macro, on its own, isn't sufficient to conduct a test:
      \let\skv@foreach@itemcounter\skv@prova
    \else
      \ifx\skv@provb\@empty\else
        % If there isn't a holder macro or quantity to test, then no
        % test is possible:
        \expandafter\skvifescapedTF\expandafter{\skv@provb}{%
          \expandafter\skvifntypeTF\expandafter{\skv@provb}{}{%
            \skv@err{Value of key 'count in': more than 1
              \MessageBreak token \skvoxdetok\skv@provb.
              \MessageBreak I can't find holder macro}\skv@ehd
          }%
        }{%
          \skv@err{Value of key 'count':\MessageBreak
            holder macro \skvoxdetok\skv@provb not escaped}\skv@ehd
        }%
        \skv@foreach@swatrue
        % \skv@tester is the second argument of \skv@foreach@maketester.
        % \skv@tester is used in pushing the item counter:
        \skvexpbracenext\skv@foreach@maketester\skv@provc\skv@tester\skvz@
      \fi
    \fi
  }%
  \skv@tempxifin{satisfying}{#1}{%
    \skv@tempxifin{all}{#1}{%
      % 'all' and 'satisfying' are present:
      \skv@tempa#1\skv@nil
    }{%
      \skv@err{Value of key 'count':
        \MessageBreak there is 'satisfying', but no 'all'}\skv@ehd
    }%
  }{%
    \skv@tempxifin{all}{#1}{%
      \skv@tempa#1satisfying\skv@nil
    }{%
      % No 'all' or 'satisfying': #1 should be only the counter macro:
      \ifx\@nnil#1\@nnil
        \skv@err{Value of key 'count' has no counter macro}\skv@ehd
      \else
        \skvifntypeTF{#1}{%
          \skv@tempa#1all satisfying\skv@nil
        }{%
          \skv@err{Value of key 'count in': more than 1
            \MessageBreak token '\detokenize{#1}'.
            \MessageBreak I can't find counter macro}\skv@ehd
        }%
      \fi
    }%
  }%
  \ifskv@foreach@swa
    \skv@foreach@addtocallback{afterpre}{%
      \noexpand\ifnum\noexpand\foreachitemcount=\@ne
        \def\skvexpandonce\skv@prova{\number\skv@prova}%
      \noexpand\fi
      \skvexpandonce\skv@tester{%
        \noexpand\skvpushnumber\skvexpandonce\skv@prova
      }{}%
    }%
  \fi
  \skvexpanded{\endgroup
    \ifskv@foreach@swa
      \skvcmdexit\skv@foreach@afterprecallback
    \else
      \skvcmdexit\skv@foreach@itemcounter
    \fi
  }%
}

% remember=<holder.macro> as <child.macro> initially <value>
%
\skvrobustdef*\skv@foreach@parseremember#1{%
  \begingroup
  \def\skv@tempxifin##1##2{%
    \skvxifinTF{\detokenize{##1}}{\detokenize{##2}}%
  }%
  \skv@tempxifin{(}{#1}{%
    \skv@err{Value of key 'remember': '(' found.
      \MessageBreak I don't accept this PGF format.
      \MessageBreak Remove the parenthesis '(<your input>)'}\skv@ehd
  }{}%
  \def\skv@tempa##1as##2initially##3\skv@nil{%
    \edef\skv@prova{\skvtrimspace{##1}}%
    \edef\skv@provb{\skvtrimspace{##2}}%
    \edef\skv@provc{\skvtrimspace{##3}}%
    \skv@foreach@swafalse
    \ifx\skv@prova\@empty
      \skv@err{Value of key 'remember' has no holder macro:
        \MessageBreak i.e., no macro that holds input}\skv@ehd
    \else
      \expandafter\skvifescapedTF\expandafter{\skv@prova}{}{%
        \skv@err{Value of key 'remember':
          \MessageBreak Holder macro \skvoxdetok\skv@prova not escaped}\skv@ehd
      }%
    \fi
    \ifx\skv@provb\@empty
      \skv@err{Value of key 'remember' has no child macro;
        \MessageBreak i.e., no macro after 'as'}\skv@ehd
    \else
      \expandafter\skvifescapedTF\expandafter{\skv@provb}{%
        \skv@foreach@swatrue
      }{%
        \skv@err{Value of key 'remember':
          \MessageBreak Child \skvoxdetok\skv@provb not escaped}\skv@ehd
      }%
    \fi
  }%
  \skv@tempxifin{initially}{#1}{%
    \skv@tempxifin{as}{#1}{%
      \skv@tempa#1\skv@nil
    }{%
      \skv@err{Value of key 'remember':
        \MessageBreak There is 'initially', but no 'as'}\skv@ehd
    }%
  }{%
    \skv@tempxifin{as}{#1}{%
      \skv@tempa#1initially\skv@nil
    }{%
      % No 'as' and 'initially':
      \edef\skv@prova{\skvtrimspace{#1}}%
      \ifx\skv@prova\@empty\else
        % Go and raise error in \skv@tempa:
        \skv@tempa#1as initially\skv@nil
      \fi
    }%
  }%
  \ifskv@foreach@swa
    % Initially:
    \skv@foreach@addtocallback{pre}{%
      % Don't remove this \ifnum, otherwise the initial assignment
      % will be overwritten on subsequent returns:
      \noexpand\ifnum\noexpand\foreachitemcount=\@ne
        \edef\skvexpandonce\skv@provb{%
          \noexpand\unexpanded{\skvexpandonce\skv@provc}%
        }%
      \noexpand\fi
    }%
    \skv@foreach@addtocallback{post}{%
      \let\skvexpandonce\skv@provb\skvexpandonce\skv@prova
    }%
  \fi
  \skvexpanded{\endgroup
    \ifskv@foreach@swa
      \skvcmdexit\skv@foreach@precallback
      \skvcmdexit\skv@foreach@postcallback
    \fi
  }%
}

% recall=<holder.macro> initially <value>.
%
% This builds a retainer macro of the form \<foreachlast><holder.name>.
%
% 'as' is invalid/illegal here, since a retainer macro is built internally.
%
\skvrobustdef*\skv@foreach@parserecall#1{%
  \begingroup
  \def\skv@tempxifin##1##2{%
    \skvxifinTF{\detokenize{##1}}{\detokenize{##2}}%
  }%
  \skv@tempxifin{(}{#1}{%
    \skv@err{Value of key 'recall': '(' found.
      \MessageBreak I don't accept this PGF format.
      \MessageBreak remove the parenthesis '()'}\skv@ehd
  }{}%
  \skv@foreach@swafalse
  \def\skv@tempa##1initially##2\skv@nil{%
    \edef\skv@prova{\skvtrimspace{##1}}%
    \edef\skv@provb{\skvtrimspace{##2}}%
    \ifx\skv@prova\@empty
      \skv@err{Value of key 'recall' has no holder macro:
        \MessageBreak i.e., no macro that holds input}\skv@ehd
    \else
      \expandafter\skvifntypeTF\expandafter{\skv@prova}{%
        \expandafter\skvifescapedTF\expandafter{\skv@prova}{%
          \edef\skv@elt{\expandafter\skvremovescape\skv@prova}%
          \skv@foreach@swatrue
          % Initially:
          \skv@foreach@addtocallback{pre}{%
            % Don't remove this \ifnum, otherwise the initial assignment
            % will be overwritten on subsequent returns:
            \noexpand\ifnum\noexpand\foreachitemcount=\@ne
              \skvcsedef{foreachlast\skv@elt}{%
                \noexpand\unexpanded{\skvexpandonce\skv@provb}%
              }%
            \noexpand\fi
          }%
          \skv@foreach@addtocallback{post}{%
            \skvcslet{foreachlast\skv@elt}\skvexpandonce\skv@prova
          }%
        }{%
          \skv@err{Value of key 'recall':
            \MessageBreak \detokenize{#1} is not escaped}\skv@ehd
        }%
      }{%
        \skv@err{Value of key 'recall':
          \MessageBreak \detokenize{#1} is not one token}\skv@ehd
      }%
    \fi
  }%
  \skv@tempxifin{as}{#1}{%
    \skv@err{Value of key 'recall': invalid 'as' found.
      \MessageBreak This key doesn't expect 'as' since
      \MessageBreak it automatically builds a retainer macro
      \MessageBreak of the form \<foreachlast><holder.name>}\skv@ehd
  }{%
    \skv@tempxifin{initially}{#1}{%
      \skv@tempa#1\skv@nil
    }{%
      \ifx\@nnil#1\@nnil\else
        \skv@tempa#1initially\skv@nil
      \fi
    }%
  }%
  \skvexpanded{\endgroup
    \ifskv@foreach@swa
      \skvcmdexit\skv@foreach@precallback
      \skvcmdexit\skv@foreach@postcallback
    \fi
  }%
}
% \skv@foreach@doreverselist{<parser>}{<listcmd>}
\skvnewdef*\skv@foreach@doreverselist#1#2{%
  \begingroup
  \def\skv@tempb{}%
  \def\skv@tempa##1#1##2\skv@reverse@stop{%
    \if\relax\detokenize{##2}\relax\skv@reverse@stop\fi
    \skv@tempa##2\skv@reverse@stop
    \edef\skv@tempb{%
      \skvexpandonce\skv@tempb\ifx\skv@tempb\@empty\else#1\fi
      \unexpanded{##1}%
    }%
  }%
  \def\skv@reverse@stop##1\skv@reverse@stop{\fi}%
  \expandafter\skv@tempa#2#1\skv@reverse@stop
  \let#2\skv@tempb
  \skvaftergroupdef#2\endgroup
}

% Eg, \skv@dots@in<value>\skv@nil...\skv@nnil\skv@stop
\skvnewdef*\skv@dots@in#1...#2#3\skv@stop{%
	\ifx\skv@nnil#2\in@false\else\in@true\fi
}

\skvrobustdef*\skv@foreach@latehookerr{%
  \def\skv@foreach@latehook{%
    \begingroup
    \let\s\string
    \skv@err{A \noexpand\newforeach hook (\s\prependtobeginforeach,
      \MessageBreak\s\appendtobeginforeach, \s\atbeginforeach,
      \MessageBreak\s\prependtoendforeach, \s\appendtoendforeach,
      \MessageBreak or \s\atendforeach) has been illegally
      \MessageBreak issued within \s\newforeach}
      {\s\newforeach\space hook command shouldn't be issued
        within \s\newforeach.}%
    \endgroup
  }%
  \skvletmanytocmd{%
    \prependtobeginforeach,\appendtobeginforeach,\atbeginforeach,
    \prependtoendforeach,\appendtoendforeach,\atendforeach
  }\skv@foreach@latehook
}

\skvrobustdef*\skv@foreach@pushstate{%
  \skvsavestate\skv@foreach@stack{%
    \do\skv@foreach@starform\do\skv@foreach@parser
    \do\skv@foreach@subparser\do\skv@foreach@listisamacro
    \do\skv@foreach@processupto\do\skv@foreach@processempty
    \do\skv@foreach@exittester\do\skv@foreach@continuetester
    \do\skv@foreach@grow\do\skv@foreach@growleft\do\skv@foreach@growright
    \do\skv@foreach@terminator\do\skv@foreach@recoverholders
    \do\skv@foreach@normalizelist\do\skv@foreach@callback
    \do\skv@foreach@hideparameters\do\skv@foreach@callback@hiddenparameters
    \do\skv@foreach@auxcallback\do\skv@foreach@precallback
    \do\skv@foreach@afterprecallback\do\skv@foreach@postcallback
    \do\skv@foreach@onlyinitially
    \do\foreachlistremainder\do\skv@foreach@mainloop
    \do\skv@foreach@getnext\do\skv@foreach@picknext\do\skv@foreach@getrm
    \do\skv@foreach@do@a\do\skv@foreach@do@b
    % Macros '...lookahead...' need stacking in \foreachfox and when
    % \newforeach is nested with \foreachfox:
    \do\skv@foreach@lookahead@a\do\skv@foreach@lookahead@b
    \do\skv@foreach@lookahead@c\do\skv@foreach@lookahead@d
    \do\skv@foreach@paramlist\do\skv@foreach@holderlist
    \do\skv@foreach@userlist\do\skv@foreach@inherit
    \do\skv@foreach@keepdecimals\do\skv@foreach@keephighdecimals
    \do\skv@foreach@itemcounter\do\skv@foreach@link
    \do\skv@foreach@expandbeforefill\do\skv@foreach@expandlistonce
    \do\skv@foreach@expandlisttwice\do\skv@foreach@expandlistfully
    \do\skv@listbreakertoks\do\skv@listpausertoks
    \do\skv@foreach@reverselist\do\foreachcurrentitem
    \do\foreachnextitem\do\foreachitemcount\do\foreachprevitem
    % The following commands are disabled on entry into the loop.
    % Hence they need to be stacked here:
    \do\prependtobeginforeach\do\appendtobeginforeach\do\atbeginforeach
    \do\prependtoendforeach\do\appendtoendforeach\do\atendforeach
  }\foreachnestdepth
}
\skvrobustdef*\skv@foreach@popstate{%
  \skvrestorestate\skv@foreach@stack\foreachnestdepth
}
\skvnewlet\skv@foreach@nil\relax
\skvnewdef*\skv@foreach@nnil{\skv@foreach@nil}
\skvrobustdef*\newforeach{\skv@testst\skv@newforeach@beginprescan}
\skvrobustdef*\skv@newforeach@beginprescan{%
  \skv@inforeachtrue
  \edef\skv@foreach@starform{0\ifskv@tempst0\else1\fi}%
  \begingroup
  \def\skv@foreach@holderlist{}%
  \def\skv@tempa{%
    \skvexpanded{\endgroup
      \noexpand\skv@foreach@endprescan
        {\skvexpandonce\skv@foreach@holderlist}%
    }%
  }%
  \let\bgroup\relax
  \skvifnextchar[{%
    \endgroup\skv@foreach@scanarg
  }{%
    \skvifnextchar i{%
      \endgroup
      \skv@err{\string\newforeach: no holder macro seen}\skv@ehd
    }{%
      \skvifnextchar\skv@orig@bgroup{%
        \endgroup
        \skv@err{\string\newforeach: no holder macro seen}\skv@ehd
      }{%
        \skv@foreach@collectholders
      }%
    }%
  }%
}
\skvrobustdef*\skv@foreach@collectholders#1{%
  \edef\skv@foreach@holderlist{%
    \skvexpandonce\skv@foreach@holderlist\skvtrimspace{#1}%
  }%
  \skvifnextchar[{%
    \skv@tempa
  }{%
    \skvifnextchar i{%
      \skv@tempa[]%
    }{%
      \skvifnextchar\skv@orig@bgroup{%
        \skv@tempa[]%
      }{%
        \skv@foreach@collectholders
      }%
    }%
  }%
}
\skvrobustdef*\skv@foreach@endprescan#1[#2]{%
  \skvifblankTF{#1}{%
    \skv@err{\string\newforeach: no holder macros seen}\skv@ehd
  }{%
    \skv@foreach@scanarg[#2]#1%
  }%
}
\skvrobustdef*\skv@foreach@scanarg{\skv@testopt\skv@foreach@scanarg@a{}}
\skvrobustdef*\skv@foreach@scanarg@a[#1]{%
  \skv@foreach@pushstate
  \skv@foreach@latehookerr
  % \foreachitemcount must be a macro, not a counter, because it is stacked:
  \def\foreachitemcount{0}%
  % Don't confuse macros of various depths; reset them here:
  \def\do##1{\def##1{}}%
  \do\skv@foreach@itemcounter\do\skv@foreach@processupto
  \do\skv@foreach@callback\do\skv@foreach@auxcallback
  \do\skv@foreach@callback@hiddenparameters
  \do\skv@foreach@precallback\do\skv@foreach@afterprecallback
  \do\skv@foreach@postcallback\do\skv@foreach@onlyinitially
  % The keys have to be set here, to determine if the list is a macro, etc.
  % Since \skv@foreach@precallback are initialized in each nest, the
  % keys have to be reset here. Reset all keys: they might have been
  % fixed by the outer loop and the inner loop might assume the default
  % values of the keys are those being used.
  \skv@foreach@setkeys{#1}%
  % We've set the keys; let's overrule \skv@foreach@expandlistonce if
  % we had seen a star suffix. Don't overrule \skv@foreach@expandlisttwice
  % and \skv@foreach@expandlistfully.
  \if\skv@foreach@starform
    \def\skv@foreach@expandlistonce{00}%
  \fi
  \ifcase0%
    % Take only one case:
    \if\skv@foreach@expandlistonce\else
    \if\skv@foreach@expandlisttwice\else
    \if\skv@foreach@expandlistfully\else 1\fi\fi\fi\relax
    \def\skv@foreach@listisamacro{00}%
  \else
    \def\skv@foreach@listisamacro{01}%
  \fi
  \begingroup
  % Collect item holders. Don't confuse explicit \bgroup for left brace:
  \skv@cnta\skvz@
  \def\skv@foreach@holderlist{}%
  \let\bgroup\relax
  \skvifnextchar i\skv@foreach@scanarg@c{%
    \skvifnextchar\skv@orig@bgroup
      \skv@foreach@scanarg@d\skv@foreach@scanarg@b
  }%
}
% #1: one holer macro or subparser.
\skvrobustdef*\skv@foreach@scanarg@b#1{%
  % Odd items must be subparser:
  \ifodd\skv@cnta
    \ifnum\skv@cnta=\@ne
      \skvifescapedTF{#1}{%
        \skv@err{Token '\noexpand#1' cannot be a subparser;
          \MessageBreak it seems to be a holder macro. I expected
          \MessageBreak the subparser to be the token here.}\skv@ehd
      }{%
        \edef\skv@prova{\skvtrimspace{#1}}%
        \let\elt\skvexpandonce
        \let\skv@elt\skv@foreach@subparser
        \if\elt\skv@prova\elt\skv@elt\else
          % Don't stack \skv@warnsubparser, so that the following
          % warning isn't called more than once in the inner loop.
          \ifnum\skv@warnsubparser=\skvz@
            \skvgadvanceno\skv@warnsubparser\@ne
            \skv@warn{Scanned subparser '\elt\skv@prova' is different from
              \MessageBreak the default or user-supplied subparser '\elt\skv@elt'.
              \MessageBreak I have used '\elt\skv@prova', but please submit
              \MessageBreak '\elt\skv@prova' as the value of the key
              'subparser'
              \MessageBreak so that I can stop giving this warning.
            }%
          \fi
          \let\skv@foreach@subparser\skv@prova
        \fi
      }%
    \fi
  \else
    \skvifescapedTF{#1}{}{%
      \skv@err{Token '\noexpand#1' is not escaped
        \MessageBreak and can't be a holder macro}\skv@ehd
    }%
  \fi
  \advance\skv@cnta\@ne
  \edef\skv@foreach@holderlist{%
    \skvexpandonce\skv@foreach@holderlist\skvtrimspace{#1}%
  }%
  \skvifnextchar i\skv@foreach@scanarg@c{%
    \skvifnextchar\skv@orig@bgroup
      \skv@foreach@scanarg@d\skv@foreach@scanarg@b
  }%
}
\skvrobustdef*\skv@foreach@scanarg@c#1#2{%
  \skvifstrcmpTF{#1#2}{in}{%
    \skv@foreach@scanarg@d
  }{%
    \skv@err{I have seen 'i' but no expected 'in'}\skv@ehd
  }%
}
\skvrobustdef*\skv@foreach@scanarg@d{%
  \ifx\skv@foreach@holderlist\@empty
    \skv@err{No item holder macros before 'in'
      \MessageBreak or before left brace}\skv@ehd
  \fi
  \skvifnextchar\skv@orig@bgroup{%
    \skv@foreach@scanarg@e
  }{%
    \if\skv@foreach@listisamacro
      \expandafter\skv@foreach@scanarg@e
    \else
      \def\reserved@a##1{%
        \skvifmacroTF{##1}{%
          \def\skv@tempehd{Maybe a star (*) suffix after
            \noexpand\newforeach or key 'expand list once', etc.,
            \MessageBreak is missing.}%
        }{%
          \let\skv@tempehd\skv@ehd
        }%
        \skv@err{I expected a left brace for beginning of list,
          \MessageBreak since you haven't told me that your
          \MessageBreak list is a macro. Instead I found '\detokenize{##1}'.
          \MessageBreak If your list is indeed a macro, you can
          \MessageBreak either put star (*) after \noexpand\newforeach
          \MessageBreak or use the key 'expand list once'
          \MessageBreak or 'expand list twice' or 'list is a macro', etc.%
        }\skv@tempehd
      }%
      \expandafter\reserved@a
    \fi
  }%
}
% #1: <list> or <listcmd>
\skvrobustdef*\skv@foreach@scanarg@e#1{%
  \edef\skv@foreach@userlist{\unexpanded{#1}}%
  \skvifnextchar\skv@orig@bgroup\skv@foreach@scanarg@h{%
    \skvifnextchar d\skv@foreach@scanarg@f\skv@foreach@scanarg@g
  }%
}
\skvrobustdef*\skv@foreach@scanarg@f#1#2{%
  \skvifstrcmpTF{#1#2}{do}{%
    \skvifnextchar\skv@orig@bgroup
      \skv@foreach@scanarg@h\skv@foreach@scanarg@g
  }{%
    \skv@err{I have seen 'd' but no the expected 'do'}\skv@ehd
  }%
}
% We've exhausted all options for grabbing the callback, so now
% look for terminator (default ;).
%
% 1. If there is no terminator ahead, the use of \skv@prova will trigger
%    'the use of ... does not match its definition' or
%    'runaway argument ...'.
% 2. This covers the case when \newforeach or \foreach comes next in
%    the callback.
\skvrobustdef*\skv@foreach@scanarg@g{%
  \def\skv@prova##1{%
    \def\skv@prova####1##1{%
      % Look out for a case like 'parser=<parser>'.
      % Eg, \newforeach[parser=;]. In this case, the value ';' of
      % key 'parser' will mistakenly be assumed to be the callback
      % terminator. It should be enclosed in braces.
      \skvxifinTF{\detokenize{parser=}\relax}{\detokenize{####1}\relax}{%
        \skvxifinTF{[}{\detokenize{####1}}{%
          \skv@err{Put '##1' in braces for key 'parser=##1'.
            \MessageBreak Try [parser={##1}]}
            {Maybe parser '##1' is the value of a key/option of
            \noexpand\newforeach and needs to be enclosed in braces.
            The '##1' I have just encountered doesn't seem to be the
            one ending a TikZ object. Maybe you need to do [parser={##1}].}%
        }{%
          % Otherwise, let's try continue:
          \skvexpanded{%
            \noexpand\skv@foreach@scanarg@h{\skvtrimspace{####1}##1}%
          }%
        }%
      }{%
        \skvexpanded{%
          \noexpand\skv@foreach@scanarg@h{\skvtrimspace{####1}##1}%
        }%
      }%
    }%
    \skv@prova
  }%
  % In case callback terminator is currently active, rescan it.
  \skvrescan\skv@foreach@terminator
  \expandafter\skv@prova\expandafter{\skv@foreach@terminator}%
}
% #1: callback
\skvrobustdef*\skv@foreach@scanarg@h#1{%
  \skvexpanded{\endgroup
    % The subparser may have changed along the way
    % (see \skv@foreach@scanarg@b):
    \skvcmdexit\skv@foreach@subparser
    \skv@foreach@mainprocess
      {\skvexpandonce\skv@foreach@holderlist}%
      {\skvexpandonce\skv@foreach@userlist}%
      {\skvtrimspace{#1}}%
  }%
}
% #1: holder macros
% #2: List or list command
% #3: Callback
\skvrobustdef*\skv@foreach@mainprocess#1#2#3{%
  \edef\skv@foreach@userlist{%
    \if\skv@foreach@expandlistonce
      \expandafter\skvexpandonce
    \else
      \if\skv@foreach@expandlisttwice
        \expandafter\expandafter\expandafter\skvexpandtwice
      \else
        \if\skv@foreach@expandlistfully
          \expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\@iden
        \else
          \expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\unexpanded
        \fi
      \fi
    \fi
    {#2}%
  }%
  % Initial code, if any:
  \skvcsuse{skv@foreach@atbeginhook@\skvrom\foreachnestdepth}%
  \skvifdefTF\foreachprevitem{}{\def\foreachprevitem{}}%
  \expandafter\skv@foreach@normalize\expandafter[\skv@foreach@parser]%
    \skv@foreach@userlist
  % Why 'keep double parser' here? Think of a list like 32//13,11/23/,...
  \skvexpbracenext\skvdefinekeepdoubleparsernormalizer
    \skv@foreach@subparser\skv@tempa
  \edef\skv@foreach@userlist{\skvexpbracenext\skv@tempa\skv@foreach@userlist}%
  \ifnum\foreachnestdepth=\skvz@
    \breakallforeachloopsfalse
  \fi
  \skvbreakloopfalse
  \foreachlastitemfalse
  \def\skv@foreach@lookahead@a##1{%
    \def\skv@foreach@picknext{##1.}%
    \futurelet\skv@foreach@next\skv@foreach@lookahead@b
  }%
  \def\skv@foreach@lookahead@b{%
    \ifx\skv@foreach@next[%
      \expandafter\skv@foreach@lookahead@c
    \else
      \ifx\skv@foreach@next(%
        \expandafter\expandafter\expandafter\skv@foreach@lookahead@d
      \else
        \expandafter\expandafter\expandafter\skv@foreach@picknext
      \fi
    \fi
  }%
  \def\skv@foreach@lookahead@c[##1]{\skv@foreach@picknext[{##1}]}%
  \def\skv@foreach@lookahead@d(##1){\skv@foreach@picknext({##1})}%
  \def\skv@foreach@mainloop##1{%
    \def\skv@foreach@getnext####1##1####2\skv@foreach@stop{%
      \edef\foreachnextitem{\skvexpandonce{\@gobble####1}}%
      \ifx\foreachnextitem\skv@foreach@nnil
        \foreachlastitemtrue
        \def\foreachnextitem{}%
      \fi
    }%
    \def\skv@foreach@do@a####1##1####2\skv@foreach@stop{%
      \edef\foreachcurrentitem{\skvexpandonce{\@gobble####1}}%
      \skvifxTF\foreachcurrentitem\skv@foreach@nnil{%
        \skvbreakloopfalse
        \foreachlastitemfalse
      }{%
        \skvifxTF\foreachcurrentitem\skv@listbreakertoks{%
          \skv@foreach@getrm{####2}%
        }{%
          \skvifxTF\foreachcurrentitem\skv@listpausertoks{%
            \message{^^J! List pause:
              ^^JType x or X to quit, or <RETURN> to proceed^^J}%
            \begingroup
            \endlinechar\m@ne\global\read-1 to\@gtempa
            \endgroup
            \skvexpandarg\lowercase{\def\noexpand\@gtempa{\@gtempa}}%
            \skvxifstrcmpTF\@gtempa{x}{%
              \skv@foreach@getrm{####2}%
            }{%
              \skv@foreach@do@b{####2}%
            }%
          }{%
            \skv@foreach@do@b{####2}%
          }%
        }%
      }%
    }%
    \def\skv@foreach@do@b####1{%
      \edef\foreachitemcount{\the\numexpr\foreachitemcount+1}%
      \ifx\skv@foreach@itemcounter\@empty\else
        \expandafter\let\skv@foreach@itemcounter\foreachitemcount
      \fi
      \skv@foreach@lookahead@a\skv@foreach@getnext####1\skv@foreach@stop
      % If the user decides to continue after \foreachlistpauser is picked up,
      % don't use \foreachlistpauser as an item:
      \skvifxTF\foreachcurrentitem\skv@listpausertoks{}{%
        \skvexpbracenext\skv@foreach@callback\foreachcurrentitem
        \let\foreachprevitem\foreachcurrentitem
      }%
      \ifx\skv@foreach@processupto\@empty\else
        \ifnum\foreachitemcount<\skv@foreach@processupto\relax\else
          \skvbreakloop
        \fi
      \fi
      \skvifdefboolTF{skvbreakloop}{%
        \skv@foreach@getrm{####1}%
      }{%
        \skv@foreach@lookahead@a\skv@foreach@do@a####1\skv@foreach@stop
      }%
    }%
    \def\skv@foreach@getrm####1{%
      \ifbreakallforeachloops\else
        \skvbreakloopfalse
      \fi
      \foreachlastitemfalse
      \def\skv@prova########1\skv@foreach@nil##1{%
        \edef\foreachlistremainder{\unexpanded{########1}}%
        \skv@removetrailingparser{##1}\foreachlistremainder
      }%
      \skv@prova####1%
    }%
    \skvifxTF\skv@foreach@userlist\@empty{%
      \if\skv@foreach@processempty\skvafterfi
        \skv@foreach@callback{}%
      \fi
    }{%
      \def\do####1{\if####1true\else false\fi}%
      \skvexpandsecond{\skvautocompletelist*}{[%
        % Note: the value of 'expand list once', etc., can't be
        % transferred automatically to \skvautocompletelist since they
        % have been used above to expand list.
        parser={\skv@foreach@parser},
        link={\skvexpandonce\skv@foreach@link},
        grow left=\do\skv@foreach@growleft,
        grow right=\do\skv@foreach@growright,
        keep decimals=\do\skv@foreach@keepdecimals,
        keep high decimals=\do\skv@foreach@keephighdecimals,
        expand before fill=\do\skv@foreach@expandbeforefill
      ]}\skv@foreach@userlist\skv@foreach@userlist
      \if\skv@foreach@reverselist\skvafterfi
        \expandafter\skv@foreach@doreverselist\expandafter
          {\skv@foreach@parser}\skv@foreach@userlist
      \fi
      \expandafter\skv@foreach@lookahead@a\expandafter\skv@foreach@do@a
        \skv@foreach@userlist##1\skv@foreach@nil##1\skv@foreach@stop
    }%
  }%
  \skv@foreach@makeprecode{#1}%
  \if\skv@foreach@recoverholders\else
    \expandafter\skvsavestate\expandafter\skv@foreach@holderstate
      \expandafter{\skv@foreach@holderlist}\skv@foreach@holderdepth
  \fi
  \skv@foreach@makeauxcallback{#3}%
  \skvexpandbracenext\skv@foreach@mainloop\skv@foreach@parser
  \skvcsuse{skv@foreach@atendhook@\skvrom\foreachnestdepth}%
  \if\skv@foreach@recoverholders\else
    \skvrestorestate\skv@foreach@holderstate\skv@foreach@holderdepth
  \fi
  \skv@foreach@popstate
  \ifnum\foreachnestdepth=\skvz@
    \def\skv@warnsubparser{0}%
  \fi
  \skv@inforeachfalse
}

% \skv@foreach@makeprecode{<holder.list>}
%
% 'Holder macro' here means, eg, \x and \y in
%
%    \newforeach \x/\y in {1/a,2/b,3/c}{<code>}
%
\skvrobustdef*\skv@foreach@makeprecode#1{%
  \begingroup
  \skv@cnta\skvz@
  \def\skv@foreach@holderlist{}%
  \def\skv@foreach@paramlist{}%
  \def\skv@prevholder{}%
  \def\skv@tempa{#1}%
  \expandafter\skv@foreach@normalize\expandafter
    [\skv@foreach@subparser]\skv@tempa
  \skvtfor*\skv@prova:=\skv@tempa\do{%
    \ifx\skv@prova\skv@foreach@subparser
      \ifnum\skv@cnta=\skvz@
        \skv@err{Subparser '\skvoxdetok\skv@foreach@subparser' can't come
          first in the list\MessageBreak of holder macros}\skv@ehd
      \else
        % Eg, if subparser is slash (/), \skv@foreach@paramlist will have
        % the syntax: ##1/##2/...:
        \edef\skv@foreach@paramlist{%
          \skvexpandonce\skv@foreach@paramlist\skvexpandonce\skv@prova
        }%
      \fi
    \else
      \advance\skv@cnta\@ne
      \edef\skv@elt{\expandafter\skvremovescape\skv@prova}%
      \edef\skv@foreach@precallback{%
        \skvexpandonce\skv@foreach@precallback
        % Each given item-holder macro is now defined in terms of
        % parameters of skv@foreach@auxcallback:
        \edef\skvexpandonce\skv@prova{%
          \noexpand\unexpanded{####\number\skv@cnta}%
        }%
        % If the current holder has no value, use the value of last holder:
        \ifnum\skv@cnta>\@ne
          \if\skv@foreach@inherit
            \noexpand\ifx\skvexpandonce\skv@prova\noexpand\@empty
              \let\skvexpandonce\skv@prova\skvexpandonce\skv@prevholder
            \noexpand\fi
          \fi
        \fi
      }%
      \edef\skv@foreach@holderlist{%
        \skvexpandonce\skv@foreach@holderlist
        % The \do is for the individual entries of the stack of
        % \skv@foreach@holderlist. It is required for stacking the
        % holder list:
        \noexpand\do\skvexpandonce\skv@prova
      }%
      \edef\skv@foreach@paramlist{%
        \skvexpandonce\skv@foreach@paramlist########\number\skv@cnta
      }%
      \let\skv@prevholder\skv@prova
    \fi
  }%
  % Add one extra parameter character to absorb extra subparsers that are
  % added for incomplete list items:
  \edef\skv@foreach@paramlist{%
    \skvexpandonce\skv@foreach@paramlist
    \skvexpandonce\skv@foreach@subparser
    ########\number\numexpr\skv@cnta+1\relax
  }%
  \skvexpanded{\endgroup
    \skvcmdexit\skv@foreach@holderlist
    \skvcmdexit\skv@foreach@paramlist
    \skvcmdexit\skv@foreach@precallback
  }%
}
% Example (*):
%
% This example demonstrates why \skv@foreach@continuetester must be
% located delicately, at where it is currently.
%
% \def\ditem{D}
% \newforeach [
%   continue=\ifx\x\ditem\fi, remember=\x as \rx initially A
% ] \x in {
%   B,(C1),D,E,[F1],G,H
% }{%
%   $\overrightarrow{\rx\x}$\ifforeachlastitem.\else,\space\fi
% }
%
% #1: callback
\skvrobustdef*\skv@foreach@makeauxcallback#1{%
  \begingroup
  \def\skv@generatesubparser##1{%
    \ifnum##1<10 \skvexpandonce\skv@foreach@subparser
      \expandafter\skv@generatesubparser
      \expandafter{\number\numexpr##1+1\expandafter}%
    \fi
  }%
  % Add extra subparsers in case some items aren't subparser-complete:
  \edef\skv@tempa{\skv@generatesubparser{1}}%
  \edef\skv@foreach@callback@hiddenparameters{\unexpanded{#1}}%
  \let\foreacheov\relax
  \let\do\noexpand
  \skvexpanded{\endgroup
    \skvcmdexit\skv@foreach@callback@hiddenparameters
    % Define auxiliary callback:
    \def\do\skv@foreach@auxcallback\skv@foreach@paramlist\foreacheov{%
      % Holder macro assignments:
      \skvexpandonce\skv@foreach@precallback
      % User tests/tasks, eg, if requested from 'evaluate' key:
      \skvexpandonce\skv@foreach@afterprecallback
      \do\ifnum\do\foreachitemcount=\@ne
        \do\skv@foreach@onlyinitially
      \do\fi
      \ifx\skv@foreach@continuetester\@secondoftwo
        \noexpand\skv@foreach@continuetester
      \else
        % Expose the parameter characters in \skv@foreach@continuetester.
        % If the user wants to ignore the callback for some items, he can
        % use the key 'continue=<condition>':
        \skvexpandonce\skv@foreach@continuetester
      \fi
      {%
        \relax
      }{%
        \if\skv@foreach@hideparameters
          \expandafter\@firstoftwo
        \else
          \expandafter\@secondoftwo
        \fi
        {%
          \noexpand\skv@foreach@callback@hiddenparameters
        }{%
          \unexpanded{#1}%
        }%
        % User tests/tasks, eg, if requested from the keys 'remember',
        % 'exit when', etc:
        \skvexpandonce\skv@foreach@postcallback
      }%
    }%
    % Define the real callback:
    \def\do\skv@foreach@callback####1{%
      \do\skv@foreach@auxcallback####1\skvxonce\skv@tempa\foreacheov
    }%
  }%
}
\skvnewdef*\skv@ucalpha#1{%
	\ifcase#1\or A\or B\or C\or D\or E\or F\or G\or H\or I\or J\or
  K\or L\or M\or N\or O\or P\or Q\or R\or S\or T\or U\or V\or W\or
  X\or Y\or Z\else?\fi
}
\skvnewdef*\skv@lcalpha#1{%
	\ifcase#1\or a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or
  k\or l\or m\or n\or o\or p\or q\or r\or s\or t\or u\or v\or w\or
  x\or y\or z\else?\fi
}
\skvnewdef*\skv@alphamap{%
  {A}{a}{1}{B}{b}{2}{C}{c}{3}{D}{d}{4}{E}{e}{5}{F}{f}{6}{G}{g}{7}{H}{h}{8}%
  {I}{i}{9}{J}{j}{10}{K}{k}{11}{L}{l}{12}{M}{m}{13}{N}{n}{14}{O}{o}{15}%
  {P}{p}{16}{Q}{q}{17}{R}{r}{18}{S}{s}{19}{T}{t}{20}{U}{u}{21}{V}{v}{22}%
  {W}{w}{23}{X}{x}{24}{Y}{y}{25}{Z}{z}{26}%
}
\skvrobustdef*\skv@reverselumap#1{%
  \def\skv@prova##1##2##3##4\skv@nil{%
    \ifx\@nnil##1%
      \expandafter\@gobble
    \else
      \expandafter\@iden
    \fi
    {\skv@prova##4\skv@nil{##1}{##2}{##3}}%
  }%
  \edef#1{\expandafter\skv@prova\skv@alphamap\@nnil{}{}\skv@nil}
}


\skvquickkeys.define{skeyval/autocomplete}{%
  .exec/\def\skv@autocomplete@parser{,};
  parser/{,}/
    \edef\skv@autocomplete@parser{\unexpanded{#1}}
    \skvstripouterbraces{2}\skv@autocomplete@parser
    \skvxifntypeTF{\detokenize{#1}}{%
      \begingroup
      % It is assumed that every n-type parser and subparser
      % must have catcode 12:
      \skvexpandnext{\catcode`}\skv@autocomplete@parser=12\relax
      \skvrescan\skv@autocomplete@parser
      \skvaftergroupdef\skv@autocomplete@parser\endgroup
    }{}
  ;
  % This default value of 'link' is required by \skvautocompletelist:
  .exec code/\def\skv@autocomplete@link{\@nil};
  link/\@nil/
    \edef\skv@prova{\unexpanded{#1}}%
    \ifcase0%
      \ifx\skv@prova\@empty 1\fi
      \ifx\skv@prova\@nnil 1\fi\relax
      \edef\skv@autocomplete@link{\unexpanded{#1}}%
      \skvstripouterbraces{2}\skv@autocomplete@link
    \fi
  ;
  grow/\@nil/
    \edef\skv@prova{\unexpanded{#1}}%
    \ifx\skv@prova\@nnil\else
      \skvcsedef{skv@autocomplete@grow#1}{00}
      \edef\skv@prova{\skvifstrcmpTF{#1}{left}{right}{left}}%
      \skvcsedef{skv@autocomplete@grow\skv@prova}{01}%
    \fi
    /left,right
  ;
  .exec/
    \def\skv@autocomplete@growleft{01}
    \def\skv@autocomplete@growright{01}
  ;
  grow left/true/
    \edef\skv@autocomplete@growleft{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  grow right/true/
    \edef\skv@autocomplete@growright{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  % Keep the decimals in rounded numbers or dimensions when list is
  % auto-completed. The value value of this key is 'true'.
  keep decimals/true/
    \edef\skv@autocomplete@keepdecimals{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  keep high decimals,keep only high decimals/true/
    \edef\skv@autocomplete@keephighdecimals{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
  expand before fill,expand list before fill/true/
    \edef\skv@autocomplete@expandbeforefill{0\skvifstrcmpTF{true}{#1}01}
    /true,false
  ;
}

% The keys 'link,grow' don't need presetting. The user must supply
% values when they are called. In internal loops, their values will
% have to be revised from those of the outer loop.
%
\skvquickkeys.preset{skeyval/autocomplete}{%
  parser,grow left=false,grow right=false,
  keep decimals=true,keep high decimals=false,
  expand before fill=false
}

% \skv@autocomplete@addtolist<parser><add.new><listcmd>
\skvrobustdef*\skv@autocomplete@addtolist#1#2#3{%
  \edef#3{\skvexpandonce#3\ifx#3\@empty\else\unexpanded{#1}\fi#2}%
}
% \skv@autocomplete@zerostepwarn{<lower>}{<upper>}{<pt.or.nil>}
\skvrobustdef*\skv@autocomplete@zerostepwarn#1#2#3{%
  \skv@warn{The tokens '\detokenize{#1}', '\detokenize{#2}'
    give nil step; '1#3' used.\MessageBreak
    Maybe you used the font-dependent units\MessageBreak
    'ex' or 'em' \ifskv@latex before \skv@begindoctoks\fi}%
}
% \skvautocompletelist[<kvlist>]{<list>}{<returncmd>}
% \skvautocompletelist*[<kvlist>]{<listcmd>}{<returncmd>}
%
% 1. Parse list of type {1,2,...,n,1,...,m} for auto completion.
%    Return outcome in <listcmd> or \skvcompletedlist.
%
\skvrobustdef*\skvautocompletelist{\skv@teststopt\skv@autocompletelist@a{}}
\skvrobustdef*\skv@autocompletelist@a[#1]#2#3{%
  \skv@usetempst{#2}\skv@autocomplete@userlist
  \skvquickkeys.set{skeyval/autocomplete}{#1}%
  \def\skv@inalphabetic{01}%
  \def\skv@isupperalpha{01}%
  \def\skv@preandpostdotspresent{01}%
  % If the list is alphabetic or numbers, original unit is nil:
  \def\skv@autocomplete@origunit{}%
  \def\skvcompletedlist{}%
  \skvexpandtwoargsonce
    \skv@autocompletelist@b\skv@autocomplete@parser\skv@autocomplete@userlist
  \let#3\skvcompletedlist
}
% \skv@autocompletelist@b{<parser>}{<list>}
\skvrobustdef*\skv@autocompletelist@b#1#2{%
  \edef\skv@tempa{\unexpanded{#2}}%
  \skv@foreach@normalize[#1]\skv@tempa
  \def\skv@prova##1{%
    \skvxifinTF{...}{\detokenize{##1}}{%
      \if\skv@autocomplete@expandbeforefill
        \edef\skv@tempa{##1}%
        \skv@foreach@normalize[#1]\skv@tempa
      \else
        \edef\skv@tempa{\unexpanded{##1}}%
      \fi
      \skvexpandargonce{\skv@autocompletelist@c{#1}}\skv@tempa
      \skv@foreach@normalize[#1]\skvcompletedlist
    }{%
      \edef\skvcompletedlist{%
        \skvaddlist{#1}\skvcompletedlist\skvtrimspace{##1}%
      }%
    }%
  }%
  \expandafter\skv@prova\expandafter{\skv@tempa}%
}
% \skv@autocompletelist@c{<parser>}{<list>}
\skvrobustdef*\skv@autocompletelist@c#1#2{%
  \skvxiffound{\relax...}\in{\relax\detokenize{#2}}\then
    \skv@err{I can't find lower limit before '...'}\skv@ehd
  \else
    \skvxiffound{\relax\detokenize{#1}...}\in{\relax\detokenize{#2}}\then
      \skv@err{I can't find lower limit before '...'}\skv@ehd
    \fi
  \fi
  % \newforeach format is '<parser>...<parser>':
  \skvxifinTF{\detokenize{#1...#1}}{\detokenize{#2}}{%
    \skv@autocomplete@splitbeforedots{#1}{#2}%
    \def\skv@prova##1#1##2#1...#1##3#1##4#1##5\skv@nil{%
      \skvifblankTF{##3}{%
        \skv@err{I can't find upper limit number or dimension,
          \MessageBreak i.e., after symbool '...'}\skv@ehd
      }{%
        % \skv@autocompletelist@b may be reentered. Hence accumulate
        % filled list:
        \skviflacus{##1}\then\else
          \edef\skvcompletedlist{%
            \skvaddlist{#1}\skvcompletedlist\unexpanded{##1}%
          }%
        \fi
        % Complete the list:
        \skv@autocompletelist@d{#1}{##1}{##2}{##3}%
        % In case the list is folded on ellipsis (...):
        \skvifblankTF{##4}{}{\skv@autocompletelist@b{#1}{##4#1##5}}%
      }%
    }%
    \expandafter\skv@prova\skv@tempa#1#1\skv@nil
  }{%
    \skv@autocompletelist@e{#1}{#2}%
  }%
}
% skv@autocompletelist@d{<parser>}{<lower1>}{<lower2>}{<upperbound>}
%
% 1. No <guide> here.
%
\skvrobustdef*\skv@autocompletelist@d#1#2#3#4{%
  \skvifxTF\skv@autocomplete@link\@nnil{%
    % No <link> has been given. The list has '...' but presumably no link.
    %
    % \skv@autocompletelist@h{<parser>}{<guide>}{<lower1>}{<lower2>}{<upper>}
    \skv@autocompletelist@h{#1}{}{#2}{#3}{#4}%
  }{%
    % <link> has been given by the user:
    \skv@autocomplete@splitandgrow{#1}{#2}{#3}{#4}%
  }%
}
%
% \skv@autocompletelist@e{<parser>}{<list>}
%
% \skv@autocompletelist@e will auto-complete this list without
% knowledge of the values of the keys 'link' and 'grow'. The syntax at (*)
% above isn't recognized by the auto-completion scheme of skeyval.
%
% skeyval formats:
%
%    {1pt,4pt,...pt,10pt}        : no additional info. required
%    {A_2pt,A_4pt,A_...,A_10pt}  : no additional info. required
%    {\pi0,\pi0.5,\pi...,\pi3}   : no additional info. required
%    {0\pi,0.5\pi,...\pi,3\pi}   : no additional info. required
%    {1pt,4pt,...,10pt}          : link = pt, grow=left, or no addit. info.
%    {A_2pt,A_4pt,...,A_10pt}    : link =_,   grow=right
%
% The general PGF format with left and right guides (given as 'A_'
% and 'pt') in
%
%    {A_2pt,A_4pt,A_...pt,A_10pt}
%
% is still legal in skeyval.
%
\skvrobustdef*\skv@autocompletelist@e#1#2{%
  \skv@autocomplete@splitbeforedots{#1}{#2}%
  \def\skv@checkguideinbounds##1##2{%
    \skv@foreach@swafalse
    \def\do####1{%
      \ifx\do####1\else
        \skviflacus####1\then\else
          \skvifinTF{##1}{####1}{}\skv@foreach@swatrue
        \fi
        \expandafter\do
      \fi
    }%
    \do##2\do
    \ifskv@foreach@swa
      \skv@err{Guide token '\detokenize{#1}' not found in some
        \MessageBreak of the elements: I can't complete
        \MessageBreak the current list. This may be
        \MessageBreak due to wrong direction of growth}\skv@ehd
    \fi
  }%
  \def\skv@prova##1#1##2#1##3...##4#1##5#1##6#1##7\skv@nil{%
    \skvifblankTF{##5}{%
      \skv@err{I can't find upper limit number or dimension,
        \MessageBreak i.e., after symbool '...'}\skv@ehd
    }{%
      % \skv@autocompletelist@b may be reentered. Hence
      \skviflacus{##1}\then\else
        \edef\skvcompletedlist{%
          \skvaddlist{#1}\skvcompletedlist
          \skvtrimspace{##1}%
        }%
      \fi
      \let\do\unexpanded
      \skvifblankTF{##3}{%
        \skvifblankTF{##4}{%
          \skv@err{No direction of growth before and/or after
            \MessageBreak symbol '...'}\skv@ehd
        }{%
          % Eg, {2pt_A,4pt_A,...pt_A,10pt_A}. Here ##3 is nil, grow left.
          \def\skv@autocomplete@growleft{00}%
          \def\skv@autocomplete@growright{01}%
          \skvexpanded{%
            \skv@autocompletelist@f
              {\do{#1}}{\do{##4}}{\do{##1}}{\do{##2}}{\do{##5}}%
          }%
        }%
      }{%
        \skvifblankTF{##4}{%
          % Eg, {A_2pt,A_4pt,A_...,A_10pt}. Here ##4 is nil, grow right.
          \def\skv@autocomplete@growright{00}%
          \def\skv@autocomplete@growleft{01}%
          \skvexpanded{%
            \skv@autocompletelist@f
              {\do{#1}}{\do{##3}}{\do{##1}}{\do{##2}}{\do{##5}}%
          }%
        }{%
          % Eg, {A_2pt,A_4pt,A_...pt,A_10pt}.
          \skvexpanded{%
            \skv@autocompletelist@g
              {\do{#1}}{\do{##3}}{\do{##4}}{\do{##1}}{\do{##2}}{\do{##5}}%
          }%
        }%
      }%
      % In case the list is folded on ellipsis (...):
      \skvifblankTF{##6}{}{\skv@autocompletelist@b{#1}{##6#1##7}}%
    }%
  }%
  \expandafter\skv@prova\skv@tempa#1#1#1\skv@nil
}
% \skv@autocompletelist@f
%       {<parser>}{<guide>}{<lower1>}{<lower2>}{<upper>}
%
% 1. Use the <guide> to get the constant and variable parts of the
%    elements.
% 2. Use the variable parts to determine if the list is Alpah, alpha or
%    number type. In this format, the unit in dimension type of list may
%    appear in <guide>.
% 3. Use the variable parts to work out the <step>.
% 4. Call the relevant macro to fill the list.
% 5. <lower1> has already been saved in \skvcompletedlist.
%
\skvrobustdef*\skv@autocompletelist@f#1#2#3#4#5{%
  \skv@checkguideinbounds{#2}{{#3}{#4}{#5}}%
  % Use the 'link' (#2) to get from {<lower1>}, {<lower2>} and {<upper>}
  % the left or right sides of the elements that should be grown:
  \def\skv@prova##1#2##2\skv@nil##3{%
    \edef##3{\if\skv@autocomplete@growleft##1\else##2\fi}%
  }%
  % <lower1> is empty when there is only one element before ellipsis:
  \skviflacus#3\then
    \def\skv@tempa{}%
  \else
    \skv@prova#3\skv@nil\skv@tempa
  \fi
  \skv@prova#4\skv@nil\skv@tempb
  \skv@prova#5\skv@nil\skv@tempc
  \let\do\skvexpandonce
  \skvexpandsecond
    {\skv@autocompletelist@h{#1}{#2}}%
    {{\do\skv@tempa}{\do\skv@tempb}{\do\skv@tempc}}%
}
% \skv@autocompletelist@g
%     {<parser>}{<predots>}{<postdots>}{<lower1>}{<lower2>}{<upper>}
\skvrobustdef*\skv@autocompletelist@g#1#2#3#4#5#6{%
  \def\skv@preandpostdotspresent{00}%
  \skv@checkguideinbounds{#2}{{#4}{#5}{#6}}%
  \skv@checkguideinbounds{#3}{{#4}{#5}{#6}}%
  % For <lower1>, <lower2> and <upper>, get the tokens between
  % <predots> and <postdots>. They are the ones to be grown.
  \def\skv@prova##1#2##2#3##3\skv@nil##4{%
    \edef##4{##2}%
  }%
  \ifx\@nnil#4\@nnil
    \let\skv@tempa\@empty
  \else
    \skv@prova#4\skv@nil\skv@tempa
  \fi
  \skv@prova#5\skv@nil\skv@tempb
  \skv@prova#6\skv@nil\skv@tempc
  % Pass <guide> as empty to \skv@autocompletelist@h. Through out, the only
  % reason for passing <guide> to \skv@autocompletelist@h is to restore
  % it in \skv@autocomplete@restore. But while
  % \skv@preandpostdotspresent is true, we won't do anything in
  % \skv@autocomplete@restore.
  \skvexpandsecond
    {\skv@autocompletelist@h{#1}{}}%
    {{\skv@tempa}{\skv@tempb}{\skv@tempc}}%
  % Restore <predots> and <postdots>:
  \def\do##1#1{%
    \ifx\do##1\else
      \edef\skvcompletedlist{%
        \skvaddlist{#1}\skvcompletedlist
        \unexpanded{#2}##1\unexpanded{#3}\skv@autocomplete@origunit
      }%
      \expandafter\do
    \fi
  }%
  \expandafter\do\skv@completedlist@partial#1\do#1%
}
% \skv@autocompletelist@h{<parser>}{<guide>}{<lower1>}{<lower2>}{<upper>}
%
% 1. Use the variable parts to determine if the list is Alpah, alpha or
%    number type. In this format, the unit in dimension type of list may
%    appear in <guide>.
% 2. Use the variable parts to work out the <step>.
% 3. Call the relevant macro to fill the list.
% 4. <lower1> has already been saved in \skvcompletedlist.
%
\skvrobustdef*\skv@autocompletelist@h#1#2#3#4#5{%
  \def\skv@completedlist@partial{}%
  \edef\skv@lowerlower{\ifx\@nnil#3\@nnil\else\unexpanded{#3}, \fi}%
  \skvifloweralpha{#4}{%
    \skv@foreach@swatrue
    \ifx\@nnil#3\@nnil\else
      \skvifloweralpha{#3}{}\skv@foreach@swafalse
    \fi
    \skvifloweralpha{#5}{}\skv@foreach@swafalse
    \ifskv@foreach@swa
      \ifx\@nnil#3\@nnil
        \def\skv@autocomplete@step{1}%
      \else
        \edef\skv@autocomplete@step{\the\numexpr\lccode`#4-\lccode`#3}%
        \ifnum\skv@autocomplete@step=\skvz@
          \def\skv@autocomplete@step{1}%
          \skv@autocomplete@zerostepwarn{#3}{#4}{}%
        \fi
      \fi
      \def\skv@isupperalpha{01}%
      % \skv@autocomplete@origunit remains nil on this branch.
      \skv@autocomplete@fillalphabetic{#1}{#4}{#5}\skv@completedlist@partial
      % Also update the items already entered in \skvcompletedlist.
      \skv@autocomplete@restore{#1}{#2}\skv@completedlist@partial
    \else
      \skv@err{The tokens '\detokenize\expandafter{\skv@lowerlower#4, #5}'
        \MessageBreak aren't of the same type}\skv@ehd
    \fi
  }{%
    \skvifupperalpha{#4}{%
      \skv@foreach@swatrue
      \ifx\@nnil#3\@nnil\else
        \skvifupperalpha{#3}{}\skv@foreach@swafalse
      \fi
      \skvifupperalpha{#5}{}\skv@foreach@swafalse
      \ifskv@foreach@swa
        \ifx\@nnil#3\@nnil
          \def\skv@autocomplete@step{1}%
        \else
          \edef\skv@autocomplete@step{\the\numexpr\uccode`#4-\uccode`#3}%
          \ifnum\skv@autocomplete@step=\skvz@
            \def\skv@autocomplete@step{1}%
            \skv@autocomplete@zerostepwarn{#3}{#4}{}%
          \fi
        \fi
        \def\skv@isupperalpha{00}%
        % \skv@autocomplete@origunit remains nil on this branch.
        \skv@autocomplete@fillalphabetic{#1}{#4}{#5}\skv@completedlist@partial
        \skv@autocomplete@restore{#1}{#2}\skv@completedlist@partial
      \else
        \skv@err{The tokens '\detokenize\expandafter{\skv@lowerlower#4, #5}'
          \MessageBreak aren't of the same type}\skv@ehd
      \fi
    }{%
      \skv@foreach@swatrue
      \ifx\@nnil#3\@nnil\else
        \skvifdimensionable{#3}{}\skv@foreach@swafalse
      \fi
      \skvifdimensionable{#4}{}\skv@foreach@swafalse
      \let\skv@autocomplete@origunit\skv@dimunit
      \skvifdimensionable{#5}{}\skv@foreach@swafalse
      \ifx\skv@autocomplete@origunit\skv@dimunit\else
        \skv@err{The units on \detokenize{'#4', '#5'} are different}\skv@ehd
      \fi
      \ifskv@foreach@swa
        \ifx\@nnil#3\@nnil
          \def\skv@autocomplete@step{1pt}%
        \else
          \edef\skv@autocomplete@step{\the\dimexpr#4-#3\relax}%
          \ifdim\skv@autocomplete@step=\skvz@
            \def\skv@autocomplete@step{1pt}%
            \skv@autocomplete@zerostepwarn{#3}{#4}{pt}%
          \fi
        \fi
        \skvexpandsecond
          {\skv@autocomplete@fillnumordim{#1}}{{#4}{#5}}%
          \skv@completedlist@partial
        \skv@autocomplete@strippoint{#1}\skv@completedlist@partial
        % Attach the constant part to the elements of the completed list.
        % <lower1> was saved earlier in \skv@autocompletelist@e, and
        % <lower2> and <upper> have been saved while filling the list.
        % Always strip point and restore original unit here.
        \skv@autocomplete@restore{#1}{#2}\skv@completedlist@partial
      \else
        \skv@foreach@swatrue
        \ifx\@nnil#3\@nnil\else
          \skvifdimensionable{#3pt}{}\skv@foreach@swafalse
        \fi
        \skvifdimensionable{#4pt}{}\skv@foreach@swafalse
        \skvifdimensionable{#5pt}{}\skv@foreach@swafalse
        \ifskv@foreach@swa
          \ifx\@nnil#3\@nnil
            \def\skv@autocomplete@step{1pt}%
          \else
            \edef\skv@autocomplete@step{\the\dimexpr#4pt-#3pt\relax}%
            \ifdim\skv@autocomplete@step=\skvz@
              \def\skv@autocomplete@step{1pt}%
              \skv@autocomplete@zerostepwarn{#3}{#4}{pt}%
            \fi
          \fi
          % \skv@autocomplete@origunit remains nil on this branch.
          \skvexpandsecondonce
            {\skv@autocomplete@fillnumordim{#1}}{{#4pt}{#5pt}}%
            \skv@completedlist@partial
          \skv@autocomplete@strippoint{#1}\skv@completedlist@partial
          \skv@autocomplete@restore{#1}{#2}\skv@completedlist@partial
        \else
          \skv@err{Sorry, the tokens
            '\detokenize\expandafter{\skv@lowerlower#4, #5}'
            \MessageBreak are unparsable. I have given up on them.
            \MessageBreak Did you miss something syntactic?
            \MessageBreak See manual for acceptable syntaxes}\skv@ehd
        \fi
      \fi
    }%
  }%
}
% \skv@autocomplete@fillnumordim<parser><lower><upper><listcmd>
\skvrobustdef*\skv@autocomplete@fillnumordim#1#2#3#4{%
  \begingroup
  \skv@autocomplete@getcomparator
  \if\skv@autocomplete@stepisneg
    \ifdim#3\skv@autocomplete@unit>#2\skv@autocomplete@unit\relax
      \skv@err{Step '\skv@autocomplete@step' is negative but upperbound
        \MessageBreak '\detokenize{#3}' is greater than lowerbound
        '\detokenize{#2}'}\skv@ehd
    \fi
  \else
    \ifdim#3\skv@autocomplete@unit<#2\skv@autocomplete@unit\relax
      \skv@err{Step '\skv@autocomplete@step' is nonnegative but upperbound
        \MessageBreak '\detokenize{#3}' is less than lowerbound
        '\detokenize{#2}'}\skv@ehd
    \fi
  \fi
  % The bounds may have decimal places. So the calculation has to be
  % done with \dimexpr:
  \edef\skv@upperlimit{\the\dimexpr#3\skv@autocomplete@unit}%
  \edef\skv@lowerlimit{\the\dimexpr#2\skv@autocomplete@unit}%
  \skv@autocomplete@addtolist{#1}\skv@lowerlimit#4%
  \ifdim\skv@lowerlimit\skv@comparator\skv@upperlimit\relax
    \def\do{%
      \edef\skv@lowerlimit{%
        \the\dimexpr\skv@lowerlimit
        +\skv@autocomplete@step\skv@autocomplete@unit\relax
      }%
      \ifdim\skv@lowerlimit\skv@comparator\skv@upperlimit\relax
        \skv@autocomplete@addtolist{#1}\skv@lowerlimit#4%
        \expandafter\do
      \fi
    }%
    \do
    % The last item has to in 'pt', so that 'pt' can be stripped.
    % Hence \dimexpr.
    \skv@autocomplete@addtolist{#1}\skv@upperlimit#4%
  \fi
  \skvaftergroupdef#4\endgroup
}
% Fill Alpha or alpha.
% \skv@autocomplete@fillalphabetic<parser><lower><upper><listcmd>
\skvrobustdef*\skv@autocomplete@fillalphabetic#1#2#3#4{%
  \begingroup
  \def\skv@inalphabetic{00}%
  \skv@autocomplete@getcomparator
  \edef\skv@type{%
    \if\skv@isupperalpha Upper\else Lower\fi case alphabetic%
  }%
  \edef\reserved@a{\if-\skv@autocomplete@step\else\skv@autocomplete@step\fi}%
  \skvoifinteger\reserved@a{}{%
    \skv@err{List is '\skv@type' type but\MessageBreak
      step '\skv@autocomplete@step' isn't an integer}\skv@ehd
  }%
  \skv@autocomplete@addtolist{#1}{#2}#4%
  \skvifstrcmpTF{#2}{#3}{}{%
    \edef\skv@lowerlimit{#2}%
    \edef\skv@upperlimit{#3}%
    \skvexpandnext{\chardef\skv@lowerlimit`}\skv@lowerlimit\relax
    \skvexpandnext{\chardef\skv@upperlimit`}\skv@upperlimit\relax
    \edef\skv@lowerlimit{%
      \the\numexpr\skv@lowerlimit-\if\skv@isupperalpha 64\else 96\fi
    }%
    \edef\skv@upperlimit{%
      \the\numexpr\skv@upperlimit-\if\skv@isupperalpha 64\else 96\fi
    }%
    \edef\skv@charcase{\the\numexpr\skv@lowerlimit+\skv@autocomplete@step}%
    \skvrecurse
      \if\skv@isupperalpha
        \edef\skv@tempa{\skv@ucalpha\skv@charcase}%
      \else
        \edef\skv@tempa{\skv@lcalpha\skv@charcase}%
      \fi
      \skv@autocomplete@addtolist{#1}\skv@tempa#4%
      \edef\skv@charcase{\the\numexpr\skv@charcase+\skv@autocomplete@step}%
    \while
      \ifnum\skv@charcase\skv@comparator\skv@upperlimit\relax
    \fi
    \skv@autocomplete@addtolist{#1}{#3}#4%
  }%
  \skvaftergroupdef#4\endgroup
}
%
% \skv@autocomplete@splitbeforedots{<parser>}{<list>}
%
% Get the one or two elements before '...' or before '<guide>,...'.
%
%    {A_2pt,A_4pt,A_...pt,A_10pt} : no additional info. required
%    {a^1,a^3,a^...,a^9}          : no additional info. required
%    {A_1,B_1,..._1,E_1}          : no additional info. required
%    {1--,4--,...--,16--}         : no additional info. required
%    {1pt,4pt,...pt,10pt}         : no additional info. required
%    {A_2pt,A_4pt,A_...,A_10pt}   : no additional info. required
%
%    {a^1,a^3,...,a^9}            : link = ^,   grow = right
%    {A_1,B_1,...,E_1}            : link = _,   grow = left
%    {1--,4--,...,16--}           : link = --,  grow = left
%    {1pt,4pt,...,10pt}           : link = pt,  grow = left, or no addit. info.
%    {A_2pt,A_4pt,...,A_10pt}     : link = _,   grow = right
%
% The items prior to the two before '<guide>...' or before '...'
% are called 'all-before-the-two' (AB2). Collect in \skv@tempa the two
% items before '<guide>...' or before '...' together with the rest of the
% list. Save the AB2 items in \skvcompletedlist.
%
% Return \skvcompletedlist and \skv@tempa.
%
\skvrobustdef*\skv@autocomplete@splitbeforedots#1#2{%
  % First count all the elements before '<guide><parser>...' or '...'.
  % We're already sure that argument #2 contains '<guide><parser>...'
  % or '...'. \skvcompletedlist has been initialized before here.
  \begingroup
  \skv@cnta\skvz@
  \def\do##1#1{%
    \skvifinTF{...}{##1}{%
      % Gobble the rest:
      \def\do####1\skv@nil{}%
    }{%
      \advance\skv@cnta\@ne
    }%
    \do
  }%
  \do#2#1\skv@nil
  \ifnum\skv@cnta>\tw@
    \@tempcnta\m@ne
    \def\do##1#1{%
      \advance\@tempcnta\@ne
      \ifnum\@tempcnta=\numexpr\skv@cnta-\tw@\relax
        \def\do####1\skv@nil{\def\skv@tempa{##1#1####1}}%
      \else
        \edef\skvcompletedlist{%
          \skvaddlist{#1}\skvcompletedlist\unexpanded{##1}%
        }%
      \fi
      \do
    }%
    \do#2#1\skv@nil
  \else
    \ifnum\skv@cnta=\@ne
      % There is only one element before '<guide><parser>...' or '...'.
      % Hence simply left-pad argument #2 with <parser> to give the
      % impression of at least 2 elements:
      \def\skv@tempa{#1#2}%
    \else
      \ifnum\skv@cnta=\tw@
        \def\skv@tempa{#2}%
      \else
        \ifnum\skv@cnta=\skvz@
          \skv@err{List <<\detokenize{#2}>>\MessageBreak
            contains symbol '...' but not a lowerbound}\skv@ehd
        \fi
      \fi
    \fi
  \fi
  \skvexpanded{\endgroup
    \skvcmdexit\skvcompletedlist\skvcmdexit\skv@tempa
  }%
}
% \skv@autocomplete@splitandgrow{<parser>}{<lower1>}{<lower2>}{<upperbound>}
%
%    {0\pi,0.5\pi,...,3\pi} : link = \pi ; grow left
%    {1--,4--,...,10--}     : link = --  ; grow left
%    {2pt,4pt,...,10pt}     : link = pt  ; grow left (or no additional info.)
%    {A_1,C_1,...,Q_1}      : link = _   ; grow left
%    {2^a,2^c,...,2^q}      : link = ^   ; grow right
%
% 1. Providing the link avoids the need to use the syntax of PGF's
%    \foreach, such as {0\pi,0.5\pi,...\pi,3\pi}. But skeyval can also
%    autocomplete lists like {0\pi,0.5\pi,...\pi,3\pi}.
% 2. We already know that the key 'link' will reject empty values.
%
\skvrobustdef*\skv@autocomplete@splitandgrow#1#2#3#4{%
  \ifx\skv@autocomplete@growleft\skv@autocomplete@growright
    \skv@err{I can't grow the list in both directions.
      \MessageBreak Maybe you haven't indicated the
      \MessageBreak direction of growth (left or right),
      \MessageBreak or both directions are 'true'.}
      {Try one of the keys 'grow=left or right',
      \MessageBreak 'grow left=true or false',
      'grow right=true or false'}\skv@ehd
  \fi
  \begingroup
  \def\skv@prova##1{%
    \skv@foreach@swatrue
    \skviflacus#2\then\else
      \skvifinTF{##1}{#2}{}\skv@foreach@swafalse
    \fi
    \skvifinTF{##1}{#3}{}\skv@foreach@swafalse
    \skvifinTF{##1}{#4}{}\skv@foreach@swafalse
    \ifskv@foreach@swa\else
      \edef\skv@provb{\ifx\@nnil#2\@nnil\else\unexpanded{#2}, \fi}%
      \skv@err{No link '##1' in one of
        '\detokenize\expandafter{\skv@provb#3, #4}'}\skv@ehd
    \fi
    \def\skv@prova####1##1####2\skv@nil{%
      \if\skv@autocomplete@growright
        \edef\skv@prova{\skvtrimspace{####1##1}}%
      \else
        \edef\skv@prova{\skvtrimspace{##1####2}}%
      \fi
      \def\do########1{{\skvtrimspace{########1}}}%
      % \skv@autocompletelist@f<parser><guide><lower1><lower2><upper>
      \skvexpanded{\endgroup
        \noexpand\skv@autocompletelist@f
        {\unexpanded{#1}}{\skvexpandonce\skv@prova}\do{#2}\do{#3}\do{#4}%
      }%
    }%
    \skv@prova#3\skv@nil
  }%
  \expandafter\skv@prova\expandafter{\skv@autocomplete@link}%
}
\skvrobustdef*\skv@autocomplete@getcomparator{%
  \begingroup
  % <unit> isn't required in alphabetic sequences:
  \if\skv@inalphabetic\else
    \let\skvreversedo\@iden
    \edef\skv@provb{\skvexpbracenext\skvreverse\skv@autocomplete@step}%
    \def\skv@prova##1##2##3\skv@nil{%
      \skvxifinTF{,\detokenize{##2##1},}{,\skvoxdetok\skv@validunit,}{%
        % That is, the sequence is made up of dimensions.
        \def\skv@autocomplete@unit{}%
      }{%
        \def\skv@autocomplete@unit{pt}%
      }%
    }%
    \expandafter\skv@prova\skv@provb\skv@nil
  \fi
  % You can't use \ifnum or \ifdim here, since for alphanumeric sequences
  % \skv@autocomplete@step isn't a dimension.
  \def\skv@prova##1##2\skv@nil{%
    \edef\skv@autocomplete@stepisneg{0\if-##10\else1\fi}%
  }%
  \expandafter\skv@prova\skv@autocomplete@step\skv@nil
  \edef\skv@comparator{\if\skv@autocomplete@stepisneg>\else<\fi}%
  \let\do\skvcmdexit
  \skvexpanded{\endgroup
    \do\skv@autocomplete@stepisneg\do\skv@comparator
    \if\skv@inalphabetic\else\do\skv@autocomplete@unit\fi
  }%
}
\begingroup
\catcode`P=12 \lccode`P=112
\catcode`T=12 \lccode`T=116
\lowercase{\endgroup
  \def\skv@autocomplete@strippoint#1#2{%
    \def\reserved@a##1#1\relax{\def#2{##1}}%
    \def\do##1.##2PT#1{%
      \ifx\do##1\else##1%
        \if\skv@autocomplete@keephighdecimals
          \ifdim.##2pt>.5pt\relax##2\fi
        \else
          \if\skv@autocomplete@keepdecimals
            \ifnum##2>\skvz@.##2\fi
          \fi
        \fi
        \unexpanded{#1}%
        \expandafter\do
      \fi
    }%
    \edef#2{\expandafter\do#2#1\do.PT#1}%
    \expandafter\reserved@a#2\relax
  }
}
% \skv@autocomplete@restore{<parser>}{<guide>}{<listcmd>}
%
% Restore guide and, in the case of dimension sequences, 'original unit'.
%
\skvrobustdef*\skv@autocomplete@restore#1#2#3{%
  \if\skv@preandpostdotspresent
    % Leave it: <predots> and <postdots> will be restored in
    % \skv@autocompletelist@g.
  \else
    \def\do##1#1{%
      \ifx\do##1\else
        \edef\skvcompletedlist{%
          \skvaddlist{#1}\skvcompletedlist
          \if\skv@autocomplete@growleft
            ##1\skv@autocomplete@origunit\unexpanded{#2}%
          \else
            \unexpanded{#2}##1\skv@autocomplete@origunit
          \fi
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do#3#1\do#1%
  \fi
}


\skv@for@restorecatcodes
\endinput

